"I Want to Figure Things Out": Supporting Exploration in Navigation for People with Visual Impairments

Navigation assistance systems (NASs) aim to help visually impaired people (VIPs) navigate unfamiliar environments. Most of today's NASs support VIPs via turn-by-turn navigation, but a growing body of work highlights the importance of exploration as well. It is unclear, however, how NASs should be designed to help VIPs explore unfamiliar environments. In this paper, we perform a qualitative study to understand VIPs' information needs and challenges with respect to exploring unfamiliar environments, with the aim of informing the design of NASs that support exploration. Our findings reveal the types of spatial information that VIPs need as well as factors that affect VIPs' information preferences. We also discover specific challenges that VIPs face that future NASs can address such as orientation and mobility education and collaborating effectively with others. We present design implications for NASs that support exploration, and we identify specific research opportunities and discuss open socio-technical challenges for making such NASs possible. We conclude by reflecting on our study procedure to inform future approaches in research on ethical considerations that may be adopted while interacting with the broader VIP community.

==> 1-Intro/v1.tex <==
For visually impaired people (VIPs), navigation in unfamiliar environments poses a critical challenge. 
Even for simple daily life activities -- buying groceries, finding a classroom at school, or casually walking up to a colleague's desk at work -- VIPs rely on assistance from sighted people.
Their inability to perform basic navigation severely impacts their personal, social, and professional autonomy~\cite{passini1988wayfinding}:  
% ------------------------------------------------------------------
% These stats either need to be connected, or can even be removed completely.
only 22\% of the visually impaired workforce is employed in the United States~\cite{kirchner1999looking, American2017Interpreting}, and their average income is 30-40\% lower than that of people who are sighted~\cite{frick2007economic}.
% ------------------------------------------------------------------



Many researchers have sought to make independent navigation possible for VIPs. However, none of the existing solutions are being adopted widely. 

For visually impaired people (VIPs), independent navigation in indoor environments is a challenging task. Even for simple daily life activities -- buying groceries, finding a classroom at school, or casually walking up to a colleague's desk at work -- VIPs rely on assistance from sighted people. Their inability to perform such basic activities often leads to social isolation~\cite{williams2013pray}, and lack of professional opportunities: only 22\% of the visually impaired workforce is employed in the United States~\cite{kirchner1999looking, American2017Interpreting}. 




Several navigation assistance systems (NASs) have been studied to help VIPs navigate in unfamiliar environments. However, existing NASs have failed to become a part of the daily life of VIPs. VIPs still rely on assistance from others when navigating unfamiliar environments. 

% From \cite{passini1988wayfinding}: 
% - Wayfinding refers to a person's abilities, both cognitive and behavioural, to reach destinations in the everyday environments. The VIP who wants to live an \textbf{active} life... 
% - Not being mobile on their own brings about a loss of personal, social, and professional independence.
% - Wf, defined in terms of spatial problem solving, is a composite of three interrelated processes: (1) decision making (plan of action to reach destination), (2) decision executing (transform plan into overt spatial behaviour and movement at the right place in space), (3) information processing (making up environmental perception and cognition that permits the above two decision-related processes to occur), where cognitive mapping is an integral part of \#3.


% Object detection helps in wayfinding
% Scene Descriptions help in wayfinding

\begin{itemize}
    \setlength{\itemindent}{.3in}
    \item [(\textbf{RQ-1})] What are VIPs' navigation goals \textit{beyond guidance}, i.e., besides going from one point to another?
    \item [(\textbf{RQ-2})] What factors influence the importance of these navigation goals between different individuals?
    \item [(\textbf{RQ-3})] What functionalities should NASs offer VIPs that they do not already offer?
    \item [(\textbf{RQ-4})] How can we refine existing NASs to accommodate these functionalities such that they enable VIPs' navigation goals, \textit{beyond guidance}?
\end{itemize}


% navigation difficult in unfamiliar env. \cite{corn2010foundations}



-- -- -- 

Introduction


Para 1: NASs only guide VIPs
Navigation in unfamiliar environments is a critical challenge for VIPs.
It affects their social, personal and professional life.
Many researchers have sought to make it possible for them to navigate, but they are only able to ‘guide’ VIPs from one point to another (which is the most primary (or simplified version) form of navigation.)
As a result, none of them are being adopted. VIPs still rely on sighted people to navigate.


Para 2: Navigation has 3 components, NASs remove them from all
Navigation/Wayfinding involves three major sub-tasks (Passini et. al):
Planning: deciding which path to take
Implementation: walking to the destination
Collect Information: gather information from the environment, which feeds into #1 and #2
Although VIPs struggle most with #3 — which affects #1 and #2, existing NASs ignore VIPs through all these three sub-tasks, essentially guiding them to their destination.


Para 3: Ability-based Design (what should we be doing instead)
Although existing systems help VIPs in reaching a destination, this does not provide them an experience equivalent to what sighted people have, or what they get in a familiar environment.
Like Google Maps is used by sighted people for navigation, it only helps them with their missing ‘ability’, and does not ask them to sit on a ‘wheelchair’. VIPs should also only be helped in aspects that they are not abled, and not removed from the loop of decision making. (cite Wobbrock’s paper on Ability-based Design).


Para 4: Examples of how NASs fail in navigation and ability-based design
For instance, in indoor navigation [NavCog, CaBot]: 
Guides them via turn-by-turn directions through a specified route, that are computed for only ‘efficiency’ - does not allow users to decide the path (no agency) [removes them from sub-task #1 and #2] — show how para #2 and #3 are not being met 
Another issue in indoor environments is availability of maps, that is a prerequisite for these systems to work. In the ‘guidance model’ there is a need for a map. But if we provide VIPs with information that they need (parallel to how VIPs use sight), we can help them navigate without maps (like sighted people do). [removes them from sub-task #3] — show how para #2 and #3 are not being met 
Let’s user select destination from a set of POIs - does not allow users to explore the space and decide on the fly where they wanna go or through which routes. — show how para #2 and #3 are not being met 


Para 4.5.1: Outdoor Navigation (do we need this?)
For instance, in outdoor navigation, Google Maps:
Issue #1
Issue #2


Para 4.5.2: Some successful ‘attempts’?
NavStick
Scene Descriptions
Object Detections
But there is still a gap where NAS designers are making up stuff, but no work has talked to VIPs specifically about their beyond navigation goals.


Para 5: Main research question [Stress unfamiliar environments somewhere]
Hence, there are clearly more things that VIPs need help with, that go beyond guidance. To inform the design of NASs, we aim to the fundamental question:

What are VIPs’ navigation goals that go beyond guidance, i.e., besides going from one point to another, and How should NASs help VIPs with them?

OR

RQ-1: What are VIPs' navigation goals ‘beyond guidance’, i.e., besides going from one point to another?
RQ-2: What factors influence the importance of these navigation goals between different individuals?
RQ-3: What functionalities should NASs offer VIPs that they do not already offer?
RQ-4: How can we refine existing NASs to accommodate these functionalities such that they enable VIPs' navigation goals,‘beyond guidance’ ?

In this work… we answer the above research questions through a qualitative study.


Para 6: Major Findings (RQ-1 + RQ-2)
To answer RQ-1, we designed and implemented a qualitative study with 8 VIPs. 
Through in-depth semi-structured interviews we found that there are in-fact two groups of VIPs: one that have beyond navigation goals, i.e. have an active attitude, and the others that don’t, i.e. have a passive attitude towards navigation. 
VIPs with an active attitude demonstrated that beyond guidance navigation goals were important for them, and demonstrated the need to:
Goal 1
Goal 2
Goal 3 …
Further, to answer RQ-2, we also interview non-VIPs and understand the factors that influence their goals.
There were two factors, internal and external.
Internal: The major factor that distinguishes the two groups were their O&M and non-visual skills.
External: behaviour of others, that affects their ability to be passive or active
Hence, based upon these factors, active may be passive and passive may be active. 
Thus there is even a need for passive to play active sometimes.


Para 7: What did we do with the findings? (RQ-3, and RQ-4)
Based upon our findings, we created a new list of design requirements that will help refine NASs to help VIPs complete these new goals. [what facilities]
Further, we outline some system sketches to visualize how some of these systems might look like and work. [how would these facilities be incorporated]



==> 1-Intro/v2.tex <==
For visually impaired people (VIPs), navigation in unfamiliar environments poses a critical challenge. 
Even for simple daily-life activities -- buying groceries, finding a classroom at school, or exploring a new shopping mall -- VIPs are required to perform navigation.
Their inability to navigate within new or rarely visit environments severely impacts their personal~\cite{williams2013pray}, professional~\cite{kirchner1999looking, American2017Interpreting}, and social autonomy~\cite{passini1988wayfinding}. 
% Many researchers have sought to make independent navigation possible for VIPs~\cite{}.
% % but 
% However, most existing systems are greatly limited in that their goal is only to \textit{guide} VIPs to the destination, hindering VIPs' ability to gain spatial awareness of the surrounding environment. \todo{Option \#1}
% % promoting a passive spatial navigation which leads to poor spatial learning of the environment~\cite{}.  
Many researchers have sought to make independent navigation possible for VIPs, but existing solutions are insufficient because their goal is only to \textit{guide} VIPs to the destination. A ``\textit{guidance only}'' approach hinders VIPs' ability to gain spatial awareness of the surrounding environment, and hence, no solutions have been widely adopted.
% [VIPs mostly rely on sighted assistance for navigation].
% [providing a passive navigation experience~\cite{clemenson_rethinking_2021}. \todo{Option \#2}]



% guidance + predefined routes + exclude users from the env. + ...
Although a variety of navigation assistance systems (NASs) have been proposed, they only support VIPs to go from point A to point B via predefined routes.
% A variety of navigation assistance systems (NASs) have been proposed, but most of them exclude VIPs from any decision making process in the name of lowering their cognitive load.
\textit{NavCog}~\cite{ahmetovic_navcog_2016}, perhaps one of the most influential work in the blind navigation space, follows a turn-by-turn assistance paradigm to \textit{guide} VIPs from one point of interest (POI) to another. CaBot~\cite{guerreiro_cabot_2019} offers guided assistance to VIPs in a suitcase form-factor, where the system mimics a guide dog and drags(need a softer word) user to the destination. Although both these approaches perform well for guidance [reduce the cognitive load onto VIPs], they do not grant users the ability to obtain spatial information about the environment, and is very different from how VIPs navigate in a familiar environment [or in real-life]. For instance, both these approach only provide information about physical landmarks that [are important] may act as source or destinations for the routes in the environment. Whereas in real life, VIPs employ sensory [any others ...] landmarks as well, that helps them create a better understanding of the space in general. Further, the paths that the users are guided through are based on `efficiency', but efficiency may not always be the best criteria for a situation -- they may want to explore a space, or take a different path that they like to be around, or pass through their favourite restaurant to feel the aroma of that cuisine. The user only has control over setting the destination, and the rest is done by the system -- keeping the user out of the decision-making loop. There is no active engagement of VIPs into navigation, and hence creating a representation of the space becomes difficult.


- Navigation requires the coordination of numerous perceptual and sensory processes that are further supported by several brain regions, including the hippocampus, retrosplenial cortex, striatum and entorhinal cortex, to create successful representations of space. [from MSR paper refs 3-8]
- At the most fundamental level, cognitive maps are formed through exploration[from MSR paper refs 8,9,25-28]
- a successful creation of cognitive maps requires active engagement in the navigation process as spatial decision making is the primary component of active learning for the acquisition of map based knowledge [from MSR paper refs 3, 32]


Navigation systems that work with GPS, for instance Google Maps~\cite{}, uses similar turn-by-turn navigation assistance, which has been shown to promote a passive spatial navigation and ultimately poor spatial learning of the surrounding environment~\cite{clemenson_rethinking_2021}. [end by saying that surrounding/environment info is important for better navigation, which will lead to next para that talks about additional pieces of information]



Several approaches have been proposed to provide additional information to the user about the environment, they are still meant [to improve/complement] for route following [guidance]. 
% 1 - NavCog3: announces POIs in the vicinity
NavCog3~\cite{sato_navcog3_2019}, for instance, extends NavCog~\cite{ahmetovic_navcog_2016} to provide users information about the presence of semantic features and POIs (and a11y information) in the vicinity (e.g., doorways, shops). But this only adds information about a specific route, and not about an environment. Also, instead of providing this information, NASs should help VIPs explore these POIs through an active engagement with the environment --- helps build a better cognitive map of the space.
% 2 - Virtual Routes: helps learn routes before going to that place
Guerreiro et al.~\cite{guerreiro_virtual_2020} allows users to preview routes virtually before they visit the environment. However, the authors observed that while using a guidance system such as NavCog after virtually viewing the route, users tend to rely on the system and not on their prior learnings about the route. Furthermore, the system was only able to help with short routes, and not cognitive maps of the environments. [Cognitive maps are formed by active engagement with the environment.] 
% 3a - Bbeep: Dynamic obstacle avoidance
BBeep~\cite{kayukawa_bbeep_2019}, another example, helps VIPs avoid dynamic obstacle such as the pedestrians on the route. [a path clearing system]. Using a suite of sensors, fitted on a suitcase, it computes if a collision may happen with a walking pedestrian and then creates a sound to help non-VIPs (sighted pedestrians) to get out of the way. [doesn't make sense to include it here].
% 3b - Airport A11y and Nav.: 
NASs were also tailored to serve well in different environments. For instance, Guerreiro et al.~\cite{guerreiro_airport_2019} adapted NavCog~\cite{ahmetovic_navcog_2016} to solve a11y challenges in a complex and large open space such as the airport. Particularly, additional mechanisms were added to prevent veering and changes to the motion model were made for the system to accurately compute location of the user as they used moving walkways. Although the system allows VIPs to not take help from airport staff, it still does not help them make their own representations or explore the space, i.e., does nothing beyond guidance.
% 4 - Turn Right: fixing rotation errors
Ahmetovic et al.~\cite{ahmetovic_turn_2018} highlighted rotation errors that happen due to imprecise turn-by-turn navigation instructions, and proposed a deep learning framework to predict over-rotations~\cite{ahmetovic2019deep}. Even though this helps improve VIPs' accuracy in following directions, it hampers their ability to form maps or explore an environment even more. The litlle active engagement that they had would now be lost, since they know that the system will guide them, without really worrying about bumping into an obstacle or turning incorrectly. 


% 5 - Impact of expertise: personalise navigation instructions/messages
Ahmetovic et al.~\cite{ahmetovic_impact_2019} explore explore how the desirability of messages provided during assisted navigation varies based on users’ navigation preferences and expertise. The authors proposed verbosity level personalization in order to keep the users engaged in the current situational context while minimizing distractions.
keep users engaged. The authors found VIPs' need for navigation instructions reduces over time as their become more familiar with the environment. Although, this is a step towards thinking more about how would VIPs want to navigate with an NAS, what kind of help do they need from them, it is still based on the same turn-by-turn guidance approach which does not consider VIPs' desire for abilities beyond guidance.


% Ability-based design
Despite extensive research in blind navigation, most existing systems are limited by \textit{guiding}-based approach. Such an approach goes against the idea of ability-based design~\cite{wobbrock2018ability}, which calls for a shift in focus from disability to ability. Current systems do not consider VIPs' abilities: O\&M skills, non-visual sensory capabilities; while designing systems. Instead, these systems replace the capabilities [or abilities] of VIPs and remove them from the decision-making process, guiding them between predefined points through a fixed path that is optimized for efficiency. Clearly, there is a lack of understanding of what abilities do VIPs ``\textit{beyond guidance}'', and how should NASs be designed to offer VIPs these abilities.


---
% When using NavCog (after virtual route learning),  -- good for short routes though.



% [from MSR paper] Nevertheless, auditory beacon navigation is a step into a new era in which automation does not simply replace our evolutionary functions and remove us from our environment, but rather feeds into our sensory inputs to promote active engagement with the world around us. 



% There is a lack of understanding about the abilities, ``\textit{beyond guidance}'', that are most valuable to VIPs.

% We explore the beyond guidance space by first asking VIPs, then proposing design guidelines and finally proposing specific solutions that confirm to these design guidelines.





% - ability is not static; it is influenced by the context in which it is exercised~\cite{newell1995extra}.

% - interactive system design from system to user.
% - disability to ability-based design: In making the shift to ability-based design, we move away from assisting human users to conform to inflexible computer systems, and instead consider how systems can be made to fit the abilities of whoever uses them. 
% - Although existing approaches do consider existing abilities of the user, but we make it the central focus.
% -  It is the authors’ hope to advance the conversation surrounding “people with disabilities” to one that primarily considers “people with abilities” in their contexts of technology use.



In this paper, we investigate [the behaviours and opinions of VIPs that go beyond guidance] with the aim of informing the design of future NASs.
Specifically, we investigate the following research questions:
\begin{itemize}
    \setlength{\itemindent}{.3in}
    \item [(\textbf{RQ-1})] What abilities do VIPs want from NASs ‘\textit{beyond guidance}’, based on their experience navigating unfamiliar environments?
    \item [(\textbf{RQ-2})] What design guidelines should NASs follow in order to offer VIPs these new abilities?
    \item [(\textbf{RQ-3})] What are some specific ways in which NASs could work in order to follow these design guidelines?
\end{itemize}



To answer these questions, we performed a qualitative study with eight VIPs and six other people who the VIPs reported as playing a big part in shaping their opinions and behaviors around navigation. The other people included orientation and mobility (O\&M) trainers, local store employees, and leaders of VIP-serving organizations.


We found three major abilities ‘beyond guidance’ that VIPs said they wanted NASs to provide them: (1) ---, (2) ---, (3) ---. 
Half of the VIPs and all six of the non-VIPs corroborated the need for these abilities, but the other half of the VIPs seemed content with receiving guidance only, suggesting that a “beyond guidance” approach to NAS design is important but only to a subset of VIPs [due to their cognitive abilities]. 
Based on these findings, we propose XX design guidelines for future NASs, including --- and ---. 
Further, we elaborate on possible visions for future NAS designs that can incorporate these new design guidelines.
We [It is the authors'] hope that these visions [advance conversations around designing systems that cater to VIPs beyond guidance, complementing route following with ....] can spark a new era of ‘beyond guidance’ NASs that serves the abilities of VIPs and complements route following with spatial exploration, social facilitation, and skill-building as well.



==> 1-Intro/v3.tex <==
% Guidance is not enough for navigation, you need active engagement.
Active engagement in navigation is central to how people form mental maps of the world. Successful creation of this map requires people to play an active role in spatial decision making for acquisition of map based knowledge during navigation~\cite{chrastil2013active, chrastil2015there}. For example, exploring a space, understanding one's current location, planning route to the destination, and retracing steps to go back --- are all part of navigation~\cite{carr2014glass}. However, performing these tasks may become challenging in unfamiliar environments. As a result, people often get help from other people in the environment or from specialized tools such as GPS-based navigation systems. Although existing tools help people reach their destination, they do not help people gain a spatial understanding of the space. For instance, it has been recently shown that turn-by-turn navigation promotes passive spatial navigation, which leads to poor spatial learning of the space~\cite{clemenson_rethinking_2021}.


Visually impaired people (VIPs), despite the absence of visual information, also build and use mental maps during navigation~\cite{hersh_mental_2020}. In fact, it is recognized that visual information is neither necessary nor sufficient to build mental maps of a space~\cite{millar1988models}. However, most existing navigation assistance systems (NASs) for VIPs, \textit{guide} them their destination through fixed routes via turn-by-turn instructions~\cite{ahmetovic_navcog_2016, guerreiro_cabot_2019, yoon2019leveraging, ...}




------------


------------



------------



For visually impaired people (VIPs), navigation in unfamiliar environments poses a critical challenge. 
Even simple daily-life activities such as buying groceries, finding a classroom at school, or exploring a new shopping mall can be overwhelming for VIPs.
VIPs' inability to navigate within new or rarely visited environments severely impacts their personal~\cite{williams2013pray}, professional~\cite{kirchner1999looking, American2017Interpreting}, and social autonomy~\cite{passini1988wayfinding}. 
Many researchers have sought to make independent navigation possible for VIPs, but existing solutions are insufficient because their goal is only to \textit{guide} VIPs to a destination. A guidance-based approach hinders VIPs' ability to gain spatial awareness of the environment, limiting their navigation experience. Hence, there is a need to explore solutions that offer ``beyond guidance'' navigation to VIPs.

% As a result, no solutions have been widely adopted.

% guide A to B + fixed POIs +  user has no control
Existing navigation assistance systems (NASs) only assist VIPs in getting from point `A' to point `B' via routes that are optimized for efficiency. 
For instance, \textit{NavCog}~\cite{ahmetovic_navcog_2016} is a smartphone-based turn-by-turn navigation system that guides users to a limited set of pre-defined points of interests (POIs), while
\textit{CaBot}~\cite{guerreiro_cabot_2019} is a suitcase-shaped robot that users grab in order to be guided to their destination.
With most such systems, the user has no control over their route to the destination.
Although these systems reduce cognitive load onto VIPs, they do so by requiring VIPs to play a passive role in navigation --- by simply following orders from the system.
% \todo{Navigation constitutes much more than following a route to destination}
 
\todo{not sure if this fits in here.}GPS-based systems like Google Maps~\cite{} also follow a similar guidance-based approach, and have been shown to promote passive navigation, leading to poor spatial understanding of the environment~\cite{clemenson_rethinking_2021}.




% other approaches that 'try' to go beyond guidance.
Navigation goes beyond just being guided, requiring the coordination of numerous perceptual and sensory processes~\cite{MSR paper 3-8} and an active engagement with the environment. Although VIPs do not have visual senses, systems exclude VIPs' other senses and do not consider them as part of their navigation. Their senses are merely considered as output channels from the system to inform VIPs about the next instruction they need to follow. Several efforts have been made to extend guidance systems to (1) provide additional information about the information (e.g., POIs~\cite{sato_navcog3_2019}, pedestrians~\cite{kayukawa_bbeep_2019}), (2) adapt to work in large open-spaces (e.g., airports~\cite{guerreiro_airport_2019}), (3) address technical challenges (e.g., rotation errors caused by delayed instructions~\cite{ahmetovic_turn_2018, ahmetovic2019deep}), and (4) rehearse routes virtually (e.g., NavCog preview~\cite{guerreiro_virtual_2020}). However, the underlying focus in all these systems is still to \textit{guide} VIPs to their destination. Consequently, these efforts have mostly been tangential to exploring ``beyond guidance'' navigation, failing to offer VIPs new abilities.



% Ability-based design
In order to offer VIPs new abilities ``beyond guidance'', NASs must first consider their existing behaviors, practices, and opinions. We build on \textit{ability-based design}~\cite{wobbrock2018ability}, which calls for a shift in focus from disability to ability while designing NASs. Current NASs do not consider VIPs' abilities, such as their O\&M skills, and non-visual sensory capabilities. We believe that instead focusing on their disability, i.e., lack of visual perception, we must build a complete understanding of VIPs' abilities to design NASs that fit into their real-life navigation practices/behaviors. In fact, abilities are not static; but dependent upon context which is influenced by other factors~\cite{newell1995extra}. Hence, there is a lack of understanding of what abilities do VIPs desire ``\textit{beyond guidance}'', and how should NASs be designed to offer VIPs these abilities given their behaviors navigating unfamiliar environments.


In this paper, we investigate VIPs' behaviors and opinions toward the abilities they want NASs to offer ``beyond guidance,'' with the aim of informing the design of future NASs.
Specifically, we investigate the following research questions:
\begin{itemize}
    \setlength{\itemindent}{.3in}
    \item [(\textbf{RQ-1})] What are VIPs' active engagement needs for navigating unfamiliar environments?
    What abilities do VIPs need in order to actively engage when navigating unfamiliar environments?
    What does active engagement mean for VIPs?
    In what ways do VIPs want to actively engage while navigating unfamiliar environments?
    What aspects of navigation do VIPs want to actively engage with the environment?
    What abilities do VIPs want from NASs ``\textit{beyond guidance},'' based on their experience navigating unfamiliar environments?
    \item [(\textbf{RQ-2})] What design guidelines should NASs follow in order to facilitate active engagement for VIPs?
    \item [(\textbf{RQ-3})] What are some specific ways in which NASs could work in order to follow these design guidelines?
\end{itemize}
What abilities
To answer these questions, we performed a qualitative study with eight VIPs and six other people who the VIPs reported as playing a big part in shaping their opinions and behaviors around navigation. The other people included orientation and mobility (O\&M) trainers, local store employees, and leaders of blind serving organizations. 


We found three major abilities ``beyond guidance'' that VIPs said they wanted NASs to provide them: (1) active engagement in navigation, (2) effective assistance from sighted people, (3) maintain and learn O\&M skills. Half of the VIPs and all six of the non-VIPs corroborated the need for these abilities, but the other half of the VIPs seemed content with receiving \textit{guidance only}, suggesting that a “beyond guidance” approach to NAS design is important but only to a subset of VIPs. We discovered that this split in half was largely affected by the VIPs' O\&M skills and cognitive capabilities. 
Based on these findings, we propose seven design guidelines for future NASs, which outline (1) what kind of information VIPs want, (2) how NASs should process this information, and (3) what forms of interaction NASs should employ to give VIPs this information.


Finally, we elaborate on specific visions for future NAS designs that can incorporate these new design guidelines.
We hope that these visions spark a new era of ``beyond guidance'' NASs that serves VIPs' abilities and complements route following with spatial exploration, social facilitation, and skill-building.






==> 1-Intro/v4.tex <==
NASs -- research purpose. What are the main challenges? (generally for NASs). 



% Guidance is not enough for navigation, you need active engagement.
Active engagement in navigation is central to how people form mental maps of the world. Successful creation of this map requires people to play an active role in spatial decision-making for acquisition of map-based knowledge during navigation~\cite{chrastil2013active, chrastil2015there}. For example, exploring a space, understanding one's current location, planning route to the destination, and retracing steps to go back, are all part of navigation~\cite{carr2014glass}. 
% 
However, performing these tasks may become challenging in unfamiliar environments. As a result, people often seek help from other people in the environment or from specialized tools such as GPS-based navigation systems. Although existing tools help people reach their destination, they do not help people gain a spatial understanding of the space. For instance, it has been recently shown that turn-by-turn navigation promotes passive spatial navigation, which leads to poor spatial learning of the environment~\cite{clemenson_rethinking_2021}.


% VIPs also use mental maps, but existing NASs guide them in a passive manner.
Visually impaired people (VIPs), despite the absence of visual information, also build and use mental maps during navigation~\cite{hersh_mental_2020}. In fact, it is known that visual information is neither necessary nor sufficient to build mental maps of a space~\cite{millar1988models}. 
% This is mostly because vision provides larger amount and more precise spatial information over other modalities, and construction of cognitive maps based on nonvisual information is difficult [ref 35 from Banovic's paper].
However, most existing navigation assistance systems (NASs) for VIPs guide them to their destination through fixed routes, delegating all decisions to the NASs~\cite{ahmetovic_navcog_2016, guerreiro_cabot_2019, yoon2019leveraging}. Some approaches have attempted to provide additional information about the environment to the VIPs during navigation. For instance, information about nearby landmarks~\cite{sato_navcog3_2019}, dynamic obstacles such as pedestrians~\cite{kayukawa_bbeep_2019}, and route previews~\cite{guerreiro_virtual_2020}. But they still focus on getting VIPs from point A to point B, without facilitating active engagement with this additional information. In fact, Guerreiro et al.~\cite{bai_virtual-blind-road_2018} found that providing route previews did not improve VIPs' navigation performance when used in conjunction with \textit{guidance-based} NASs.
% While traditional turn-by-turn navigation is effective in its ability to lead us to a desired location, this passive form of navigation does not support spatial learning, thus having a detrimental impact on humans navigation skills and spatial cognition


% 
% Despite widespread consensus about the benefits of active engagement in navigation, there is a lack of research on how NASs should facilitate active engagement for VIPs.
Clearly, there is a lack of research on how NASs should facilitate active engagement for VIPs.
Prior work on design requirements for NASs is mostly directed towards enhancing guidance-based approaches to create a richer navigation experience for VIPs.
% understanding the information needs~\cite{banovic_uncovering_2013} and interaction preferences~\cite{lewis_hearing_2015} to enhance guidance-based approaches. 
Banovic et al.~\cite{banovic_uncovering_2013} explored VIPs' information needs  for better spatial learning, assuming a passive role for VIPs. While Lewis et al.~\cite{lewis_hearing_2015} examined VIPs' preference for receiving audio cues to support \textit{guidance}. 
Our work, on the other hand, is built on the premise of exploring opportunities for NASs that go ``beyond-guidance'' and towards active engagement for VIPs.
% We examine the behaviors of VIPs when navigating unfamiliar environments in order to learn insights about their ``beyond guidance'' needs. Based on these insights, we propose a new set of design guidelines that feed into specific visions for future NASs that actively engage VIPs in navigation. 


In this paper, we perform a qualitative study with fourteen people --- eight VIPs and six other people who contribute significantly to VIPs' navigation decisions --- in order to inform the design of future NASs to facilitate active engagement.
% VIPs' behaviors and opinions toward the abilities they want NASs to offer ``beyond guidance'', with the aim of informing the design of future NASs to facilitate active engagement.
Specifically, we investigate the following research questions:
\begin{itemize}
    \setlength{\itemindent}{.3in}
    \item [(\textbf{RQ-1})] What forms of active engagement are important for VIPs when navigating unfamiliar environments?
    \item [(\textbf{RQ-2})] What design guidelines should NASs follow in order to facilitate active engagement for VIPs?
    \item [(\textbf{RQ-3})] What are some specific ways in which NASs could work in order to follow these design guidelines?
\end{itemize}
% What abilities
% The six other people who the VIPs reported as playing a big part in shaping their opinions and behaviors around navigation. 
The six other people included orientation and mobility (O\&M) trainers, local store employees, and leaders of blind serving organizations. 


We found three major forms of active engagement that VIPs said they wanted NASs to facilitate, in order to actively engage during navigation: (1) active engagement with the \textit{environment}, (2) effective assistance from sighted people, (3) means to maintain and learn O\&M skills. Half of the VIPs and all six of the non-VIPs corroborated the need for these abilities, but the other half of the VIPs seemed content with receiving \textit{guidance only}, suggesting that a “beyond guidance” approach to NAS design is important but only to a subset of VIPs. We discovered that this split in half was largely affected by the VIPs' O\&M skills and cognitive capabilities.


Based on our findings, we propose seven design guidelines for future NASs to support active engagement in navigation, which outline 
(1) \textit{information units}: what type of information do VIPs want, 
(2) \textit{information representation}: how should the information be organized and be interacted with, and
(3) \textit{agency-building}: how should NASs nudge VIPs to take an active role in navigation.
% what forms of interaction NASs should employ to give VIPs this information. 
Finally, we elaborate on specific visions for future NAS designs that can incorporate these new design guidelines.
We hope that these visions spark a new era of NASs that facilitate active engagement in navigation for VIPs.

% allow VIPs to actively engage in navigation in order   
% serves VIPs' abilities and complements route following with spatial exploration, social facilitation, and skill-building.










% ------------------------ 





% mental maps do not require 'vision'
% It is now recognised that representing space is not a purely visual activity and that vision is neither necessary nor sufficient on its own for spatial coding~\cite{millar1988models}. 
% many VIPs are active and others rarely go out on their own
% Many blind and partially sighted people are very successful (independent) travellers, though others rarely go out on their own.~\cite{hersh_mental_2020}
% this is dependent upon their skills (hersh paper also says this somewhere).




% Low vision causes high cognitive load when it comes to active navigation~\cite{https://link.springer.com/content/pdf/10.3758/s13414-020-02038-7.pdf}, and hence most existing systems work with guidance only.
% - cognitive maps
% - flexible and use from any point





% ~\cite{hersh_mental_2020}


%---------------------- notes-------------
% - It helps build a mental map of the environment aka spatial awareness
% - Especially in unfamiliar environments, navigation is often reduced (or simplified) to guidance which has been shown to promote passive spatial navigation, leading to poor spatial learning of the environment.
% - [Benefits] Active engagement has many positives:
%     - It helps learn a space, leading to independence.
%     - Better use of your brain, which becomes even faster in exploring and navigating spaces.
%     - actively engage in their navigation, leading to more accurate cognitive maps
% - exploring a new space, understanding current location, and being able to go back are all part of navigation~\cite{carr2014glass}
% - Navigation requires multiple different senses and different parts of the brain to create successful representation of the space. Guidance, on the contrary, does not allow any of this and hence poor cognitive maps are being formed.
% - hippocampus plays a role in spatial learning, memory and navigation and contains the cognitive map
% -  In fact, the creation of cognitive maps, development of spatial expertise, and exploration of novel environments
% - cognitive maps at the most fundamental level are formed through exploration of the environment

% two types of nav. strategies:
% 1. how env. cues relate to the individual (directions)
% 2. how env. cues relate to each other (map)
% -- Both operate independently and in parallel
% -- cognitive maps requires 2., s.t. the spatial information is flexible and can be used from any location

% - successful creation of this map requires active engagement in navigation as spatial decision making is primary component of active learning for acquisition of map based knowledge. 
% - e.g., turn-by-turn direction promotes a passive form of navigation that does not support learning or formation of spatial maps.
% --- 






% --- 



==> 1-Intro/v5.tex <==
  \label{sec:intrduction}
Navigation assistance systems (NASs) help visually impaired people (VIPs) navigate unfamiliar environments independently, specifically by assisting them with orientation and mobility (O\&M). %The key challenge in NAS design is determining out how best to support VIPs' independent navigation. 
Most existing NASs such as NavCog3~\cite{sato_navcog3_2019}, Microsoft Soundscape~\cite{MSsoundscape}, and CaBot~\cite{guerreiro_cabot_2019}
% , Navatar~\cite{fallah2012user}, 
have supported independent navigation via \textit{guidance}, usually in the form of turn-by-turn directions~\cite{ahmetovic_navcog_2016, fallah2012user, sato_navcog3_2019, bai_virtual-blind-road_2018, yoon2019leveraging}, or by acting as a metaphorical ``guide dog'' ~\cite{guerreiro_cabot_2019, kayukawa_bbeep_2019, kayukawa2020guiding}. 

While NASs that focus on \textit{guidance} are successful at getting VIPs from one destination to another, recent research in both cognitive science and human--computer interaction has found that other aspects such as \textit{exploration} are just as critical for helping VIPs navigate the world independently.
Specifically, cognitive science research shows that the ability to explore and to play an active role in navigation is important for one's spatial learning, cognitive development, self-confidence, sense of independence, and agency in making wayfinding decisions~\cite{golledge1997attitudes, golledge1999wayfinding, chrastil2012active, chrastil2013active, chrastil2015there, charmaz2014constructing}. 
Likewise, human--computer interaction (HCI) researchers have
found that VIPs can benefit from navigation assistance beyond turn-by-turn directions~\cite{clemenson_rethinking_2021, fenech2010effects, leshed2008car, nair_toward_2020}, specifically emphasizing the benefits to looking around~\cite{nair_toward_2020} and spatial learning~\cite{clemenson_rethinking_2021} in understanding one's environment.


\cite{fenech2010effects} "show that using a turn-by-turn navigation system negates route
learning and impairs scene recognition. These findings suggest that using a navigation system while driving
creates inattention blindness, a failure to “see” elements in the environment."

"Since this guidance method does not require any contextual knowledge about the surroundings~\cite{fenech2010effects}, it is suitable for navigation assistance of blind or visually impaired (BVI) people." -- \cite{ahmetovic_turn_2018}. 


Although recent research has uncovered that exploration is important to independent navigation, 
% the literature lacks a recent articulation of its meaning in the context of assistive technology.
the literature has been quiet on several key issues that would help researchers design new NASs, including (1) what means of exploration VIPs find most challenging when navigating unfamiliar environments, and (2) how NASs can ameliorate those challenges.
Moreover, in order to foster self-directed exploration, it would benefit researchers to understand how NASs can \textit{support}, and not \textit{replace}, VIPs' existing cognitive capabilities. 

% \textcolor{magenta}{with the ageing population, VIPs percentage will increase over time [cite a paper], and hence people who became VIPs later in life will increase, and hence their need for exploration -- in terms of more description will also be important -- this comes when we say that people who are congenitally blind have a different set of environment description needs than those who became blind later in life.}



In this paper, we perform a qualitative study with fourteen participants in order to understand how NASs can facilitate exploration for VIPs. In our study, we performed two series of semi-structured interviews: the first with eight VIPs, the second with six other people who the VIPs identified as significantly affecting their navigation behaviors. These six people included orientation and mobility O\&M trainers, local store employees, and leaders of blind serving organizations. In addition, our research team included two VIPs, who helped us connect with participants, form our interview structure, and interpret our findings.

Through these interviews, we investigate the following research questions:
\begin{itemize}
    \setlength{\itemindent}{.3in}
    \item [\textbf{RQ1.}] \textcolor{black}{What information do VIPs need to explore unfamiliar environments, and what factors influence these needs between individuals?}
    \item [\textbf{RQ2.}] \textcolor{black}{What challenges do VIPs face while exploring, both independently and collaboratively?}
\end{itemize}


We discovered three means of exploration that are challenging to VIPs: (1) gathering information about the environment in a self-directed manner, (2) receiving effective navigational help from others around them, and (3) building and maintaining orientation and mobility (O\&M) skills. 
We also found that VIPs have mixed opinions on the need for exploration, opinions that are largely informed by VIPs' previous exposure to O\&M training.
Half of the VIPs that we interviewed expressed a strong desire for more help exploring unfamiliar environments, while the other half felt content with receiving guidance-based help only. The former half had significant exposure to O\&M training, while the latter half had much less.


\color{magenta}{Define what exploration means. How does it differ from Guidance? -- see Lets get lost paper - What's the layout subsection.}
\color{black}{}



Based on our findings, we propose a new set of design guidelines that NASs should follow in order to facilitate exploration for VIPs (RQ2). 
These guidelines cover three aspects of NAS design:
(1) \textit{information collection}: what types of raw information NASs should gather from the environment, 
(2) \textit{information representation}: how this information should be processed and organized, 
(3) \textit{agency in requesting information from others}: how NASs should provide VIPs the control over getting information from others, and
(4) \textit{skill-building}: how should NASs assist VIPs in developing their cognitive abilities and O\&M skills.


Finally, we articulate visions for future NAS research that emerge from the design guidelines (RQ3). We identify future research opportunities such as active surveying of the environment, the concept of \textit{exploratory landmarks}, and real-time O\&M tutoring via the NAS itself.
We hope this effort can help the community adopt a broader view of NASs and ultimately empower VIPs in a more comprehensive way.

==> 1-Intro/v6.tex <==
% \newpage

\label{sec:intrduction}
Navigating unfamiliar environments is extremely difficult for visually impaired people (VIPs). 
Most navigation assistance systems (NASs) such as NavCog~\cite{ahmetovic_navcog_2016} and CaBot~\cite{guerreiro_cabot_2019} help VIPs navigate unfamiliar environments via turn-by-turn navigation: guiding users with verbal instructions (e.g., `turn left in 2 metres')~\cite{ahmetovic_navcog_2016, fallah_user_2012, sato_navcog3_2019, bai_virtual-blind-road_2018} or by acting as a metaphorical ``guide dog'' ~\cite{guerreiro_cabot_2019, kayukawa_bbeep_2019, kayukawa_guiding_2020}.
Although NASs focusing on turn-by-turn navigation are successful at getting users to their destination, research shows that it promotes a passive form of navigation which 

negates route learning and impairs scene recognition~\cite{fenech_effects_2010}. 


More recently, Clemenson et al.~\cite{clemenson_rethinking_2021} 


demonstrated that turn-by-turn navigation systems promote user to play a passive role in their navigation.

% \todo{concerns have been raised about ... \cite{clemenson_rethinking_2021}}
% they do so by requiring VIPs to play a passive role --- by simply following orders from the system --- instead of giving VIPs the freedom to explore and understand a space themselves.
% they require VIPs to play a passive role in their navigation; simply following orders from the NAS without making any wayfinding decisions. 
% In figure~\ref{fig:teaser}~(a), we illustrate how the turn-by-turn navigation oriented approach offers a limited view of the environment and restricts VIPs' access to the complete environment.


 
Research in cognitive science has found that the ability to explore and to play an active role in navigation is crucial for one's spatial learning, cognitive development, contextual awareness, sense of independence, and agency in making wayfinding decisions~\cite{golledge1997attitudes, golledge_wayfinding_1999, chrastil_active_2012, chrastil_active_2013, chrastil_there_2015, chrastil_active_2014}.
% Likewise, research in human-computer interaction (HCI) have found that VIPs can benefit from navigation assistance beyond turn-by-turn directions~\cite{clemenson_rethinking_2021, fenech2010effects, leshed2008car, nair_toward_2020}, specifically emphasizing the benefits to looking around~\cite{nair_toward_2020} and spatial learning~\cite{clemenson_rethinking_2021} in understanding one's environment.
Much of VIPs' navigation has been scaffolded around an end goal, yet \textit{exploration} and \textit{spontaneity} remain understudied in NAS design.


Efforts have been made to move beyond turn-by-turn navigation by providing additional information \textit{en route} to the destination~\cite{MSsoundscape, sato_navcog3_2019, paneels_listen_2013}. However, the route-centric nature of these approaches limit VIPs' ability to explore the complete environment. 
% \Cref{fig:teaser} (a) shows how a turn-by-turn navigation-based approach enables access to a part of the environment (highlighted in blue) along the route to the destination.


To our knowledge, only few researchers have tried to understand how NASs should support exploration --- primarily by enhancing VIPs' spatial learning in navigation~\cite{lahav_blindaid_2008, banovic_uncovering_2013, schneider_constructive_2000}.
% ~\cite{banovic_uncovering_2013}, but the literature has been quiet on several key issues that would help researchers design new NASs to support \textit{in-situ} exploration in unfamiliar environments. 
\hl{Banovic et al.}~\cite{banovic_uncovering_2013} investigate VIPs' information needs for spatial learning by examining their strategies for building cognitive maps of spaces. While cognitive maps of \textit{familiar} environments help VIPs explore in situ, the same is not true for \textit{unfamiliar} environments. Tversky~\cite{tversky1993cognitive} suggests that cognitive maps of unfamiliar environments are merely collages or ``thematic overlay of multimedia from different points of views'' and thus, VIPs cannot act upon them confidently in situ. 
% However, cognitive maps only support in-situ exploration in familiar environments. Tversky suggests that cognitive maps of 
% While robust cognitive maps help VIPs in exploration, doing so requires several visits before VIPs get familiar enough to confidently act upon them in situ. 
Supporting spatial learning alone is not sufficient to facilitate exploration in unfamiliar environments, especially places that VIPs do not visit regularly such as hotels, airports, or restaurants.


Therefore, we see an opportunity for NASs to facilitate in-situ exploration in unfamiliar environments for VIPs. More specifically, we envision NASs helping VIPs ``figure things out'' in \textit{any} unfamiliar environment so they can make navigation decisions on the fly, just like sighted people can do using vision. \todo{Add: Since navigating with vision is significantly different from that without vision~\cite{swobodzinski_indoor_2009}}. To realize our vision of such NASs, it is important to first examine specific practices that VIPs use to explore unfamiliar environments, the information they need to make in-situ navigation decisions, the factors that influence these needs, and the challenges they face while exploring environments. 
% --- both by themselves and by seeking assistance from people around them.
Moreover, to gain a comprehensive understanding about VIPs' practices surrounding exploration, we should also investigate challenges that VIPs face while exploring environments with the help of other people --- shown to significantly affect VIPs' navigation behaviors~\cite{williams_just_2014, thieme_i_2018, easley_lets_2016}.


In this paper, we perform a qualitative study designed to establish a holistic understanding of VIPs' practices for in-situ exploration in unfamiliar environments, aimed at guiding design of future NASs. In our study, we first performed a series of semi-structured interviews with 12 VIPs with short follow up interviews with six other people who the VIPs identified as significantly affecting their navigation behaviors. These six people included orientation and mobility O\&M trainers, local store employees, and leaders of blind serving organizations.
In addition, our research team hosted two VIPs who helped us connect with participants, refined our interview protocol, and interpret our findings.
Through these interviews, we investigate the following research questions:\\
\vspace{0.05cm}
\begin{tabular}{{p{0.05\textwidth}p{0.85\textwidth}}}
 \textbf{RQ1.} &  What information do VIPs need to explore unfamiliar environments, and what factors influence these needs between individuals? \\
 \textbf{RQ2.} & What challenges do VIPs face while exploring unfamiliar environments, both independently and collaboratively? 
\end{tabular} \\


We discovered that VIPs need two types of spatial information for in-situ exploration: \textit{shape information} and \textit{layout information}, in addition to route-based information (e.g., route to the destination, safety information, POIs). We also identified three factors that influence VIPs’ preferences for spatial information: (1) their onset of vision impairments, (2) their inherent sociability, and (3) their O\&M proficiency and choice of mobility aid. These factors were found to dictate participants' preference for the \textit{format} of information (i.e., non-visual cues or descriptions), the \textit{source} of information (i.e., others or self), and the \textit{amount} of information (i.e., level of detail). 
% Although some of these points may appear obvious in retrospect, they are often ignored by designers in practice.
\Cref{fig:teaser} \hl{shows} ----- \todo{How much detail about the figure here, and how much in the caption?}

We also identified several challenges that VIPs face in independent exploration including difficulties in gather spatial information and acquiring O\&M training, along with challenges that VIPs face in collaborative exploration such as issues with social pressures on the helper and difficulties in comprehending assistance from other people. 
While some of these challenges, specifically ones in collaborative exploration, may have been identified in prior research for turn-by-turn navigation, the design implications for exploration have not been addressed.\todo{reframe this para after Findings is revised.}


Our findings highlight key insights that inform design implications for future NASs that support in-situ exploration in unfamiliar environments for VIPs. Throughout our discussion, we articulate our visions for future NASs such as ---, ---, and ---;\todo{complete this para after Discussion section} highlighting research opportunities and challenges in realizing those visions. 
Finally, we discuss VIPs' nuanced preference for both exploration \textit{and} turn-by-turn navigation, and how does that inform accessibility research at large. We hope this effort can help the HCI community gain design inspiration for systems that enable users to initiate decisions and stay in control, instead of the system.










% \todo{Cite where relevant: \cite{swobodzinski2009indoor} -- navigation without vision is different from that with vision}








% Consequently, efforts have been made to promote exploration in navigation for VIPs by supporting contextual awareness~\cite{MSsoundscape, sato_navcog3_2019, paneels2013listen} and independent spatial learning~\cite{banovic_uncovering_2013, clemenson_rethinking_2021}.
% For example, Microsoft Soundscape\cite{MSsoundscape} and NavCog3~\cite{sato_navcog3_2019} support VIPs' contextual awareness by announcing points of interests in user's vicinity, en-route to the destination. However, most of these systems still use a turn-by-turn navigation approach in which VIPs still do not have the agency to make spontaneous navigation decisions.


% Banovic et al.~\cite{banovic_uncovering_2013} uncover VIPs' information needs for spatial learning by examining VIPs' strategies for building and refining cognitive maps of a space. While robust cognitive maps allow VIPs to make wayfinding decisions \textit{in situ}, doing so requires several visits before VIPs get familiar enough to do so. As a result, spatial learning is not enough to support exploration in unfamiliar environments, particularly places that VIPs do not visit on a regular basis.








% , or by supporting spatial learning~\cite{clemenson_rethinking_2021} as they navigate to a destination. 


% Although these efforts enhance user's spatial awareness, it does not allow them to make their own navigation decisions.



% for independent spatial learning, focusing on how NASs can support VIPs in refining their cognitive maps of an environment. 

% can master and navigate an environment over time.  


% We are interested in understanding how NASs should be designed so that they can facilitate \textit{in-situ} exploration in unfamiliar environment for VIPs.  

% However, there is a lack of understanding about how NASs should support VIPs in exploring unfamiliar environments by making \textit{in-situ} navigation decisions. 



% We are interested in understanding how should NASs support VIPs in exploring unfamiliar environments by making \textit{in-situ} navigation decisions. Banovic et al.~\cite{banovic_uncovering_2013} uncovers VIPs' information needs for spatial learning to facilitate exploration


% Efforts have been made to promote exploration in navigation for VIPs, but most of them are focused on improving turn-by-turn navigation by increase spatial awareness or by supporting spatial learning 




% Research efforts have been made to move beyond turn-by-turn navigation by improving 

% to support exploration either by improving VIPs' spatial awareness~\cite{MSsoundscape, paneels2013listen}, or by supporting their spatial learning~\cite{clemenson_rethinking_2021, banovic_uncovering_2013}, but still do not fully support 


% Research efforts have been made to promote exploration by supporting spatial learning~\cite{} in familiar and unfamiliar environments but, most approaches still focus on a route-based navigation which does not enable VIPs to be capable of making in-situ navigation decisions when exploring unfamiliar environments. For instance, Microsoft Soundscape~\cite{MSsoundscape} and ISAS~\cite{paneels2013listen}

% Banovic et al.~\cite{}




% Likewise, human--computer interaction (HCI) researchers have found that VIPs can benefit from navigation assistance beyond turn-by-turn directions~\cite{clemenson_rethinking_2021, fenech2010effects, leshed2008car, nair_toward_2020}, specifically emphasizing the benefits to looking around~\cite{nair_toward_2020} and spatial learning~\cite{clemenson_rethinking_2021} in understanding one's environment.




% research in both cognitive science and human--computer interaction has found that other aspects such as \textit{exploration} are just as critical for helping VIPs navigate the world independently.
% Specifically, cognitive science research shows that the ability to explore and to play an active role in navigation is important for one's spatial learning, cognitive development, self-confidence, sense of independence, and agency in making wayfinding decisions~\cite{golledge1997attitudes, golledge1999wayfinding, chrastil2012active, chrastil2013active, chrastil2015there, charmaz2014constructing}. 
% Likewise, human--computer interaction (HCI) researchers have found that VIPs can benefit from navigation assistance beyond turn-by-turn directions~\cite{clemenson_rethinking_2021, fenech2010effects, leshed2008car, nair_toward_2020}, specifically emphasizing the benefits to looking around~\cite{nair_toward_2020} and spatial learning~\cite{clemenson_rethinking_2021} in understanding one's environment.







%  --- shown to be just as critical to navigation in both cognitive science research~\cite{golledge1997attitudes, golledge1999wayfinding, chrastil2012active, chrastil2013active, chrastil2015there} and human-computer interaction research~\cite{clemenson_rethinking_2021, fenech2010effects, leshed2008car} --- 

% Consequently, we do not yet see NASs supporting VIPs exploration in unfamiliar environments, enabling them to make \textit{in situ} wayfinding decisions.



% Recently, much research has been directed towards promoting exploration in unfamiliar
% Researchers have made efforts in promoting exploration by providing additional information about VIPs' surrounding environment, they are still aimed at 


% Recently, researchers have sought to move beyond turn-by-turn navigation --- towards exploration --- but even these systems do not enable VIPs to make 




% Consequently, VIPs still cannot explore unfamiliar environments unlike sighted people, who 



% Despite the understanding that exploration is important to independent navigation, the literature has been quiet on several key issues that would help researchers design new NASs, including (1) (2). Moreover,

% Cognitive science research shows that the ability to explore and to play an active role in navigation is important for one's spatial learning, cognitive development, self-confidence, sense of independence, and agency in making wayfinding decisions~\cite{golledge1997attitudes, golledge1999wayfinding, chrastil2012active, chrastil2013active, chrastil2015there}. 


% Navigation assistance systems (NASs) help visually impaired people (VIPs) navigate unfamiliar environments independently, specifically by assisting them with orientation and mobility (O\&M).
% Most existing NASs such as NavCog3~\cite{sato_navcog3_2019} and CaBot~\cite{guerreiro_cabot_2019} support VIPs via turn-by-turn navigation: guiding users via verbal instructions (e.g., `turn left in 2 metres')~\cite{ahmetovic_navcog_2016, fallah2012user, sato_navcog3_2019, bai_virtual-blind-road_2018, yoon2019leveraging}, or by acting as a metaphorical ``guide dog'' ~\cite{guerreiro_cabot_2019, kayukawa_bbeep_2019, kayukawa2020guiding}.








% \newpage





% --- --- --- 

% \novelty{While the role of sighted people has been extensively studied in designing for guidance-based systems~\cite{williams_just_2014}, we know that others have a role to play -- 1st thing, and 2nd thing -- we want to understand what their role is and how can NASs help support both VIPs and other people since it has been shown that VIPs collaborate with other people during navigation in general~\cite{vincenzi_interdependence_2021, bennett2018interdependence}}

% \cite{paneels2013listen} -- focuses on increasing spatial awareness by conveying points of interest as they walk down the street using a low cost device.


% Alternate story: how sighted people get to choose their next decision based on visual information, but VIPs cannot. What are VIPs' info needs that would enable them navigate independently by exploring unfamiliar environments.


% % % 
% % Most existing NASs such as NavCog3~\cite{sato_navcog3_2019} and CaBot~\cite{guerreiro_cabot_2019} have supported VIPs' navigation in unfamiliar environments by guiding them to a destination, or by a turn-by-turn navigation paradigm, usually guiding users from 
% % usually in the form of verbal instructions (e.g., `turn left in 2 metres')~\cite{ahmetovic_navcog_2016, fallah2012user, sato_navcog3_2019, bai_virtual-blind-road_2018, yoon2019leveraging}, or by acting as a metaphorical ``guide dog'' ~\cite{guerreiro_cabot_2019, kayukawa_bbeep_2019, kayukawa2020guiding}. 


% Most existing NASs such as NavCog3~\cite{sato_navcog3_2019}
% % , Microsoft Soundscape~\cite{MSsoundscape},
% and CaBot~\cite{guerreiro_cabot_2019}
% % , Navatar~\cite{fallah2012user}, 
% have supported independent navigation by guiding users from one point to another, usually in the form of turn-by-turn directions~\cite{ahmetovic_navcog_2016, fallah2012user, sato_navcog3_2019, bai_virtual-blind-road_2018, yoon2019leveraging}
% % , by placing audio beacons in the environment~\cite{MSsoundscape}, 
% or by acting as a metaphorical ``guide dog'' ~\cite{guerreiro_cabot_2019, kayukawa_bbeep_2019, kayukawa2020guiding}. 

% While NASs that focus on \textit{guidance} are successful at getting VIPs from one destination to another, recent research in both cognitive science and human--computer interaction has found that other aspects such as \textit{exploration} are just as critical for helping VIPs navigate the world independently.
% Specifically, cognitive science research shows that the ability to explore and to play an active role in navigation is important for one's spatial learning, cognitive development, self-confidence, sense of independence, and agency in making wayfinding decisions~\cite{golledge1997attitudes, golledge1999wayfinding, chrastil2012active, chrastil2013active, chrastil2015there, charmaz2014constructing}. 
% Likewise, human--computer interaction (HCI) researchers have found that VIPs can benefit from navigation assistance beyond turn-by-turn directions~\cite{clemenson_rethinking_2021, fenech2010effects, leshed2008car, nair_toward_2020}, specifically emphasizing the benefits to looking around~\cite{nair_toward_2020} and spatial learning~\cite{clemenson_rethinking_2021} in understanding one's environment.


% \cite{fenech2010effects} "show that using a turn-by-turn navigation system negates route
% learning and impairs scene recognition. These findings suggest that using a navigation system while driving
% creates inattention blindness, a failure to “see” elements in the environment."

% "Since this guidance method does not require any contextual knowledge about the surroundings~\cite{fenech2010effects}, it is suitable for navigation assistance of blind or visually impaired (BVI) people." -- \cite{ahmetovic_turn_2018}. 


% Although recent research has uncovered that exploration is important to independent navigation, 
% % the literature lacks a recent articulation of its meaning in the context of assistive technology.
% the literature has been quiet on several key issues that would help researchers design new NASs, including (1) what means of exploration VIPs find most challenging when navigating unfamiliar environments, and (2) how NASs can ameliorate those challenges.
% Moreover, in order to foster self-directed exploration, it would benefit researchers to understand how NASs can \textit{support}, and not \textit{replace}, VIPs' existing cognitive capabilities. 




% In this paper, we perform a qualitative study with fourteen participants in order to understand how NASs can facilitate exploration for VIPs. In our study, we performed two series of semi-structured interviews: the first with eight VIPs, the second with six other people who the VIPs identified as significantly affecting their navigation behaviors. These six people included orientation and mobility O\&M trainers, local store employees, and leaders of blind serving organizations. In addition, our research team included two VIPs, who helped us connect with participants, form our interview structure, and interpret our findings.

% Through these interviews, we investigate the following research questions:
% \begin{itemize}
%     \setlength{\itemindent}{.3in}
%     \item [\textbf{RQ1.}] \textcolor{black}{What information do VIPs need to explore unfamiliar environments, and what factors influence these needs between individuals?}
%     \item [\textbf{RQ2.}] \textcolor{black}{What challenges do VIPs face while exploring, both independently and collaboratively?}
% \end{itemize}


% We discovered three means of exploration that are challenging to VIPs: (1) gathering information about the environment in a self-directed manner, (2) receiving effective navigational help from others around them, and (3) building and maintaining orientation and mobility (O\&M) skills. 
% We also found that VIPs have mixed opinions on the need for exploration, opinions that are largely informed by VIPs' previous exposure to O\&M training.
% Half of the VIPs that we interviewed expressed a strong desire for more help exploring unfamiliar environments, while the other half felt content with receiving guidance-based help only. The former half had significant exposure to O\&M training, while the latter half had much less.


% \color{magenta}{Define what exploration means. How does it differ from Guidance? -- see Lets get lost paper - What's the layout subsection.}
% \color{black}{}



% Based on our findings, we propose a new set of design guidelines that NASs should follow in order to facilitate exploration for VIPs (RQ2). 
% These guidelines cover three aspects of NAS design:
% (1) \textit{information collection}: what types of raw information NASs should gather from the environment, 
% (2) \textit{information representation}: how this information should be processed and organized, 
% (3) \textit{agency in requesting information from others}: how NASs should provide VIPs the control over getting information from others, and
% (4) \textit{skill-building}: how should NASs assist VIPs in developing their cognitive abilities and O\&M skills.


% Finally, we articulate visions for future NAS research that emerge from the design guidelines (RQ3). We identify future research opportunities such as active surveying of the environment, the concept of \textit{exploratory landmarks}, and real-time O\&M tutoring via the NAS itself.
% We hope this effort can help the community adopt a broader view of NASs and ultimately empower VIPs in a more comprehensive way.




% \textbf{May add these lines later:}

% - Although some of these points may appear obvious in retrospect, they are often ignored by designers in practice.

% - 




% --- --- --- ---


% are valuable forms of navigation understudied in accessibility research.


% The trend of scaffolding VIPs' navigation around an end goal 

% Navigation for VIPs is scaffolded around an end goal, yet exploration and spontaneity 
 
%  are a valuable forms of navigation understudied in accessibility research. Research in cognitive science and has found that other


% Exploration has been shown to be an important aspect of navigation, with both cogsci and hci research stating its significance. In cogsci research, .... . In HCI, ..... . Whereas, 






% understands navigation as social and contextual, and
%     thus holistically details the process of exploring




% % Independent navigation is a fundamental human behavior with several aspects including exploring new environments. Research in cognitive sciences ha


% Recent research in both cognitive science and human--computer interaction (HCI) has found that other aspects such as \textit{exploration} are just as critical for helping VIPs navigate the world independently.
% Specifically, cognitive science research shows that the ability to explore and to play an active role in navigation is important for one's spatial learning, cognitive development, self-confidence, sense of independence, and agency in making wayfinding decisions~\cite{golledge1997attitudes, golledge1999wayfinding, chrastil2012active, chrastil2013active, chrastil2015there, charmaz2014constructing}. 
% Likewise, human--computer interaction (HCI) researchers have found that VIPs can benefit from navigation assistance beyond turn-by-turn directions~\cite{clemenson_rethinking_2021, fenech2010effects, leshed2008car, nair_toward_2020}, specifically emphasizing the benefits to looking around~\cite{nair_toward_2020} and spatial learning~\cite{clemenson_rethinking_2021} in understanding one's environment.





% - explain why decision making is important.

% VIPs inability to take navigation into their own hands is important because ----


% Several researchers have promoted exploration in navigation to assist VIPs in being able to do ---





% % Consequently, VIPs rely on NASs to navigate unfamiliar environments.



==> 2-RW/v1.tex <==
Our work builds on two areas of related work: research on NASs that aim to help VIPs navigate unfamiliar environments independently and research on understanding VIPs' navigation behaviors and preferences.
While several research efforts have been made in both these areas, our work differs in two major ways. 

First, we focus on understanding the challenges faced by VIPs specifically in their endeavour to explore an unfamiliar environment. Prior work is primarily focused on understanding VIPs' navigation goals in general. Second, we propose a new research direction for future NASs that support ``beyond guidance'' navigation for VIPs. Most existing research takes a guidance-based stance to achieving independent navigation for VIPs.

Below, we start by discussing existing NAS technologies and highlight how they only focus on guiding VIPs to the destination. Next, we review literature in cognitive science in order to understand the importance of exploration in independent navigation. Finally, we elaborate on research efforts at the intersection of these two areas to highlight the research gap our work aims to address.




\subsection{Navigation Assistance Systems (NAS)}


Many researchers have sought to make independent navigation possible for VIPs, but existing solutions are insufficient as their goal is only to guide VIPs to a destination.
% Their goal is only to guide VIPs to a destination via fixed routes that are optimized for efficiency. 
For instance, \textit{NavCog}~\cite{ahmetovic_navcog_2016} is a smartphone-based turn-by-turn navigation system that guides users to a limited set of pre-defined points of interests (POIs), while
\textit{CaBot}~\cite{guerreiro_cabot_2019} is a suitcase-shaped robot that users grab in order to be guided to their destination via fixed routes that are optimized for efficiency. 
With most such systems, the user has no control over their route to the destination.
Although these systems reduce cognitive load onto VIPs, they do so by requiring VIPs to play a passive role in navigation --- by simply following orders from the system. A guidance-based approach hinders VIPs' ability to gain spatial awareness of the environment.

% A guidance-based approach hinders VIPs' ability to gain spatial awareness of the environment, limiting their navigation experience. Hence, there is a need to explore solutions that offer ``beyond guidance'' navigation to VIPs.

% [ALTERNATE] Many researchers have sought to make independent navigation possible for VIPs. One approach is to use fixed environment infrastructure such as BLE beacons~\cite{ahmetovic_navcog_2016, sato_navcog3_2019, kim_navigating_2016, guerreiro_airport_2019}, RFID tags~\cite{ganz2011percept, ganz2012percept, ganz2015percept}, WiFi~\cite{dias2014navpal}, and IR transmitters~\cite{mehta2011vi} to localize the user on a predefined map of the environment. 
% Another approach uses computer vision~\cite{lee2016rgb, fusco2018indoor, bai_wearable_2019, guerreiro_cabot_2019}. Specifically, they employ sensors such as cameras, LiDARs, inertial measurement units (IMU), or a suite of several sensors to locate the user on the map. 




% For instance, an influential system named NavCog~\cite{ahmetovic_navcog_2016} uses a network of BLE beacons installed in the environment along with a smartphone’s inertial sensor to estimate the user’s location and guide them using turn-by-turn directions.
 
% Although these systems have been shown to perform well even in complex environments such as airports~\cite{guerreiro_airport_2019} and train-stations~\cite{kim2016navigating}, their primary purpose is still to guide VIPs to the destination.
% Users are not involved in the navigation process, they just select a destination --- from a predefined set of points of interests (POIs) --- and follow a fixed route until they reach the destination. These systems do not support VIPs to gather additional information about the surrounding environment, 


% Without any additional information about the surrounding environment, users fail to build spatial awareness


% One shortcoming of these systems is that they use a predefined set of points of interests (POIs) such as doors, elevators, stairs, restrooms, offices, or shops. 

% These approaches use a predefined set of points of interests (POIs) from which the user gets to choose the destination. 



% One shortcoming of this approach, however, is that they require the environment to be instrumented with a dense array of BLE beacons in order to properly localize the user. VIPs must therefore depend on a different stakeholder — namely, building administrators — in order to install the hardware and make indoor environments navigable to VIPs.

% The second class of NASs use computer vision~\cite{lee2016rgb, fusco2018indoor, bai_wearable_2019, guerreiro_cabot_2019}. Specifically, they employ sensors such as cameras, LiDARs, inertial measurement units (IMU), or a suite of several sensors for both mapping and localization. CaBot~\cite{guerreiro_cabot_2019}, for example, uses the combination of a stereo camera and LiDAR, mounted on a suitcase, in order to guide VIPs in a manner similar to guide dogs. 
% Unlike fixed environment infrastructure approaches, computer vision approaches provide information about dynamic objects such as obstacles in the path. However, even these approaches focus on guiding VIPs from point A to point B. Even in 




% The third class uses real-time remote assistance from sighted people to 

% avoid the need to map the environment altogether and to localize the user within the environment. 

% VizWiz~\cite{bigham2010vizwiz}, for example, is a smartphone app that lets VIPs take pictures, then share them with crowd-sourced communities of sighted people to get their assistance. BeMyEyes~\cite{holton2015review}, another smartphone app, employs a video chat interface for mutual collaboration between VIPs and sighted volunteers. AIRA~\cite{aira} is a for-hire service that uses video calling to connect VIPs with trained experts who can guide them.


% Unlike fixed environment infrastructure and computer vision approaches, these solutions do not require the environment to be mapped or instrumented at all. They also take advantage of interdependence by enabling the collective effort between VIPs and sighted allies. One problem with these approaches, however, is that they rely solely on human effort --- they take little advantage of the capability that assistive technologies can bring as a stakeholder [CITE] to the collective effort of making indoor spaces navigable.  

% In summary, most existing NASs tend to focus on guiding VIPs to their destination, without facilitating other aspects of navigation such as exploration.

% Although guidance is an important part of navigation, the research in cognitive sciences on navigation 



Both Microsoft Soundscape~\cite{MSsoundscape}, and NavCog3~\cite{sato_navcog3_2019}


, delegating all decisions to the NASs




While these approaches provide an important functionality, i.e., getting from point A to point B, but navigation goes beyond guidance. Next, we discuss literature in wayfinding and navigation to elaborate

% just one stakeholder: VIPs, and do not take adequate account of the critical role that other stakeholders play in making indoor spaces navigable for VIPs. 

most existing navigation assistance systems (NASs) for VIPs guide them to their destination through fixed routes, delegating all decisions to the NASs~\cite{ahmetovic_navcog_2016, guerreiro_cabot_2019, yoon2019leveraging}. 

Some approaches have attempted to provide additional information about the environment to the VIPs during navigation. For instance, information about nearby landmarks~\cite{sato_navcog3_2019}, dynamic obstacles such as pedestrians~\cite{kayukawa_bbeep_2019}, and route previews~\cite{guerreiro_virtual_2020}. But they still focus on getting VIPs from point A to point B, without facilitating active engagement with this additional information. In fact, Guerreiro et al.~\cite{bai_virtual-blind-road_2018} found that providing route previews did not improve VIPs' navigation performance when used in conjunction with \textit{guidance-based} NASs.




Several approaches have been proposed to provide additional information to the user about the environment, they are still meant [to improve/complement] for route following [guidance]. 
% 1 - NavCog3: announces POIs in the vicinity
NavCog3~\cite{sato_navcog3_2019}, for instance, extends NavCog~\cite{ahmetovic_navcog_2016} to provide users information about the presence of semantic features and POIs (and a11y information) in the vicinity (e.g., doorways, shops). But this only adds information about a specific route, and not about an environment. Also, instead of providing this information, NASs should help VIPs explore these POIs through an active engagement with the environment --- helps build a better cognitive map of the space.
% 2 - Virtual Routes: helps learn routes before going to that place
Guerreiro et al.~\cite{guerreiro_virtual_2020} allows users to preview routes virtually before they visit the environment. However, the authors observed that while using a guidance system such as NavCog after virtually viewing the route, users tend to rely on the system and not on their prior learnings about the route. Furthermore, the system was only able to help with short routes, and not cognitive maps of the environments. [Cognitive maps are formed by active engagement with the environment.] 
% 3a - Bbeep: Dynamic obstacle avoidance
BBeep~\cite{kayukawa_bbeep_2019}, another example, helps VIPs avoid dynamic obstacle such as the pedestrians on the route. [a path clearing system]. Using a suite of sensors, fitted on a suitcase, it computes if a collision may happen with a walking pedestrian and then creates a sound to help non-VIPs (sighted pedestrians) to get out of the way. [doesn't make sense to include it here].
% 3b - Airport A11y and Nav.: 
NASs were also tailored to serve well in different environments. For instance, Guerreiro et al.~\cite{guerreiro_airport_2019} adapted NavCog~\cite{ahmetovic_navcog_2016} to solve a11y challenges in a complex and large open space such as the airport. Particularly, additional mechanisms were added to prevent veering and changes to the motion model were made for the system to accurately compute location of the user as they used moving walkways. Although the system allows VIPs to not take help from airport staff, it still does not help them make their own representations or explore the space, i.e., does nothing beyond guidance.
% 4 - Turn Right: fixing rotation errors
Ahmetovic et al.~\cite{ahmetovic_turn_2018} highlighted rotation errors that happen due to imprecise turn-by-turn navigation instructions, and proposed a deep learning framework to predict over-rotations~\cite{ahmetovic2019deep}. Even though this helps improve VIPs' accuracy in following directions, it hampers their ability to form maps or explore an environment even more. The litlle active engagement that they had would now be lost, since they know that the system will guide them, without really worrying about bumping into an obstacle or turning incorrectly. 


% 5 - Impact of expertise: personalise navigation instructions/messages
Ahmetovic et al.~\cite{ahmetovic_impact_2019} explore explore how the desirability of messages provided during assisted navigation varies based on users’ navigation preferences and expertise. The authors proposed verbosity level personalization in order to keep the users engaged in the current situational context while minimizing distractions.
keep users engaged. The authors found VIPs' need for navigation instructions reduces over time as their become more familiar with the environment. Although, this is a step towards thinking more about how would VIPs want to navigate with an NAS, what kind of help do they need from them, it is still based on the same turn-by-turn guidance approach which does not consider VIPs' desire for abilities beyond guidance.










\subsection{Importance of Exploration in Navigation}
% Various strands of research in cognitive science indicate the importance of exploration in independent navigation. For instance, ....



\subsection{Support for Exploration via Navigation Assistance Systems}
Various strands of research in cognitive science indicate the importance of exploration in independent navigation. 


Prior work on design requirements for NASs is mostly directed towards enhancing guidance-based approaches to create a richer navigation experience for VIPs.
% understanding the information needs~\cite{banovic_uncovering_2013} and interaction preferences~\cite{lewis_hearing_2015} to enhance guidance-based approaches. 
Banovic et al.~\cite{banovic_uncovering_2013} explored VIPs' information needs  for better spatial learning, assuming a passive role for VIPs. While Lewis et al.~\cite{lewis_hearing_2015} examined VIPs' preference for receiving audio cues to support \textit{guidance}. 
Our work, on the other hand, is built on the premise of exploring opportunities for NASs that go ``beyond-guidance'' and towards active engagement for VIPs.
% We examine the behaviors of VIPs when navigating unfamiliar environments in order to learn insights about their ``beyond guidance'' needs. Based on these insights, we propose a new set of design guidelines that feed into specific visions for future NASs that actively engage VIPs in navigation. 




% Despite extensive research in blind navigation, most existing systems are limited by \textit{guiding}-based approach. Such an approach goes against the idea of ability-based design~\cite{wobbrock2018ability}, which calls for a shift in focus from disability to ability. Current systems do not consider VIPs' abilities: O\&M skills, non-visual sensory capabilities; while designing systems. Instead, these systems replace the capabilities [or abilities] of VIPs and remove them from the decision-making process, guiding them between predefined points through a fixed path that is optimized for efficiency. Clearly, there is a lack of understanding of what abilities do VIPs ``\textit{beyond guidance}'', and how should NASs be designed to offer VIPs these abilities.

The broader challenge of supporting exploration in navigation has been approached from a variety of perspectives. These efforts largely fall under two main categories: 








% Ability-based design
Despite extensive research in blind navigation, most existing systems are limited by \textit{guiding}-based approach. Such an approach goes against the idea of ability-based design~\cite{wobbrock2018ability}, which calls for a shift in focus from disability to ability. Current systems do not consider VIPs' abilities: O\&M skills, non-visual sensory capabilities; while designing systems. Instead, these systems replace the capabilities [or abilities] of VIPs and remove them from the decision-making process, guiding them between predefined points through a fixed path that is optimized for efficiency. Clearly, there is a lack of understanding of what abilities do VIPs ``\textit{beyond guidance}'', and how should NASs be designed to offer VIPs these abilities.


To this end, we investigate the roles, capabilities, and needs of all relevant stakeholders --- heeding the call for an interdependence perspective [cite] in assistive technology design --- to discover a new set of design guidelines for NASs.

==> 2-RW/v2.tex <==
Our work builds on two areas of related work: research on NASs that aim to help VIPs navigate unfamiliar environments independently and research on understanding VIPs' navigation behaviors and preferences.
%While several research efforts have been made in both these areas, our work differs in two major ways. 
%First, we focus on understanding the challenges faced by VIPs specifically in their endeavour to explore an unfamiliar environment. Prior work is primarily focused on understanding VIPs' navigation goals in general. Second, we propose a new research direction for future NASs that support ``beyond guidance'' navigation for VIPs. Most existing research takes a guidance-based stance to achieving independent navigation for VIPs.

%Below, we start by discussing existing NAS technologies and highlight how they only focus on guiding VIPs to the destination. Next, we review literature in cognitive science in order to understand the importance of exploration in independent navigation. Finally, we elaborate on research efforts at the intersection of these two areas to highlight the research gap our work aims to address.




\subsection{Navigation Assistance Systems (NAS)}


Many researchers have sought to make independent navigation possible for VIPs, and the overarching approach is to do so by guiding VIPs to their destination.
% [Guidance only]
NavCog~\cite{ahmetovic_navcog_2016}, for instance, is a smartphone-based turn-by-turn navigation system that guides users to a limited set of pre-defined points of interests (POIs), while
CaBot~\cite{guerreiro_cabot_2019} is a suitcase-shaped robot that users grab in order to be guided to their destination. 
Although these systems reduce VIPs' cognitive load, they do so by requiring VIPs to play a passive role in navigation --- by simply following orders from the system. 
[Cognitive science research says the next line]
A guidance-based approach hinders VIPs' ability to gain exploration of the environment. 

Recent research ... inject spatial awareness via additional info..
% [Announcing POIs to increase knowledge --- still guidance]
In order to provide additional information about the environment [additional info, why?], both Microsoft Soundscape~\cite{MSsoundscape} and NavCog3~\cite{sato_navcog3_2019} announce POIs and landmarks such as doors, elevators, and stairs in the user's vicinity.
% Another approach, named BBeep~\cite{kayukawa_bbeep_2019} provides detects pedestrians in the path
However, this feature is primarily meant to help users reaffirm their location as they follow routes, with the underlying goal still being getting users to their destination.
% Moreover, these announcements compete for attention with VIPs' other senses which they use to gather information when navigating an environment. 
Although POIs and landmarks form an integral part of VIPs' navigation, there is a lack of research on what other kinds of information VIPs need in order to explore environments. 
% Consequently, these efforts have mostly been tangential to ``beyond guidance'' navigation, and do not facilitate exploration.

% In addition, announcing POIs requires NASs to do all the work, with VIPs merely waiting for the system to confirm their location. This again leads to VIPs not being able to explore a space on their own.
% [However, the underlying focus in all these systems is still to \textit{guide} VIPs to their destination. Consequently, these efforts have mostly been tangential to exploring ``beyond guidance'' navigation, failing to offer VIPs new abilities.]

% [Route preview --- doesn't support map knowldge] 
Guerreiro et al.~\cite{guerreiro_virtual_2020} took a more indirect approach in increasing user's knowledge about the environment. The authors proposed an interactive virtual navigation app which allows users to preview routes before they actually visit the environment. 
One shortcoming of this approach, however, is that it focuses on \textit{route knowledge}, and not \textit{map knowledge}. While route knowledge enables path following, it does not provide a spatial understanding of the space. Map knowledge, on the other hand, gives users the ability to take navigation decisions such as choosing a path, taking shortcuts, or exploring new spaces~\cite{chrastil2012active}. 


% Difference in route knowledge and map knowledge and their advantages.
% Route knowledge enables one to follow
% a known path from one location to another, whereas survey
% knowledge includes some configural information and gives
% one the ability to take novel shortcuts and detours between
% locations, traversing paths that have never been taken
% before. There are thus different types of spatial knowledge
% that a navigator might acquire during exploration of a new
% environment, which could depend on the structure of that
% environment, how it is explored, or the effort devoted to
% learning it.


% that allows users to preview routes virtually before they visit the environment. However, 


% the authors observed that while using a guidance system such as NavCog after virtually viewing the route, users tend to rely on the system and not on their prior learnings about the route. Furthermore, the system was only able to help with short routes, and not cognitive maps of the environments. 

% This was indirect, and hence ...


% [Cognitive maps are formed by active engagement with the environment.]
% Another interesting work by  
% Ahmetovic et al.~\cite{ahmetovic_impact_2019} explore how the desirability of messages provided during assisted navigation varies based on users’ navigation preferences and expertise. The authors proposed verbosity level personalization in order to keep the users engaged in the current situational context while minimizing distractions.
% keep users engaged. The authors found VIPs' need for navigation instructions reduces over time as their become more familiar with the environment. Although, this is a step towards thinking more about how would VIPs want to navigate with an NAS, what kind of help do they need from them, it is still based on the same turn-by-turn guidance approach which does not consider VIPs' desire for abilities beyond guidance.

% [Recently, several researchers have argued for ....~\cite{clemenson_rethinking_2021}]
NavStick~\cite{nair_toward_2020}, an audio navigation tool, allows users to survey virtual environments. Users point to a specific direction using a game controller's thumbstick in order to hear what lies there via spatialized sound.
While this approach does explore ``beyond guidance'' abilities for VIPs --- enabling VIPs to \textit{look-around} --- it is primarily designed to work in virtual environments to make video games and mixed reality experiences blind accessible. 
% In real world, however, there are several confounding factors such as presence of other people and availability of assistance, that influence VIPs' navigation behaviors.

Hence, we aim to investigate VIPs' real-life challenges to inform the design of more such ``beyond guidance'' navigation technologies, with special emphasis on supporting exploration in unfamiliar environments.












\subsection{Importance of Exploration in Navigation}
Various strands of research in cognitive science indicate the importance of exploration in independent navigation. For instance, .... [Need an intro paragraph to contain all 3 points]


% [Point1: Turn-by-turn and exploration are two parallel aspects of navigation]

Neuroscience research identifies two independent and parallel neural processes in navigation, one process follows cues pointing to directions, and the other process finds location based on environmental information in a spatial layout~\cite{ferbinteanu2016contributions}. The navigation ability of following directions is well supported by turn-by-turn instructions in NAS. However, exploration using environmental information deserves more attention in NAS research. 

% [Point2: Exploration is human nature, essential for human identity]

Exploration practice in navigation is an essential and inherent aspect of humanity, critical to our ancestral survival and manifested in our DNA. A gene coding the human trait for exploration and seeking is linked to our ancestors’ mass migration out of Africa, a critical step to survival as a species~\cite{matthews2011novelty}. As a result of natural selection, the need for exploration is hereditary and programmed in our DNA. The practice of exploration, although no longer a survival skill, is a matter of self-determination as a human being~\cite{o2019wayfinding}. Thus, NASs have the duty to support and enable exploration for VIPs. 

% [Point3: Exploration is learnable by anyone, and good for cognitive improvement]

Exploration expertise is learnable and sustainable through active practice. Research finds evidence that exploration expertise is not a talent but rather plastic skills. Active effort in practicing exploration is linked to positive change of brain structure and cognitive advantages~\cite{woollett2009talent}. Therefore, despite the lack of vision posing a challenge, with the support from NASs, there should be a potential for all VIPs to practice and build exploration skills. 



% [CITE1]Ferbinteanu, J. (2016). Contributions of hippocampus and striatum To memory-guided behavior depend on past experience. The Journal of Neuroscience, 36(24), 6459–6470. https://doi.org/10.1523/jneurosci.0840-16.2016 = ferbinteanu2016contributions


% [CITE2]Matthews, L. J., & Butler, P. M. (2011). Novelty-seeking drd4 polymorphisms are associated with human migration distance out-of-africa after controlling for neutral population gene structure. American Journal of Physical Anthropology, 145(3), 382–389. https://doi.org/10.1002/ajpa.21507 = matthews2011novelty


% [CITE3]O'Connor, M. R. (2019). Wayfinding: The science and mystery of how humans navigate the world. St. Martin’s Press. New York. = o2019wayfinding


% [CITE4]Woollett, K., Spiers, H. J., & Maguire, E. A. (2009). Talent in the taxi: A model system for exploring expertise. Philosophical Transactions of the Royal Society B: Biological Sciences, 364(1522), 1407–1416. https://doi.org/10.1098/rstb.2008.0288 = woollett2009talent










\subsection{Navigation Assistance System Design to Support VIPs' Preferences}

% The broader challenge of investigating exploration in navigation for VIPs has been approached from a variety of perspectives. These efforts largely fall under two main categories: 

Informed by the research studies in cognitive science, various research efforts have been made to understand VIPs' navigation needs, preferences, and behaviors. Prior work on design requirements for NASs, however, is mostly directed toward enhancing guidance-based NASs either by providing additional information about the surroundings~\cite{banovic_uncovering_2013}, or by understanding interaction preferences to receive audio cues~\cite{lewis_hearing_2015}.

% [Add another paragraph with details of what these papers do?]

% create a richer navigation experience for VIPs.  
% Various strands of research in cognitive science indicate the importance of exploration in independent navigation. 
% Prior work on design requirements for NASs is mostly directed towards 
% understanding the information needs~\cite{banovic_uncovering_2013} and interaction preferences~\cite{lewis_hearing_2015} to enhance guidance-based approaches. 
Banovic et al.~\cite{banovic_uncovering_2013} uncover VIPs' information needs for better spatial learning. The authors conducted interviews with both VIPs and O\&M trainers to outline the different types of information that NASs should provide VIPs. In contrast, we focus on NAS design that \textit{facilitate} exploration and do not directly provide VIPs the information needed for exploration.
Lewis et al.~\cite{lewis_hearing_2015} examined VIPs' preferences for receiving audio cues to support guidance. On the other hand, we advocate rethinking NAS design that go ``beyond guidance'' and empower VIPs to explore an environment on their own.

In summary...?

% Our work is built on the premise of exploring opportunities for NAS design that go ``beyond-guidance'', and towards supporting VIPs exploration.
% We examine the behaviors of VIPs when navigating unfamiliar environments in order to learn insights about their ``beyond guidance'' needs. Based on these insights, we propose a new set of design guidelines that feed into specific visions for future NASs that actively engage VIPs in navigation. 













% -----------COMMENTED OUT---------------

% Despite extensive research in blind navigation, most existing systems are limited by \textit{guiding}-based approach. Such an approach goes against the idea of ability-based design~\cite{wobbrock2018ability}, which calls for a shift in focus from disability to ability. Current systems do not consider VIPs' abilities: O\&M skills, non-visual sensory capabilities; while designing systems. Instead, these systems replace the capabilities [or abilities] of VIPs and remove them from the decision-making process, guiding them between predefined points through a fixed path that is optimized for efficiency. Clearly, there is a lack of understanding of what abilities do VIPs ``\textit{beyond guidance}'', and how should NASs be designed to offer VIPs these abilities.










% Ability-based design
% Despite extensive research in blind navigation, most existing systems are limited by \textit{guiding}-based approach. Such an approach goes against the idea of ability-based design~\cite{wobbrock2018ability}, which calls for a shift in focus from disability to ability. Current systems do not consider VIPs' abilities: O\&M skills, non-visual sensory capabilities; while designing systems. Instead, these systems replace the capabilities [or abilities] of VIPs and remove them from the decision-making process, guiding them between predefined points through a fixed path that is optimized for efficiency. Clearly, there is a lack of understanding of what abilities do VIPs ``\textit{beyond guidance}'', and how should NASs be designed to offer VIPs these abilities.


% To this end, we investigate the roles, capabilities, and needs of all relevant stakeholders --- heeding the call for an interdependence perspective [cite] in assistive technology design --- to discover a new set of design guidelines for NASs.




















\begin{comment}

, delegating all decisions to the NASs




While these approaches provide an important functionality, i.e., getting from point A to point B, but navigation goes beyond guidance. Next, we discuss literature in wayfinding and navigation to elaborate

% just one stakeholder: VIPs, and do not take adequate account of the critical role that other stakeholders play in making indoor spaces navigable for VIPs. 

most existing navigation assistance systems (NASs) for VIPs guide them to their destination through fixed routes, delegating all decisions to the NASs~\cite{ahmetovic_navcog_2016, guerreiro_cabot_2019, yoon2019leveraging}. 

Some approaches have attempted to provide additional information about the environment to the VIPs during navigation. For instance, information about nearby landmarks~\cite{sato_navcog3_2019}, dynamic obstacles such as pedestrians~\cite{kayukawa_bbeep_2019}, and route previews~\cite{guerreiro_virtual_2020}. But they still focus on getting VIPs from point A to point B, without facilitating active engagement with this additional information. In fact, Guerreiro et al.~\cite{bai_virtual-blind-road_2018} found that providing route previews did not improve VIPs' navigation performance when used in conjunction with \textit{guidance-based} NASs.




Several approaches have been proposed to provide additional information to the user about the environment, they are still meant [to improve/complement] for route following [guidance]. 
% 1 - NavCog3: announces POIs in the vicinity
NavCog3~\cite{sato_navcog3_2019}, for instance, extends NavCog~\cite{ahmetovic_navcog_2016} to provide users information about the presence of semantic features and POIs (and a11y information) in the vicinity (e.g., doorways, shops). But this only adds information about a specific route, and not about an environment. Also, instead of providing this information, NASs should help VIPs explore these POIs through an active engagement with the environment --- helps build a better cognitive map of the space.
% 2 - Virtual Routes: helps learn routes before going to that place
Guerreiro et al.~\cite{guerreiro_virtual_2020} allows users to preview routes virtually before they visit the environment. However, the authors observed that while using a guidance system such as NavCog after virtually viewing the route, users tend to rely on the system and not on their prior learnings about the route. Furthermore, the system was only able to help with short routes, and not cognitive maps of the environments. [Cognitive maps are formed by active engagement with the environment.] 
% 3a - Bbeep: Dynamic obstacle avoidance
BBeep~\cite{kayukawa_bbeep_2019}, another example, helps VIPs avoid dynamic obstacle such as the pedestrians on the route. [a path clearing system]. Using a suite of sensors, fitted on a suitcase, it computes if a collision may happen with a walking pedestrian and then creates a sound to help non-VIPs (sighted pedestrians) to get out of the way. [doesn't make sense to include it here].
% 3b - Airport A11y and Nav.: 
NASs were also tailored to serve well in different environments. For instance, Guerreiro et al.~\cite{guerreiro_airport_2019} adapted NavCog~\cite{ahmetovic_navcog_2016} to solve a11y challenges in a complex and large open space such as the airport. Particularly, additional mechanisms were added to prevent veering and changes to the motion model were made for the system to accurately compute location of the user as they used moving walkways. Although the system allows VIPs to not take help from airport staff, it still does not help them make their own representations or explore the space, i.e., does nothing beyond guidance.
% 4 - Turn Right: fixing rotation errors
Ahmetovic et al.~\cite{ahmetovic_turn_2018} highlighted rotation errors that happen due to imprecise turn-by-turn navigation instructions, and proposed a deep learning framework to predict over-rotations~\cite{ahmetovic2019deep}. Even though this helps improve VIPs' accuracy in following directions, it hampers their ability to form maps or explore an environment even more. The litlle active engagement that they had would now be lost, since they know that the system will guide them, without really worrying about bumping into an obstacle or turning incorrectly. 


% 5 - Impact of expertise: personalise navigation instructions/messages
Ahmetovic et al.~\cite{ahmetovic_impact_2019} explore how the desirability of messages provided during assisted navigation varies based on users’ navigation preferences and expertise. The authors proposed verbosity level personalization in order to keep the users engaged in the current situational context while minimizing distractions.
keep users engaged. The authors found VIPs' need for navigation instructions reduces over time as their become more familiar with the environment. Although, this is a step towards thinking more about how would VIPs want to navigate with an NAS, what kind of help do they need from them, it is still based on the same turn-by-turn guidance approach which does not consider VIPs' desire for abilities beyond guidance.


\end{comment}

==> 2-RW/v3.tex <==
Our work builds on two areas of related work: research on NASs that aims to help VIPs navigate unfamiliar environments independently, and research on understanding VIPs' navigation needs and behaviors.


\subsection{Navigation Assistance Systems Approaches}

%Many researchers have sought to make independent navigation possible for VIPs. 
% Predominantly, most NASs do so by guiding VIPs to their destination.
Predominantly, NASs have followed a guidance-based approach that assists VIPs in getting from point A to point B.
% The predominant approach is to \textit{guide} VIPs to their destination.
For instance, NavCog~\cite{ahmetovic_navcog_2016} is a smartphone-based turn-by-turn navigation system that guides users to pre-defined points of interests (POIs) in the environment. 
CaBot~\cite{guerreiro_cabot_2019} is a suitcase-shaped robot that users grab in order to be guided to their destination, similar to how VIPs navigate with a guide dog. 
Although these systems reduce VIPs' cognitive load during navigation, they do so by requiring VIPs to play a passive role --- by simply following orders from the system --- instead of giving VIPs the freedom to explore and understand a space themselves. 


More recently, developers have begun to include more contextual and environmental information in their guidance-based NASs,
% to help VIPs get additional information along the routes to their destination.
to provide VIPs a better understanding of the environment.
For example, both Microsoft Soundscape~\cite{MSsoundscape} and NavCog3~\cite{sato_navcog3_2019} provide users additional information about the surroundings by announcing POIs and landmarks in their vicinity.
Guerreiro et al.~\cite{guerreiro_virtual_2020} propose an interactive virtual navigation app which allows users to preview and rehearse routes before they actually visit the environment.



Other accessibility- and navigation-related work in HCI has highlighted how crucial exploration is to navigation, arguing that guidance alone is not enough for independent navigation.
For example, Nair et. al~\cite{nair_toward_2020} describe the importance of looking around in navigation and propose a system called NavStick for making adventure video games more blind-accessible. Clemenson et. al~\cite{clemenson_rethinking_2021} recently argued that NAS designers need to rethink the role of GPS navigation systems so that they can facilitate active engagement with the world, rather than acting as simple guides from point A to point B.



Although recent research has emphasized the crucial role that exploration plays in navigation, most NAS research is still directed toward facilitating guidance only. In order for NAS research to begin facilitating \textit{exploration}, we need to understand
% in these other related fields, most NASs facilitate guidance only.
% However, despite the consensus about including these other aspects of navigation that emerge from exploration, we do not yet 
what means of exploration NASs should support and how NASs should support them.
Our work aims to address this research gap by investigating VIPs' needs and behaviors when navigating unfamiliar environments.

% Specifically, we identify different forms of exploration that VIPs find challenging to inform the design of NASs.
% In addition, our findings also inform design of future NASs that support exploration.
% VIPs' independent navigation endeavors.





\subsection{Importance of Exploration in Navigation}
Various strands of research in cognitive science indicate the importance of exploration in independent navigation. Specifically, the ability to explore environments leads to two primary cognitive benefits: formation of cognitive maps~\cite{o1978hippocampus, tolman1948cognitive} and active engagement with the environment~\cite{chrastil2015there, chrastil2013active}. Regarding cognitive maps, Tolman et al.~\cite{tolman1948cognitive} found that maps created via exploration have a flexible spatial information which allows for the maps to be accessed from any location. 

Regarding active engagement, Chrastil et al.~\cite{chrastil2015there} report that playing an active role in spatial decision making leads to a better spatial understanding of the environment. Furthermore, active engagement  contributes to spatial knowledge which can be useful in finding alternative routes~\cite{chrastil2013active}.

In addition to formation of cognitive maps and active engagement with the environment, many researchers have shown that the ability to explore unfamiliar environments has additional benefits --- specifically, development of cognitive abilities and improved overall brain health~\cite{clemenson2018environmental, clemenson2019improving, maguire1998knowing, maguire2000navigation, woollett2011acquiring}.

Our work is motivated by this cognitive science perspective. Given the importance of exploration in navigation, we see an opportunity to facilitate exploration for VIPs. To this end, we aim to understand challenges that VIPs face while exploring unfamiliar environments.


\subsection{VIPs' Navigation Needs and Behaviors}
Past research also examines VIPs' navigational needs and behaviors for the purpose of informing NAS design. 
% VIPs' needs are crucial in defining the goals of an NAS, while understanding their behaviors help determine the interaction design.
% While investigating user's needs help answer the question, `what should NASs do?', understanding the behaviors help answer the question, `how should NASs do it?'.
Lewis et al.~\cite{lewis_hearing_2015} interview a focus group of VIPs to determine users' requirements for effective guidance using NASs.
Similarly, Banovic et al.~\cite{banovic_uncovering_2013} interview both VIPs and O\&M trainers to understand the guidance that NASs provide can be made more informative to foster spatial learning.
By contrast, we seek to understand how NASs can be designed to facilitate exploration rather than guidance.



Ahmetovic et al.~\cite{ahmetovic_turn_2018} investigate VIPs' behaviors when following turn-by-turn directions to understand why VIPs sometimes make rotation errors when being guided. In a follow-up work, their findings informed the design of a deep learning framework that prevents over-rotations in guidance-based NASs~\cite{ahmetovic2019deep}.
In addition, Ahmetovic and another set of colleagues~\cite{ahmetovic_impact_2019} study how VIPs' information needs varies based on their navigation expertise. They find that NASs should adapt the verbosity of its instructions for VIPs to suit their level of expertise and enable them to stay engaged in the environment while navigating. 
Last, Scheuerman et al.~\cite{scheuerman2017learning} investigate how VIPs write navigation instructions to each other to inform the design of effective text-to-speech systems for giving directions to VIPs.


Our work focuses on understanding what means of exploration are challenging for VIPs when navigating unfamiliar environments, so that we can propose design guidelines and new types of functionality for NASs. We hope that our findings can lead to NASs becoming exploration assistance systems rather than guidance systems.  


\subsection{Collaboration in Navigation}



==> 2-RW/v4.tex <==


Research in cognitive science (Section~\ref{sec:cog-sci-RW}) has shown the importance of exploration to navigation~\cite{chrastil_active_2012, maguire_navigationrelated_2000, clemenson_improving_2019, konishi_spatial_2013, giudice_navigating_2018, golledge_geography_1993, clark-carter_efficiency_1986, chrastil_there_2015, chrastil_active_2013, tolman_cognitive_1948, okeefe_hippocampus_1978}, 
yet most NASs focus on guiding VIPs via turn-by-turn navigation~\cite{ahmetovic_navcog_2016, fallah_user_2012, bai_virtual-blind-road_2018,murata_smartphone-based_2018, ran_drishti_2004, riehle_indoor_2008, guerreiro_cabot_2019, kayukawa_bbeep_2019, kayukawa_guiding_2020, avila_soto_dronenavigator_2017, peng_indoor_2017, saegusa_development_2011, scheggi_cooperative_2014}. 
Although recent NAS approaches have taken important first steps toward facilitating exploration for VIPs~\cite{blum_spatialized_2013, paneels_listen_2013, MSsoundscape, sato_navcog3_2019}, many questions remain.
Here, we summarize the evolution of exploration in NASs (Section~\ref{sec:NAS-design-approaches}) and work on understanding VIPs' navigational needs and challenges
(Section~\ref{sec:understanding-needs-prefs}), describing how the present work advances these efforts.


% Motivated by the cognitive science perspective
% % (Section~\ref{sec:cog-sci-RW})
% , we focus on opportunities for rethinking current NAS design approaches (Section~\ref{sec:NAS-design-approaches}) to support exploration for VIPs. To this end, we address the research gaps in understanding VIPs' information needs and challenges around exploration to inform the design of future NASs (Section~\ref{sec:understanding-needs-prefs}).


% we 

\subsection{The Importance of Exploration in Navigation}
\label{sec:cog-sci-RW}


\revision{
% 
In general, two main forms of knowledge have been described in literature on navigation: \textit{route} knowledge and \textit{survey} knowledge~\cite{golledge_wayfinding_1999, ggolledge_cognitive_2000}. Route knowledge includes path from one point to another and landmarks along the path and is acquired via an egocentric reference frame (person-centered). In contrast, survey knowledge includes configuration of the space and is acquired via an allocentric reference frame (environment-centered). The process of exploration uses a combination of these to learn about the space and make navigation decisions on the fly.
% 
}


Various strands of cognitive science research indicate the importance of exploration to navigation. Specifically, the ability to explore environments leads to two primary cognitive benefits: the formation of cognitive maps~\cite{okeefe_hippocampus_1978, tolman_cognitive_1948} and the promotion of active engagement with the environment~\cite{chrastil_there_2015, chrastil_active_2013}. Regarding the formation of cognitive maps, Tolman et al.~\cite{tolman_cognitive_1948} 
found that maps created via exploration 
% have a flexible spatial information which allows for the maps to 
can be accessed and used from any location in the environment and not just from specific places or routes. 
Regarding the promotion of active engagement, Chrastil et al.~\cite{chrastil_there_2015} report that playing an active role in spatial decision-making leads to a better spatial understanding of the environment. This understanding can be useful in many situations, such as when the need to find an alternative route arises~\cite{chrastil_active_2013}.
In addition to these two benefits, many researchers have shown that the ability to explore unfamiliar environments can improve the development of cognitive abilities and improve overall brain health~\cite{maguire_navigationrelated_2000, clemenson_improving_2019, konishi_spatial_2013}.

This body of work reveals
% Inspired by these demonstrated benefits of exploration, we see 
the potential benefits that NASs could bring by facilitating exploration for VIPs. Since we do not yet understand how exactly NASs should be designed to support exploration for VIPs, our work aims to address this research gap.

% which has not yet been fully adopted by current NAS approaches due to lack of understanding about VIPs' needs and challenges around exploration.




% \subsection{Navigation Assistance System (NAS) Approaches}
\subsection{\revision{Tools for Supporting Exploration in Navigation}}
\label{sec:NAS-design-approaches}
%Many researchers have sought to make independent navigation possible for VIPs. 
% Predominantly, most NASs do so by guiding VIPs to their destination.
% NASs have predominantly followed a turn-by-turn navigation approach \cite{ahmetovic_navcog_2016, fallah_user_2012, bai_virtual-blind-road_2018,murata_smartphone-based_2018, ran_drishti_2004, riehle_indoor_2008, guerreiro_cabot_2019, kayukawa_bbeep_2019, kayukawa_guiding_2020, avila_soto_dronenavigator_2017, peng_indoor_2017, saegusa_development_2011, scheggi_cooperative_2014}.
% that assists VIPs in getting from point A to point B.
% % The predominant approach is to \textit{guide} VIPs to their destination.
% For instance, NavCog~\cite{ahmetovic_navcog_2016} is a smartphone-based turn-by-turn navigation system that guides users to pre-defined points of interests (POIs) in the environment. 
% CaBot~\cite{guerreiro_cabot_2019} is a suitcase-shaped robot that users grab in order to be guided to their destination, similar to how VIPs navigate with a guide dog. 
% Although these systems reduce VIPs' cognitive load during navigation, 
% such a destination-oriented approach results in a poor understanding of the environment~\cite{fenech_effects_2010, ishikawa_wayfinding_2008}, inhibits the process of ``experiencing the physical world''~\cite{leshed_car_2008}, and the user becomes a ``passenger of their own body''~\cite{ingold_being_2011}.


% Accessibility- and navigation-related work in human--computer interaction (HCI)~\cite{nair_toward_2020, clemenson_rethinking_2021} has highlighted how important exploration is to navigation, arguing that turn-by-turn navigation alone is not enough to support exploration in unfamiliar environments.
% For example, 

\revision{

}

Several recent works in human--computer interaction (HCI) have argued for NASs to facilitate exploration in addition to turn-by-turn guidance.
% have tried to incorporate certain elements of exploration to navigation- and accessibility-related . For example, 
Nair et al.~\cite{Nair2021a} recently highlighted the importance of exploration and the ability to look around when navigating, creating a system called NavStick for giving VIP players the ability to look around within adventure video games. Clemenson et al.~\cite{clemenson_rethinking_2021} recently argued that NAS designers should rethink the role of turn-by-turn navigation systems so that they can facilitate active engagement with the world.



NAS developers have also made efforts to facilitate exploration~\cite{blum_spatialized_2013, paneels_listen_2013, sato_navcog3_2019, MSsoundscape}. 
% and to learn about unfamiliar environments~\cite{guerreiro_virtual_2017, guerreiro_virtual_2020}
In-Situ Audio Services (ISAS)~\cite{blum_spatialized_2013} and NavCog3~\cite{sato_navcog3_2019}, for example, announce nearby points of interests (POIs) via speech and 3D-spatialized audio either during a route (via ``pushes'') or via search (``pulls''). Microsoft Soundscape~\cite{MSsoundscape} places audio beacons directly at the destination instead of giving them instructions at every turn, allowing users to determine their own routes. 





% While Guerreiro et al.~\cite{guerreiro_virtual_2020} propose an interactive virtual navigation application which allows users to preview and rehearse routes before they actually visit the environment. 


% More recently, developers have begun to enhance the turn-by-turn navigation approach by supporting more contextual information~\cite{paneels_listen_2013}, or by supporting spatial learning~\cite{guerreiro_virtual_2020}. However, these approaches limit VIPs' exploration to route-based context and learning. For example, both Microsoft Soundscape~\cite{MSsoundscape} and NavCog3~\cite{sato_navcog3_2019} announce points of interests (POIs) and landmarks in user's vicinity \textit{en route} to the destination. 
% These systems help VIPs answer the question ``what's around me?''~\cite{paneels2013listen}.





% --- allowing users to make their own navigation decisions, rather than acting as guides between two POIs.


% Question:
Although recent research has emphasized the crucial role that exploration plays in navigation and has made some notable contributions towards it, research in accessibility and cognitive science shows there is more to exploration than learning nearby POIs and the routes to destinations. Exploration in navigation includes learning about spaces and building an environment-centered cognitive map of spaces to make navigation decisions from~\cite{banovic_uncovering_2013, hersh_mental_2020, long_establishing_nodate}. 
Before our community can ever develop NASs to support these aspects, it is important for us to take a step back and gain a holistic understanding about what information VIPs need in order to explore and why VIPs find it difficult to gather this information in the first place.
Hence, our work does not introduce new technology, but instead aims to broaden our understanding about VIPs' needs and challenges around exploration.

% there is a lack of understanding about specific information that VIPs need and the challenges they face when exploring unfamiliar environments. Our work does not introduce new technology, but instead 
% aims to address this research gap by investigating VIPs' needs and challenges to inform the design of future NASs.
% when navigating environments by themselves, and by seeking assistance from others.

% Specifically, we identify different forms of exploration that VIPs find challenging to inform the design of NASs.
% In addition, our findings also inform design of future NASs that support exploration.
% VIPs' independent navigation endeavors.




% highlight the gap -> but we don't know 







\subsection{Understanding VIPs' Navigation Needs and Challenges}
\label{sec:understanding-needs-prefs}
% VIPs make up for their inability to gather visual information by seeking external support either from NASs or from other people in the environment. 
% We focus on identifying VIPs' information needs for in-situ exploration in unfamiliar environments (~section~\ref{sec:info-needs-RW}) and the challenges they face while collecting this information --- both by themselves and by seeking assistance from other people (section~\ref{sec:challenges-RW}).


Several studies have identified VIPs' information needs while navigating \cite{ahmetovic_impact_2019, williams_pray_2013, quinones_supporting_2011, lewis_hearing_2015, van_der_bie_guiding_2016, scheuerman_learning_2017, guerreiro_virtual_2020} and the challenges that VIPs face~\cite{giudice_use_2020, williams_just_2014, easley_lets_2016, thieme_i_2018, langdon_better_2016}, but most of them are aimed at informing the design of NASs that support turn-by-turn navigation. Our focus, on the other hand, is to understand VIPs' information needs and challenges regarding \textit{exploring} unfamiliar environments, which remains understudied~\cite{banovic_uncovering_2013}.




% \subsubsection{Information needs for navigation}
% \label{sec:info-needs-RW}

% Many reports have studied VIPs' information needs with an to inform the design of turn-by-turn navigation systems~\cite{lewis_hearing_2015, scheuerman_learning_2017}, but VIPs' information needs for exploration still remain understudied~\cite{banovic_uncovering_2013}. 
Lewis et al.~\cite{lewis_hearing_2015} interviewed a focus group of VIPs to determine user requirements for NASs, but only in the context of turn-by-turn navigation.
\revision{Specifically, most of their findings correlate with information about POIs, updates on progress about routes to the destination, and preference for notifications about whether users are following the system-generated routes or not. 
Unlike our work, which focuses on NASs that support exploration, Lewis et al.\ made proposals to \textit{guide} users to a destination instead of giving them the freedom to choose their own routes.}
Similarly, Scheuerman et al.~\cite{scheuerman_learning_2017} investigate how VIPs write navigation instructions to each other to better inform the design of turn-by-turn navigation systems. \revision{The authors study how VIPs represent distances, indicate directions, and reference landmarks; with an aim to propose design implications for providing NASs 
}



Banovic et al.~\cite{banovic_uncovering_2013} interview both VIPs and O\&M trainers to uncover VIPs' information needs for spatial learning. 
% The authors found that VIPs need four types of spatial information: high-level overview of the space, safety information (e.g., obstacles), information about places and activities of interest, and navigation information (e.g., routes and POIs). 
% While these findings establish that VIPs' information needs for exploration differ from that of turn-by-turn navigation, the specifications for each of these spatial information types is not concrete enough for NASs. For instance, we do not yet understand what it means to provide VIPs a ``high-level overview'' of the space to effectively support VIPs' exploration. 
Our work builds on Banovic et al.'s work in two ways. First, we shift our focus from spatial learning to in-situ exploration. In other words, we envision NASs helping users to ``figure things out'' on their own and make navigation decisions on the fly instead of learning a space to visit later on. 
% Second, we zoom-in on the specifications of spatial information that requires NASs' support.
Second, we investigate the exploration affordances that NASs should offer on a more specific level (RQ1). Banovic et al.\ found that VIPs desire a ``high-level overview'' of spaces, while we find in Sections~\ref{sec:RQ1-findings} and \ref{sec:RQ2-findings} that NASs should afford \textit{\revision{area} shape} information, \textit{layout} information, and assistance in communicating needs with others specifically, as Figure~\ref{fig:teaser}b illustrates.
% We also uncover the factors that affect VIPs' choice of spatial information (the second part of RQ1), building on prior work finding that variations in navigation preferences and behaviors  between individuals play an important role in designing NASs~\cite{ahmetovic_impact_2019, williams_pray_2013}. 


Researchers have found that
VIPs' navigation strategies are different from sighted people's~\cite{swobodzinski_indoor_2009} and that
variations in individual VIPs' navigation preferences and behaviors play an important role in designing NASs~\cite{ahmetovic_impact_2019, williams_pray_2013}. 
\revision{For instance, Williams et al.~\cite{williams_pray_2013} identify personality and scenario attributes that impact VIPs' daily-life navigation preferences. Ahmetovic et al.~\cite{ahmetovic_impact_2019} made proposals for NASs to adapt to the verbosity of navigation instructions to suit user's level of expertise, ensuring that they stay engaged in the during navigation.}
As a result, as part of our RQ1 investigation,
% We follow this research in two ways. First, 
we also uncover the factors that affect VIPs' choice of spatial information (Section~\ref{sec:factors-info-needs}) \revision{to identify factors that influence VIPs preferences for spatial information and to understand which specific dimensions of spatial information does each of these factors dictate.}


% Williams et al~\cite{williams_pray_2013} revealed that VIPs' navigation behaviors change based on both internal factors (such as individual personalities) and external factors (such as location). 


% Ingunn Moser [37] who describes how disability is configured through the social and material environment. Interactions within the social and material world that ability or disability is constructed [cf. 23]. As a result, "ability is not something a person is, but something a person becomes".


% To build an understanding of the interactions that create disability, we draw on work by Ingunn Moser [37], who describes how disability is configured through the social and material environment. Interactions within the social and material world that ability or disability is constructed [cf. 23]. As a result, ability or 3dis-
%  [37, p.668]. For example, whether a person is more or less able to climb a mountain may not only be determined by bodily fitness, but by how they interact with the physical world (using e.g. ladders, climbing tools or GPS devices) and other people, who may offer help in critical moments. By understanding how such situated negotiations oc-
% cur, our interests lie not just in overcoming bodily limits or disabilities, but in extending ability, or enlarging capability.


% FACTORS AND DIMENSIONS:
% We also identified three factors that influence preferences for spatial information between individuals: 
% (1) their onset of vision impairments, (2) their inherent sociability, and (3) their O\&M proficiency and choice of mobility aid. Understanding \textit{how} these factors dictate the format, source, and amount of spatial information VIPs need leads to an inclusive design of future NASs that support VIPs' exploration.


% Ahmetovic et al.~\cite{ahmetovic_turn_2018} investigate VIPs' behaviors when following turn-by-turn directions to understand why VIPs sometimes make rotation errors when being guided. In a follow-up work, their findings informed the design of a deep learning framework that prevents over-rotations in guidance-based NASs~\cite{ahmetovic_deep_2020}.
% In addition, Ahmetovic and another set of colleagues~\cite{ahmetovic_impact_2019} study how VIPs' information needs varies based on their navigation expertise. They find that NASs should adapt the verbosity of its instructions for VIPs to suit their level of expertise and enable them to stay engaged in the environment while navigating. The present research informs 


% VIPs' information needs have been shown to differ from that of sighted people~\cite{}. As s result, it is important to understand VIPs' information needs. Prior work has identified VIPs' information needs with respect to descriptions for grocery~\cite{}


% \subsubsection{Challenges in navigation}
% \label{sec:challenges-RW}


% Research shows that VIPs' navigation strategies differ from that of sighted people~\cite{swobodzinski_indoor_2009}. As a result,

Last, prior work has identified many \textit{social} challenges related to navigation that VIPs face as well: specifically, challenges in comprehending assistance from other people~\cite{williams_just_2014, guerreiro_airport_2019}, in navigating through environments that are predominantly occupied by sighted people~\cite{easley_lets_2016}, and in negotiating these differences with other people~\cite{thieme_i_2018}. 
VIPs' ability to explore is best viewed within an interdependence framework~\cite{bennett_interdependence_2018, vincenzi_interdependence_2021} --- that is, as a collective effort involving other people, as Figure~\ref{fig:teaser}(b) illustrates.
In this spirit, in RQ2
% we study how NASs can explicitly help VIPs communicate  into exploration tools by designing NASs that act as an intermediary between VIPs and sighted people around them.
we investigate not only VIPs' internal challenges when trying to explore, but also 
% we investigate
how VIPs interact with people when trying to explore. 
Our aim with this latter aspect of RQ2 is to understand how NASs can bridge communication gaps and foster collaboration as yet another means of exploration.



% Our work also understands this difference between VIPs and sighted people, but in the context of collaboratively exploring unfamiliar environments (Section~\ref{sec:colab_exploration}) as opposed to sighted people taking the lead in guiding VIPs. We find many of the same challenges such as social pressures due to others in the environment and comprehending verbal assistance, but the design implications differ because of our interdependence perspective~\cite{bennett_interdependence_2018, vincenzi_interdependence_2021} and our focus on informing NASs that support exploration instead of turn-by-turn navigation.


% % We also found some of the same issues that VIPs face in exploration as well. However, unlike these papers that only understand these issues to later replace people with NASs, we found that in context of exploration that instead of replacing people we could in fact 
% transform them into exploration tools by designing NASs that act as an intermediary between VIPs and sighted people around them.



% "we suggest that technology should not try and replace human assistance, but instead enable people with VI to better identify and interact with other people in-situ." -- \cite{thieme_i_2018}


% Research shows that VIPs' navigation strategies are different from that of sighted people~\cite{swobodzinski_indoor_2009}. 
% As a result, 
% several researchers have studied how these differences cause NAS designers' bias towards building technologies that VIPs find hard to use~\cite{williams_just_2014} and how they affect VIPs' ability to receive guidance assistance from sighted people when navigating collaboratively~\cite{thieme_i_2018, easley_lets_2016, vincenzi_interdependence_2021}. 
% We take up this call and identify challenges that VIPs face in exploring unfamiliar environments collaboratively. While some challenges that prior research discovered in context of turn-by-turn navigation systems also came up in during our interviews, the design implication differ in context of our work that focuses on informing design of NASs that support exploration.










% We conducted a
% similar study with blind participants and sighted companions,
% finding many of the same teamwork negotiations and social
% interactions. Following we explain the findings from this study as
% well as findings from single-person observations and focus group
% discussions related to navigation technology needs.


% the difference in our aim to inform the design NASs  

% Williams and another set of colleagues~\cite{williams_just_2014} point out that current NASs should consider these differences when guiding users. W


% inform the design of a personal pedestrian navigation device (is turn by turn). how sighted assistance creates complications for VIPs -- mismatch between info provided and what VIPs need. Their main aim was to understand where other people were failing, and how can NASs do that part better. Also, path and route oriented instead of in-situ decision making, Their view of NASs is to replace people with NAS.


% Thieme et al.~\cite{thieme_i_2018}
% explore how abilities become negotiated. six athletes and spectators during Rio Olympics. Their approach is to see where people are failing and suggest how NASs can smooth this interaction -- instead of replacing them with NASs (like \cite{williams_just_2014} does). We follow this second approach wherever possible.


% Easley et al.~\cite{easley_lets_2016} 
% exploring social norms in predominantly blind environments and discuss how how these may be different from what sighted people expect. Design tech that can bridge the gap between this mismatch so that VIPs can navigate in environments with sighted people in them. Design for both social acceptance and social interactions -- we consider these differences in context of in-situ exploration.


% so that we can propose design guidelines and new types of functionality for NASs. We hope that our findings can lead to NASs becoming exploration assistance systems rather than just being turn-by-turn navigation systems.  




% ------------------------------------
% ------------------------------------


% VIPs' needs are crucial in defining the goals of an NAS, while understanding their behaviors help determine the interaction design.
% While investigating user's needs help answer the question, `what should NASs do?', understanding the behaviors help answer the question, `how should NASs do it?'.
% Lewis et al.~\cite{lewis_hearing_2015} interview a focus group of VIPs to determine users' requirements for effective guidance using NASs.
% Similarly, Banovic et al.~\cite{banovic_uncovering_2013} interview both VIPs and O\&M trainers to understand the guidance that NASs provide can be made more informative to foster spatial learning.
% By contrast, we seek to understand how NASs can be designed to facilitate exploration rather than guidance.



% Ahmetovic et al.~\cite{ahmetovic_turn_2018} investigate VIPs' behaviors when following turn-by-turn directions to understand why VIPs sometimes make rotation errors when being guided. In a follow-up work, their findings informed the design of a deep learning framework that prevents over-rotations in guidance-based NASs~\cite{ahmetovic2019deep}.
% In addition, Ahmetovic and another set of colleagues~\cite{ahmetovic_impact_2019} study how VIPs' information needs varies based on their navigation expertise. They find that NASs should adapt the verbosity of its instructions for VIPs to suit their level of expertise and enable them to stay engaged in the environment while navigating. 
% Last, Scheuerman et al.~\cite{scheuerman2017learning} investigate how VIPs write navigation instructions to each other to inform the design of effective text-to-speech systems for giving directions to VIPs.



% \cite{williams_pray_2013} -- how people use tech in daily life navigation and what factors (personal and situational) affect the use of tech. How differences between individuals play an important role in designing tech. Our work furthers these by understanding what factors influence VIPs' need for spatial information and then discuss how NASs should incorporate these specific differences. Personas --- should we use these personas to say who needs what kind of navigation? CHALLENGES IN NAVIGATION AND HOW DO THEY USE TECH TO SOLVE IT? O\&M training part is common. We identify SPECIFIC factors that affect exploration difference between individuals.

% While some are common, we note that the design implications for these factors is different because the aim in to design tech to support exploration.

% \cite{williams_just_2014} inform the design of a personal pedestrian navigation device (is turn by turn). how sighted assistance creates complications for VIPs -- mismatch between info provided and what VIPs need. Their main aim was to understand where other people were failing, and how can NASs do that part better. Also, path and route oriented instead of in-situ decision making, Their view of NASs is to replace people with NAS.


% \cite{thieme_i_2018} explore how abilities become negotiated. six athletes and spectators during Rio Olympics. Their approach is to see where people are failing and suggest how NASs can smooth this interaction -- instead of replacing them with NASs (like \cite{williams_just_2014} does). We follow this second approach wherever possible.


% Easley et al.~\cite{easley_lets_2016} 
% exploring social norms in predominantly blind environments and discuss how how these may be different from what sighted people expect. Design tech that can bridge the gap between this mismatch so that VIPs can navigate in environments with sighted people in them. Design for both social acceptance and social interactions -- we consider these differences in context of in-situ exploration.


% Our work focuses on understanding what means of exploration are challenging for VIPs when navigating unfamiliar environments, 





% Errors are not all bad: abdolrahmani2017embracing, abdolrahmani2016not




% --------------------------------------------
% |-------------- WRITING DUMP --------------|
% --------------------------------------------


% \todo{can be removed}\hl{Specifically, we aim at understand \textit{what} information do VIPs need and \textit{how} should NASs support VIPs in gathering this information.}




% VIPs miss out on the rich visual information about the environment and hence, interact with external aids such as NASs or other people to 

% VIPs' inability to gather information visually \hl{makes them}\todo{fix} interact with the

% VIPs' inability to gather visual information requires them to interact with the environment to fill this gap. 



% Past research examines VIPs' needs and challenges to inform NAS design. More specifically, understanding the information needs help identify \textit{what} VIPs want assistance with (section~\ref{sec:info-needs-RW}) and understanding the challenges help identify \textit{how} VIPs should be assisted (section~\ref{sec:challenges-RW}). In our work, we investigate VIPs' information needs for exploring unfamiliar environments in situ and the challenges they face while doing so.


% Past research also examines VIPs' navigational needs and challenges for the purpose of informing NAS design. While some people understand only in context of VIPs alone, and other do so when they navigate with the assistance of others. To obtain a holistic understanding, we investigate both these perspectives --- independent and collaborative --- specifically with respect to supporting in-situ exploration. \todo{Improve language}

==> 3-Methods/v1.tex <==
% List as RQs (navstick, acoustic minimap paper) 
% We conducted a series of ... We investigate the following two RQs
% RQ-1: What factors shape VIPs' O\&M practices, navigation goals, and challenges when navigating unfamiliar environments?
% RQ-2: How do the behaviour of non-VIPs supports and/or hinders VIPs’ navigation goals
% In order to investigate the first, we asked VIPs to share their experiences and challenges faced by them in specific environments. ....
% RQ-3: What are the design requirements for an NAS that arise from RQ-1 and RQ-2?
% In order to investigate the second, we asked VIP participants to share their prior interactions with different people. We then asked non-VIP participants about their interactions with VIPs to better understand both perspectives. ... remove repitition

% RQ-1: What factors characterize VIPs' attitudes toward navigation in unfamiliar environments?

(more empirical by asking /walking through different people, diff scenarios. in contrast to just getting what users prefer) (compare to prior work, what's diff we did)

% RQ-2: What are the O\&M practices, goals, challenges,and preference in assistance from others when navigating unfamiliar environments
We conducted a series of semi-structured interviews with VIPs and non-VIPs who influence their navigation attitudes: O\&M trainers, staff members of businesses, and leaders of VIP-serving organizations. Our goal is to investigate VIPs’ O\&M practices, navigation goals, and challenges, and we do this by understanding VIPs' past experiences and their interactions with others in everyday situations. We also want to understand how the behaviour of non-VIPs supports and/or hinders VIPs’ navigation goals. To this end, we asked VIP participants to share their experiences and challenges faced by them in specific environments. Further, to elicit the impact of non-VIPs on the attitudes of VIPs, we first asked VIP participants to share their prior interactions with different people, and then asked non-VIP participants about their interactions with VIPs to better understand both perspectives. Finally, we explored possible ways in which NASs can better serve VIPs with diverse preferences, and also mitigate challenges that are caused due to the behaviour of non-VIPs.
% Add Table with VIPs info

\subsection{Participants}

We recruited a total of fourteen participants: eight visually impaired people (seven male and one female; aged 18 to 36), two O\&M trainers (two females), two leaders of VIP-serving organizations (one male and one female), and two business staff members working who interact with VIP customers (one male and one female). 

We recruited VIPs through online social media platforms such as Reddit (r/blind), and private Facebook groups. All eight participants were white cane users. Six of them were totally blind, and two were legally blind. Six were blind by birth, and two developed vision impairments at the ages of one and four. Three identified they had color perception and three did not use vision information in their daily lives at all. All participants had experience of using navigation technologies such as AIRA~\cite{} and Google Maps~\cite{}. All eight participants live in the U.S.

We collaborated with a leading blind serving organization in a major metropolitan city in the U.S. The organization offers a wide variety of services, including training in orientation and mobility, assistive technology ,and daily living skills; low vision eye care; employment/placement services; and rehabilitation programs designed specifically for children and senior citizens. In addition, we recruited the leader of the Office of Disability Services(ODS) of a large university. 

We recruited one O\&M trainer through each of these organizations as part of ---. One has been working with --- over the past --- years. They specialize in ---. Whereas the other O\&M trainer has been working over the --- years… [find more descriptors]

We recruited two staff members: one works at a local bookstore near our institution, and the other worked at a major department store. We met the bookstore employee by visiting local businesses around our institution and identifying employees who interact with VIP customers frequently. To recruit the department store employee, we sent out emails through our personal network and snow-balling.

% why did we recruit them? We recruited them as part of research questions 2, Why these people? 
% the two can be directly referred.

\subsection{Procedure}

% RQ-1 and RQ-2

We conducted the interviews using open-ended, semi-structured questions. The questions consisted of four major subsections, and for different stakeholders, we followed different structures of sections and questions generated before the interview through discussion and pilot interviews.  Each section comprised of 6-8 open-ended questions and lasted 10-20 minutes. We interviewed the bookstore employee  at the store itself, and we interviewed all other participants via a video-conference. Each interview lasted 60-90 minutes in total, and we compensated participants \$25 for their time. The study was approved by our institution's IRB. 

% RQ-1
% For our interviews with VIPs as part of RQ1, we [BLANK].
For VIPs, in order to fully understand participants’ current indoor navigation situation and possible future technology solution, we divided the interview into four sections, each discussing a different topic: VIPs’ background and history of O\&M practices, walk-through, interaction with other stakeholders, and use of assistive technology. In the first session, we investigated participants’ background including their level of vision loss and their reliance on vision information, which could help us determine the current vision situation of participants. In the second session, we walked through with participants about their indoor navigation experience and opinions to understand their navigation approach. In the third part, we asked them about their interaction with other stakeholders such as O\&M trainers, friends/families and strangers, and this could help us acquire their attitude of asking for help from others. At last, we let the participants describe the technologies they use in their daily life through indoor navigation.

% RQ-2
For other stakeholders, we also divided the questions into four parts but different from Questions for VIPS because we want to investigate their experience in terms of helping VIPs more. First, we let them walk through the experience of them helping VIPs. Second, we focused on their roles and capabilities in terms of helping VIPs. After that, we obtained the collaboration between them and other stakeholders. At last, we asked them about technologies that could help them, which help us understand current technologies they use to help blind people and their opinions on future technology development. Note that since these stakeholders had different capabilities and needs, questions within each section were slightly different and the sequence might differ.



\subsection{Data Analysis}

Having participants’ consent, we recorded full interviews with all 13 participants and transcribed all the recordings into text. After transcribing, iterative and inductive approaches were taken during qualitative coding by all researchers. Each text was distributed to at least two researchers and was fully gone over to discover bullet points and patterns individually. The two researchers periodically discussed their individual coding efforts for reconciliation through group consensus. After multiple rounds of coding and several group discussions, we defined topics and themes for each stakeholder and group these quotes into points matched with the topics. The findings were generated and examined through patterns of the topics and quotes. 
% how many researchers went through it, unclear
% Cohen Kappa score? [-] Collectively work and come to consensus [x]

% For our thematic analysis process, we first transcribed each semi-structured interview, then one authors performed open-coding [1] on the transcripts. Following best practices for grounded theory as described by Charmaz [2], we were simultaneously engaged in analysis and data collection, iteratively constructing our analytic frame and updating our question prompts for future interviews as we synthesized and identified emerging themes. We iteratively reviewed and refined these into a closed set of codes, which we then re-applied to the transcripts as we performed additional interviews. Because we were following a grounded theory approach, we did not need to compute inter-rater reliability [3].

% [1] Anselm Strauss and Juliet Corbin. 1990. Open coding. Basics of qualitative research: Grounded theory procedures and techniques 2, 1990 (1990), 101–121
% [2] Charmaz, Kathy. Constructing grounded theory. sage, 2014.
% [3] McDonald, Nora, Sarita Schoenebeck, and Andrea Forte. "Reliability and inter-rater reliability in qualitative research: Norms and guidelines for CSCW and HCI practice." Proceedings of the ACM on Human-Computer Interaction 3.CSCW (2019): 1-23. 

==> 3-Methods/v2.tex <==
We conducted a series of semi-structured interviews, first with VIPs and then with people who they constantly mentioned during the interviews as having influenced their navigation goals and preferences --- namely, O\&M trainers, store employees (of nearby stores), and people who are in leadership positions of blind-serving organizations. Through these interviews, we aim to answer the first research questions: \textit{What abilities do VIPs want from NASs ‘\textit{beyond guidance}’, based on their experience navigating unfamiliar environments?}
% \begin{itemize}
%     \setlength{\itemindent}{.3in}
%     \item [(\textbf{RQ-1})] What are VIPs' navigation goals \textit{beyond guidance}, i.e., besides simply going from one point to another? 
%     \item [(\textbf{RQ-2})] What factors influence how important individual VIPs view these navigation goals?
% \end{itemize}
In order to investigate this research question, we conducted extensive interviews with VIPs to understand their background, their history of O\&M practices, walkthroughs of daily navigational routines and challenges, how they interact with other people in those scenarios, anspecific instancesd their use of assistive technologies. 
We asked both VIP and non-VIP participants to recall and walk us through examples of their past encounters and interactions with each other. Soliciting experiences from both perspectives helped us corroborate the findings.\todo{update this}
% identify both internal and external factors that may influence VIPs' navigation goals.


% Internal: O&M Skills and non-visual skills
% External: How others can force VIPs to change their goals and play an active or passive role.

%Based on our findings, we explored possible ways in which NASs can help VIPs achieve these navigation goals while keeping in mind the factors that influence these goals.

% VIPs’ background and history of O\&M practices,  walk-through (recall), interaction with other stakeholders, and use of assistive technology.

% we asked non-VIP participants to walk through an experience of them helping a VIP.


\subsection{Participants}
% \todo{Ready!}
\begin{table*}[t]
  \centering
    \begin{tabular}{ c  c  c  c  c c} 
    \hline
     \textbf{ID} & \textbf{Age} & \textbf{Gender} & \textbf{Visual Impairment} & \textbf{Mobility Aid} & \textbf{Development of Impairment} \\
    \hline
    P1 & 18 & Female & No usable vision & White cane & From birth\\
    P2 & 22 & Male & Otherwise visually impaired & White cane & From birth\\
    P3 & 36 & Male & No usable vision & White cane & From birth\\
    P4 & 25 & Male & No usable vision & White cane & four years old\\
    P5 & 21 & Male & No usable vision & White cane & From birth\\
    P6 & 23 & Male & No usable vision & White cane & From birth\\
    P7 & 25 & Male & Otherwise visually impaired & White cane & one year old\\
    P8 & 33 & Male & No usable vision & White cane & From birth\\
    \hline
    \end{tabular}
    \caption{Demographics of visually impaired participants.}
    \label{tab:participants}
\end{table*}

We recruited a total of fourteen participants, eight VIPs (Table~\ref{tab:participants}) and six other people from groups who the VIPs reported as playing a big part in shaping their opinions and behaviors around navigation. The other people, i.e., non-VIPs, included two O\&M trainers, one of whom leads O\&M services at a major blind-serving organization; two other leaders of VIP-serving organizations; and two employees of local stores who regularly interact with VIP customers. 


We recruited the visually impaired participants by posting to online forums and social media platforms popular among the community \textit{(exact forums and platforms anonymized for submission)}. All eight visually impaired participants were white cane users. Six participants (P1, P3-6, P8) had no usable vision, and the other two (P2, P7) identified themselves as being otherwise visually impaired. Six participants were blind from birth, while two developed vision impairments at the ages of one (P7) and four (P4). Three of the totally blind participants (P1, P6, P8) reported that they could perceive light slightly but that their perception of light does not help them with navigation. The other Three totally blind participants (P3, P4, P5) reported to have no visual perception whatsoever. All eight participants lived in the United States, spread across seven different states.

% We collaborated on this research with a leading blind-serving organization in the United States.
In addition to the VIPs, we recruited two leaders from a leading blind-serving organization in the United States as participants: their assistive technology director and their director of O\&M services. 
% (Gus: Program Director of Assistive Technology Services)
% Caitlin: Vision Rehabilitation Therapist, Orientation and Mobility Specialist
%We recruited one of the leaders of this organization, who has been working with the organization over the past decade, as a participant in our study, and the organization .
In addition, we recruited the assistive technology manager of the Office of Disability Services (ODS) of a large university. Both organizations offer a wide range of services to VIPs, including resources for O\&M training, rehabilitation programs, and assistive devices. We recruited our second O\&M trainer through the ODS. 
% The O\&M trainer at the blind-serving organization also leads the O\&M efforts at the organization. 
The O\&M trainers have over 10 and 15 years of experience in providing O\&M training to VIPs, respectively.


Last, we recruited two store employees: one from a local bookstore and one from a major department store. We became acquainted with the bookstore employee by visiting local businesses around our institution and asking employees about the extent that they interact with VIP customers. We recruited the department store employee by emailing major department store managers in our institution's surrounding area.

\subsection{Procedure}
% Structure it this way:
% We had two different sets of questions for each RQ. 
% For RQ-1, we ....
% For RQ-2, - for VIPs, and then for non-VIPs

We conducted the interviews using open-ended, semi-structured questions. We interviewed the bookstore employee in person during working hours and all other participants via video-conference. Each interview lasted 60-90 minutes and the participants were compensated \$25 for their time. The study was approved by our institution's IRB. 



\todo{review}
To investigate the proposed research questions, all interviews consisted of four major subsections. The interviews with VIPs contained: VIPs’ background and history of O\&M practices,  walk-through, interaction with other stakeholders, and use of assistive technology. The interviews with non-VIPs contained: experiences helping VIPs, stakeholder roles, interactions with other stakeholders, and current technologies used. Each section comprised of 6-8 open-ended questions and lasted 10-20 minutes. To formulate the open-ended questions for each section, we conducted pilot interviews with different stakeholders.  

We interviewed VIPs to understand their navigation goals and experiences  with NASs. All of the subsections in the interviews with VIPs(listed above) helped us to explore RQ-1. To investigate participants’ level of vision loss and their reliance on visual information, the first section covered participants’ basic background. Then, to learn about VIPs' navigation goals we used the second section to ask participants to walk through their experiences and opinions regarding indoor navigation. We also used the third section to ask participants about their interactions and expectations with other stakeholders such as O\&M trainers, friends/families and strangers. Lastly, to learn about VIPs' experiences with current NASs, the fourth section asked participants to describe the technologies they use in their daily life when navigating indoors.

The subsection regarding VIP participants' interaction with other stakeholders also helped us to explore RQ-2. To better understand the factors that impact VIPs' navigation goals, this section asked participants about their interactions and expectations with other stakeholders. We also interviewed other stakeholders to understand current VIPs' navigation goals from various perspectives. The subsection regarding non-VIP participants' experiences helping VIPs allowed us to further understand RQ-2. In order to learn about how other stakeholders interact with VIPs, we asked non-VIP participants' to walk through an experience of them helping a VIP. Understanding the interactions between VIPs and other stakeholders enabled us to identify various factors that impact VIPs' navigation goals. 

\subsection{Data Analysis}
We audio-recorded all interviews during the study, which produced over 18 hours of recordings. For our thematic analysis, we first transcribed each semi-structured interview, then the primary author along with one researcher collaboratively performed open-coding~\cite{strauss1998open} on these transcripts. Following the grounded theory approach~\cite{charmaz2014constructing}, we simultaneously performed data analysis and collection, iteratively refining our analytic frame while also updating the questions for future interviews as we identified emerging themes. During the process of data collection, the primary author conducted weekly meetings to review the themes and refine them into a closed set of codes, which the research team re-applied to the transcripts to reach a "group consensus"~\cite{saldana2021coding}. Since we followed a grounded theory approach, we did not seek agreement via measures like Cohen's Kappa to establish inter-rater reliability ~\cite{mcdonald2019reliability}.

==> 3-Methods/v3.tex <==
We conducted a series of semi-structured interviews, first with VIPs and then with people who they constantly mentioned during the interviews as having influenced their navigation behaviors. 
Through these interviews, we aim to answer our first research question (RQ1): \textit{What means of exploration are challenging for VIPs when navigating unfamiliar environments?} We will use our findings from RQ1 to form design 
guidelines for NASs (RQ2; Section~\ref{sec:DGs}) and suggest specific visions for future research on NASs (RQ3; Section~\ref{sec:visions}).
% We asked VIPs questions to 
% % we conducted extensive interviews with VIPs to
% understand their background, their history of O\&M practices, their daily navigational routines and challenges, how they interact with other people in those scenarios, and their use of assistive technologies for navigation. 
% We asked both VIP and non-VIP participants to recall and walk us through examples of their past encounters and interactions with each other. Soliciting experiences from both perspectives helped us corroborate the findings.\todo{update this}

\subsection{Participants}
% \todo{Ready!}
\begin{table*}[t]
  \centering
    \begin{tabular}{ l  c  c  l  c} 
    \hline
     \textbf{ID} & \textbf{Age} & \textbf{Gender} & \textbf{Visual Impairment (Onset)} & \textbf{Mobility Aid}  \\
    \hline
    P1 & 18-25 & Female & No usable vision (from birth) & White cane \\
    P2 & 18-25 & Male & Otherwise visually impaired (from birth) & White cane \\
    P3 & 26-35 & Male & No usable vision (from birth) & White cane \\
    P4 & 18-25 & Male & No usable vision (from the age of four) & White cane \\
    P5 & 18-25 & Male & No usable vision (from birth) & White cane \\
    P6 & 18-25 & Male & No usable vision (from birth) & White cane \\
    P7 & 18-25 & Male & Otherwise visually impaired (from the age of one) & White cane \\
    P8 & 26-35 & Male & No usable vision (from birth) & White cane \\
    \color{magenta}{P9} & \color{magenta}{18-25} & \color{magenta}{Female} & \color{magenta}{Otherwise visually impaired (from birth)} & \color{magenta}{White cane} \\
    \color{magenta}{P10} & \color{magenta}{26-35} & \color{magenta}{Female} & \color{magenta}{No usable vision (from the age of four)} & \color{magenta}{White cane} \\
    \color{magenta}{P11} & \color{magenta}{56-65} & \color{magenta}{Female} & \color{magenta}{No usable vision (from the age of 20)} & \color{magenta}{Guide dog} \\
    \color{magenta}{P12} & \color{magenta}{66-75} & \color{magenta}{Female} & \color{magenta}{No usable vision (from the age of 26)} & \color{magenta}{Guide dog} \\
    \hline
    \end{tabular}
    \caption{Demographic information of visually impaired participants.}
    \label{tab:participants}
\end{table*}\todo{pending interview for P12}

We recruited a total of fourteen participants: eight VIPs and six other people from groups who the VIPs reported as playing a big part in shaping their behaviors around navigation. Table~\ref{tab:participants} summarizes the demographics of our eight visually impaired participants.
The six other people included two leaders of a major blind-serving organization, a manager of disability services at a large university, an O\&M trainer, and two employees of local stores who regularly interact with VIP customers. 


We recruited the visually impaired participants by posting to online forums and social media platforms popular among the community \textit{(exact forums and platforms anonymized for submission)}. 
All eight visually impaired participants were white cane users. 
Six participants (P1, P3-6, P8) had no usable vision, and the other two (P2, P7) identified themselves as being otherwise visually impaired. 
Six participants were blind from birth, while two developed vision impairments at the ages of one (P7) and four (P4). 
Three of the blind participants (P1, P6, P8) reported that they have limited light perception but it does not help them with navigation. 
The other three totally blind participants (P3, P4, P5) reported to have no visual perception whatsoever. 
All eight participants lived in the United States, spread across seven different states.

% Through our collaboration with a leading blind-serving organization, we recruited two of its leaders as participants: their assistive technology director and their director of O\&M services.


The two leaders that we recruited from the major blind-serving organization were their assistive technology director and their director of O\&M services. We recruited them through our collaboration with the organization. 
We recruited the manager of disability services for the large university via email. 
Both the blind-serving organization and the university's disability services department offer a wide range of services to VIPs, including resources for O\&M training, rehabilitation programs, and assistive devices.

We recruited the O\&M trainer with the help of the university's disability services department. They self-reported as having over 15 years of experience providing O\&M services to VIPs.

Lastly, the two store employees that we recruited were from a local bookstore and a major department store. 
We met the bookstore employee after we visited local businesses around our institution and asked employees about the extent to which they interact with VIP customers. 
We recruited the department store employee by emailing major department store managers in our institution's surrounding area.

\subsection{Procedure}
We performed two series of semi-structured interviews: the first with visually impaired participants, and the second with people who the VIPs stated as significantly affecting their everyday navigation behaviors. We refined our interview questions through pilot interviews and additional discussion with the VIPs on our research team.

In the first series of interviews, we asked VIPs open-ended questions to understand their background, role of visual information (if any), their history of O\&M practices, and their use of assistive technologies for navigation. In order to understand their daily navigational challenges even further, along with how they interact with other people in those scenarios to overcome those challenges, we then asked the VIPs to recall and walk us through specific examples of their past experiences of navigating unfamiliar environments.

In the second series of interviews, we asked the six non-VIPs about their backgrounds, their frequency of interactions with VIPs, their role in assisting VIPs in navigation, and their experience with assistive technologies for VIPs (if any). We then ask them to recall and walk us through their past experiences interacting with VIPs, specifically instances in which they helped VIPs with navigation-related tasks. Soliciting experiences from both VIP and non-VIP perspectives helped us corroborate our findings.

We interviewed the bookstore employee in person during working hours and all other participants via video-conference. Each interview lasted 60--90 minutes and the participants were compensated \$25 for their time. The study was approved by our institution's IRB. 




% We asked both VIP and non-VIP participants to recall and walk us through examples of their past encounters and interactions with each other. Soliciting experiences from both perspectives helped us corroborate the findings.\todo{update this}



% \todo{review}
% Each interview was composed of four major subsections in order to help us investigate which forms of exploration are challenging for VIPs when navigating unfamiliar environments. 
% The interviews with VIPs contained: VIPs’ background and history of O\&M practices,  walk-through, interaction with other stakeholders, and use of assistive technology. 
% The interviews with non-VIPs contained: experiences helping VIPs, stakeholder roles, interactions with other stakeholders, and current technologies used. Each section comprised of 6-8 open-ended questions and lasted 10-20 minutes. 
% To formulate the open-ended questions for each section, we conducted pilot interviews with different stakeholders.  


% We also interviewed other stakeholders to further answer RQ1, by understanding current VIPs' exploratory navigation goals from various perspectives. 
% In order to learn about how other stakeholders interact with VIPs, we asked non-VIP participants' to walk through an experience of them helping a VIP. 
% Understanding the interactions between VIPs and other stakeholders enabled us to identify various factors that impact VIPs' ability to fulfill their exploration preferences when navigating. 

\subsection{Data Analysis}
We analyzed our interview data via a thematic analysis process. We started by transcribing each semi-structured interview (over 18 hours of recordings in total), then performed open-coding~\cite{strauss1998open} on these transcripts to arrive at an initial set of codes. While we were still interviewing the participants, the primary author and one of the other researchers collaboratively performed the open coding.
Following the grounded theory approach~\cite{charmaz2014constructing}, we simultaneously performed data analysis and collection, iteratively refining our analytic frame while also updating the questions for future interviews as we identified emerging themes. Involvement of two VIPs in our research team helped us follow a co-design process while creating these themes. 

After interviewing the participants and arriving at an initial set of codes, we conducted weekly meetings to review the codes and refine them into a closed set of codes, which we then re-applied to the transcripts to reach a "group consensus"~\cite{saldana2021coding}. 
Since we followed a grounded theory approach, we did not seek agreement via measures like Cohen's Kappa to establish inter-rater reliability ~\cite{mcdonald2019reliability}.

==> 3-Methods/v4.tex <==
We performed a qualitative study guided by our two research questions 
% regarding VIPs' information needs (RQ1) and the challenges they face while exploring unfamiliar environments (RQ2).
RQ1 and RQ2.
Here we describe our recruitment process (Section~\ref{sec:ptcpts}), experimental procedure (Section~\ref{sec:procedure}), and data analysis procedure  (Section~\ref{sec:dataAnalysis}).
% series of semi-structured interviews with VIPs to answer two research questions: 
% \vspace{0.05cm}
% \begin{tabular}{{p{0.05\textwidth}p{0.85\textwidth}}}
%  \textbf{RQ1.} &  What information do VIPs need to explore unfamiliar environments, and what factors influence these needs between individuals? \\
%  \textbf{RQ2.} & What challenges do VIPs face while exploring unfamiliar environments, both independently and collaboratively? 
% \end{tabular} \\
% \begin{itemize}
%     \setlength{\itemindent}{.3in}
%     \item [\textbf{RQ1.}] 
%     % What information do VIPs need to explore unfamiliar environments, and how does that differ from the information needed for turn-by-turn navigation?
%     What information do VIPs need to explore unfamiliar environments, and what factors influence these needs between individuals? 
%     % - directed navigation
%     % - turn-by-turn navigation <---
%     % [would have to motivate the need for why we thought about these factors being present.]
% % How does VIPs' information needs differ between exploring unfamiliar environments and traversing to a destination, i.e., exploration versus guidance?
%     \item [\textbf{RQ2.}] What challenges do VIPs face while exploring unfamiliar environments, both independently and collaboratively?
% \end{itemize}%
% \vspace{-0.1cm}
% \noindent 
% To answer these research questions, we conducted a series of semi-structured interviews with VIPs and asked them to share their experiences of exploring unfamiliar environments, describing the \textit{information} they seek and the \textit{challenges} they face while
% gathering information by themselves (i.e., independently) and by seeking assistance from other people (i.e., collaboratively). 
% The interviews offered insights into VIPs' information needs and challenges while exploring unfamiliar environments, in comparison to traversing to a destination, i.e. guidance.
% To further investigate the challenges faced during collaborative exploration, we conducted short follow-up interviews with other people who the VIPs constantly mentioned as influencing their navigation behavior.
% These other people --- or stakeholders, as we like to call them --- include leaders of a blind-serving organization, O\&M trainer, manager of disability services at a university, and store employees.
% We interpret and synthesize our study findings from RQ1 (Section~\ref{sec:RQ1-findings}) and RQ2 (Section~\ref{sec:RQ2-findings}) to form design guidelines for NASs (Section~\ref{sec:DGs}) and suggest specific visions for future research on NASs that facilitate exploration, in addition to guidance (Section~\ref{sec:visions}).


\subsection{Participants}
\label{sec:ptcpts}
We recruited 12 visually impaired participants (VIPs) --- seven men and five women --- with a wide range of ages (18 to 72). Table~\ref{tab:participants} summarizes participants' demographics; all participants' names in the table are pseudonyms. 
Participants had diverse visual abilities, onset of vision impairment, and mobility aid preferences. 
% --> omit this line (already in the table) Eight participants had no usable vision, and four participants identified themselves as being legally blind with limited light perception to no usable vision in one eye and with some residual vision in the other eye. Eight participants are blind from birth while four developed vision impairments later in life at the ages of one (Charles), four (James), 20 (Harper), and 26 (Emily).
% The majority of our participants are white cane users except for Harper and Emily, who use guide dogs as their primary mobility aid. 
Ten are white cane users and two use guide dogs.
All live in the United States, spread across nine different states.


We recruited the VIPs from several sources. 
First, we posted to online forums and social media platforms popular among the visually impaired community \textit{(exact forums/platforms anonymized for submission)}, recruiting six participants in the process. Second, we connected with two participants through our research team's ongoing collaboration with a major blind-serving organization. We recruited the last four participants via snowball sampling~\cite{goodman_snowball_1961}.
% ; Leo put us in touch with Harper and Emily, and Nora referred us to Grace and Olivia. 


\begin{table*}[t]
\caption{
    \textcolor{black}{Self-reported demographic information of our visually impaired participants.}
    }
    \label{tab:participants}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcclll}
\hline 
\textbf{Pseudonym} & \textbf{Gender} & \textbf{Age} & \textbf{Onset} & \textbf{Mobility Aid} & \textbf{Nature of Vision Impairment}                                           
\\ \hline
\textcolor{black}{Harper}  & F & 59 & Age 20    & Guide dog  & Total blindness \\
Aaron       & M               & 22  & Birth & White cane   & No vision in left eye; Shape, color, and movement in right \\
\textcolor{black}{Emily} & F & 72 & Age 26 & Guide dog & Total blindness \\
James   & M & 25 & Age 4     & White cane & Total blindness \\
Daniel  & M & 21 & Birth & White cane & Total blindness \\
Leo     & M & 33 & Birth & White cane & Total blindness \\
\textcolor{black}{Grace}       & F               & 19  & Birth & White cane   & Light perception, shapes, color in left eye; No vision in right       \\
William & M & 23 & Birth & White cane & Total blindness \\
Charles       & M               & 25  & Age 1     & White cane   & Light, shape, color, and movement in left eye; No vision in right \\
Nora    & F & 18 & Birth & White cane & Total blindness \\
Lucas   & M & 36 & Birth & White cane & Total blindness \\
\textcolor{black}{Olivia}      & F               & 21  & Birth & White cane   & Light perception in left eye; Color, contour, and shadow in right     \\ \hline
\end{tabular}
}
    
\end{table*}

 


In addition to the VIPs, we recruited six other participants from groups who the VIPs reported as often collaborating with and who play a big part in shaping VIPs' behaviors around navigation. The six others include two leaders of a major blind-serving organization (their assistive technology director and their director of O\&M services), a manager of disability services at a large university, an O\&M trainer, and two store employees (one working at a small bookstore and the other at a major department store).
% -> omit this line Both the blind-serving organization and the university's disability services department offer a wide range of services to VIPs, including resources for O\&M training, rehabilitation programs, and assistive devices. 
We selected these two store employees because they self-reported as regularly interacting with visually impaired customers.



\subsection{Procedure}
\label{sec:procedure}

To develop our interview protocol and study procedure, we hosted two VIPs who are not trained in research in our lab for several months. We conducted multiple pilot interviews and brainstorming sessions with them in order to begin understanding VIPs' experiences in exploring unfamiliar environments. We then developed the interview protocol together using this new understanding.
% began recruiting participants as described above. % <-- feels redundant having already said that
% To inform the design of future NASs that facilitate exploration, in addition to guidance, we performed a qualitative study to understand VIPs' information needs for exploration (RQ1) and VIPs' challenges in gathering this information independently and collaboratively (RQ2). 
% Our study involved two phases: a \textit{formative study} (Section~\ref{sec:formative-study}) with two VIPs working with our research team, and the \textit{main study} (Section~\ref{sec:main-study}) that constituted 
% interviews with 12 VIPs and short follow-up interviews with the six others who help shape VIPs' exploration behaviors. 


% \subsubsection{Formative study}
% \label{sec:formative-study}
% % We started with a formative study with two VIPs to gather an initial data sample of VIPs' experiences in exploring unfamiliar environments, with an aim to refine the interview protocol --- both the structure and the questions --- to effectively answer our two research questions.
% We hosted two VIPs who are not trained in research in our lab for several months, conducting multiple pilot interviews and brainstorming sessions in order to begin understanding VIPs' experiences in exploring unfamiliar environments. Through this collaboration, we developed the main study interview protocol to investigate RQ1 and RQ2 and began recruiting participants as described above.
% , iteratively refining our interview protocol for the main study.
% Through this process we gained two major insights, one relating to each research question.
% With respect to RQ1, 
% we learned that VIPs' information needs are sensitive to their navigation goal: exploration versus guidance. Since our goal is to identify VIPs' information needs for exploration, we restructured our interview protocol to deliberately ask VIPs to recall their prior visits to locations where they had no specific destination in mind, i.e., \textit{exploration}; and also to locations where they traversed to a specific destination within the environment, i.e., \textit{guidance}. 
% With respect to RQ2, 
% we learned that collaboration is a key aspect to VIPs' exploration strategies and that some of the challenges they face during exploration arise from these collaborations with other people. This insight led us to refine our interview questions to \textit{identify} these other people and to \textit{gauge their effect}, both positive and negative, on VIPs' ability to successfully explore unfamiliar environments. The formative study concluded with a refined interview protocol for our main study with VIPs, which we describe next.

% \subsubsection{Main study}
% \label{sec:main-study}
% We conducted our main study by interviewing 12 visually impaired participants to investigate RQ1 and RQ2. 
Our final interview protocol was organized as follows.
We began each interview by collecting participants' background information, including their demographics (age, gender, location), onset and level of vision impairment, history of O\&M practices, mobility aid preference, and use of assistive technologies for navigation.
Collecting this background information helped us identify correlations between different individuals' exploration preferences and their past experiences.
% For example,
% Next, to learn about VIPs' information needs and the challenges they face when exploring environments, we used 
We then turned to RQ1 and RQ2 by employing
a recent critical incidence technique~\cite{flanagan_critical_1954},
% , chell1998critical
in which we asked participants to recall and walk us through specific instances of their past experiences of navigating unfamiliar environments. 


In the interviews, we encouraged participants to describe these instances in as much as detail as possible. For example, we first asked participants to name a specific location they recently visited and then asked them to elaborate on their navigation goal (i.e., exploration vs. guidance): ``\textit{So, you mentioned visiting a shopping mall. What was the purpose of your visit?}'' 
Then, we initiated a back-and-forth discussion 
% And then, the primary researcher would initiate the discussion 
by re-establishing the scenario for them: ``\textit{Now, let’s walk through your visit to the shopping mall. Suppose, I spotted you at the shopping mall. What would I observe? Let’s start with you getting off the bus.}''
During these discussions, we asked follow-up questions to understand participants’ information needs, challenges, and workarounds to address these challenges. 
% information that they need when exploring unfamiliar environments and what challenges do they face while doing so.
% Note that we were cognizant of VIPs' navigation goal (exploration or guidance) throughout their account of incidents. % <-- 
% Participants described information that they need when exploring unfamiliar environments and what challenges do they face while doing so. 


% We began our interviews with a script but also asked follow-up questions to gain more context\todo{may omit this para.} on specific incidents and challenges that the participants reported~\cite{hesse-biber_practice_2011}.
% For each interview, we asked the participant to walk us through at least one location that they wanted to explore, and at least one location that they mentioned as wanting to traverse through with a destination in mind, i.e., guidance. Doing so enabled us to tease apart the information needs for exploration from guidance, comprehensively answering RQ1.


During the interviews, we made special note of people who the VIPs mentioned as often collaborating with and their effect on the VIPs' navigation behaviour. To further investigate RQ2 from the perspective of these other people, we conducted short follow-up interviews with six representative non-VIP participants, described in Section~\ref{sec:ptcpts}.
Soliciting experiences from both VIP and non-VIP perspectives helped us find the root cause of the challenges that VIPs --- and in some case these non-VIPs --- face when exploring unfamiliar environments collaboratively.
% including two leaders of blind-serving organizations, a manager of disability services department at a university, an O\&M trainer, and two store employees. 

We asked these six others about their backgrounds, their frequency of interactions with VIPs, their role in assisting VIPs in navigation, and their experience with assistive technologies for VIPs (if any). We used the same critical incident technique~\cite{flanagan_critical_1954} as before, but we asked these participants to recall and walk us through their past experiences interacting with VIPs, specifically instances in which they helped VIPs with navigation-related tasks. 



We conducted all interviews via a Zoom video-conference, except for two: the bookstore employee preferred to be interviewed in person during working hours, and Emily preferred a telephone interview since she was not comfortable using Zoom. \Cref{fig:interview-screenshot} shows screenshots of the remote interviews conducted with four of our participants. All interviews were recorded with participants' consent.
Each interview lasted 60--90 minutes and the participants were compensated \$25 for their time. We collected over \textcolor{black}{23 hours} of recordings in total. The study was approved by our institution's IRB. 
% We next describe 


\begin{figure*} [t]
    \centering
    \includegraphics[width=0.7\textwidth]{images/screenshots-zoom.pdf}
    \caption{Screenshots of remote interviews with four of our participants. Each of these participants granted us written consent to record the audio and video of their interviews. Faces have been obscured to protect anonymity.}
    \label{fig:interview-screenshot}
\end{figure*}




\subsection{Data Analysis}
\label{sec:dataAnalysis}
We analyzed our interview data via a grounded theory approach~\cite{charmaz_constructing_2006}. Following grounded theory, we simultaneously performed data analysis and collection, iteratively refining our analytic frame while also updating the questions for future interviews as we identified emerging themes.
The primary author and a co-author collaboratively performed open coding~\cite{strauss_basics_1990} on the interview transcripts while interviews were still ongoing to arrive at an initial set of codes.
We also held brainstorming sessions with the two VIPs on our research team to validate and refine some of these themes.
Later, we conducted weekly meetings to review the codes and refine them into a closed set of codes, which we then re-applied to the transcripts to reach a ``group consensus''~\cite{saldana_coding_2013}. Since we followed a grounded theory approach, we did not seek agreement via measures like Cohen's Kappa to establish inter-rater reliability ~\cite{mcdonald_reliability_2019}.
% ) --- then performed open-coding~\cite{strauss_basics_1990} on these transcripts to arrive at an initial set of codes. 
% Following the grounded theory approach~\cite{charmaz_constructing_2006}, we simultaneously performed data analysis and collection, iteratively refining our analytic frame while also updating the questions for future interviews as we identified emerging themes. 


% After interviewing the participants and arriving at an initial set of codes, we conducted weekly meetings to review the codes and refine them into a closed set of codes, which we then re-applied to the transcripts to reach a ``group consensus''~\cite{saldana_coding_2013}. 
% Since we followed a grounded theory approach, we did not seek agreement via measures like Cohen's Kappa to establish inter-rater reliability ~\cite{mcdonald_reliability_2019}.



























% These additional six participants represent a subset of p
% \textcolor{magenta}{While there have been considerable research efforts in understanding VIPs' collaboration with their friends and family~\cite{williams_just_2014, vincenzi_interdependence_2021}, our research focuses on corroborating our findings from VIPs with people that are not a part of their immediate social circle.}\todo{Trying to answer the question: Why didn't we recruit friends/family? Needs another draft.} 
% Reviewers comment: "Six additional stakeholders were also interviewed. It is not clear why these particular stakeholders were chosen and I was surprised to see only one O&M trainer on this list and no family members/friends/assistance workers who regularly accompany people who are vision impaired."

% The two leaders that we recruited from the major blind-serving organization were their assistive technology director and their director of O\&M services. We recruited them through our collaboration with the organization. 
% We recruited the manager of disability services for the large university via email. 
% Both the blind-serving organization and the university's disability services department offer a wide range of services to VIPs, including resources for O\&M training, rehabilitation programs, and assistive devices.
% \todo{Feels like too much detail (and space) on other stakeholders.}

%The O\&M trainer that we recruited self-reported as having over 15 years of experience providing O\&M services to VIPs.
%The two store employees that we recruited were from a local bookstore and a major department store. 
%We met the bookstore employee after we visited local businesses around our institution and asked employees about the extent to which they interact with VIP customers. 
%We recruited the department store employee by emailing major department store managers in our institution's surrounding area, asking if they knew of any employees who frequently interact with VIP customers.




% More language from a paper: "In the interviews, we asked people about the diferent technologies they used to get around, circumstances that prompted their use, challenges they encountered, and how they worked around the challenges."


% Copied from the paper: "We concluded the study by giving participants an opportunity to ask questions about our research, future directions, or to elaborate on topics they wished to discuss." ~ (Understanding Everyday Experiences of Reminiscence for People with Blindness: Practices, Tensions and Probing New Design Possibilities)



% Copied from Co-located interactions paper: "we started the interviews by following a script but also used unscripted questions to gather more information about the specific context and experiences of in-person activities mentioned by the participants [30]." ~\cite{hesse2010practice}

% As a result, we also performed follow-up interviews with these other people that VIPs constantly mentioned as having significantly affected their navigation behavior. % <---- May be added here, or later when we talk about RQ2 in detail.

% 1. there is a nuanced difference between exploration and guidance information needs, and we had to be cognizant about the experiences that VIPs share with us during the interviews and carefully define/understand the context in which VIPs explored a specific space.



% - that there is a nuanced difference between VIPs' information needs for exploration and guidance and hence, we had to be deliberate about asking VIPs about differentiating exploration from guidance. 


% To design NASs that facilitate exploration in addition to guidance, our aim is to first understand what information is important for exploration (RQ1), and also identify challenges do VIPs face while exploring unfamiliar environments (RQ2). 


% We performed two series of semi-structured interviews: the first with our 12 visually impaired participants, and the second with six people who the VIPs 
% stated as \textcolor{magenta}{often collaborating and} significantly affecting their everyday navigation behaviors \textcolor{magenta}{in shared environments}. 
% \textcolor{magenta}{We hosted two VIPs, who are not trained in research, at our lab for several months to help us refine our interview questions. We conducted pilot interviews with the two VIPs to identify our initial set of research questions. Through several brainstorming sessions with the two VIPs, we also refined our interview questions over multiple iterations. The involvement of VIPs on our team benefited us in identifying the two means of exploration --- independent and collaborative --- before we begun investigating it in detail with our 12 participants.}

% In the first series of interviews, we asked VIPs open-ended questions to understand their background, role of visual information (if any), their history of O\&M practices, and their use of assistive technologies for navigation. In order to understand their daily navigational challenges even further, along with how they interact with other people in those scenarios to overcome those challenges, we then asked the VIPs to recall and walk us through specific examples of their past experiences of navigating unfamiliar environments.

% In the second series of interviews, we asked the six non-VIPs about their backgrounds, their frequency of interactions with VIPs, their role in assisting VIPs in navigation, and their experience with assistive technologies for VIPs (if any). We then ask them to recall and walk us through their past experiences interacting with VIPs, specifically instances in which they helped VIPs with navigation-related tasks. Soliciting experiences from both VIP and non-VIP perspectives helped us corroborate our findings. \textcolor{magenta}{Since VIPs do not navigate with these people as often, as they do with their friends and family, it was important to understand any communication gap between the two parties.}



% dump: 
% Give a similar example about how we asked them to tell us what would happen if we were there. "For example, at the beginning of discussions regarding arrival at an airport, the primary researcher described a typical scenario such as, “Now, let’s talk about the arrivals. You have landed. You need to claim your baggage and leave the airport to your destination. Or maybe other things you need to do in between.” During these discussions, we particularly aimed to understand participants’ navigation and information needs, frustrations, and workarounds to address these needs, as well as the situational and environmental factors impacting their experiences at each of these stages." -- Abdolrahmani et al. (Towards more transactional...)
% 
% "We used open-ended, semi-structured questions as a guide for conducting the interviews."
% We asked the agents to share their experiences

==> 4-Findings/v1.tex <==
% What are these attitudes, and what defines them?
% These continuums emerged from the themes. relate to different feelings of ---- Define the continuums first, and then say that these form two diffrent clusters and we call them: active and passive
We found the VIPs that we interviewed to adopt two major attitudes towards navigation in unfamiliar environments, which we call an [active?] attitude and a [passive?] attitude.  [ppl tended to have one of two primary attitudes towards navigating unfamiliar env., which we will call an active att and a passive att. These atts shape our ptcpts' feelings and preferences over x (agency over convenience), y (independence/self-reliance), z (safety vs adventure example) - tendancy to think of spaces/nav in terms of maps or routes.]: \textit{active} and \textit{passive}. 

% Where do active fall on this continuum
VIPs display an \textit{active} attitude when they value agency over convenience, are self-reliant, and display a higher proficiency in O\&M skills that renders their preference to explore and navigate via mental maps. 

% Where do passive fall on this continuum
VIPs show a \textit{passive} attitude, on the other hand, [when they] value convenience over agency, rely on assistance from others, and display a lower proficiency in O\&M skills that renders their preference to be guided or navigate via memorized routes (and not maps). 

% fluidity and contextual nature, why we cluster them in this situation in unfamiliar environments
We also discovered that these attitudes are largely dependent on context. In fact, many VIPs that we interviewed fluidly move on the continuum between active and passive attitudes in different environments. They may, for example, have an active attitute toward navigation in their home but a passive attitude in unfamiliar environments. Our work primarily focuses on unfamiliar or rarely visited environments where the two attitudes are most distinguishable (also NASs come into play in these cases more -- ??).
% give an example of what a ptcpt said about being independent in a specific location.
% Names of the attitudes
% Language too strong - not a property of the person, 
% These are the trends that we found in our group, 

These attitudes [in unfamiliar environments] were primarily shaped by the VIP participant's exposure to O\&M training. All participants [most of the times when they navigate in an unfamiliar environments] displaying an active attitude towards navigation (n=4) reported to have received extensive O\&M training spanning over several years, as opposed to participants with a passive attitude (n=4) who reported to have received only limited O\&M training -- mostly via short vocational rehabilitation programs spanning over 1-2 months that are meant to help them navigate a specific location such as their workplace. We found that the level of vision impairment did not play a major role in shaping the navigation attitudes. Two participants (P2, P7) -- who identified themselves as otherwise visually impaired, i.e., had low-vision -- portrayed different attitudes despite having a comparable amount of visual information to support their navigation. 


We observe that the attitudes influence participants' navigation goals, navigation challenges, and their preference in assistance from others. Participants with an active attitude expressed their need to be in control during navigation, trying to figure things out on their own. However, existing NASs require VIPs to play a passive role. They do not accommodate VIPs with an active attitude towards navigation at all. In the following subsections, we explore the difference between these passive and active attitudes towards navigation in detail. Through this exploration, we reveal insights that lead to a new set of design requirements (Section~\ref{sec:Drs}) which can help refine existing NASs to provide a more agency-oriented experience to the VIPs during navigation.


\subsection{O\&M Skills and Cognitive Abilities}


Participants' prior experience with O\&M training was found to be a key factor in shaping their attitudes. All our participants with an active attitude (n=4) highlighted the importance of O\&M skills in their lives, empowering them with independence and autonomy during navigation. As P4 explains:  

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[O\&M skills are] vital because the world will walk over you if you [don’t] take control of your own abilities. [...] People will tell you where you can go and what you can do if you do not interject. And if you don't know how to do those things, then you're just kind of meekly following along. It's self esteem shattering, [and] reduces your individuality.”} - \textbf{P4} & \\
\end{tabu}

\subsubsection{\textbf{Access to O\&M Training}}
All participants with a passive attitude (n=4), in contrast, reported to only have receive limited O\&M training. Lack of access to O\&M training was found to be the reason behind the divide between the two categories. There were several factors that affected access:

\textit{{Eligibility for benefits during K-12 school}:} For VIPs who develop vision impairments earlier in life or are blind by birth have easy access to O\&M training through their schools. However, VIPs that develop visual impairments later in life often find it difficult to arrange one. All our participants developed vision impairment either from birth (P2, P3, P5, P6, P8, P16), or earlier in life (P4: by the age of four, P7: by the age of one). All of them stated that they were assigned an O\&M trainer in school. However, many participants (n=6) stated that it is much more difficult to set up an O\&M session as an adult, compared to getting one as a child in school. As a result, most of their O\&M training was done during K-12 school. For instance, P16 (who is blind by birth) explains:

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“For earlier years, I d[id]n't need to reach out [to O\&M trainers] because that's something that like, we automatically get [in schools]. Now, I definitely would have to advocate for myself [by reaching out to] the Rehab Center or something like that. [...] I can’t expect them to reach out to me.”} - \textbf{P16} & \\
\end{tabu}
\vspace{0.2cm}

\textit{{Availability of O\&M trainers}:} Despite being eligible for benefits during K-12 school, there may still be a possibility that VIPs did not receive appropriate O\&M training during school. This is primarily due to shortage of O\&M trainers and decentralization. O\&M trainers are assigned multiple students scattered over a geographical area, which makes it difficult for them to be physically present and provide enough time to all their students. P7, who was assigned an O\&M trainer during middle school, describes the reason behind their lack of access to an O\&M trainer:

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I was told that I would get an O\&M trainer back in middle school [...] I never received that trainer. She came in once within the six years she was supposed to be training me. [...] I actually had my English teacher in middle school, walking around campus with me after the classes being like, 'Hey, here's what this class is'. 
%  [...] So she was kind of more of a navigation instructor than the O\&M instructor that was supposed to be assigned to me.
 ”} - \textbf{P7} & \\
\end{tabu}
\vspace{0.2cm}


% [Maybe] Add few more points here
% - as an adult it is difficult because of shortage
% - ?




% "I actually was never given O\&M instruction. [...] I was never taught how to properly use a cane [...] I've never communicated with [O\&M instructors]"


\textit{{Availability of state funding}:} All our participants reported that they are dependent upon the state to receive O\&M training facilities. A few participants (n=2) highlighted that their state provides limited resources due to shortage of funds, thereby affecting their ability to receive O\&M training:

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“It's just very hard to get [O\&M training here] because [anonymized state] is out of money. [...] it's very hard to [receive O\&M training because] you've got to prove that you’re working.”} - \textbf{P3} & \\
\end{tabu}
\vspace{0.2cm}





\textit{{Type of training received}:} Most participants (n=3) with a passive attitude indicated that they possessed limited O\&M skills that they had acquired through short vocational rehabilitation programs. For instance, the participants mentioned that they only knew the basics of how to use their white cane, but did not have the confidence to trust their skills. These programs are geared towards helping VIPs memorize the space, instead of building their O\&M skills in general.
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“Usually, [the state provides] vocational rehab and [gives you a] caseworker. And the caseworker is supposed to get you from not working to working, whether [by providing you with] mobility training, or whatever.”} - \textbf{P3} & \\
\end{tabu}
\vspace{0.2cm}


\noindent In contrast, all participants with an active attitude displayed confidence in their O\&M skills, so much so that they trusted their white cane more than sighted guides in many scenarios. These participants highlighted that they were exposed to extensive training, geared towards enabling independent navigation.


\subsubsection{\textbf{Initiative Towards Maintaining O\&M Skills.}} Most participants with an active attitude (n=3) preferred to use their O\&M skills as much as possible. Participants highlighted how they want to constantly keep working on their skills to feel more independent by not relying on assistance from others, practice and develop them further; to ultimately offer them the agency to make their own choices during navigation. For instance, P4 explains:
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"It is very easy to let your [O\&M] skills atrophy as a blind person if you rely overly on sighted people and it's an easy trap to fall into. It's easy to [use a] sighted guide and become complacent and [not pay attention to] what turns you have taken and where you are in relation to other things." } - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm}

On the other hand, most participants with a passive attitude preferred sighted assistance over using their O\&M skills for navigation -- primarily due to convenience. However, a few participants (n=2) in this category expressed their desire to obtain better O\&M training from an instructor, rather than practicing themselves.


\subsubsection{\textbf{Level of Attention Towards Other Senses.}} 
Another key difference between the two attitudes came to the fore when  participants were asked to describe the information that they acquired from other senses (such as touch, smell, and hearing) while navigating an environment that they visited in the past one month. Most participants with an active attitude (n=3) articulated in much higher fidelity about the information they could gather through their other senses. For instance, P8 provides a description of the information that they could gather from their first visit at a client's home: % Add "bandwidth"
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"
%  [I rely on] sound and touch certainly [the most]. 
 [I can use] ambient sounds [for] figuring out [...] where an object is. So for example, [I know] a refrigerator makes a hum so I know where the refrigerator is. [I can also use] ambient sounds [such as] the sound of the air flowing through the ducts, an HVAC system, a refrigerator. [or] a clock ticking, [which] provide location data in and of themselves, [to create] an auditory environment based on the [occlusion] of sound" } - \textbf{P8} & \\
\end{tabu}
\vspace{0.2cm}


\noindent On similar lines, P4 describes their use of sense of smell at a shopping mall that they recently visited.

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"
%  I also use [my] sense of smell [for navigating]. [...] 
 Clothing stores smell different from jewellery stores, or at least tend to." } - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm}

\noindent Although participants with a passive attitude also used their other senses for navigation, most (n=3) of them provided vague descriptions of the sensory information that they gathered. For instance, P6 explains their use of other sensory cues:
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“Everything I can get like sound, texture of the floors, location of things. Yeah, everything I can get from the place I am. Particularly any information that can be useful.” } - \textbf{P6} & \\
\end{tabu}
\vspace{0.2cm}


As a consequence, participants with an active attitude rely heavily on their other senses in order to navigate independently. Whereas, participants from the other category simply preferred to rely on sighted assistance without having to put in the effort to gather this information. The active attitude calls for assistance that supplements their existing cognitive capabilities or information that VIPs can acquire themselves. Participants with a passive attitude, instead, indicated that they would be open to completely relying on any external source of information.

% \cite{}

\subsection{Navigation Goals}
For both attitudes, the underlying aim of navigation is to find their way around an environment. However, we discovered some navigation goals that are more important for VIPs with an active attitude, than their counterpart. In addition, the VIPs with active attitude highlighted how they acquired information from the environment like participants with a passive attitude, but use it for different purposes. Below, we outline these navigation goals to highlight the difference between the two attitudes, while also pointing out the gaps in how existing NASs do not accommodate the navigation goals of VIPs with an active attitude.


\subsubsection{\textbf{Learning about General Layout of the Space.}} 
VIP-participants with an active attitude reported the need to learn about the general shape and layout of an environment, both prior to visiting the environment and then during navigation. All participants in this category (n=4), expressed their desire to first learn about the general shape and then figure things out on their own during navigation. This preference resulted from the participants' need to build a mental map of the space that will assist them in finding their way around the space in a much more independent fashion by using their O\&M skills. As P4 puts it:\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``[When I receive help] I will [ask], ‘what does this building generally look like?’ Because I want to understand [the shape of the building]. That's one of [the] first things [I want] to understand and that is a difficult thing to do as a blind person because I cannot look at satellite maps and it takes me a long time to [understand] the general shape [of a space], personally."} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm}

On the contrary, most (n=3) participants with a passive attitude stated that learning about the layout is not as important. Instead, they prefer to receive direct assistance from others -- either from sighted people or a system. This reliance on sighted assistance meant that their decision to visit an unfamiliar environment is dependent on availability of sighted assistance, including their friends and family. \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``Usually for groceries, I ask somebody to assist me because [...] I feel like [the shape of the store is] really complicated to learn."} - \textbf{P6} & \\
\end{tabu}
\vspace{0.2cm}

In some scenarios, a few participants (n=2) with a passive attitude highlighted that even they ask for a general layout of the space. However, unlike active attitude, they shifted quickly towards getting assistance as the space becomes more and more complex to navigate. We found a direct relationship between the speed of this shift towards assistance and the participant's confidence in their O\&M skills.  This directly supports our hypothesis that O\&M training forms the basis of navigation preferences for both the categories.

Most existing NASs focus on providing turn-by-turn directions, without enabling the users to learn the general layout of the environment. Only a handful of approaches focus on this aspect of navigation. NavCog~\cite{}, for instance, uses a route preview feature that helps build a general understanding of the relative location of the different landmarks in an environment. Similarly, authors et al. \cite{} allow users to rehearse specific routes in an environment. Although these approaches help users build a better mental map of the indoor space, they do not provide the user with layout of the environment like: How wide is the hallway? What is the shape of the room? We found that these kinds of information are more valued by participants with an active attitude than their counterpart.

\subsubsection{\textbf{Adding Landmarks to Mental Maps.}} 
All participants highlighted that landmarks play a major role in being able to successfully navigate through a space. Both groups reported the use landmarks to follow routes and to form mental map of the space. The two groups differ, however, in the format of the mental maps that they form with the landmarks. % supported by existing work~\cite{}

In particular, participants with active attitude state that once they had a mental map with a general layout of the space, participants incorporated landmark information on top of the general layout to solidify their mental maps. For instance, P2 mentioned how they focused on understanding the general layout of a grocery store, and then supplemented their initial mental map with landmarks that were relevant to them. \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``So [during my first visit, I was] essentially going through the whole grocery section [while looking for] the bathroom. I'm [asking to myself], ‘Where is everything else? There's bread here [...] Where's everything?’"} - \textbf{P2} & \\
\end{tabu}
\vspace{0.2cm}

Participants with a passive attitude, on the other hand, use landmark information to memorize the routes and not to create more complete mental maps of the environment. Consequently, existing approaches for route preview or route rehearsal serve these groups of participants well. For instance, P6 highlights this "route specific" behaviour of the participants in this group: \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"I try to use the wall like a  landmark [or I use] the doors that are near. [I use them] to follow just a straight line. "} - \textbf{P6} & \\
\end{tabu}
\vspace{0.2cm}


We also found an interesting nuance in how active attitudes stressed on creating a more robust set of landmarks. Given the dynamic nature of the environment, location of landmarks may change over time and landmarks created in previous visits may not be valid anymore. To mitigate this, participants reported that they created redundant landmarks such that even if one of the moves, or they end up missing one, others can be used to accurately orient themselves. In addition, participants mentioned building a hierarchy of importance of landmarks. Based upon the relative importance of the landmarks,
participants mentioned that they look for certain landmarks first and the redundant landmarks are used for confirmation. \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"I've learned that you cannot rely [only] on one landmark [for navigation] because things change and the world is not static. [...] you may miss one landmark, but not the other so context is important. If you can find three landmarks in a location, then if you miss one or even two, you'll still have the third [which can help you] go back and find the other two to make sure that you're in the right place. [...] I found in my neighbourhood, for instance, there are very many fences that feel very similar within the four block radius of my house. So I can't say, ‘Okay, I will only pay attention to this type of fence’ because I will probably find [a similar fence] again on another block even though it's not the same one. I have to say, ‘this fence next to this telephone pole, with gravel.’ I need multiple layers [of information] But sometimes [the supplementary information] can be as simple as the traffic is closer here. [...]  So landmarks have a hierarchy of importance in my mind."} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\
Note that while this practice is common for both the groups, it is less prominent amongst the passive attitudes since they already rely on sighted assistance during navigation.









\subsubsection{\textbf{Self-exploration for Robust Mental Maps.}}
Participants mentioned that often, their mental maps are not robust enough for them to rely on them completely for navigation. Since the format of mental maps is different for active (complete maps), and passive (routes) attitudes; the two groups reported different approaches to fill-out the gaps in their mental maps for subsequent visits. Most participants (n=3) with an active attitude stated that they prefer to explore the environment themselves to augment their sensory cues. This not only helps them in getting familiar with the environment but also feel more independent. \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[When I enter the mall] the echolocation can tell me some things [about the shape of a space], but I want specifics. So I will go to each side [of the entrance] and [check] how big [the entrance is]. And then I will see that there are two large openings from this foyer, one on either side, left and right, after a ways of wall. [I also learn that] there's a large opening into the main part of the mall. [From this information] I know that [the shape of the entrance] is probably a sort of long wide corridor, stretched out [perpendicularly] in front of me [...]”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\
Most participants with the passive attitude, on the other hand, prefer to update their mental maps -- which consist of routes, and not complete maps -- by asking for directions. For instance, P5 describe their approach: \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"Anything [that could be] as simple as finding a room that is not braille signed or a checkout counter [...] would require me to ask for directions."} - \textbf{P5} & \\
\end{tabu}
\vspace{0.2cm} \\





\subsection{Preference in Assistance from Others}
\subsubsection{\textbf{Frequency of Asking for Assistance.}}
The two attitudes differ in reliance on assistance from others for navigation. Active attitudes value agency over convenience, and hence do not ask for assistance unless absolutely necessary. We found that most participants with the active attitudes used sighted assistance sparingly, often turning to non-VIPs to only supplement their existing knowledge. Participants reported several different reasons behind this, such as not wanting to bother others (P2), relinquish control (P4) or becoming complacent (P2, P4, P16); not trusting others with their safety (P4, P16); and believing in their abilities to be independent (P2, P4, P8, P16).  \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"Generally I don't like to ask for help unless I absolutely need it.  I don't want to [...] make a person busy or inconvenience them [...]  unless [...] I'm having legitimate difficulties that I can't solve through a bit more effort, especially when it comes to like navigation. [...] Essentially, [...] I want to [...] keep reaffirming to myself [that] I can navigate spaces by myself."} - \textbf{P2} & \\
\end{tabu}
\vspace{0.2cm} \\

Most participants on the other side of the spectrum, reported a much more comfortable interaction loop with others. We found that these participants were open to receiving help from others whenever they needed it, without evoking the feeling that they were bothering someone or asking for help would lessen their agency. For instance, P6 share their grocery shopping experience: \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"[I think that] people are really helpful. [...] if I don't find somebody [to go to the store with me], I just ask [a stranger if they] can help me out. [...] [They do] their own groceries and I[ do] mine and we talk and it's really nice."} - \textbf{P6} & \\
\end{tabu}
\vspace{0.2cm} \\









\subsubsection{\textbf{Preference in Type of Assistance.}}
Despite the fact that participants with an active attitude preferred not to receive assistance from others, both groups ended up receiving help in environments that were completely unfamiliar to them. However, we found that their attitudes govern the type of help they wish to receive from others.

Participants with active attitudes strongly preferred to receive only verbal instructions regarding directions and general layout of the space, navigating to their destination on their own. Most participants (n=3) reported to avoid sighted guide assistance, because they backed their O\&M skills to help navigate to the destination if they had a bit more information about the environment. As P4 and P16 explain: \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"Occasionally, I will use a sighted guide but I'm trying to do that less. [Instead] I will tend to ask people questions. [I prefer to] have them point things out [to me] and not lead me."} - \textbf{P4} & \\ 
 & \textit{“I never usually ask for a sighted guide. I just ask for directions. [For example, I ask,] `Okay can you tell me where this is?'"} - \textbf{P16} & \\
\end{tabu}
\vspace{0.2cm} \\


In contrast, all participants with a passive attitude preferred to received a more closely guided form assistance such as having the other person walk with them to the destination, or sighted guide assistance. We observe that most participants in this group go for assistance because it is much more hassle free for them, as P3 and P5 describe:\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I'll always take [sighted assistance] if someone's offering it. If somebody comes up to me [and asks], ‘do you need assistance?’ I'm taking [the assistance] because it's there.”} - \textbf{P3} & \\ 
 & \textit{“[I do not go alone] to places like stores [...] unless [I plan to] be going straight to find a personal shopper.”} - \textbf{P5} & \\
\end{tabu}
\vspace{0.2cm} \\



Despite their preferences, participants with an active attitude may sometimes end up choosing sighted assistance over verbal instructions. We found that this usually happens when VIPs do not feel like putting in the effort, i.e., for \textit{convenience}. Another reason this might happen is due to a \textit{time constraint}, for example: when they are supposed to catch a flight or a train. P4, on their recent trip to a clothing store, says: \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I relied on my sister [as a sighted guide]  more than I would like to have. But it was [a matter of] convenience [...] I wasn't really there to learn the stores. I was there to shop and get out of there as quickly as possible because I hate shopping." } - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\



\subsection{Socio-navigational Challenges }



\subsubsection{\textbf{Communicating Needs and Receiving Environment Information.}}
VIPs often ask for assistance from non-VIPs that may not be their friends or family. All participants, irrespective of their attitude, reported that non-VIPs struggled to understand their needs, leaving them frustrated. Participants with an active attitude, who prefer to receive verbal description, often found it difficult to understand the shape and layout of the environment based on non-VIP's descriptions. Our finding reinforces prior work that highlights the mismatch between how space is perceived by VIPs and non-VIPs. \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"[I need to ask for clarification] because a lot of people describe [shapes with letters] like U shaped or H shaped. I know what U shaped is, but sometimes I forget what H shaped means [because] I don’t really use it. [I need to clarify that] I just prefer geometric shapes [for descriptions.]"} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\ 
In addition to reinforcing prior findings, we also found that all participants almost always asked for descriptions from their VIP-friends and family, who have been to a space before. P16 provides an example of how their VIP-friend helped them:
\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“So for example, [before I go to a train station] my friend will tell me this train [...] doesn't talk. And that's actually a big thing when it comes to travelling because then I'm really gonna have to pay attention and count the stops […] So my friend will let me know [that I am] really gonna have to pay attention [when riding that train] because this train doesn't talk and it doesn't let you know [what station you are at]”} - \textbf{P16} & \\
\end{tabu}
\vspace{0.2cm} \\ 


Most participants with a passive attitude reported frustration mostly in cases where non-VIPs do not how to assist them. This finding reinforces the findings by Authors et al.~\cite{}. \\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I had somebody once when I was travelling grab the end of my cane and [try] to pull me along by my cane, and that’s not [the correct way to assist]”} - \textbf{P3} & \\
\end{tabu}
\vspace{0.2cm} \\ 
Despite the frustration and such experiences, all participants agreed that they did not expect non-VIPs to know the right way to help them, and hence expressed the need to be able to lead communication and work with non-VIPs in order to help non-VIPs assist VIPs. 



\subsubsection{\textbf{Social Pressure.}}
We found that participants with an active attitude were more cognizant towards social factors compared to the other group. All participants (n=4) with an active attitude stated that were often apprehended by other people's perception of them, and sometimes their sighted guides as well. This caused participants to feel anxious and negatively impacted their ability to navigate environments. We observed that this feeling escalated when they received assistance from their friends and/or family. For example, P4 says:\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I know that my sister gets looks from people all the time [when she acts as my sighted guide], because of foolish assumptions they make out of ignorance. [People think] that she is my caretaker, [and that] anything that they perceive as her not doing her job is wrong.”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\
Since the active group valued autonomy and independence more, they did not want people to perceive them as relying on others. On the contrary, most participants with a passive attitude did not seem to be affected by what other people's perception of them. Unlike the other, passive attitudes remained unaffected, irrespective of who assisted them.

==> 4-Findings/v2.tex <==
% This is where to talk about the groups, make more important
\subsection{Beyond Guidance Abilities}
Our thematic analysis revealed three beyond guidance abilities, which emerged as major themes:

Ability 1 - Agency in Navigation

Ability 2 -  Get Navigation help from non-VIPs effectively

Ability 3 - : Maintain or Learn O&M Skills

Interestingly, these three abilities emerged from our interviews with four of our eight participants.
These abilities emerged from our interviews with all parties. Interestingly, however, only half (4/8) of the VIPs spoke to a need for these abilities. 

Participants were split on their attitudes towards wanting these abilities, with half of the participants strongly wanting all three and the other half being much more satisfied with receiving guidance only.
This means, if our sample of VIPs is representative of the VIP population at large, that the status quo of guidance-based NASs satisfy half of VIPs very well, but does not meet the more agency-oriented needs of the other half of VIPs.

The experiences of 

Below we discuss these abilities in detail. We also discuss how their everyday navigation experiences 


\subsection{Perspective from Ptcpts Favouring Guidance Only}
Our findings about the other people reinforce prior work that builds off of this perspective prefers to be guided. With respect to Ability \#1 they said...., wrt ability \#2 they said...



The first ability that we learnt was about agency in navigation. Specifically we heard remarks about [that they love to be able to learn about the general layout of the space subsection 1], [subsection 2]. Here we describe these findings in more detail

and this emerged from the subsection headings
Half seemed satisfied, but other half revealed beyond navigation goals
% 

% \subsection{Two Attitudes Towards Navigation}

Through our semi-structured interviews, we found that the responses of our VIP participants formed two major clusters of thought towards navigation: one having \textbf{beyond guidance} navigation goals, and the other not. We will label these two groups as \textit{active} and \textit{passive} attitudes respectively. Our work primarily focuses on unfamiliar or rarely visited environments where the two attitudes are most distinguishable among the people we interviewed. However, we note that these attitudes are ultimately dependent on context. In fact, many VIPs that we interviewed fluidly move on the continuum between active and passive attitudes in different environments. They may, for example, have an active attitude toward navigation in their home but a passive attitude in unfamiliar environments. 

In unfamiliar environments, we found that these attitudes are largely shaped by the participant's access to O\&M training, and are most distinguishable through their level of attention towards other sensory details when performing non-visual skills and preference for asking for assistance. VIPs who show an \textit{active} attitude often display a higher proficiency in O\&M skills and a higher level of attention towards other senses, which lead to a preference to explore and navigate via mental maps. VIPs who show a \textit{passive} attitude, on the other hand, often display a lower proficiency in O\&M skills and a lower level of attention towards other senses, which lead to a preference to be guided or navigate via memorized routes.

In the following sections, we explore VIPs' \textbf{beyond guidance} navigation goals by examining the differences between \textit{active} and \textit{passive} attitudes. 


% Emphasize goal not difference
% + add current NAS do not address/ current NAS address only passive goal
% Active ~ 3/4 Passive ~ 1/4

\subsection{Goal 1: Agency in Navigation}


VIPs with an active attitude value agency over convenience, and thus have corresponding navigation goals to achieve more control and independence in their navigation experience. Even though for both groups, active and passive, the underlying aim of navigation is to find their way around an environment, we discovered that VIPs with active attitudes rank beyond guidance navigation goals higher than their counterparts.
% some navigation goals that are more important for VIPs with an active attitude than their counterpart. Particularly, we find that VIPs with active attitude value agency over convenience, and thus have corresponding navigation goals to achieve more control and independence in their navigation experience. 
Below, we outline these agency driven navigation goals by highlighting the difference between the two attitudes, while also pointing out the gaps in how existing NASs do not accommodate the navigation goals of VIPs with an active attitude.

\subsubsection{\textbf{Learning about General Layout of the Space.}}
VIP-participants with an active attitude reported the need to learn about the general shape and layout of an environment, both prior to visiting the environment and then during navigation. All participants in this category (n=4), expressed their desire to first learn about the general shape and then figure things out on their own during navigation. This preference resulted from the participants' need to build a mental map of the space that will assist them in finding their way around the space in a much more independent fashion by using their O\&M skills. As P4 puts it:\\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``[When I receive help] I will [ask], ‘what does this building generally look like?’ Because I want to understand [the shape of the building]. That's one of [the] first things [I want] to understand and that is a difficult thing to do as a blind person because I cannot look at satellite maps and it takes me a long time to [understand] the general shape [of a space], personally."} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm}

On the contrary, most (n=3) participants with a passive attitude stated that learning about the layout is not as important. Instead, they prefer to receive direct assistance from others -- either from sighted people or a system. This reliance on sighted assistance meant that their decision to visit an unfamiliar environment is dependent on availability of sighted assistance, including their friends and family. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``Usually for groceries, I ask somebody to assist me because [...] I feel like [the shape of the store is] really complicated to learn."} - \textbf{P6} & \\
\end{tabu}
\vspace{0.2cm}

In some scenarios, a few participants (n=2) with a passive attitude highlighted that even they ask for a general layout of the space. However, they shifted quickly towards getting assistance as the space becomes more and more complex to navigate. We found a direct relationship between the speed of this shift towards assistance and the participant's confidence in their O\&M skills.  This directly supports our hypothesis that O\&M training forms the basis of navigation preferences for both the categories.

Most existing NASs focus on providing turn-by-turn directions, without enabling the users to learn the general layout of the environment. Only a handful of approaches focus on this aspect of navigation. NavCog~\cite{}, for instance, uses a route preview feature that helps build a general understanding of the relative location of the different landmarks in an environment. Similarly, authors et al. ~\cite{} allow users to rehearse specific routes in an environment. Although these approaches help users build a better mental map of the indoor space, they do not provide the user with layout of the environment like: How wide is the hallway? What is the shape of the room? We found that these kinds of information are more valued by participants with an active attitude than their counterpart, and thus are a crucial part of advancing NASs to provide beyond guidance assistance.

\subsubsection{\textbf{Adding Landmarks to Mental Maps.}} 
Participants with active attitude utilize landmarks to further reinforce and their understanding of the general layout. All (n=4) participants with active attitude state that once they had a mental map with a general layout of the space, participants incorporated landmark information on top of the general layout to solidify their mental maps. For instance, P2 mentioned how they focused on understanding the general layout of a grocery store, and then supplemented their initial mental map with landmarks that were relevant to them. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``So [during my first visit, I was] essentially going through the whole grocery section [while looking for] the bathroom. I'm [asking to myself], ‘Where is everything else? There's bread here [...] Where's everything?’"} - \textbf{P2} & \\
\end{tabu}
\vspace{0.2cm}

Participants with a passive attitude, on the other hand, use landmark information to memorize the routes and not to create more complete mental maps of the environment. Consequently, existing approaches for route preview or route rehearsal serve these groups of participants well. For instance, P6 highlights this "route specific" behaviour of the participants in this group: \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"I try to use the wall like a  landmark [or I use] the doors that are near. [I use them] to follow just a straight line. "} - \textbf{P6} & \\
\end{tabu}
\vspace{0.2cm}

We also found an interesting nuance in how active attitudes stressed on creating a more robust set of landmarks. Given the dynamic nature of the environment, location of landmarks may change over time and landmarks created in previous visits may not be valid anymore. To mitigate this, participants reported that they created redundant landmarks such that even if one of the moves, or they end up missing one, others can be used to accurately orient themselves. In addition, participants mentioned building a hierarchy of importance of landmarks. Based upon the relative importance of the landmarks,
participants mentioned that they look for certain landmarks first and the redundant landmarks are used for confirmation. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"I've learned that you cannot rely [only] on one landmark [for navigation] because things change and the world is not static. [...] you may miss one landmark, but not the other so context is important. If you can find three landmarks in a location, then if you miss one or even two, you'll still have the third [which can help you] go back and find the other two to make sure that you're in the right place. [...] I found in my neighbourhood, for instance, there are very many fences that feel very similar within the four block radius of my house. So I can't say, ‘Okay, I will only pay attention to this type of fence’ because I will probably find [a similar fence] again on another block even though it's not the same one. I have to say, ‘this fence next to this telephone pole, with gravel.’ I need multiple layers [of information] But sometimes [the supplementary information] can be as simple as the traffic is closer here. [...]  So landmarks have a hierarchy of importance in my mind."} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\

Note that while this practice is common for both the groups, it is less prominent amongst the passive attitudes since they already rely on sighted assistance during navigation.

While current  NASs utilize landmarks, they do not consider their dynamic nature. 
% NavCog [], 
BLE-based systems for instance, use permanent architectural features as landmarks. This does not adequately reflect real life navigation practices, especially those of active VIPs, where many of the landmarks they depend on during navigation are in fact impermanent, and often fluid in nature.

\subsubsection{\textbf{Self-exploration for Robust Mental Maps.}}
VIPs with an active attitude preferred self-exploration over asking others for directions to complete their mental map. All participants mentioned that often, their mental maps are not robust enough to rely on completely for navigation. However, since the format of mental maps is different for active (complete maps), and passive (routes) attitudes, the two groups reported different approaches to fill-out the gaps in their mental maps for subsequent visits. Most participants (n=3) with an active attitude stated that they prefer to explore the environment themselves to augment their sensory cues. This not only helps them in getting familiar with the environment but also feel more independent. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[When I enter the mall] the echolocation can tell me some things [about the shape of a space], but I want specifics. So I will go to each side [of the entrance] and [check] how big [the entrance is]. And then I will see that there are two large openings from this foyer, one on either side, left and right, after a ways of wall. [I also learn that] there's a large opening into the main part of the mall. [From this information] I know that [the shape of the entrance] is probably a sort of long wide corridor, stretched out [perpendicularly] in front of me [...]”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\

Most participants with the passive attitude, on the other hand, prefer to update their mental maps -- which consist of routes, and not complete maps -- by asking for directions. For instance, P5 describe their approach: \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"Anything [that could be] as simple as finding a room that is not braille signed or a checkout counter [...] would require me to ask for directions."} - \textbf{P5} & \\
\end{tabu}
\vspace{0.2cm} \\

Current NASs do not offer adequate means of self-exploration. BLE based systems 


\subsection{Goal 2: Get Navigation help from non-VIPs effectively}

The two attitudes were further distinguishable through their preferences for navigation assistance. Participants showing active attitudes strongly preferred to receive only verbal instructions regarding directions and general layout of the space, navigating to their destination on their own. For example, most active participants (n=3) reported to avoid sighted guide assistance, because they backed their O\&M skills to help navigate to the destination if they had a bit more information about the environment. In contrast, all passive participants (n=4) preferred to received a more closely guided form assistance such as having the other person walk with them to the destination, or sighted guide assistance. However, both groups ended up receiving help in environments that were completely unfamiliar to them. Thus, communication with non VIPs is a crucial part of navigation for all VIPs. Below, we outline the navigation goals that emphasize VIPs' desire to communicate for and receive assistance effectively by exploring the different ways active and passive VIPs interact with others.

\subsubsection{\textbf{Communicating Needs and Receive Corresponding Assistance.}}
VIPs often ask for assistance from non-VIPs that may not be their friends or family. All participants, irrespective of their attitude, reported that non-VIPs struggled to understand their needs, leaving them frustrated. Participants with an active attitude, who prefer to receive verbal description, often found it difficult to understand the shape and layout of the environment based on non-VIP's descriptions. Our finding reinforces prior work that highlights the mismatch between how space is perceived by VIPs and non-VIPs. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"[I need to ask for clarification] because a lot of people describe [shapes with letters] like U shaped or H shaped. I know what U shaped is, but sometimes I forget what H shaped means [because] I don’t really use it. [I need to clarify that] I just prefer geometric shapes [for descriptions.]"} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\ 

In addition to reinforcing prior findings, we also found that all participants almost always asked for descriptions from their VIP-friends and family, who have been to a space before. P16 provides an example of how their VIP-friend helped them:\\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“So for example, [before I go to a train station] my friend will tell me this train [...] doesn't talk. And that's actually a big thing when it comes to travelling because then I'm really gonna have to pay attention and count the stops […] So my friend will let me know [that I am] really gonna have to pay attention [when riding that train] because this train doesn't talk and it doesn't let you know [what station you are at]”} - \textbf{P16} & \\
\end{tabu}
\vspace{0.2cm} \\ 

Most participants with a passive attitude reported frustration mostly in cases where non-VIPs do not know how to assist them. This finding reinforces the findings by Authors et al.~\cite{}. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I had somebody once when I was travelling grab the end of my cane and [try] to pull me along by my cane, and that’s not [the correct way to assist]”} - \textbf{P3} & \\
\end{tabu}
\vspace{0.2cm} \\ 

Ineffective help was not limited to inadequate assistance. In fact, VIPs often complained of cases in which non-VIPs overestimate the extent of the VIPs' disabilities, and thus offered assistance that they believed was necessary, rather than the help VIPs actually needed. For example, P4 describes an instance when non-VIPs have forced wheelchair service onto them out of ignorance.\\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[Airport staff are] relatively good at adapting [to our needs] usually, but the very first thing they always do [when they assist you] is they give you a wheelchair, and [some staff] insist that you use it. [...] I don't want to say that's insulting [...] But on the other hand, that is stupid [...] that is not their fault. It's their training.”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\ 


Despite the frustration and such experiences, all participants agreed that they did not expect non-VIPs to know the right way to help them, and hence expressed the need to be able to lead communication and work with non-VIPs in order to help non-VIPs assist VIPs. 

\subsubsection{\textbf{Get Help Without Social Pressure On the Helper.}}
Effectively receiving assistance was inhibited not only by communication but also due to external social pressures. We found that participants with an active attitude were more cognizant towards social factors compared to the other group. All participants (n=4) with an active attitude stated that were often apprehended by other people's perception of them, and sometimes their sighted guides as well. This caused participants to feel anxious and negatively impacted their ability to navigate environments. We observed that this feeling escalated when they received assistance from their friends and/or family. For example, P4 says:\\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I know that my sister gets looks from people all the time [when she acts as my sighted guide], because of foolish assumptions they make out of ignorance. [People think] that she is my caretaker, [and that] anything that they perceive as her not doing her job is wrong.”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\

%These sentiments were shared by the two business staff participants. blahblahblah

Since the active group valued autonomy and independence more, they did not want people to perceive them as relying on others. On the contrary, most participants with a passive attitude did not seem to be affected by what other people's perception of them. Unlike the other, passive attitudes remained unaffected, irrespective of who assisted them.

\subsection{Goal 3: Maintaining/Learning O\&M Skills}

\subsubsection{\textbf{Maintaining O\&M Skills.}} Most participants with an active attitude (n=3) preferred to use their O\&M skills as much as possible. Participants highlighted how they want to constantly keep working on their skills to feel more independent by not relying on assistance from others, practice and develop them further; to ultimately offer them the agency to make their own choices during navigation. For instance, P4 explains:\\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"It is very easy to let your [O\&M] skills atrophy as a blind person if you rely overly on sighted people and it's an easy trap to fall into. It's easy to [use a] sighted guide and become complacent and [not pay attention to] what turns you have taken and where you are in relation to other things." } - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\

On the other hand, most participants with a passive attitude preferred sighted assistance over using their O\&M skills for navigation -- primarily due to convenience. However, a few participants (n=2) in this category expressed their desire to obtain better O\&M training from an instructor, rather than practicing themselves.

% Shortage of O&M instructors

\subsubsection{\textbf{Learning O\&M Skills.}} Despite passive participants' preference for sighted assistance, we found sufficient evidence that even passive users may benefit from developing their O&M skills and encouraging active attitudes. 

% @David -- Might be useful to read when talking about Landmarks, Routes, and Maps: https://asisignage.com/2011/12/05/wayfinding-and-navigation-whats-the-difference/
% cool will check out

==> 4-Findings/v3.tex <==
% Structure:
    % context or build-up
    % --- main point (sub-heading)
    % --- stats
    % - Why did they want/do this?
    % What does this lead to?
    % --- Quote (if any)
    
Our thematic analysis revealed three \textit{``beyond guidance''} abilities, which emerged as major themes:
% \begin{itemize}
%     % \setlength{\itemindent}{.3in}
%     \item Agency in navigation: 
%     \item Get navigation help from non-VIPs effectively: 
%     \item Maintain and learn O\&M skills: 
% \end{itemize}
\begin{itemize}
    \setlength{\itemindent}{.3in}
    \item [(\textbf{A-1})] Active Engagement with the Environment
    \item [(\textbf{A-2})] Get Navigation help from non-VIPs effectively
    \item [(\textbf{A-3})] Maintain and Learn O\&M Skills
\end{itemize}
These abilities emerged from our interviews with all parties. Interestingly, however, only half (4/8) of the VIPs spoke to a need for these abilities. Participants were split on their attitudes towards wanting these abilities, with half of the participants strongly wanting all three and the other half being much more satisfied with receiving guidance only.
This means, if our sample of VIPs is representative of the VIP population at large, that the status quo of guidance-based NASs satisfy half of VIPs very well, but does not meet the more agency-oriented needs of the other half of VIPs. Below, we elaborate on these beyond guidance abilities in detail, and point out how current NASs are unable to address them.


% Sample: Below, we frst describe participants’ experiences when moving through the stages of airport travel. We then provide a description of perceptions of using a voice travel assistant to address the challenges encountered during this process.

\subsection{Ability 1: Active Engagement with the Environment}

The first ability that we learned was agency in navigation. Specifically, we heard remarks about VIPs' desire to learn about the general layout of the space, add dynamic landmarks to their mental map, and fortify their understanding of the space through self exploration. 
% Next, we ....
Here we describe these findings in more detail, while also pointing out the gaps in existing NASs regarding these abilities.

\subsubsection{\textbf{Learning about General Layout of the Space.}}
When navigating unfamiliar or rarely visited environments, participants expressed their desire to learn more information about the space that would help them specifically in building a mental map of that space. 
% Some VIP participants reported the need to learn about the general shape and layout of an environment, both prior to visiting the environment and then during navigation. 
Many participants (n=4) reported that knowing the overall layout of the space helped them navigate within that space more confidently, and also enabled them to explore the space and add to their mental map.
% For example, half of our participants (n=4), wanted to first learn about the general shape and then figure things out on their own during navigation. 
This preference resulted from the participants' need to build a mental map of the space that will assist them in finding their way around the space in a much more independent fashion by using their O\&M skills. As P4 puts it:\\
[why did VIPs want this?]



\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``[When I receive help] I will [ask], ‘what does this building generally look like?’ Because I want to understand [the shape of the building]. That's one of [the] first things [I want] to understand and that is a difficult thing to do as a blind person because I cannot look at satellite maps and it takes me a long time to [understand] the general shape [of a space], personally."} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm}

Most existing NASs focus on providing turn-by-turn directions, without enabling the users to learn the general layout of the environment. Only a handful of approaches focus on this aspect of navigation. %NavCog~\cite{}
BLE-based systems, for instance, use a route preview feature that helps build a general understanding of the relative location of the different landmarks in an environment. Similarly, %authors et al. ~\cite{} 
computer-vision-based systems allow users to rehearse specific routes in an environment. Although these approaches help users get acquainted to particular routes, they do not provide the user with information regarding the layout of the environment like: How wide is the hallway? What is the shape of the room? [We found that these kinds of information were extremely valuable]
We found that these kinds of information are valued by some participants, and thus are a crucial part of advancing NASs to provide beyond guidance assistance.

\subsubsection{\textbf{Adding Landmarks to Mental Maps.}} 

Our findings reinforce previous studies that VIPs utilize landmarks to further reinforce their understanding of the general layout of the environment. Half of our participants (n=4) state that once they had a mental map with a general layout of the space, they incorporated landmark information on top of the general layout to solidify their mental maps. For instance, P2 mentioned how they focused on understanding the general layout of a grocery store, and then supplemented their initial mental map with landmarks that were relevant to them. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``So [during my first visit, I was] essentially going through the whole grocery section [while looking for] the bathroom. I'm [asking to myself], ‘Where is everything else? There's bread here [...] Where's everything?’"} - \textbf{P2} & \\
\end{tabu}
\vspace{0.2cm}

We also found an interesting nuance in how VIPs created a more robust set of landmarks. Given the dynamic nature of the environment, location of landmarks may change over time and landmarks created in previous visits may not be valid anymore. To mitigate this, participants reported that they created redundant landmarks such that even if one of them moves, or they end up missing one, others can be used to accurately orient themselves. In addition, participants mentioned building a hierarchy of importance of landmarks. Based upon the relative importance of the landmarks,
participants mentioned that they look for certain landmarks first and the redundant landmarks are used for confirmation. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"I've learned that you cannot rely [only] on one landmark [for navigation] because things change and the world is not static. [...] you may miss one landmark, but not the other so context is important. If you can find three landmarks in a location, then if you miss one or even two, you'll still have the third [which can help you] go back and find the other two to make sure that you're in the right place. [...] I found in my neighbourhood, for instance, there are very many fences that feel very similar within the four block radius of my house. So I can't say, ‘Okay, I will only pay attention to this type of fence’ because I will probably find [a similar fence] again on another block even though it's not the same one. I have to say, ‘this fence next to this telephone pole, with gravel.’ I need multiple layers [of information] But sometimes [the supplementary information] can be as simple as the traffic is closer here. [...]  So landmarks have a hierarchy of importance in my mind."} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\

While current  NASs utilize landmarks, they do not consider their dynamic nature. BLE-based systems for instance, use permanent architectural features as landmarks. This does not adequately reflect the experiences of all VIPs, as we discovered many VIP depend on impermanent, and often fluid, landmarks for navigation. Similarly, computer-vision-based systems utilize a set of POIs from a pre-determined map, and hence do not provide the user with the ability to easily add and omit landmarks to reflect any changes in the location. We found that this fluidity was valued by some of our participants and thus is an integral extension for NASs to provide beyond guidance assistance. 


\subsubsection{\textbf{Self-exploration for Robust Mental Maps.}}
Often, VIPs wanted to simply learn more about a space without an actual destination in mind. 
Some VIPs preferred self-exploration over asking others for directions to complete their mental map. Half of our participants (n=4) mentioned that their mental maps are often not robust enough to rely on completely for navigation. Most of those participants (n=3) stated that they prefer to explore the environment themselves to augment their sensory cues. This not only helps them in getting familiar with the environment but also feel more independent. For example, P4 explained what type of specific information he looks for to complete his mental map.\\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[When I enter the mall] the echolocation can tell me some things [about the shape of a space], but I want specifics. So I will go to each side [of the entrance] and [check] how big [the entrance is]. And then I will see that there are two large openings from this foyer, one on either side, left and right, after a ways of wall. [I also learn that] there's a large opening into the main part of the mall. [From this information] I know that [the shape of the entrance] is probably a sort of long wide corridor, stretched out [perpendicularly] in front of me [...]”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\

While current NASs utilize the concept of mental maps and provide a means of practicing specific routes to become acquainted with the space, they do not offer adequate means of self-exploration. Both BLE based systems, and computer vision based systems use fixed POIs that are either used as end points of a route or announced to the user as they walk past them. However, they do not provide all the relevant information that VIPs may find useful in completing their mental maps. For example, they do not supplement many of the sensory details, such as sound or touch, that VIPs are already using. We found that self-exploration was an important step to navigation for many VIPs and thus providing the necessary sensory details to allow VIPs to explore and fill out their mental map is a necessary ability for NASs to provide beyond guidance assistance. 

\subsection{Ability 2: Get Nav Help from Non-VIPs effectively}

The second ability we found was receiving effective help from non-VIPs. Specifically, our participants reported their desire to communicate for and receive corresponding assistance, while avoiding any unwanted social interaction or attention. Below, we outline the navigation abilities that emphasize VIPs' desire to communicate for and receive correct assistance effectively.

\subsubsection{\textbf{Receive Correct Help.}}
Not all VIPs desire the same type of assistance. We found that some of our participants strongly preferred to receive only verbal instructions regarding directions and general layout of the space, navigating to their destination on their own. For example, nearly half (n=3) reported to avoid sighted guide assistance, because they backed their O\&M skills to help navigate to the destination if they had a bit more information about the environment. 

We further found that incorrect help was not limited to insufficient assistance. In fact, some of our VIPs (n=?) complained of cases in which non-VIPs overestimated the extent of their disabilities, and offered incorrectly excessive assistance. For example, P4 describes an instance when non-VIPs have forced wheelchair service onto them out of ignorance.\\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[Airport staff are] relatively good at adapting [to our needs] usually, but the very first thing they always do [when they assist you] is they give you a wheelchair, and [some staff] insist that you use it. [...] I don't want to say that's insulting [...] But on the other hand, that is stupid [...] that is not their fault. It's their training.”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\ 

Current guidance based NASs offer a fixed service to all users and do not consider a possible preference in level of engagement during navigation. Both BLE and computer vision based systems assume their users need as much help as they can get, and thus provide direct assistance, either through step-by-step instruction or through physical guide, but do not offer users the freedom to choose the level of help. However, this not only does not address the desires of VIP who prefer only verbal instruction, but this can also be demeaning to many VIPs. Beyond guidance NASs must enable their users in the way they prefer, and not in a way that may be most convenient. 

\subsubsection{\textbf{Communicate the Space Effectively.}}
Communication with non-VIPs is a crucial part of navigation for all VIPs that often proves to be difficult. %For example, VIPs often ask for assistance from non-VIPs that may not be their friends or family. 
All participants (n=8) reported that non-VIPs struggled to understand their needs, leaving them frustrated. Particularly, half of our participants (n=4), who prefer to receive verbal description, often found it difficult to understand the shape and layout of the environment based on non-VIP's descriptions. Our finding reinforces prior work that highlights the mismatch between how space is perceived by VIPs and non-VIPs. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"[I need to ask for clarification] because a lot of people describe [shapes with letters] like U shaped or H shaped. I know what U shaped is, but sometimes I forget what H shaped means [because] I don’t really use it. [I need to clarify that] I just prefer geometric shapes [for descriptions.]"} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\ 

In addition to reinforcing prior findings, we also found that effective communication must include relevant information. All participants almost always asked for descriptions from their VIP-friends and family, who have been to a space before. They explained that VIPs generally have a better understanding of what type of information would be useful for other VIPs than non-VIPs. P16 provides an example of how their VIP-friend helped them:\\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“So for example, [before I go to a train station] my friend will tell me this train [...] doesn't talk. And that's actually a big thing when it comes to travelling because then I'm really gonna have to pay attention and count the stops […] So my friend will let me know [that I am] really gonna have to pay attention [when riding that train] because this train doesn't talk and it doesn't let you know [what station you are at]”} - \textbf{P16} & \\
\end{tabu}
\vspace{0.2cm} \\ 

As current NASs are focused on direct guidance, they do not yet effectively communicate all the relevant information for VIPs. For example, BLE based systems use a set list of turn-by-turn instructions, but does not mention other relevant details such as the presence of other accessibility features, or notes of caution. Similarly, computer-based systems only announce POIs as the user passes them. 

\subsubsection{\textbf{Get Help Without Social Pressure On the Helper.}}
Effective assistance was prevented not only explicitly by communication, but also implicitly by external social pressures. We found that many participants were cognizant towards social factors.  Half of our  participants (n=4) stated that they were often apprehended by other people's perception of them, and sometimes their sighted guides as well. This caused participants to feel anxious and negatively impacted their ability to navigate environments. We observed that this feeling escalated when they received assistance from their friends and/or family. For example, P4 says:\\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I know that my sister gets looks from people all the time [when she acts as my sighted guide], because of foolish assumptions they make out of ignorance. [People think] that she is my caretaker, [and that] anything that they perceive as her not doing her job is wrong.”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\
Since P4 valued autonomy and independence more, they did not want people to falsely perceive them as relying on others. 

In fact, implicit social pressures was also an issue reported by the business staff. For example, P13 reported their difficulty gauging whether or not they should offer assistance. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I personally think that the tough [judgement to make] is [whether or not to offer help].  I'm always concerned with invading somebody's personal space or [disregarding] their bodily autonomy. So I think it's a matter of just trying to be cognizant and aware of [things like]  if somebody seems like they need help [or] if somebody seems like they are totally fine. [It] is not a perfect system, obviously, [and] mistakes will be made.”} - \textbf{P13} & \\
\end{tabu}
\vspace{0.2cm} \\

As current NASs offer systems solutions for guidance-based navigation assistance, they do not properly address the issue of discretion. For example, while computer-based systems, such as CaBot, have been designed to minimize public attention, they still draw attention due to the relatively larger hardware components. On the other hand, BLE-based systems have a better form-factor in that they are contained in a smartphone, they still do not address the issue of discrete communication between users and non-VIP. For example, VIPs cannot discretely request for spaces to become equipped with the necessary hardware so they may be navigable. Some systems, such as AIRA provide a means of connecting non-VIPs to VIPs without social interactions, but these are not navigation assistance systems and lack many of the other functionalities of an NAS. 


\subsection{Ability 3: Maintain and Learn O\&M skills}

The third ability was maintaining and learning O\&M Skills. Our findings supported previous studies in the importance of O\&M training. Thus, we found that O\&M skills were an integral part of VIPs' independence, especially when in terms of navigating. Below, we highlight the abilities that may benefit VIPs' need to maintain or develop their O\&M skills.

\subsubsection{\textbf{Maintaining O\&M Skills.}}
Supporting previous studies, many of our participants (n=4) highlighted the importance of O\&M skills in their lives, empowering them with independence and autonomy during navigation. As P4 explains:  \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[O\&M skills are] vital because the world will walk over you if you [don’t] take control of your own abilities. [...] People will tell you where you can go and what you can do if you do not interject. And if you don't know how to do those things, then you're just kind of meekly following along. It's self esteem shattering, [and] reduces your individuality.”} - \textbf{P4} & \\
\end{tabu} \\

On top of reinforcing previous findings, we found that some of our participants (n=3) preferred to use their O\&M skills as much as possible. These participants highlighted how they want to constantly keep working on their skills to feel more independent by not relying on assistance from others, practice and develop them further; to ultimately offer them the agency to make their own choices during navigation. In fact, they reported a need to constantly practice these skills, and how too much assistance could be detrimental to maintaining them. For instance, P4 explains:\\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"It is very easy to let your [O\&M] skills atrophy as a blind person if you rely overly on sighted people and it's an easy trap to fall into. It's easy to [use a] sighted guide and become complacent and [not pay attention to] what turns you have taken and where you are in relation to other things." } - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\

While current systems do utilize many O\&M skills in their functionality, they do not offer a means for VIPs to practice their O\&M skills. In fact, both BLE-based systems, as well as computer-vision based systems utilize step-by-step instructions or even sighted guidae style assistance, which may in fact cause VIPs' skills to deteriorate. 

\subsubsection{\textbf{Learning O\&M Skills.}}

While O\&M is a valuable skill, it is not always readily available. In fact half of our participants (n=4), reported to only have receive limited O\&M training. There were several factors that affected access.

The first reason is lack of access. For VIPs who develop vision impairments earlier in life or are blind by birth have easy access to O\&M training through their schools. However, VIPs that develop visual impairments later in life often find it difficult to arrange one. All our participants developed vision impairment either from birth (P2, P3, P5, P6, P8, P16), or earlier in life (P4: by the age of four, P7: by the age of one). All of them stated that they were assigned an O\&M trainer in school. However, many participants (n=6) stated that it is much more difficult to set up an O\&M session as an adult, compared to getting one as a child in school. As a result, most of their O\&M training was done during K-12 school. For instance, P16 (who is blind by birth) explains:

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“For earlier years, I d[id]n't need to reach out [to O\&M trainers] because that's something that like, we automatically get [in schools]. Now, I definitely would have to advocate for myself [by reaching out to] the Rehab Center or something like that. [...] I can’t expect them to reach out to me.”} - \textbf{P16} & \\
\end{tabu}
\vspace{0.2cm}

The second reason is lack of O/&M trainers. Despite being eligible for benefits during K-12 school, there may still be a possibility that VIPs did not receive appropriate O\&M training during school. This is primarily due to shortage of O\&M trainers and decentralization. O\&M trainers are assigned multiple students scattered over a geographical area, which makes it difficult for them to be physically present and provide enough time to all their students. P7, who was assigned an O\&M trainer during middle school, describes the reason behind their lack of access to an O\&M trainer:

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I was told that I would get an O\&M trainer back in middle school [...] I never received that trainer. She came in once within the six years she was supposed to be training me. [...] I actually had my English teacher in middle school, walking around campus with me after the classes being like, 'Hey, here's what this class is'. 
%  [...] So she was kind of more of a navigation instructor than the O\&M instructor that was supposed to be assigned to me.
 ”} - \textbf{P7} & \\
\end{tabu}
\vspace{0.2cm}

This was supported by our interviews with O/&M instructors. Both O\&M instructors reported that a shortage of trainers was a common problem. 

Finally, there may be lack of funding. All our participants reported that they are dependent upon the state to receive O\&M training facilities. A few participants (n=2) highlighted that their state provides limited resources due to shortage of funds, thereby affecting their ability to receive O\&M training:

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“It's just very hard to get [O\&M training here] because [anonymized state] is out of money. [...] it's very hard to [receive O\&M training because] you've got to prove that you’re working.”} - \textbf{P3} & \\
\end{tabu}
\vspace{0.2cm}

Thus, we suggest that NASs could not only provide a means of practicing but also an effective way of developing these skills.

\subsection{ Perspective from Participants Favoring Guidance only}

Our findings about the other people, who were satisfied with guidance based assistance, reinforce prior work that builds off of this perspective prefers to be guided. With respect to Active Engagement in Navigation,  they did not find a need for more agency and thus were satisfied with the route-centered nature of guidance based assistance. Similarly, for Getting Navigation Help from Non-VIP effectively, while they agreed that non-VIPs were often unhelpful, they were unphased by external social pressures. Finally, regarding Ability \# 3, while they agreed on the importance and utility of O\&M skills, they valued convenience more and thus did not want to spend the effort to practice and develop these skills. Below, we discuss in further detail how the experience of these participants reinforce prior findings. 

\subsubsection{\textbf{Agency in Navigation}}

The other half of our participants (n=4) were satisfied with the convenience of guidance based navigation assistance, and hence did not mention a need for more agency. However, their experiences support prior studies in their preference for guidance-based approaches. 

For example, some of these participants (n=3) stated that learning about the layout is not as important. Instead, they prefer to receive direct assistance from others -- either from sighted people or a system. This reliance on sighted assistance meant that their decision to visit an unfamiliar environment is dependent on availability of sighted assistance, including their friends and family. \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``Usually for groceries, I ask somebody to assist me because [...] I feel like [the shape of the store is] really complicated to learn."} - \textbf{P6} & \\
\end{tabu}
\vspace{0.2cm}

In some scenarios, a few of these participants (n=2) with a passive attitude highlighted that even they ask for a general layout of the space. However, they shifted quickly towards getting assistance as the space becomes more and more complex to navigate. We found a direct relationship between the speed of this shift towards assistance and the participant's confidence in their O\&M skills.  This directly supports our hypothesis that O\&M training forms the basis of navigation preferences for both the categories.

Similarly, these participants (n=4) use landmark information to memorize the routes and not to create more complete mental maps of the environment. Consequently, existing approaches for route preview or route rehearsal serve this group of participants well. For instance, P6 highlights this "route specific" behaviour: \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"I try to use the wall like a  landmark [or I use] the doors that are near. [I use them] to follow just a straight line. "} - \textbf{P6} & \\
\end{tabu}
\vspace{0.2cm}


This reinforces prior findings, use of non-visual cues and landmarks

Reinforcing prior findings:
- Dias et al. [20] further assessed which features support indoor navigation and orientation of PVI through an interview with 20 participants. The majority of the participants reported that they use environmental cues (e.g., smells, sounds) or landmarks (e.g., doorways, elevators) to inform their decisions during navigation --- Ref \#20 from NavCog3 paper.

\subsubsection{\textbf{ Get Navigation help from non-VIPs effectively}}

Furthermore, the other half of our participants (n=4) preferred to received a more closely guided form assistance such as having the other person walk with them to the destination, or sighted guide assistance. Thus, their experiences reinforced prior findings on the inadequacy of non-VIP assistance. 

For example, all of these participants (n=4) prefer to update their mental maps -- which consist of routes, and not complete maps -- by asking for directions. For instance, P5 describe their approach: \\

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"Anything [that could be] as simple as finding a room that is not braille signed or a checkout counter [...] would require me to ask for directions."} - \textbf{P5} & \\
\end{tabu}
\vspace{0.2cm} \\

However, for these participants, their frustration originated mostly from when non-VIPs did not know how to assist them. For example, P3 highlights an unpleasant experience receiving bad help from a non-VIP.

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I had somebody once when I was travelling grab the end of my cane and [try] to pull me along by my cane, and that’s not [the correct way to assist]”} - \textbf{P3} & \\
\end{tabu}
\vspace{0.2cm} \\ 

This finding reinforces the findings by Authors et al.~\cite{}. \\

\subsubsection{\textbf{ Maintain and Learn O\&M skills}}

The other participants preferred sighted assistance over using their O\&M skills for navigation -- primarily due to convenience. However, there experiences still support prior studies on the importance of these skills. 

In fact, a few participants (n=2) in this category expressed their desire to obtain better O\&M training. For instance, P7 shared how he believed he would have benefited from further O\&M instruction. 

\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I feel like I would have benefited [from O\&M training]. I don't want to feel like I'm overexaggerating, but [I would be] at least 10 times more [independent at navigating] if I just had that training. [I would have preferred the trainer] telling me, ‘Hey, here's where we're going. Here's what we're going to do. Here's how to do it properly.’ Instead of [having to rely on a sighted guide] just [telling me], ‘Hey, we're going here. Enjoy.’”} - \textbf{P7} & \\
\end{tabu}
\vspace{0.2cm} \\ 

However, these participants preferred to receive training from an instructor, rather than practicing themselves. Nevertheless, their experiences reinforce prior studies on the important of O\&M skills for VIP navigation. 


==> 4-Findings/v4.tex <==
In the following we present an analysis of our semi-structured interviews to answer (\textbf{RQ-1}).
Our thematic analysis revealed three forms of active engagement that are important for VIPs when navigating unfamiliar environments: 
% which emerged as major themes:
\begin{itemize}
    \setlength{\itemindent}{.3in}
    \item [(\textbf{A-1})] Engaging with the Environment
    \item [(\textbf{A-2})] Getting Effective Navigation Help from Others
    \item [(\textbf{A-3})] Maintaining and Learning O\&M Skills
\end{itemize}
These forms of active engagement emerged from our interviews with all parties and are not currently facilitated by NASs. 
Interestingly, however, only half (4/8) of the VIPs spoke to a need for these abilities. 
Participants were split on their attitudes towards wanting these abilities, with half of the participants strongly wanting all three and the other half being much more satisfied with receiving guidance only.
This means, if our sample of VIPs is representative of the VIP population at large, that the status quo of guidance-based NASs satisfy half of VIPs very well, but does not meet the more agency-oriented needs of the other half of VIPs. 
Below, we elaborate on these beyond guidance abilities in detail. 
We notice that no NASs have these abilities.

\subsection{Engaging with the Environment}
The first form of active engagement that we learned was engaging with the environment.
Specifically, we heard remarks about VIPs' desire to learn about the general layout of the space, generate a mental map through self-exploration, and add dynamic landmarks to their mental map. 
Here we report our findings and how they lead to each of these aspects of this form of active engagement.

% [each subsection is an aspect of the forms of active engagement]
\subsubsection{\textbf{Learn the General Layout of the Space.}}
We found that learning the general layout of the space was a key aspect of engaging with the environment.
When navigating unfamiliar or rarely visited environments, participants expressed their desire to learn information about the space that would help them build a mental map of that space. 
Many participants (n=4) reported that knowing the overall layout of the space helps them navigate within that space more confidently, and also enables them to explore the space independently.
As P4 put it:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``[When I receive help] I will [ask], ‘what does this building generally look like?’ Because I want to understand [the shape of the building]. That's one of [the] first things [I want] to understand and that is a difficult thing to do as a blind person because I cannot look at satellite maps and it takes me a long time to [understand] the general shape [of a space], personally."} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm}\\\\
While understanding the general layout often proves to be difficult, it allows him to find his way around the space in a much more independent fashion by using his O\&M skills. 

Most existing NASs focus on providing turn-by-turn directions, without enabling the users to learn the general layout of the environment. 
Only a handful of approaches focus on this aspect of navigation.
BLE-based systems, for instance, use a route preview feature that helps build a general understanding of the relative location of the different landmarks in an environment.
Similarly, computer-vision-based systems allow users to rehearse specific routes in an environment.
Although these approaches help users get acquainted to particular routes, they do not provide the user with information regarding the layout of the environment like: 
How wide is the hallway? 
What is the shape of the room?
We found that these kinds of information are valued by some participants, and thus are a crucial part of promoting more active engagement with the environment.

\subsubsection{\textbf{Generate a Mental Map Through Self-Exploration.}}
Our participants reported that they further engage with the environment through self-exploration.
Often, VIPs want to simply learn more about a space without an actual destination in mind. 
For many VIPs, an initial mental map consisting of the layout is not robust enough to rely on completely for navigation. 
We found that some of our participants (n=4) prefer self-exploration over asking others for directions to complete their mental maps.
%Half of our participants (n=4) mentioned that their mental maps were often not robust enough to rely on completely for navigation. 
Most of these participants (n=3) stated that they prefer to explore the environment themselves to augment their non-visual skills. 
For example, P4 explained what type of specific information he looks for to complete his mental map:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[When I enter the mall] the echolocation can tell me some things [about the shape of a space], but I want specifics. So I will go to each side [of the entrance] and [check] how big [the entrance is]. And then I will see that there are two large openings from this foyer, one on either side, left and right, after a ways of wall. [I also learn that] there's a large opening into the main part of the mall. [From this information] I know that [the shape of the entrance] is probably a sort of long wide corridor, stretched out [perpendicularly] in front of me [...]”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Through self-exploration, P4 solidified his understanding of the space by gathering supplementary information for sensory cues he was already using, such as sound. 
%This not only helped him get familiar with the environment but also feel more independent. 
Furthermore, P4 was able to learn how the foyer led to another corridor. Thus, self-exploration allowed him to combine disjoint architectural features into a more robust and complete mental map of the environment.

While current NASs utilize the concept of mental maps and provide a means of practicing specific routes to become acquainted with the space, they do not offer adequate means of self-exploration. 
Both BLE based systems, and computer vision based systems use fixed POIs that are either used as end points of a route or announced to the user as they walk past them. 
However, they do not provide all the relevant information that VIPs may find useful in completing their mental maps. 
For example, they do not supplement many of the sensory details, such as sound or touch, that VIPs are already using or show the user how the separate routes may be connected. Providing the necessary means for self-exploration can enable VIPs to generate their own routes based on their mental maps, and better engage with the environment during navigation.  

\vspace{5mm}
\fbox{\begin{minipage}{0.95\linewidth}
\textbf{Insight 1}: VIPs want to learn about the general layout of the space in a manner that engages them with the environment, i.e., via self-exploration
\end{minipage}}

\subsubsection{\textbf{Add Dynamic Landmarks to Mental Map.}}
The final step to engage with the environment involves filling the mental map with landmarks, which are often dynamic in nature.
Participants (n=4) stated that once they had a mental map with a general layout of the space, they incorporated landmark information on top of the general layout to solidify their mental maps. 
For instance, P2 mentioned how they focused on understanding the general layout of a grocery store, and then supplemented their initial mental map with landmarks that were relevant to them. \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``So [during my first visit, I was] essentially going through the whole grocery section [while looking for] the bathroom. I'm [asking to myself], ‘Where is everything else? There's bread here [...] Where's everything?’"} - \textbf{P2} & \\
\end{tabu}
\vspace{0.2cm}\\\\
This supports previous studies in that VIPs utilize landmarks to further reinforce their understanding of the general layout of the environment. 

We also found an interesting nuance in how VIPs created a more robust set of landmarks. 
Given the dynamic nature of the environment, location of landmarks may change over time and landmarks created in previous visits may not be valid anymore. 
To mitigate this, participants reported that they created redundant landmarks such that even if one of them moves, or they end up missing one, others can be used to accurately orient themselves. 
In fact, participants mentioned building a hierarchy of importance of landmarks.
Based upon the relative importance of the landmarks, participants looked for certain landmarks first and used the redundant landmarks for confirmation.
P4 explained:  \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"I've learned that you cannot rely [only] on one landmark [for navigation] because things change and the world is not static. [...] you may miss one landmark, but not the other so context is important. If you can find three landmarks in a location, then if you miss one or even two, you'll still have the third [which can help you] go back and find the other two to make sure that you're in the right place. [...] I found in my neighbourhood, for instance, there are very many fences that feel very similar within the four block radius of my house. So I can't say, ‘Okay, I will only pay attention to this type of fence’ because I will probably find [a similar fence] again on another block even though it's not the same one. I have to say, ‘this fence next to this telephone pole, with gravel.’ I need multiple layers [of information] But sometimes [the supplementary information] can be as simple as the traffic is closer here. [...]  So landmarks have a hierarchy of importance in my mind."} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Treating landmarks as static singular entities can be misleading. Multiple landmarks of different priority help VIPs get a more complete understanding of the space, and prepare for any changes that may arise in the environment.

While current  NASs utilize landmarks, they do not consider their dynamic nature. 
BLE-based systems for instance, use permanent architectural features as landmarks. 
This does not adequately reflect the experiences of all VIPs, as we discovered many VIP depend on impermanent, and often fluid, landmarks for navigation. 
Similarly, computer-vision-based systems utilize a set of POIs from a pre-determined map, and hence do not provide the user with the ability to easily add and omit landmarks to reflect any changes in the location. 
Fluid and dynamic landmarks allow for VIPs to actively engage with a dynamic environment, and ultimately adapt quicker to any changes. 

\vspace{5mm}
\fbox{\begin{minipage}{0.95\linewidth}
\textbf{Insight 2}: VIPs want to utilize dynamic landmarks to account for non-static nature of spaces.
\end{minipage}}

\subsection{Getting Effective Navigation Help from Others}
The second form of active engagement is receiving effective help from non-VIPs.
While VIPs' primary goal is to navigate independently, interacting and receiving assistance from others is also a part of VIPs' navigation.
Our participants reported their desire to avoid getting too much help, get all relevant information about a space, and get help without putting social pressure on the helper. 
We found that these aspects of receiving help lead VIPs to more actively engage with the navigation process, by receiving effective assistance without becoming too complacent or reliant on others.
Below, we outline our findings in more detail and explain how they motivate this form of active engagement.


% [May add some of this language in the preamble to address the fact that assistance from others is also a part of VIPs' navigation] VIPs often rely on multiple senses during navigation. In addition, information/assistance obtained from others in the environment forms an important aspect of their navigation. Participants mentioned their desire to actively voice their needs during navigation, which includes interaction with others in the surrounding environment, for help.

\subsubsection{\textbf{Avoid Getting Too Much Help}}
Not all VIPs desire the same type of assistance; receiving the correct amount, specifically avoiding too much, is an integral part of receiving effective help.
For example, we found that some of our participants (n=4)  strongly prefer to receive only verbal instructions regarding directions and general layout of the space, so they may navigate to their destination on their own. 
In fact, nearly half (n=3) reported to avoid sighted guide assistance in most situations, and instead opted to use their O\&M skills to help navigate to the destination despite the inconvenience. 

We further found that despite these preferences, VIPs were often offered incorrectly excessive assistance
For example, P4 described an instance when non-VIPs have forced wheelchair service onto him out of ignorance:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[Airport staff are] relatively good at adapting [to our needs] usually, but the very first thing they always do [when they assist you] is they give you a wheelchair, and [some staff] insist that you use it. [...] I don't want to say that's insulting [...] But on the other hand, that is stupid [...] that is not their fault. It's their training.”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
While wheelchair service might be more convenient, it did not match P4's preferences, specifically in that it assumed and reinforced a passive role in Excessive assistance in this case was not only unnecessary but also demeaning. 
P4's experience highlights the general mismatch between non-VIPs' expectations and VIPs' abilities. 

Current guidance based NASs offer a fixed service to all users and do not consider a possible preference in level of engagement during navigation. 
Both BLE and computer vision based systems assume their users need as much help as they can get, and thus provide direct assistance, either through step-by-step instruction or through physical guide, but do not offer users the freedom to choose the level of help. 
However, this does not address the desires of VIP who prefer only verbal instruction, and can even be degrading to many VIPs. 
Effective navigation assistance thus must enable their users in the way they prefer, and not in a way that may be most convenient. 

\subsubsection{\textbf{Get all Relevant Information.}}
Communication with non-VIPs is a crucial part of navigation for all VIPs that often proves to be difficult.
All participants (n=8) reported that non-VIPs struggled to understand their needs, leaving them frustrated. 
For example, P4 found it difficult to understand the shape and layout of the environment based on non-VIP's descriptions. 
He explained:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"[I need to ask for clarification] because a lot of people describe [shapes with letters] like U shaped or H shaped. I know what U shaped is, but sometimes I forget what H shaped means [because] I don’t really use it. [I need to clarify that] I just prefer geometric shapes [for descriptions.]"} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Non-VIPs often utilize visual details when describing a space. 
However, as P4 explained, this is not always applicable to VIPs. 
In fact, we found that VIPs often preferred non-visual descriptions for navigation, such as when the floor tile changed materials. 
Our finding reinforces prior work that highlights the mismatch between how space is perceived by VIPs and non-VIPs.

We also found that effective communication must include relevant information. 
All participants (n=8) almost always asked for descriptions from their VIP-friends and family, who have been to a space before. 
They explained that VIPs generally have a better understanding of what type of information would be useful for other VIPs than non-VIPs. 
For example, P16 reported a time when a description from a non-VIP caused confusion: \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"Sometimes there'll be a [situations] where [a non-VIP tells me], ‘Oh,[the place I’m looking for is] the third door.’ And I'm like, ‘Okay, [...] this is the third door, but [...]  it's not the [right place]’  I think they mean[t] third classroom door, but there's a storage room [next to the classrooms]. [I didn’t know] they d[id]n't count that as a door or a room."} - \textbf{P16} & \\
\end{tabu}
\vspace{0.2cm} \\\\
She further contrasted her experience with an description she received from a VIP friend: \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“So for example, [before I go to a train station] my friend will tell me this train [...] doesn't talk. And that's actually a big thing when it comes to travelling because then I'm really gonna have to pay attention and count the stops […] So my friend will let me know [that I am] really gonna have to pay attention [when riding that train] because this train doesn't talk and it doesn't let you know [what station you are at]”} - \textbf{P16} & \\
\end{tabu}
\vspace{0.2cm} \\\\ 
Descriptions from her VIP friend not only matched P16's perception of space, but also included other relevant details that P16 also found important or useful. 

As current NASs are focused on direct guidance, they only provide a limited set of verbal descriptions. 
For example, BLE based systems and computer-based systems announce the presence POIs and landmarks, but do not mention other relevant information such as the presence of other accessibility features, or notes of caution. 
We found that VIPs often need these details to successfully navigate a space, especially if they are visiting a place independently. 
A way of communicating all the relevant information in a way that is comprehensible for VIPs is a crucial step for allowing VIPs to receive navigation help from non-VIPs effectively. 



\subsubsection{\textbf{Get Help Without Putting Social Pressure On the Helper.}}
VIPs also expressed the desire to get navigational help from others without unintentionally putting social pressure on them. 

Social pressures prevent VIPs from receiving effective assistance.
%Effective assistance was prevented not only explicitly by communication, but also implicitly by external social pressures.
% Both external social pressures and comm prevented effective assistance, they do so implicitly and explicitly respectively.
We found that many participants were cognizant towards social factors.  
Half of our  participants (n=4) stated that they were often apprehended by other people's perception of them, and sometimes their sighted guides as well. 
This caused participants to feel anxious and negatively impacted their ability to navigate environments. 
We observed that this feeling escalated when they received assistance from their friends and/or family. 
For example, P4 said:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I know that my sister gets looks from people all the time [when she acts as my sighted guide], because of foolish assumptions they make out of ignorance. [People think] that she is my caretaker, [and that] anything that they perceive as her not doing her job is wrong.”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
He added that while he understood these assumptions were due to ignorance, he still felt the false perceptions was putting unwanted social pressure on his sighted guide.

The negative impact of social pressures on non-VIPs was corroborated by our interviews with business staff. 
For example, P13 reported their difficulty determining whether or not they should offer assistance: \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I personally think that the tough [judgement to make] is [whether or not to offer help].  I'm always concerned with invading somebody's personal space or [disregarding] their bodily autonomy. So I think it's a matter of just trying to be cognizant and aware of [things like]  if somebody seems like they need help [or] if somebody seems like they are totally fine. [It] is not a perfect system, obviously, [and] mistakes will be made.”} - \textbf{P13} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Non-VIP staff had difficulty deducing whether or not to assist someone, and often opted to not interfere out of fear of acting in a socially unacceptable manner. 

Current NASs do not properly address the issue of discretion. 
For example, while computer-based systems, such as CaBot, have been designed to minimize public attention, they can still draw unwanted attention due to the relatively larger hardware components. 
On the other hand, BLE-based systems have a better form-factor in that they are contained in a smartphone; however, they still do not address the issue of discrete communication between users and non-VIP. 
For example, VIPs cannot discretely request for spaces to become blind-accessible. 
Some systems, such as AIRA provide a means of connecting non-VIPs to VIPs without social interactions, but these are not navigation assistance systems and lack many of the other functionalities of an NAS. 
We found that social pressures can negatively impact both the frequency and quality of assistance to VIPs, and thus minimizing the social tensions is integral for VIPs to receive effective navigational assistance from non-VIPs.

\subsection{Maintaining and Learning O\&M skills}
The third ability was maintaining and learning O\&M Skills. 
Our findings supported previous studies in the importance of O\&M training. 
Thus, we found that O\&M skills were an integral part of VIPs' independence, especially in terms of navigating. 
Below, we highlight the abilities that may benefit VIPs' need to maintain or develop their O\&M skills.

\subsubsection{\textbf{Maintain O\&M Skills.}}
Many of our participants (n=4) highlighted the importance of O\&M skills in their lives, empowering them with independence and autonomy during navigation. 
As P4 explained:  \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[O\&M skills are] vital because the world will walk over you if you [don’t] take control of your own abilities. [...] People will tell you where you can go and what you can do if you do not interject. And if you don't know how to do those things, then you're just kind of meekly following along. It's self esteem shattering, [and] reduces your individuality.”} - \textbf{P4} & \\
\end{tabu} \\\\
P4 further elaborated that he even denied assistance out of fear of his skills deteriorating:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"It is very easy to let your [O\&M] skills atrophy as a blind person if you rely overly on sighted people and it's an easy trap to fall into. It's easy to [use a] sighted guide and become complacent and [not pay attention to] what turns you have taken and where you are in relation to other things." } - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
In fact, many of our participants (n=3) shared this sentiment, and preferred to use their O\&M skills as much as possible, even denying sighted assistance. 
While O\&M skills are critical to VIPs' autonomy, they can worsen without regular use, thus revealing VIPs' need to practice these skills. 

No current NAS systems offer an explicit means of practicing and honing the skills needed for independent navigation. 
Both BLE-based and computer-vision based systems rely on the users' O\&M skills  to follow step-by-step instructions; however, the systems do not encourage their users to actively engage with the environment.
For example, these systems do not promote the users to be more aware of the non-visual sensory cues and the orientation or mobility techniques used during navigating. 
On the other hand, \cite{min2021augmented} have explored various prototypes of augmented reality solution to practice orientation and mobility through augmenting VIPs' non-visual senses; yet these systems are not NASs in that they do not provide other key navigation functions such as directional guidance.
As O\&M skills are crucial for VIPs to remain independent, for NASs to promote active engagement in navigation, they must provide an explicit means of maintaining and preventing any deterioration of these skills.

\subsubsection{\textbf{Learn O\&M Skills.}}
Our findings further showed that O\&M training was in fact not always readily available. 
Half of our participants (n=4), reported to only have receive limited O\&M training. 
There were several factors that affected access.

The first reason was lack of access. 
For VIPs who developed vision impairments earlier in life or are blind by birth have easy access to O\&M training through their schools. 
However, VIPs that develop visual impairments later in life often find it difficult to arrange one. 
All our participants developed vision impairment either from birth (P2, P3, P5, P6, P8, P16), or earlier in life (P4: by the age of four, P7: by the age of one). 
All of them stated that they were assigned an O\&M trainer in school.  
However, many participants (n=6) stated that it became much more difficult to set up an O\&M session as an adult, compared to getting one as a child in school. 
For instance, P16 (who is blind by birth) explained:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“For earlier years, I d[id]n't need to reach out [to O\&M trainers] because that's something that like, we automatically get [in schools]. Now, I definitely would have to advocate for myself [by reaching out to] the Rehab Center or something like that. [...] I can’t expect them to reach out to me.”} - \textbf{P16} & \\
\end{tabu}
\vspace{0.2cm}\\\\
As a result most of her O\&M training was done during K-12 school.

The second reason was lack of O\&M trainers. 
Despite being eligible for benefits during K-12 school, VIPs may still not be able to receive appropriate O\&M training during school. 
Our interviews with the O\&M instructors have revealed that this is primarily due to shortage of O\&M trainers and decentralization. 
Bother instructors confirmed that O\&M trainers are assigned multiple students scattered over a geographical area, which makes it difficult for them to be physically present and provide enough time to all their students. 
Similarly, P7, who was assigned an O\&M trainer during middle school, described the reason behind their lack of access to an O\&M trainer:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I was told that I would get an O\&M trainer back in middle school [...] I never received that trainer. She came in once within the six years she was supposed to be training me. [...] I actually had my English teacher in middle school, walking around campus with me after the classes being like, 'Hey, here's what this class is'. 
%  [...] So she was kind of more of a navigation instructor than the O\&M instructor that was supposed to be assigned to me.
 ”} - \textbf{P7} & \\
\end{tabu}
\vspace{0.2cm}\\\\
Due to this reason, P7 never received formal O\&M training, despite his belief that it would have benefited him. 

Finally, there may be lack of funding. 
All our participants reported that they were dependent upon their respective states to receive O\&M training facilities. 
A few participants (n=2) highlighted that their state provided limited resources due to shortage of funds, thereby affecting their ability to receive O\&M training.
For example, P3 said:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“It's just very hard to get [O\&M training here] because [anonymized state] is out of money. [...] it's very hard to [receive O\&M training because] you've got to prove that you’re working.”} - \textbf{P3} & \\
\end{tabu}
\vspace{0.2cm}\\\\
He further explained that due to limited funding, adult VIPs were limited to vocational rehabilitation, which was a partial form of training meant only to supply the necessary skills for a VIP to perform a specific job.  Even this type of training was scarce, and VIPs had to prove their employment status.

For these reasons, lack of O\&M training is a problem faced by many VIPs. 
However, most current systems do not provide a means of learning O\&M skills, 
Providing an efficient systems solution to O\&M training could help democratize the skills necessary for VIPs navigate independently. 
Hence, we suggest that NASs could not only provide a means of practicing but also an effective way of developing these skills.

\subsection{ Perspective from Participants Favoring Guidance only}
Our findings about VIPs who were satisfied with guidance based assistance, reinforce prior work that builds off of this perspective of those who prefer to be guided. 
%With respect to Active Engagement with the environment,  they 
Half of our participants (n=4) did not find a need for more agency and thus were satisfied with the route-centered nature of guidance based assistance. 
Similarly, %for Getting Navigation Help from Non-VIP effectively, 
while they agreed that non-VIPs were often unhelpful, they were unphased by external social pressures, and were eager to accept sighted guide assistance.
Finally, while they agreed on the importance and utility of O\&M skills, they valued convenience more and thus did not want to spend the effort to practice and develop these skills. 
Below, we discuss in further detail of the experiences of these participants. 

\subsubsection{\textbf{Active Engagement with the Environment}}
Some of these participants (n=3) stated that learning about the layout was not as important as getting to the destination. 
They explained that they preferred to receive direct assistance from others -- either from sighted people or through a system. 
This reliance on sighted assistance meant that their decision to visit an unfamiliar environment was dependent on availability of sighted assistance, including their friends and family. \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``Usually for groceries, I ask somebody to assist me because [...] I feel like [the shape of the store is] really complicated to learn."} - \textbf{P6} & \\
\end{tabu}
\vspace{0.2cm}\\\\
In some scenarios, a few of these participants (n=2) highlighted that even they asked for a general layout of the space. 
However, they shifted quickly towards getting assistance as the space became more and more complex to navigate. 
We found a direct relationship between the speed of this shift towards assistance and the participant's confidence in their O\&M skills.  

Similarly, these participants (n=4) used landmark information to memorize the routes and not to create more complete mental maps of the environment. 
Consequently, existing approaches for route preview or route rehearsal serve this group of participants well. 
For instance, P6 highlighted this "route specific" behaviour: \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"I try to use the wall like a  landmark [or I use] the doors that are near. [I use them] to follow just a straight line. "} - \textbf{P6} & \\
\end{tabu}
\vspace{0.2cm}\\\\
P6 further explained that he preferred the convenience of a sighted guide and thus preferred to receive assistance rather than explore and generate a mental map for himself.
This reinforces prior findings by \cite{dias2015indoor} on VIPs' use of non-visual cues and landmarks to inform their decisions during navigation.

\subsubsection{\textbf{ Get Navigation help from non-VIPs effectively}}
Furthermore, our participants (n=4) preferred to receive a more closely guided form assistance such as having the other person walk with them to the destination, or sighted guide assistance. They preferred to update their mental maps -- which consisted of routes, and not complete maps -- by asking for directions instead of exploring. 
For instance, P5 described their approach: \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"Anything [that could be] as simple as finding a room that is not braille signed or a checkout counter [...] would require me to ask for directions."} - \textbf{P5} & \\
\end{tabu}
\vspace{0.2cm} \\\\
None of these participants mentioned discomfort due to social pressures, and were generally satisfied with receiving as much assistance as they are offered. 

However, they did report that non-VIPs often did not know how to assist them. 
For example, P3 highlighted an unpleasant experience receiving bad help from a non-VIP:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I had somebody once when I was travelling grab the end of my cane and [try] to pull me along by my cane, and that’s not [the correct way to assist]”} - \textbf{P3} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Thus, their experiences reinforced prior findings on the inadequacy of non-VIP assistance. 

\subsubsection{\textbf{ Maintain and Learn O\&M skills}}
These participants (n=4) preferred sighted assistance over using their O\&M skills for navigation -- primarily due to convenience. 
However, all of them were aware of the importance of these skills.
In fact, a few (n=2) expressed their desire to obtain better O\&M training. 
For instance, P7 shared how he believed he would have benefited from further O\&M instruction:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I feel like I would have benefited [from O\&M training]. I don't want to feel like I'm overexaggerating, but [I would be] at least 10 times more [independent at navigating] if I just had that training. [I would have preferred the trainer] telling me, ‘Hey, here's where we're going. Here's what we're going to do. Here's how to do it properly.’ Instead of [having to rely on a sighted guide] just [telling me], ‘Hey, we're going here. Enjoy.’”} - \textbf{P7} & \\
\end{tabu}
\vspace{0.2cm} \\\\
However, P7 was not eager to practice these skills independently, as he emphasized the necessity of receiving training from an instructor over being self taught. 
Nevertheless, our findings confirmed prior studies on the important of O\&M skills for VIP navigation. 
















==> 4-Findings/v5.tex <==
\section{Findings}
\label{sec:findings}


Our thematic analysis revealed three means of exploration that are challenging for VIPs when navigating unfamiliar environments: 
% which emerged as major themes:
\begin{itemize}
    \setlength{\itemindent}{.3in}
    \item [\textbf{Means 1.}] Gathering Information from the Environment in a Self-Directed Manner
    \item [\textbf{Means 2.}] Getting Information from Others
    \item [\textbf{Means 3.}] Maintaining and Learning O\&M Skills
\end{itemize}

These means of exploration emerged from our interviews with all parties --- all VIP and non-VIP participants. We note, however, that these exploration needs emerged from a subset of our VIPs: exactly half of them (four out of eight), who all had significant exposure to O\&M training. These four VIPs expressed a strong desire for all three of these means of exploration to be made easier.

The other four VIPs, who did not have as much exposure to O\&M training, did not express a desire for these means of exploration to be made easier and seemed content with receiving only guidance-based navigational assistance.
% These VIPs lacked exposure to O\&M training because of where they grew up or because they developed their visual impairment later in life.
Ultimately, we found that VIPs' stances on this issue are determined by the type of navigational help they are used to receiving.

Still, our findings reveal an opportunity for NASs to offer new means of exploration for the many VIPs who desire it --- half of all VIPs, if our sample of VIPs is representative. Facilitating these means of exploration may also shift the desires of VIPs who are content with guidance only, by showing them what is possible via exploration and by giving them access to O\&M and exploration capabilities which they previously had no exposure to.

In Sections~\ref{sec:form1}--\ref{sec:form3}, we describe each of these means of exploration in detail. In Appendix~\ref{sec:theothers}, we further describe the perspective of VIPs who favor guidance-based assistance.




\subsection{Means 1: Gathering Information from the Environment in a Self-Directed Manner}
\label{sec:form1}
The first means of exploration that VIPs find challenging is gathering information from the environment.
Specifically, VIPs described their desire to learn about the general layout of the space, generate a mental map through self-exploration, and add dynamic landmarks to their mental map. 
Here we expand on each of the desires listed above.

% [each subsection is an aspect of the means of active engagement]
\subsubsection{Learn the General Layout of the Space.}
We found that VIPs want to learn the general layout of the space when gathering information from the environment, but often find it difficult due to their low vision.
When asked about navigating unfamiliar or rarely visited spaces, participants expressed their desire to learn information that would help them build a mental map of that space. 
Many VIPs (n=4) reported that knowing the overall layout of the space helps them navigate within that space more confidently, and also enables them to explore the space independently.
As P4 put it:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``[When I receive help,] I will [ask], ‘What does this building generally look like?’ Because I want to understand [its shape]. That's one of [the] first things [I want] to understand[.]"} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm}\\\\
While understanding the general layout often proves to be difficult, it allows P4 to find his way around the space in a much more independent fashion by using his O\&M skills. 


Some VIPs place a high value on learning a place's layout, at times desiring that information even more than rehearsing specific routes. 
If a designer hopes to design an NAS that fosters exploration, that NAS should allow users to learn the general shape of the environment quickly and efficiently.

\subsubsection{Generate a Mental Map Through Self-Exploration.}
Our participants reported that they frequently lack the means to gather information from the environment via self-exploration.
Often, VIPs simply want to learn more about a space without having a specific destination in mind. 
For many VIPs, an initial mental map of the space's layout is not robust enough to fully rely on for navigation. 
We found that some of our participants (n=4) prefer self-exploration over asking others for directions to complete their mental maps.
%Half of our participants (n=4) mentioned that their mental maps were often not robust enough to rely on completely for navigation. 
Three of these four participants stated that they prefer to explore environments themselves to augment their non-visual skills. 
For example, P4 explained what type of specific information he looks for to complete his mental map:\\\\
% \begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
%  & \textit{“[When I enter a mall,] echolocation can tell me some things [about its shape], but I want specifics. So I will go to each side [of the entrance] and [check] how big [the entrance is]. And then I will see that there are two large openings from this foyer, one on either side, left and right, after a ways of wall. [From this information] I know that [the shape of the entrance] is probably a sort of long wide corridor, stretched out [perpendicularly] in front of me [...]”} - \textbf{P4} & \\
% \end{tabu}
% \vspace{0.2cm} \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[When I enter a mall,] echolocation can tell me some things [about its shape], but I want specifics. So I will go to each side [of the entrance] and [check] how big [the entrance is]. And then I [can learn] that there are two large openings from this foyer[.] 
%  I [can then deduce] that [the shape of the entrance] is probably a sort of long wide corridor, stretched out [perpendicularly] in front of me [...]
 ”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Through self-exploration, P4 solidifies his understanding of the space by gathering supplementary information for sensory cues he was already using, such as sound. 
%This not only helped him get familiar with the environment but also feel more independent. 
Furthermore, P4 was able to learn how the foyer led to another corridor. Thus, self-exploration allowed him to combine disjoint architectural features into a more robust and complete mental map of the environment.
By designing NASs that allow for self-exploration, VIPs can better engage with the environment during navigation, which, in turn, can allow them to create more robust mental maps of their environment.\\

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 1}: VIPs want to learn about the general layout of the space in a manner that engages them with the environment, i.e., via self-exploration.
\end{minipage}}
\end{center}
\vspace{2mm}

\subsubsection{Add Dynamic Landmarks to Mental Map.}
We found that VIPs find it troublesome to utilize landmarks in their mental maps to the fullest potential, due to landmarks' often dynamic nature.  
Participants (n=4) stated that once they had a mental map with a general layout of the space, they incorporated landmark information on top of the general layout to solidify their mental maps. 
For instance, P2 described how, for an unfamiliar grocery store, he first focused on understanding the general layout of the store, then supplemented his initial mental map with landmarks that were relevant to him. He explained that he sought to understand the locations of certain key points of interest such as the bathroom, specific aisles, and the cash register, to develop a more comprehensive understanding of the space.
This supports previous studies' findings that VIPs utilize landmarks to further reinforce their understanding of the general layout of the environment. 

We also found, however, that there is a more complex nuance to how VIPs use landmarks, specifically for robustness. 
Given the dynamic nature of the environment, location of landmarks may change over time, and landmarks created in previous visits may not be valid anymore. 
To mitigate this, participants reported that they create redundant landmarks such that even if one of them moves, or if they end up missing one, other landmarks can be used to accurately orient themselves. 
In fact, participants mentioned building a hierarchy of importance of landmarks.
Based upon the landmarks' relative importance, participants look for certain landmarks first and use the redundant landmarks for confirmation.
P4 explained:  \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"I've learned that you cannot rely [only] on one landmark because things change and the world is not static. [...] If you can find three landmarks in a location, then if you miss one or even two, you'll still have the third[.]"} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Treating landmarks as static singular entities can be misleading. Multiple landmarks of different priority help VIPs get a more complete understanding of the space, and prepare for any changes that may arise in the environment.
% While current  NASs utilize landmarks, they do not consider their dynamic nature. 
% BLE-based systems for instance, use permanent architectural features as landmarks. 
% This does not adequately reflect the experiences of all VIPs, as we discovered many VIP depend on impermanent, and often fluid, landmarks for navigation. 
% Similarly, computer-vision-based systems utilize a set of POIs from a pre-determined map, and hence do not provide the user with the ability to easily add and omit landmarks to reflect any changes in the location. 
Fluid and dynamic landmarks allow for VIPs to actively engage with a dynamic environment, and ultimately adapt quicker to any changes. 

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 2}: VIPs want to utilize dynamic landmarks to account for the non-static nature of spaces.
\end{minipage}}
\end{center}
\vspace{2mm}


\subsection{Means 2: Getting Information from Others}
\label{sec:form2}

The second means of exploration that we discovered as being challenging for VIPs is the ability to get information from others --- specifically, from non-VIPs. Our VIP participants (n=4) expressed a desire to ask non-VIPs for directions as a means of exploring unfamiliar environments, and to do so while maintaining their independence and continuing to navigate the environment themselves.

Specifically, the VIPs reported three challenges they often face in getting information from non-VIPs: that asking for information often leads to receiving full guidance, that the information they receive relies on having vision to understand, and that merely asking non-VIPs for information exerts social pressure on them. We describe these three challenges in the following subsections.
% While VIPs' primary goal is to navigate independently, many VIPs consider interacting with others and receiving assistance from them to be a part of navigating as well.
% Our VIP participants consider it imperative to receive help from others in an exploratory manner rather than becoming too complacent or reliant on others.
% They reported their desire to avoid getting too much help from others, to get spatial information from others explained to them in a way they can understand without vision, and to get help from others without putting social pressure on the helper. 
%We found that these aspects of receiving help lead VIPs to more actively explore the environment, by receiving effective assistance without becoming too complacent or reliant on others.
% Below, we outline our findings in more detail and explain how they motivate this meansof exploration.

\subsubsection{Avoid Getting Guided After Asking for Information.}
% Not all VIPs desire the same type of assistance. Receiving the correct amount of assistance --- and specifically avoiding too much assistance --- is an integral part of receiving effective help.
We found that some VIP participants (n=4) strongly prefer that others give them verbal directions only rather than escort them to their destination.
Nearly half (n=3) of our VIP participants reported that they avoid sighted guide assistance in most situations because the guides will be too helpful, and instead opt to use their O\&M skills to actively navigate to their destination despite the inconvenience. 

We further found that despite these preferences, VIPs are often offered inappropriately excessive assistance.
For example, P4 described an instance when non-VIPs have forced wheelchair service onto him out of ignorance:\\\\
% \begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
%  & \textit{“[Airport staff are] relatively good at adapting [to our needs] usually, but the very first thing they always do [when they assist you] is they give you a wheelchair, and [some staff] insist that you use it. [...] I don't want to say that's insulting [...] But on the other hand, that is stupid [...] that is not their fault. It's their training.”} - \textbf{P4} & \\
% \end{tabu}
\vspace{0.2cm}
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[Airport staff are] relatively good at adapting [to our needs] usually, but the very first thing they always do [when they assist you] is they give you a wheelchair, and [some staff] insist that you use it." } - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\
While wheelchair service might be more convenient, it does not match P4's preference for autonomy, specifically in that it assumes and reinforces a passive role instead of promoting exploration. VIPs often prefer to receive information from others, instead of sighted guidance.
In fact, excessive assistance in this case was not only unnecessary but also demeaning to P4. P4 explained that while he understood their actions were due to inadequate training, he still felt uncomfortable being forced to accept a type of assistance that overemphasized his level of disability and ignored his preferences.
% Current guidance based NASs offer a fixed service to all users and do not consider a possible preference for exploration during navigation. 
% Both BLE and computer vision based systems assume their users need as much help as they can get, and thus provide direct assistance, either through step-by-step instruction or through physical guide, but do not offer users the freedom to choose the level of help. 
% However, this does not address the desires of VIP who prefer only verbal instruction, and can even be degrading to many VIPs. 
% In short, we learned that non-VIPs must assist each VIP in the way that they prefer and not in the way that may be most convenient for non-VIPs. 
In short, we learned that VIPs often just want information from non-VIPs instead of being guided. \\ 
% Hence, non-VIPs must assist each VIP in the way that they prefer and not in the way that may be most convenient for non-VIPs.

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 3}: There is a mismatch between type and amount of information provided by non-VIPs and VIPs' preferences for them. 
\end{minipage}}
\end{center}
\vspace{2mm}


\subsubsection{Get Information in a Comprehensible Format.}

% to get spatial information from others explained to them in a way they can understand without vision

% When getting help, VIPs must be given all relevant details about the space in a format that they can understand without vision. 
We found that VIPs often struggle to receive information for navigating independently such as directions or room descriptions from non-VIPs, and that they struggle because the information they get requires vision to understand or interpret.
For example, P1 reported a time when a description from a non-VIP caused confusion: \\\\
% \begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
%  & \textit{"Sometimes there'll be a [situations] where [a non-VIP tells me], ‘Oh,[the place I’m looking for is] the third door.’ And I'm like, ‘Okay, [...] this is the third door, but [...]  it's not the [right place]’  I think they mean[t] third classroom door, but there's a storage room [next to the classrooms]. [I didn’t know] they d[id]n't count that as a door or a room."} - \textbf{P1} & \\
% \end{tabu}
% \vspace{0.2cm} \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"Sometimes there will be [situations] where [a non-VIP tells me], ‘Oh, [the place I’m looking for is] the third door.’ [...] But there's a storage room [next to the classroom]. [I didn’t know] they d[id]n't count that as a door or a room."} - \textbf{P1} & \\
\end{tabu}
\vspace{0.2cm} \\\\
While the presence of a fourth door may have been trivial to the non-VIP, providing this detail proved to be necessary for P1 to adequately understand the space.
She further contrasted her experience with a description she received from a VIP friend: \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“So for example, [before I go to a train station,] my friend will tell me this train [...] doesn't talk. And [that] I'm really gonna have to pay attention and count the stops. [...] So my friend will let me know [that I am] really gonna have to pay attention[.]”} - \textbf{P1} & \\
\end{tabu}
\vspace{0.2cm} \\\\ 
Descriptions from the VIP friend not only matched P1's perception of space, but also included other relevant details that P1 found important or useful. In fact, all VIP participants (n=8) almost always prefer to ask for descriptions from their friends who are visually impaired over non-VIP peers. All VIP participants (n=8) also reported that non-VIPs often struggle to match their descriptive preferences, leaving them frustrated. 
% They explained that VIPs generally have a better understanding of what types of information would be useful for other VIPs. 

As another example, P4 states that he finds it difficult to understand the shape and layout of an environment based on non-VIP's descriptions. 
He explained:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"[I need to ask for clarification] because a lot of people describe [shapes with letters] like `U' shaped or `H' shaped. I know what U shaped is, but sometimes I forget what H shaped means[.] I just prefer geometric shapes [for descriptions.]"} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Non-VIPs often utilize visual details when describing a space. 
As P4 explained, however, this is not always applicable to VIPs. 
In fact, we found that VIPs often prefer non-visual descriptions for navigation, such as describing how the floor texture changes from one location to another.

% As current NASs are focused on direct guidance, they only provide a limited set of verbal descriptions. 
% For example, BLE based systems and computer-based systems announce the presence POIs and landmarks, but do not mention other relevant information such as the presence of other accessibility features, or notes of caution. 
Last, our VIP participants expressed that they often need details beyond the presence of POIs and landmarks to successfully navigate a space, especially if they are visiting a place independently. These additional details include the presence of other accessibility features or notes of caution. 
In short, we learned that a major challenge hampering VIPs' ability to explore is ensuring that VIPs can get information from non-VIPs communicated to them in a way that they can interpret without vision. \\

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 4}: Non-VIPs' perception of spaces differ from that of VIPs, 
which causes a barrier to VIPs receiving verbal instructions or directions from non-VIPs. 
\end{minipage}}
\end{center}
\vspace{1mm}


\subsubsection{Getting Information Without Putting Social Pressure on the Helper.}

% \color{black}{}



VIPs expressed that another aspect of why getting information from others is challenging is the fact that non-VIPs often face social pressure from others whenever they are helping VIPs, even if it is just to provide information or directions.


% Many of our VIP participants are cognizant towards social factors ---  
\color{magenta}{Add: Guidance (A->B) is easier in the sense that you can ask simple questions, and get to the destination. However, when exploring environments, it is very different: (1) requires more time because you don't have anything specific in your mind; (2) more socially anxious because it takes more time, you feel like people are watching you and that is very inconvenient; (3) you cannot touch everything (that's the only way to explore) which is even more socially uncomfortable because you cannot touch something you do not know. }

\color{black}{}


% half of them (n=4) stated that they are often made to feel anxious by other people's perception of them and their sighted guides, negatively impacting their ability to navigate environments. 
We observed that this feeling applies even when VIPs receive assistance from their friends and/or family. 
For example, P4 said:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I know that my sister gets looks from people all the time [when she acts as my sighted guide], because of foolish assumptions they make out of ignorance. [People think] that she is my caretaker, [and that] anything that they perceive as her not doing her job is wrong.”} - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
He added that it is for this reason that he prefers receiving help information from professionals, such as O\&M instructors, as he feels less guilt towards having to subject them to such "embarrassment." It is clear from participants' remarks that social pressures are preventing VIPs from utilizing the full potential of non-VIP information available to them.



In addition, our interviews with business staff confirmed that non-VIPs feel social pressure when offering help to VIPs.
For example, the grocery store employee reported their difficulty determining whether or not they should offer help information to VIPs they see: \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I'm always concerned with invading somebody's personal space or [disregarding] their bodily autonomy. So I think it's a matter of just trying to be cognizant [...] if somebody seems like they need help [or] if somebody seems like they are totally fine. [It] is not a perfect system, obviously, [and] mistakes will be made.”} - \textbf{Grocery store employee} & \\
\end{tabu}
\vspace{0.2cm} \\\\

Furthermore, the grocery store employee expressed some social anxiety while helping VIP customers. As the employee explains, for him it was due to the company policies and lack of training.\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[My manager] said, if you need to help a customer [...] who's disabled, definitely try to. If they give you consent that you can drive my wheelchair, or you can grab my arm [...] Just be careful in that case, if they do say you can. But if they don't say anything, then you shouldn't do anything. Because you don't want to, you know, actually causing issues where they say, `oh, why are you touching me'?”} - \textbf{Grocery store employee} & \\
\end{tabu}
\vspace{0.2cm} \\\\



Non-VIP staff have difficulty determining whether or not to give assistive information to a VIP, and they often opt to not interfere out of fear that they may act in a socially unacceptable manner or get in trouble due to some company policies. 
% Current NASs do not properly address the issue of discretion. 
% For example, while computer-based systems, such as CaBot, have been designed to minimize public attention, they can still draw unwanted attention due to the relatively larger hardware components. 
% On the other hand, BLE-based systems have a better form-factor in that they are contained in a smartphone; however, they still do not address the issue of discrete communication between users and non-VIP. 
% For example, VIPs cannot discretely request for spaces to become blind-accessible. 
% Some systems, such as AIRA provide a means of connecting non-VIPs to VIPs without social interactions, but these are not navigation assistance systems and lack many of the other functionalities of an NAS.
In short, we find that social pressures can negatively impact both the frequency and quality of exploration information that VIPs receive. As a result, minimizing the social tensions that non-VIP helpers face is integral for VIPs to receive effective navigational information from them.\\

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 5}: Social pressure prevents VIPs from receiving and non-VIPs from providing useful information.
\end{minipage}}
\end{center}
\vspace{2mm}


\color{magenta}{Nice quote from Paige about: how some people get frustrated when they ask too many questions. Eventually, they've learned to say sorry for now reason, and that is something they don't like. This could be used to motivate why NASs can play a better role (than people), and hence motivate the translation vision.}
\color{black}{}



\subsection{Means 3: Maintaining and Learning O\&M skills}
\label{sec:form3}
The third means of exploration that we discovered as being challenging for VIPs is maintaining and learning O\&M skills. 
Confirming previous studies' findings~\cite{hersh_mental_2020}, we found that O\&M skills are an integral part of VIPs' sense of independence, especially when it comes to navigating unfamiliar environments. 
VIPs use various O\&M skills to collect various types of sensory information about the environment --- sounds, smells, air pressure, etc. --- and integrate them in order to inform their spatial decision-making.
Below, we describe our findings about VIPs' need to maintain and develop their O\&M skills in detail.

\subsubsection{Maintaining O\&M Skills.}


While O\&M skills are critical to VIPs' autonomy, they can worsen without regular use. Thus, it is important that VIPs make use of their O\&M skills on a regular basis and incorporate them for everyday navigation activities.
Many of our participants (n=4) acknowledged the importance of O\&M skills in their lives and described how these techniques empower them with independence and autonomy during navigation. 
As P4 explained:  \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[O\&M skills are] vital because the world will walk over you if you [don’t] take control of your own abilities. [...] People will tell you where you can go and what you can do[.] And if you don't know how to do those things, then you're just kind of meekly following along. It's self esteem shattering, [and] reduces your individuality.”} - \textbf{P4} & \\
\end{tabu} \\\\
P4 further elaborated that he even denies assistance out of fear of his skills deteriorating if he relied too much on sighted assistance:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"It is very easy to let your [O\&M] skills atrophy as a blind person if you rely overly on sighted people and it's an easy trap to fall into. It's easy to [use a] sighted guide and become complacent and [not pay attention to] what turns you have taken and where you are in relation to other things." } - \textbf{P4} & \\
\end{tabu}
\vspace{0.2cm} \\\\
While P4 knows that taking advantage of any assistance offered may be immediately convenient, he also understands that it may harm his ability to be independent in the long run.
% by deteriorating the skills that he needs to explore the space on his own.
Several of our participants (n=3) share this sentiment and prefer to use their O\&M skills as much as possible, denying sighted assistance whenever they can.  
As O\&M skills are crucial for VIPs to remain independent, there is an opportunity for NASs to promote exploration by providing a means of maintaining these skills and preventing them from deteriorating. \\

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 6}: VIPs express the need to use their O\&M skills as much as possible in order to maintain their ability to be independent.
\end{minipage}}
\end{center}
\vspace{2mm}

\subsubsection{Learning O\&M Skills.}
Learning is also an integral part of equipping VIPs with the necessary skills for exploratory navigation. 
Our findings further showed that some VIPs have trouble receiving O\&M training at all.
For example, half of our participants (n=4) reported that they have received only limited O\&M training in their lives. Upon further inquiry, we identified several factors that affect VIPs' access to adequate O\&M training.

The first factor is the age at which VIPs develop their visual impairments. 
VIPs who developed vision impairments earlier in life or are blind by birth tend to have easy access to O\&M training through their schools. 
On the other hand, VIPs that develop visual impairments later in life often find it difficult to arrange for such training. 
All of our VIP participants developed their vision impairment either from birth (P2, P3, P5, P6, P8, P1) or earlier in life (P4: by the age of four, P7: by the age of one). 
They all stated that they were assigned an O\&M trainer in school.  
Many participants (n=6) stated that it becomes much more difficult to set up an O\&M session as an adult, compared to getting one as a child in school. 
For instance, P1 (who is blind by birth) explained:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“For earlier years, I d[id]n't need to reach out [to O\&M trainers] because that's something that like, we automatically get [in schools]. Now, I definitely would have to advocate for myself[.]} - \textbf{P1} & \\
\end{tabu}
\vspace{0.2cm}\\\\
%  [by reaching out to] the Rehab Center or something like that. [...] I can’t expect them to reach out to me.”}
As a result, most of P1's O\&M training was done during her K-12 education.

The second reason is lack of access to O\&M trainers. 
VIPs may still not be able to receive appropriate O\&M training during school despite being eligible. 
Our interviews with the O\&M instructors have revealed that this is primarily due to shortage of O\&M trainers and decentralization. 
Both instructors confirmed that O\&M trainers are assigned multiple students scattered over a geographical area, which makes it difficult for them to be physically present and provide enough time to all their students. 
Similarly, P7, who was assigned an O\&M trainer during middle school, described the reason behind his lack of access to an O\&M trainer:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I was told that I would get an O\&M trainer back in middle school. [...] I never received that trainer. She came in once within the six years she was supposed to be training me.”} - \textbf{P7} & \\
\end{tabu}
\vspace{0.2cm}\\\\
Due to this reason, P7 never received formal O\&M training, despite his belief that it would have benefited him. 

The third reason is lack of funding. 
All our participants reported that they are dependent upon their respective states to receive O\&M training or other accessibility services or devices. 
A few participants (n=2) highlighted that their state provides limited resources due to shortage of funds, thereby affecting their ability to receive O\&M training.
For example, P3 said:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“It's just very hard to get [O\&M training here] because [anonymized state] is out of money. [...] It's very hard to [receive O\&M training because] you've got to prove that you’re working.”} - \textbf{P3} & \\
\end{tabu}
\vspace{0.2cm}\\\\
He further explained that, due to limited funding, adult VIPs are limited to vocational rehabilitation, which is a partial form of training meant only to supply the necessary skills for a VIP to perform a specific job.  
However, as P3 explained, even this type of training was scarce, and VIPs have to prove their employment status in order to receive it.

For these reasons, a lack of O\&M training is a problem affecting many VIPs. 
However, most current systems do not provide a means of learning O\&M skills. 
Providing an efficient systems-based solution to O\&M training could help democratize the skills necessary for VIPs to navigate independently. 
Hence, we suggest that in order for NASs to facilitate exploration, they should not only provide a means of practicing O\&M skills but should also provide an effective way of developing these skills in the first place.
\begin{center}
\vspace{5mm}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 7}: Many factors may prevent VIPs' access to O\&M training. Some VIPs need access to O\&M training.
\end{minipage}}
\end{center}
\vspace{2mm}

==> 4-Findings/v6.tex <==

\section{Findings}
\label{sec:findings}
% 
% 

Our thematic analysis revealed three means of exploration that are challenging for VIPs when navigating unfamiliar environments: 
% which emerged as major themes:
\begin{itemize}
    \setlength{\itemindent}{.3in}
    \item [\textbf{Means 1.}] Gathering Information from the Environment in a Self-Directed Manner
    \item [\textbf{Means 2.}] Getting Information from Others
    \item [\textbf{Means 3.}] Maintaining and Learning O\&M Skills
\end{itemize}

These means of exploration emerged from our interviews with all parties --- all VIP and non-VIP participants. We note, however, that these exploration needs emerged from a subset of our VIPs: exactly half of them (four out of eight), who all had significant exposure to O\&M training. These four VIPs expressed a strong desire for all three of these means of exploration to be made easier.

The other four VIPs, who did not have as much exposure to O\&M training, did not express a desire for these means of exploration to be made easier and seemed content with receiving only guidance-based navigational assistance.
Ultimately, we found that VIPs' stances on this issue are determined by the type of navigational help they are used to receiving.

Still, our findings reveal an opportunity for NASs to offer new means of exploration for the many VIPs who desire it --- half of all VIPs, if our sample of VIPs is representative. Facilitating these means of exploration may also shift the desires of VIPs who are content with guidance only, by showing them what is possible via exploration and by giving them access to O\&M and exploration capabilities which they previously had no exposure to.

In Sections~\ref{sec:form1}--\ref{sec:form3}, we describe each of these means of exploration in detail. In Appendix~\ref{sec:theothers}, we further describe the perspective of VIPs who favor guidance-based assistance


\subsection{\textcolor{magenta}{Information Needs for Exploration}}
% 
\textcolor{magenta}{%
Participants shared their navigation experiences and often contrasted how their information needs differ, based on their navigation 
While navigating to a specific destination, i.e., guidance, participants reported that 
}


\subsubsection{\textcolor{magenta}{}}
    

\textcolor{magenta}{%
.
}


The first means of exploration that VIPs find challenging is gathering information from the environment.
Specifically, VIPs described their desire to learn about the general layout of the space, generate a mental map through self-exploration, and add dynamic landmarks to their mental map. 
Here we expand on each of the desires listed above.

\textbf{Learn the General Layout of the Space.}
We found that VIPs want to learn the general layout of the space when gathering information from the environment, but often find it difficult due to their low vision.
When asked about navigating unfamiliar or rarely visited spaces, participants expressed their desire to learn information that would help them build a mental map of that space. 
Many VIPs (n=4) reported that knowing the overall layout of the space helps them navigate within that space more confidently, and also enables them to explore the space independently.
As James put it:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{``[When I receive help,] I will [ask], ‘What does this building generally look like?’ Because I want to understand [its shape]. That's one of [the] first things [I want] to understand[.]"} --- \textbf{James} & \\
\end{tabu}
\vspace{0.2cm}\\\\
While understanding the general layout often proves to be difficult, it allows James to find his way around the space in a much more independent fashion by using his O\&M skills. 


Some VIPs place a high value on learning a place's layout, at times desiring that information even more than rehearsing specific routes. 
If a designer hopes to design an NAS that fosters exploration, that NAS should allow users to learn the general shape of the environment quickly and efficiently.


\textbf{Add Dynamic Landmarks to Mental Map.}
We found that VIPs find it troublesome to utilize landmarks in their mental maps to the fullest potential, due to landmarks' often dynamic nature.  
Participants (n=4) stated that once they had a mental map with a general layout of the space, they incorporated landmark information on top of the general layout to solidify their mental maps. 
For instance, Aaron described how, for an unfamiliar grocery store, he first focused on understanding the general layout of the store, then supplemented his initial mental map with landmarks that were relevant to him. He explained that he sought to understand the locations of certain key points of interest such as the bathroom, specific aisles, and the cash register, to develop a more comprehensive understanding of the space.
This supports previous studies' findings that VIPs utilize landmarks to further reinforce their understanding of the general layout of the environment. 

We also found, however, that there is a more complex nuance to how VIPs use landmarks, specifically for robustness. 
Given the dynamic nature of the environment, location of landmarks may change over time, and landmarks created in previous visits may not be valid anymore. 
To mitigate this, participants reported that they create redundant landmarks such that even if one of them moves, or if they end up missing one, other landmarks can be used to accurately orient themselves. 
In fact, participants mentioned building a hierarchy of importance of landmarks.
Based upon the landmarks' relative importance, participants look for certain landmarks first and use the redundant landmarks for confirmation.
James explained:  \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"I've learned that you cannot rely [only] on one landmark because things change and the world is not static. [...] If you can find three landmarks in a location, then if you miss one or even two, you'll still have the third[.]"} - \textbf{James} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Treating landmarks as static singular entities can be misleading. Multiple landmarks of different priority help VIPs get a more complete understanding of the space, and prepare for any changes that may arise in the environment.
Fluid and dynamic landmarks allow for VIPs to actively engage with a dynamic environment, and ultimately adapt quicker to any changes. 

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 2}: VIPs want to utilize dynamic landmarks to account for the non-static nature of spaces.
\end{minipage}}
\end{center}
\vspace{2mm}
    
% 
% 
\subsection{\textcolor{magenta}{Challenges in Independent Exploration}}
% 
    \subsubsection{\textcolor{magenta}{Agency in Exploration}}
    \textbf{Generate a Mental Map Through Self-Exploration.}
Our participants reported that they frequently lack the means to gather information from the environment via self-exploration.
Often, VIPs simply want to learn more about a space without having a specific destination in mind. 
For many VIPs, an initial mental map of the space's layout is not robust enough to fully rely on for navigation. 
We found that some of our participants (n=4) prefer self-exploration over asking others for directions to complete their mental maps.
%Half of our participants (n=4) mentioned that their mental maps were often not robust enough to rely on completely for navigation. 
Three of these four participants stated that they prefer to explore environments themselves to augment their non-visual skills. 
For example, James explained what type of specific information he looks for to complete his mental map:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[When I enter a mall,] echolocation can tell me some things [about its shape], but I want specifics. So I will go to each side [of the entrance] and [check] how big [the entrance is]. And then I [can learn] that there are two large openings from this foyer[.] 
 ”} - \textbf{James} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Through self-exploration, James solidifies his understanding of the space by gathering supplementary information for sensory cues he was already using, such as sound. 
Furthermore, James was able to learn how the foyer led to another corridor. Thus, self-exploration allowed him to combine disjoint architectural features into a more robust and complete mental map of the environment.
By designing NASs that allow for self-exploration, VIPs can better engage with the environment during navigation, which, in turn, can allow them to create more robust mental maps of their environment.\\

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 1}: VIPs want to learn about the general layout of the space in a manner that engages them with the environment, i.e., via self-exploration.
\end{minipage}}
\end{center}
\vspace{2mm}
    
% 
   \subsubsection{\textcolor{magenta}{Reliance on Orientation and Mobility Skills}}
% 
The third means of exploration that we discovered as being challenging for VIPs is maintaining and learning O\&M skills. 
Confirming previous studies' findings~\cite{hersh_mental_2020}, we found that O\&M skills are an integral part of VIPs' sense of independence, especially when it comes to navigating unfamiliar environments. 
VIPs use various O\&M skills to collect various types of sensory information about the environment --- sounds, smells, air pressure, etc. --- and integrate them in order to inform their spatial decision-making.
Below, we describe our findings about VIPs' need to maintain and develop their O\&M skills in detail.

\textbf{Maintaining O\&M Skills.}
While O\&M skills are critical to VIPs' autonomy, they can worsen without regular use. Thus, it is important that VIPs make use of their O\&M skills on a regular basis and incorporate them for everyday navigation activities.
Many of our participants (n=4) acknowledged the importance of O\&M skills in their lives and described how these techniques empower them with independence and autonomy during navigation. 
As James explained:  \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[O\&M skills are] vital because the world will walk over you if you [don’t] take control of your own abilities. [...] People will tell you where you can go and what you can do[.] And if you don't know how to do those things, then you're just kind of meekly following along. It's self esteem shattering, [and] reduces your individuality.”} - \textbf{James} & \\
\end{tabu} \\\\
James further elaborated that he even denies assistance out of fear of his skills deteriorating if he relied too much on sighted assistance:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"It is very easy to let your [O\&M] skills atrophy as a blind person if you rely overly on sighted people and it's an easy trap to fall into. It's easy to [use a] sighted guide and become complacent and [not pay attention to] what turns you have taken and where you are in relation to other things." } - \textbf{James} & \\
\end{tabu}
\vspace{0.2cm} \\\\
While James knows that taking advantage of any assistance offered may be immediately convenient, he also understands that it may harm his ability to be independent in the long run.
% by deteriorating the skills that he needs to explore the space on his own.
Several of our participants (n=3) share this sentiment and prefer to use their O\&M skills as much as possible, denying sighted assistance whenever they can.  
As O\&M skills are crucial for VIPs to remain independent, there is an opportunity for NASs to promote exploration by providing a means of maintaining these skills and preventing them from deteriorating. \\

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 6}: VIPs express the need to use their O\&M skills as much as possible in order to maintain their ability to be independent.
\end{minipage}}
\end{center}
\vspace{2mm}

\textbf{Learning O\&M Skills.}
Learning is also an integral part of equipping VIPs with the necessary skills for exploratory navigation. 
Our findings further showed that some VIPs have trouble receiving O\&M training at all.
For example, half of our participants (n=4) reported that they have received only limited O\&M training in their lives. Upon further inquiry, we identified several factors that affect VIPs' access to adequate O\&M training.

The first factor is the age at which VIPs develop their visual impairments. 
VIPs who developed vision impairments earlier in life or are blind by birth tend to have easy access to O\&M training through their schools. 
On the other hand, VIPs that develop visual impairments later in life often find it difficult to arrange for such training. 
All of our VIP participants developed their vision impairment either from birth (Aaron, Lucas, Daniel, William, Leo, Nora) or earlier in life (James: by the age of four, Charles: by the age of one). 
They all stated that they were assigned an O\&M trainer in school.  
Many participants (n=6) stated that it becomes much more difficult to set up an O\&M session as an adult, compared to getting one as a child in school. 
For instance, Nora (who is blind by birth) explained:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“For earlier years, I d[id]n't need to reach out [to O\&M trainers] because that's something that like, we automatically get [in schools]. Now, I definitely would have to advocate for myself[.]} - \textbf{Nora} & \\
\end{tabu}
\vspace{0.2cm}\\\\
As a result, most of Nora's O\&M training was done during her K-12 education.

The second reason is lack of access to O\&M trainers. 
VIPs may still not be able to receive appropriate O\&M training during school despite being eligible. 
Our interviews with the O\&M instructors have revealed that this is primarily due to shortage of O\&M trainers and decentralization. 
Both instructors confirmed that O\&M trainers are assigned multiple students scattered over a geographical area, which makes it difficult for them to be physically present and provide enough time to all their students. 
Similarly, Charles, who was assigned an O\&M trainer during middle school, described the reason behind his lack of access to an O\&M trainer:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I was told that I would get an O\&M trainer back in middle school. [...] I never received that trainer. She came in once within the six years she was supposed to be training me.”} - \textbf{Charles} & \\
\end{tabu}
\vspace{0.2cm}\\\\
Due to this reason, Charles never received formal O\&M training, despite his belief that it would have benefited him. 

The third reason is lack of funding. 
All our participants reported that they are dependent upon their respective states to receive O\&M training or other accessibility services or devices. 
A few participants (n=2) highlighted that their state provides limited resources due to shortage of funds, thereby affecting their ability to receive O\&M training.
For example, Lucas said:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“It's just very hard to get [O\&M training here] because [anonymized state] is out of money. [...] It's very hard to [receive O\&M training because] you've got to prove that you’re working.”} - \textbf{Lucas} & \\
\end{tabu}
\vspace{0.2cm}\\\\
He further explained that, due to limited funding, adult VIPs are limited to vocational rehabilitation, which is a partial form of training meant only to supply the necessary skills for a VIP to perform a specific job.  
However, as Lucas explained, even this type of training was scarce, and VIPs have to prove their employment status in order to receive it.

For these reasons, a lack of O\&M training is a problem affecting many VIPs. 
However, most current systems do not provide a means of learning O\&M skills. 
Providing an efficient systems-based solution to O\&M training could help democratize the skills necessary for VIPs to navigate independently. 
Hence, we suggest that in order for NASs to facilitate exploration, they should not only provide a means of practicing O\&M skills but should also provide an effective way of developing these skills in the first place.
\begin{center}
\vspace{5mm}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 7}: Many factors may prevent VIPs' access to O\&M training. Some VIPs need access to O\&M training.
\end{minipage}}
\end{center}
\vspace{2mm}







\subsection{\textcolor{magenta}{Challenges in Collaborative Exploration}}
% 
\textit{The second means of exploration that we discovered as being challenging for VIPs is the ability to get information from others }--- specifically, from non-VIPs. Our VIP participants (n=4) expressed a desire to ask non-VIPs for directions as a means of exploring unfamiliar environments, and to do so while maintaining their independence and continuing to navigate the environment themselves.

Specifically, the VIPs reported three challenges they often face in getting information from non-VIPs: that asking for information often leads to receiving full guidance, that the information they receive relies on having vision to understand, and that merely asking non-VIPs for information exerts social pressure on them. We describe these three challenges in the following subsections.


\subsubsection{\textcolor{magenta}{Social Pressures in Collaborative Environments}}
% 
\textbf{Getting Information Without Putting Social Pressure on the Helper.}


VIPs expressed that another aspect of why getting information from others is challenging is the fact that non-VIPs often face social pressure from others whenever they are helping VIPs, even if it is just to provide information or directions.


\textcolor{magenta}{Add: Guidance (A->B) is easier in the sense that you can ask simple questions, and get to the destination. However, when exploring environments, it is very different: (1) requires more time because you don't have anything specific in your mind; (2) more socially anxious because it takes more time, you feel like people are watching you and that is very inconvenient; (3) you cannot touch everything (that's the only way to explore) which is even more socially uncomfortable because you cannot touch something you do not know. }


We observed that this feeling applies even when VIPs receive assistance from their friends and/or family. 
For example, James said:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I know that my sister gets looks from people all the time [when she acts as my sighted guide], because of foolish assumptions they make out of ignorance. [People think] that she is my caretaker, [and that] anything that they perceive as her not doing her job is wrong.”} - \textbf{James} & \\
\end{tabu}
\vspace{0.2cm} \\\\
He added that it is for this reason that he prefers receiving help information from professionals, such as O\&M instructors, as he feels less guilt towards having to subject them to such "embarrassment." It is clear from participants' remarks that social pressures are preventing VIPs from utilizing the full potential of non-VIP information available to them.



In addition, our interviews with business staff confirmed that non-VIPs feel social pressure when offering help to VIPs.
For example, the grocery store employee reported their difficulty determining whether or not they should offer help information to VIPs they see: \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“I'm always concerned with invading somebody's personal space or [disregarding] their bodily autonomy. So I think it's a matter of just trying to be cognizant [...] if somebody seems like they need help [or] if somebody seems like they are totally fine. [It] is not a perfect system, obviously, [and] mistakes will be made.”} - \textbf{Grocery store employee} & \\
\end{tabu}
\vspace{0.2cm} \\\\

Furthermore, the grocery store employee expressed some social anxiety while helping VIP customers. As the employee explains, for him it was due to the company policies and lack of training.\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[My manager] said, if you need to help a customer [...] who's disabled, definitely try to. If they give you consent that you can drive my wheelchair, or you can grab my arm [...] Just be careful in that case, if they do say you can. But if they don't say anything, then you shouldn't do anything. Because you don't want to, you know, actually causing issues where they say, `oh, why are you touching me'?”} - \textbf{Grocery store employee} & \\
\end{tabu}
\vspace{0.2cm} \\\\



Non-VIP staff have difficulty determining whether or not to give assistive information to a VIP, and they often opt to not interfere out of fear that they may act in a socially unacceptable manner or get in trouble due to some company policies. 
In short, we find that social pressures can negatively impact both the frequency and quality of exploration information that VIPs receive. As a result, minimizing the social tensions that non-VIP helpers face is integral for VIPs to receive effective navigational information from them.\\

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 5}: Social pressure prevents VIPs from receiving and non-VIPs from providing useful information.
\end{minipage}}
\end{center}
\vspace{2mm}


\textcolor{magenta}{Nice quote from Paige about: how some people get frustrated when they ask too many questions. Eventually, they've learned to say sorry for now reason, and that is something they don't like. This could be used to motivate why NASs can play a better role (than people), and hence motivate the translation vision.}




\subsubsection{\textcolor{magenta}{Communicating Form and Type of Assistance during Collaboration}}


\textbf{Avoid Getting Guided After Asking for Information.}
We found that some VIP participants (n=4) strongly prefer that others give them verbal directions only rather than escort them to their destination.
Nearly half (n=3) of our VIP participants reported that they avoid sighted guide assistance in most situations because the guides will be too helpful, and instead opt to use their O\&M skills to actively navigate to their destination despite the inconvenience. 

We further found that despite these preferences, VIPs are often offered inappropriately excessive assistance.
For example, James described an instance when non-VIPs have forced wheelchair service onto him out of ignorance:\\\\
\vspace{0.2cm}
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“[Airport staff are] relatively good at adapting [to our needs] usually, but the very first thing they always do [when they assist you] is they give you a wheelchair, and [some staff] insist that you use it." } - \textbf{James} & \\
\end{tabu}
\vspace{0.2cm} \\
While wheelchair service might be more convenient, it does not match James's preference for autonomy, specifically in that it assumes and reinforces a passive role instead of promoting exploration. VIPs often prefer to receive information from others, instead of sighted guidance.
In fact, excessive assistance in this case was not only unnecessary but also demeaning to James. James explained that while he understood their actions were due to inadequate training, he still felt uncomfortable being forced to accept a type of assistance that overemphasized his level of disability and ignored his preferences.
In short, we learned that VIPs often just want information from non-VIPs instead of being guided. \\

\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 3}: There is a mismatch between type and amount of information provided by non-VIPs and VIPs' preferences for them. 
\end{minipage}}
\end{center}
\vspace{2mm}


\textbf{Get Information in a Comprehensible Format.}


We found that VIPs often struggle to receive information for navigating independently such as directions or room descriptions from non-VIPs, and that they struggle because the information they get requires vision to understand or interpret.
For example, Nora reported a time when a description from a non-VIP caused confusion: \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"Sometimes there will be [situations] where [a non-VIP tells me], ‘Oh, [the place I’m looking for is] the third door.’ [...] But there's a storage room [next to the classroom]. [I didn’t know] they d[id]n't count that as a door or a room."} - \textbf{Nora} & \\
\end{tabu}
\vspace{0.2cm} \\\\
While the presence of a fourth door may have been trivial to the non-VIP, providing this detail proved to be necessary for Nora to adequately understand the space.
She further contrasted her experience with a description she received from a VIP friend: \\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{“So for example, [before I go to a train station,] my friend will tell me this train [...] doesn't talk. And [that] I'm really gonna have to pay attention and count the stops. [...] So my friend will let me know [that I am] really gonna have to pay attention[.]”} - \textbf{Nora} & \\
\end{tabu}
\vspace{0.2cm} \\\\ 
Descriptions from the VIP friend not only matched Nora's perception of space, but also included other relevant details that Nora found important or useful. In fact, all VIP participants (n=8) almost always prefer to ask for descriptions from their friends who are visually impaired over non-VIP peers. All VIP participants (n=8) also reported that non-VIPs often struggle to match their descriptive preferences, leaving them frustrated. 

As another example, James states that he finds it difficult to understand the shape and layout of an environment based on non-VIP's descriptions. 
He explained:\\\\
\begin{tabu} to \linewidth { X[l] X[27l] X[2l]}
 & \textit{"[I need to ask for clarification] because a lot of people describe [shapes with letters] like `U' shaped or `H' shaped. I know what U shaped is, but sometimes I forget what H shaped means[.] I just prefer geometric shapes [for descriptions.]"} - \textbf{James} & \\
\end{tabu}
\vspace{0.2cm} \\\\
Non-VIPs often utilize visual details when describing a space. 
As James explained, however, this is not always applicable to VIPs. 
In fact, we found that VIPs often prefer non-visual descriptions for navigation, such as describing how the floor texture changes from one location to another.


Last, our VIP participants expressed that they often need details beyond the presence of POIs and landmarks to successfully navigate a space, especially if they are visiting a place independently. These additional details include the presence of other accessibility features or notes of caution. 
In short, we learned that a major challenge hampering VIPs' ability to explore is ensuring that VIPs can get information from non-VIPs communicated to them in a way that they can interpret without vision. \\
% 
\begin{center}
\fbox{\begin{minipage}{0.5\linewidth}
\textbf{Insight 4}: Non-VIPs' perception of spaces differ from that of VIPs, 
which causes a barrier to VIPs receiving verbal instructions or directions from non-VIPs. 
\end{minipage}}
\end{center}
\vspace{1mm}


==> 4-Findings/v7.tex <==
\label{sec:findings}

% \newpage
\section{RQ1 Findings: Information Needs for Exploration}
\label{sec:RQ1-findings}
In this section, we present our findings for RQ1: What information do VIPs need to explore unfamiliar environments, and what factors influence these needs between individuals? 
Our interviews revealed that VIPs need two types of spatial information (Section~\ref{sec:informationNeeds}) for exploration --- shape information and layout information --- in addition to the information they need for turn-by-turn navigation (i.e., POIs and route information). 
We also discovered factors that influence these information needs between individuals 
% : their onset of vision impairments, their inherent sociability, their O\&M proficiency and mobility aid preference
(Section~\ref{sec:factors-info-needs}).
Throughout our results, we highlight key insights that inform the design of future NASs supporting VIPs' exploration in navigation.

% that inform design of future NASs supporting exploration in navigation for VIPs.


% Our analysis revealed a significant difference in VIPs’ information needs when exploring unfamiliar environment versus traversing to a destination within that environment. In line with prior research~\cite{banovic_uncovering_2013}, we found that participants wanted information about route to the destination with notifications (find better word) POIs and obstacles along the way. In contrast, while exploring environments, participants found information about the structural layout of the space potentially helpful. 
% Below, we elaborate on how VIPs use this information for exploration and further elaborate on factors that influence the importance of this information for different individuals with visual impairments.


\subsection{Spatial Information}
\label{sec:informationNeeds}
% We discovered that route-based information, usually appropriate for turn-by-turn navigation, is not enough for exploration. Instead, VIPs expressed desire to learn the overall structure of the environment via shape and layout information, which we collectively call \textit{spatial information}. Our choice of the term \textit{spatial information} stems from the fact that this information --- both shape and layout --- provide VIPs an understanding of the spatial structure of the environment, which as the participants described is important for exploration. 

We found that participants want to learn spatial information in a hierarchy --- first, the shape information, then the layout information, followed by specific details about the route to a destination. Participants noted that the shape and layout information give them a high-level overview of the environment, allowing them to decide their route to the destination by themselves. Our findings extend prior work~\cite{banovic_uncovering_2013} by specifying what it means for VIPs to obtain a ``high-level'' overview of a space.

We note an important difference between what VIPs want during exploration and how current NASs facilitate exploration. While current NASs' approach of announcing nearby POIs~\cite{paneels_listen_2013, blum_spatialized_2013, sato_navcog3_2019} promotes a body-centred reference frame (i.e., egocentric), we found that VIPs want to build their cognitive maps in an environment-centred reference frame (i.e., allocentric) via shape and layout information.
Next, we describe the two types of spatial information: shape information (Section~\ref{sec:shapeInfo}) and layout information (Section~\ref{sec:layoutInfo}).


% Participants wanted to learn the overall structure of unfamiliar environments, first the shape of the space and then the layout of objects within them.. 
% Collectively, we refer to these two pieces of information, i.e., shape information and layout information, as \textit{spatial information}. Par
% because it provides VIPs an understanding of the spatial structure of the environment. 

% Not surprising

% Not surprisingly, participants noted that route-based information such as information about route to the destination and information about obstacles and landmarks along the path were important when navigating to a destination, reinforcing prior work~\cite{banovic_uncovering_2013}.
% the information needs uncovered by Banovic et al.~\cite{banovic_uncovering_2013}. 

% Interestingly, participants indicated that this route-based information alone was not sufficient to explore unfamiliar environments, emphasizing the need for shape information and layout information, which we describe in the following sections. \novelty{Furthermore, existing NASs improve spatial awareness by announcing POIs~\cite{paneels_listen_2013}, but what we learned is that VIPs want for allocentric\todo{cite allo and ego papers} view of the space instead of a egocentric view and that POI-based navigation is not enough for in-situ exploration. }

% ( such as route to the destination, safety information, ,) is not enough for exploration. In

% In line with information Banovic et al.~\cite{banovic_uncovering_2013}

% More specifically, we found that information about route to the destination along with notifications about obstacles and landmarks along the route was more important when they had a specific destination in mind. 

% For exploration however, 

% However, this route-based information was not enough to give participants information about the environment's overall structure, needed for exploration.

% in line with Banovic et al.'s

% Our participants suggested that while

% safety and landmark information are crucial to their

% Our choice of the term \textit{spatial information} stems from the fact that this information --- both shape and layout --- provide VIPs an understanding of the spatial structure of the environment, which as the participants described is important for exploration.
% route-based information, usually appropriate for turn-by-turn navigation, is not enough for exploration. Instead, VIPs expressed desire to learn the overall structure of the environment via shape and layout information, which we collectively call \textit{spatial information}. Our choice of the term \textit{spatial information} stems from the fact that this information --- both shape and layout --- provide VIPs an understanding of the spatial structure of the environment, which as the participants described is important for exploration. 


% We now detail the two components of spatial information.

% We discovered that participants want information about the overall structure of the space, 

% Prior research on identifying information needs for VIPs primarily focused on identifying instances where VIPs navigated in an unfamiliar environment with an aim to learn the space, or 

% Prior\todo{may omit this para; shift to intro perhaps?} research on information needs investigate VIPs' ability to reach a specific destination, while also receiving some additional information along the route~\cite{banovic_uncovering_2013}. Most NASs understand VIPs information needs in context of guiding them between destinations via a turn-by-turn navigation paradigm. As a consequence, VIPs usually `see' a part of the environment and are restricted to performing navigation-related activities along the route to the destination. By facilitating exploration, VIPs will be able to access the whole environment, not just a part of it along the route, and make navigation decisions on the fly in any unfamiliar environment. While we do not propose to cease research in turn-by-turn navigation, we sought to define and recognize exploration as an important aspect in VIPs' navigation.


% to either reach a specific destination~\cite{} or to learn

% While some of our findings correspond 

% \textit{learn} information about unfamiliar environment, with an aim to 

% Participants revealed that route-based information is not enough to explore environments, and described wanting to learn about the shape of the space, layout of different landmarks within that space and finally, information about how spaces are connected with each other via connections such as doors, stairs, escalators, pathways, etc. 
% Below, we elaborate on each of these in detail.


\subsubsection{Shape information}
\label{sec:shapeInfo}
Participants described shape information as a skeletal wire-frame of the unfamiliar environment, marking its bounds. Shape information provides VIPs with a high-level overview of the structure of the space very quickly.
Many participants (n=4) indicated that shape information forms the basis of their mental map, onto which they append other pieces of information including object layouts and routes. James, recollecting his recent visit to an office complex, explained how he would ask for shape information before anything else:
\vspace{-0.25cm} \\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & \textit{``[I ask] ... `What does this building generally look like?' Because I want to understand its shape. That’s one of the first things [I want] to understand.''} --James  & \\
\end{tabu} \vspace{-0.1cm} \\



Participants described using shape in context of both indoor and outdoor environments. For indoors, shape is understood to be the boundary or walls of a room and thus, can be represented in the form of geometric shapes such as squares (e.g., offices) or rectangles (e.g., hallways).
% As Leo explained:
% \vspace{-0.25cm} \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{``I'm going to probably start by examining the exterior of the room, the perimeter of the room [...] I go around [and] I've got a scope for the size and the shape of the room''} -Leo  & \\
% \end{tabu} \\\\
For outdoors, participants referred to the environment's general dimensions as its shape. For instance, Olivia explained how she values information about width of the sidewalk and the streets when the environment may require crossing streets. 



Participants reported using their white cane and/or non-visual senses to collect shape information. 
Some participants (n=4) mentioned walking along the boundary of the walls (or  sidewalks in outdoor spaces) to gather shape information. Other participants (n=3) reported using their sense of hearing (e.g., echolocation) to obtain an estimate of the environment's shape. However, both techniques caused VIPs' difficulties in gathering shape information, which we describe later in Section~\ref{sec:ind_exploration}.
% \todo{para can be removed.}


Interestingly, we learned that VIPs use shape information differently for turn-by-turn navigation and exploration. Williams et al.~\cite{williams_just_2014} found that boundaries --- indicating the shape --- help VIPs to orient themselves and walk in a straight line when receiving guidance to a destination. In contrast, we found that VIPs use shape information to get a sense of the environment's high-level overview during exploration.



% IF HINTS ARE TO BE ADDED: LEO SAID IT WAS DIFFICULT TO NAVIGATE THROUGH COMPLEX SHAPED GROCERY STORE AND HOW SHAPE INFO IS NOT PRECISE ENOUGH.


% We found that participants want information about general shape of the space in order to explore environments. 
% Participants mentioned walking along the boundary of the walls, or using their white cane to graze along the pathway to get a better sense of the environment. BOUNDARY
% Additional cues such as sound, primarily echolocation, also provide VIPs a decent estimate of the environment’s shape. 
% Many VIPs reported that knowing the overall shape of the space helps them navigate within that space more confidently, and also enables them to explore the space independently. As James put it: \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{“I will [ask], ‘What does this building generally look like?’ Because I want to understand its shape. That’s one of the first things [I want] to understand.”} --- \textbf{James}% 
%  & \\
% \end{tabu}
% \vspace{-0.4cm}\\\\

% Environments, especially indoors, are characterized by their boundaries which may be represented in the form of geometric shapes such as squares (for rooms) or rectangles (for hallways). These shapes form the first layer of VIPs’ mental map, which develops over time as they explore the space more. In practice, however, VIPs find it challenging to gather this formation. They may acquire this information by asking for verbal descriptions from others, which is seldom accurate. Alternatively, they may also trace along the boundaries using their tactile senses which is time consuming and tedious. 
% - Shape can also be defined by bound of walkable path. For example, in outdoors, it could be ....



% "it's kind of hard to tell, because, like, I can't, like, see how long a hallway is. But I can feel like how long a hallway is, like, you know, depending on how people like how close people are walking into, like, towards you, you know, because when people see the cane, they move out of your way, for the most part. So like, you can tell like, either they're super close to you, because the hallways kind of narrow. They're like super far, because they just bought on the opposite side. So like, that's easy to tell." -Olivia

\subsubsection{Layout information}
\label{sec:layoutInfo}
Participants described layout information as the arrangement of different objects within the space --- both with respect to them (egocentric)  and with respect to the environment (allocentric). The objects constitute several categories including points of interests (POIs) (e.g., stairs, elevators, restrooms), landmarks (e.g., change in flooring, curbs), obstacles, and other people in the environment who the VIPs often see as potential collaborators in exploration. 

For example, Aaron recalled his visit to an unfamiliar grocery store where he first focused on understanding the shape of the store, and then populated this structure with layout information.
He explained that he sought to understand the locations of certain key points of interest such as the bathroom, specific aisles, and the cash register to develop a more comprehensive understanding of the space and to ultimately allow him to explore the grocery store. Charles described the layout of a space he recently visited with the help of verbal descriptions from his friend: \vspace{-0.25cm} \\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & \textit{``... it's two floors, there's a restroom down the hall on the way as soon as you get in, there is a large step up on to the porch. And then there is double doors leading out to the pool. And there's no gate around the pool.''} --Charles  & \\
\end{tabu} \\

We noticed subtle differences in VIPs' use of landmarks and POIs between navigating to a destination and exploring unfamiliar environments. On one hand, participants described using landmarks and POIs either as potential destinations or as locations to reorient themselves along the route; pointed out by prior work ~\cite{giudice_navigating_2018}. For exploration, on the other hand, participants mentioned using landmarks to create a more comprehensive mental map of the space with the aim to eventually make navigation decisions in situ.


% Once participants had an overview of the shape, essentially the bounds of the space, they found information about arrangement of different landmarks within that space important for exploration. Note that during guidance, VIPs treat POIs as source and destination between routes, and also to reorient themselves [cite a paper]. During exploration, however, VIPs use landmarks to create a more comprehensive mental map that would eventually help them avoid obstacles, choose and stop by destinations on the fly, and confirm their location.  

% [Doesn’t fit in here. Either needs more explanation, or can be removed.] We also found that participants want not just one, but several landmarks for a specific location in the environment. Given the dynamic nature of the environment, location of landmarks may change over time, and landmarks created in previous visits may not be valid anymore. To mitigate this, participants reported that they create redundant landmarks such that even if one of them moves, or if they end up missing one, other landmarks can be used to accurately orient themselves. In fact, participants mentioned building a hierarchy of importance of landmarks. Based upon the landmarks’ relative importance, participants look for certain landmarks first and use the redundant landmarks for confirmation. James explained: \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{“I’ve learned that you cannot rely [only] on one landmark because things change and the world is not static. [...] If you can find three landmarks in a location, then if you miss one or even two, you’ll still have the third[.]”} --- \textbf{James}% 
%  & \\
% \end{tabu}
% \vspace{-0.4cm}\\\\




% \textit{Charles:
% "Yes, actually, so I'm actually going through some of that preparation right now, because I'm going to a new house next Wednesday to go swimming. So I'm in contact with someone who's been there before."" — 16:32
% [example of a space description] ""And what they've taught me so far as it's two floors, there's a restroom down the hall on the way as soon as you get in, there is a large step up on to the porch. And then there is double doors leading out to the pool. And there's no gate around the pool."" — 17:00}



% \subsubsection{Connection information} [not enough support... going through the interview data to see if this is indeed the truth.]


\vspace{2mm}
\begin{center}
\setlength{\fboxsep}{0.8em}
\fbox{\begin{minipage}{0.5\textwidth}
\textbf{Insight 1}: VIPs need two types of spatial information: shape information and layout information, to get a high-level overview of a space.
\end{minipage}}
\end{center}
\vspace{1mm}


% \yy{Hi Gaurav, here is my thought for your consideration - comparing our finding to RW "Uncovering Information Needs for Independent Spatial Learning for Users who are Visually Impaired" and our previous CHI submission:  Do we find a hierarchical framework for the spatial information needed? 
% (1) High level - shape
% (2) Mid level - layout objects
% (3) low level - landmarks (spots) relationships between layout objects, denoted by multimodal senses (CHI submission)
% (4) minute level - precision required, especially for VIPs with no usable vision. 
% Perhaps say more about how the hierarchical framework help VIPs to organize mental map and come up with their own routes when navigating independently.
% This can also help with Theme 3 Independent exploration
% }


\subsection{Factors Influencing Information Preferences Between Individuals}
\label{sec:factors-info-needs}
We discovered three factors that influence VIPs' preferences for spatial information: 
 (1) their onset of vision impairments, (2) their inherent sociability, and 
(3) their O\&M proficiency and mobility aid preference. Not surprisingly, many of these factors have been observed to affect VIPs' navigation behavior in different contexts ~\cite{long_establishing_nodate, wiener_foundations_2010, schinazi_spatial_2016, thinus-blanc_representation_1997, williams_just_2014, williams_pray_2013}. Thus, we identified dimensions of information needs --- specifically, spatial information --- dictated by these factors in context of exploring unfamiliar environments. 
VIPs' preferences dictated information needs along three dimensions, (1) preferred format of spatial information: sensory augmentation vs. detailed descriptions, (2) preferred source of spatial information: via other people vs. via self, and (3) amount of support for gathering spatial information: minimal vs. maximal support; respectively.


% While we discovered a strong correlation between these factors and VIPs' preferences for spatial information, we note that given our sample size it may not be ideal to extend our study results to infer ratio of people with certain preferences in the visually impaired community at large.

% It is important to note that our findings stem from our interviewees with our sample of participants. While we notice a clear influence of the factors we present, it may not be ideal to infer percentage of people with a specific preference based on our small sample. 

% However, the importance of this information was influenced by four key factors: (1) onset of blindness, (2) level of O\&M training, (3) primary mobility aid, (4) personality traits such as inherent curiosity and sociability. 
% These factors characterize the importance of exploration, to some extent, in the lives of our participants.

% We acknowledge that our findings are derived from our interviews with our sample of participants. While we are certain that these factors influence VIPs’ information needs, it is still unclear as to what extent does each of these factors influence VIPs’ preferences at large.


\subsubsection{Onset of vision impairment and preferred `format' of spatial information}
\label{sec:spatial-info-format}

We observed differences in VIPs' preferred \textit{format} for spatial information, which depended on when their onset of vision impairment came about.
% in which early-blind and late-blind individuals wanted to receive spatial information.
% Our early-blind participants --- people who are blind by birth or developed vision impairments early in life --- expressed a preference for receiving spatial information. By contrast, the late blind participants expressed preference for receiving spatial information in the form of verbal descriptions with as much detail as possible.

Many early-blind participants (n=3) --- people who are blind by birth or developed vision impairments early in life --- shared that they have learned to trust their non-visual senses to collect spatial information over time. These participants further explained that they prefer receiving \textit{confirmation} of their sensed information either from other people or through their other senses, instead of receiving complete \textit{descriptions}, and that they prefer their non-visual senses to be amplified (e.g., through a more powerful echolocation ability) rather than mutated (e.g., through system-provided labels). These participants noted that doing so helps them maintain their sense of independence, which is important to VIPs as reported by Lee et al.~\cite{lee_designingIndep_2021}.






By contrast, the late-blind participants expressed preference for receiving spatial information in the form of verbal descriptions with as much visual detail as possible.
Two of our late-blind participants, Emily and Harper, attributed their preference for descriptions of spatial information to their having had vision in the past, allowing them to visualize spaces. \vspace{-0.25cm}\\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & %
 \textit{``I have a pretty good running movie of the world and what it looks like around me and a picture of it. [T]his knowledge [of] how things are put together and look like is definitely [an] advantage of having seen for 25 years.''}  --Emily 
 & \\
\end{tabu} \\\\
Harper noted that she wanted the verbal descriptions to include visual details such as color. Highly visual descriptions help her visualize spaces and memorize them. None of the early-blind participants showed interest in learning or referring to visual concepts such as color when receiving spatial information.




% (people who develop vision impairments later in life)
% We noticed two major difference between early blind and late blind participants' preference for spatial information. First, early blind participants indicated that they trusted information collected via their non-visual senses more than their counterparts. Second, late blind participants valued more detailed 

% differences in our participants' trust on spatial information that they collected via their non-visual senses and their ability to visualize spaces. 
% Congenitally blind participants expressed much more confidence in 


% Our finding reinforce prior research in cognitive sciences, which has shown that congenitally blind people develop different mechanisms due to neuroplasticity of the brain to perform cognitive tasks extremely well with their other senses \cite{chebat2020spatial}. As a consequence, they are relatively better than late blind people in using their non-visual senses effectively. However, all participants noted that information was still not reliable enough (more on this in Section~\ref{sec:ind_exploration}).

% Another difference 

% they are able to infer spatial information with touch and sound.

\subsubsection{Inherent sociability and preferred `source' of spatial information}
We found that participants' preference for seeking assistance from others to collect spatial information --- i.e., \textit{collaborative exploration} --- is correlated to their inherent sociability and prior experiences of being assisted by others. 
While all participants described instances of seeking assistance from others, many (n=5) expressed their preference for using other people as a source of spatial information, instead of doing it all by themselves.


For some of these participants it was easier (William) and faster (Lucas) to gather information via others. Many others (n=4) felt independence in seeking help from others, stating that \textit{``independence also has to do with self-advocating for [oneself]''} (Nora). Most participants who preferred collaborative exploration shared positive experiences of receiving help, even from strangers, and self-reported as being socially adept. %\todo{Is this the correct way to say they were social?}

Interestingly, Emily mentioned that asking for spatial information from others was also a way for her to connect with people. She further explained that she prefers to go shop at CVS in-person, rather than getting items delivered, as it gives her an opportunity for her to interact with people and connect with the outside world. She shared instances of building relationships with several people who help her on a regular basis.
\vspace{-0.25cm}\\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & %
 \textit{`` I could do online shopping or delivery shopping with CVS, but I don't want to. These people become my friends. 
 [...] 
%  Same with my bank, I could do online banking, but I choose not to. 
 I like going up and connecting with the people.''} --Emily
 & \\
\end{tabu} \\


% `` I could do online shopping or delivery shopping with CVS, but I don't want to these people become my friends. Same with my bank, I could do online banking, but I choose not to I like going up and connecting with the people.'' -Emily


Other participants (n=4) expressed their preference for gathering spatial information by themselves --- i.e., \textit{independent exploration} --- whenever it was possible. For most of these participants, we found that they value their ability to explore independently above everything else, and some expressed discomfort in interacting with other people due to negative experiences of seeking help from others. We heard many stories about people not knowing how to help VIPs, similar to what Williams et al.~\cite{williams_just_2014}, Guerreiro et al.~\cite{guerreiro_airport_2019}, and others have reported.


% we found a split between our participants' preference for collaborating with other people for exploration, attributed mainly to their personality traits such as inherent sociability and curiosity. 
% Many participants (n=5) preferred to ask for spatial information from people around them whenever necessary while many others (n=4) preferred to seek assistance from people only as a last resort and wanted to gather information by themselves. Lastly, some participants (n=3) expressed no preference between the two whatsoever. 







% while many other participants wanted to gather spatial information by themselves


\subsubsection{O\&M proficiency/mobility aid preference and preferred `amount of support'}
Participants were split on the amount of support they need to gather spatial information in order to successfully explore unfamiliar environments. These differences were found to be correlated with VIPs' self-reported proficiency in O\&M skills (being exposed to limited/no training vs. sufficient training) and their mobility aid preference (guide dog vs. white cane).

Most participants who self-reported as having limited exposure to O\&M training (n=3) described wanting a higher degree of support from NASs, i.e., detailed spatial information, compared to those who had a greater exposure to O\&M training. In fact, some of the participants with limited O\&M exposure reported to be content with turn-by-turn navigation and did not express a strong desire for the ability to explore unfamiliar environments. As a consequence, they found it extremely hard to infer spatial information on their own.
\vspace{-0.25cm} \\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & %
 \textit{``Usually for groceries, I ask somebody to assist me because [...] I feel like the shape of the store is really complicated to learn.''} --William
 & \\
\end{tabu} \\


We also observed a similar pattern with mobility aid preference. Both of our participants who use a guide dog --- Emily and Harper --- exclaimed that it is extremely hard for them to explore environments with the help of a guide dog. 
Harper explained that while her guide dog is instrumental in ensuring her safety, exploring environments with its help is even more challenging than with a white cane.\vspace{-0.25cm} \\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & %
 \textit{``That's the real downside for my seeing eye dog. To explore a new space, I am supposed to tell him, give him commands. If I don't know where I'm going, I can't tell him. The only thing he can do is get me out [...] and he will keep me from falling.''} --Harper
 & \\
\end{tabu}
\vspace{-0.4cm}\\\\ 


% Our findings revealed another interesting insight about the challenges faced when using different mobility aids, despite both being a part of VIP's independent exploration. Not surprisingly, we observe that all participants who use a white cane regularly (n=10) experienced independence when exploring environments with their cane
% ~\cite{lee2021designingIndependence}. Interestingly, we found that both Emily and Harper --- who are guide dog users --- expressed similar feelings of independence when navigating with their guide dogs.\vspace{-0.2cm} \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{``I will ask for people assistance in my life where I need it, you know, but not a whole lot that way. I pretty much am on my own. When I when we go on our walks around, [my dog] and I are by ourselves.''} -Emily
%  & \\
% \end{tabu} \\\\
% As discussed, while it is challenging to gather information in a self-directed manner for our participants with a white cane, we found that it is almost impossible to explore environments with a guide dog. Harper explains how her guide dog is instrumental in ensuring her safety, but exploring environments with its help is even more challenging than with a white cane.\vspace{-0.2cm} \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{``That's the only thing. That's the real downside for my seeing eye dog. To explore a new space, I am supposed to tell him, give him commands left right forward. If I don't know where I'm going, I can't tell him. So he is not good. The only thing he can do is get me out [...] and he will keep me from falling down steps.''} -Harper
%  & \\
% \end{tabu}
% \vspace{-0.4cm}\\\\ 


% Finally, Grace expressed frustration about not being able to explore environments independently in a self-directed manner. She further reinforces the fact that landmarks and GPS-based systems primarily support guidance-based navigation~\cite{clemenson_rethinking_2021}, and do not facilitate exploration. \vspace{-0.25cm}\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{``You can't really go anywhere unless you have like a plan and you know where you're going. And you have like a set address and like, route to go [and] you have [to have] like a plan B if you get lost [...] Coz like, we can't look at signs and be like, Oh, I'm in this street. You either use landmarks or your GPS or something.''} -Grace
%  & \\
% \end{tabu}
% \vspace{-0.4cm}\\\\ 





% \begin{comment}
% Congenitally blind people (people who are blind by birth) develop different mechanisms due to neuroplasticity of the brain to perform cognitive tasks extremely well with their other senses \cite{}. As a consequence, they are able to infer spatial information with touch and sound. On the other hand, individuals who developed blindness later in life have the ability to visualize spatial information because of their prior experiences when they used to have vision. These differences in their lived experiences causes participants to value different forms of information more than the other. Hence, congenitally blind participants value sensory substitutions more than late blind participants, whereas late blind participants value descriptions that are visual in nature. We describe some examples of these two preferences below.

% Several of our early blind participants (n = 7) described using echolocation as an effective way of obtaining a rough understanding of the shape and size of the environment. In contrast, almost all our late blind participants did not rely on echolocation as much. Grace, who was legally blind by birth, but only in the past year and a half developed severe blindness described some difficulties in relying on echolocation as a means to obtain spatial information. On the other hand, Emily (aged 72), who developed blindness in her mid-twenties mentioned that she has gotten much more comfortable with using touch and sound as a means to get textural and spatial information. During our interviews, Emily shared an anecdote about how she is able to gather information about the texture of the floor with her ‘smart toes’: \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{“I can tell where I am in a room if my toes are telling me I'm on a hardwood floor or carpeted floor. 
% %  [and]
%  I'm talking about with shoes on, so I rely on my ‘smart toes’. It's amazing how much that, almost subconsciously, now information gets through.”} --- \textbf{Emily}% 
%  & \\
% \end{tabu}
% \vspace{-0.4cm}\\\\


% Hence, it is important for NASs to augment VIPs’ senses to either support (for late blind people) or solidify (for congenitally blind people) information gathered about the environment. NASs should be designed to account for these varying levels of information support (or augmentation) requirements.

% Though congenitally blind individuals have a significant advantage (change the word advantage here) in terms of relying on their other senses, late blind people have the ability to visualize spaces due to their prior experiences when they used to have vision. As a result, all our late blind participants expressed the need to get visual information about their environment such as color. Harper (aged 59), who developed blindness at the age of twenty shared that her colleague would describe her visual information at a fundraiser event (not sure if this is very relevant because we are talking about exploration):\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{“She would describe every lady’s gown and what they were wearing, and what it looked like, and what their jewelry looked like, and what their hair looked like, and that sort of thing. Thankfully, I was able to see when I was younger and so, when she says midnight blue, or teal blue, or royal blue or sky blue. I know what color she's talking about.”}   --- \textbf{Harper}% 
%  & \\
% \end{tabu}
% \vspace{-0.4cm}\\\\



% Emily adds further: \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{“I can't speak for all blind people, but I saw until I was 25. Right? So, I have a pretty good running movie of the world and what it looks like around me and a picture of it. [T]his knowledge of the world and how things are put together and look like is definitely advantage of having seen for 25 years.”} --- \textbf{Emily}% 
%  & \\
% \end{tabu}
% \vspace{-0.4cm}\\\\


% On the other hand, all participants who are totally blind by birth expressed no interest whatsoever in visual information because they have no such concept as color. 

% For NASs to support exploration, it is important to design for VIPs’ varying preference for visual information that is influenced by when they developed vision impairment. \\
% \end{comment}


\vspace{2mm}
\begin{center}
\setlength{\fboxsep}{0.8em}
\fbox{\begin{minipage}{0.5\textwidth}
\textbf{Insight 2}: VIPs' preferred format, source, and amount of spatial information support vary between individuals depending upon their \mbox{onset} of vision impairment, their inherent sociability, and their O\&M proficiency and mobility aid \mbox{preference}, respectively.
\end{minipage}}
\end{center}
\vspace{1mm}







% \newpage % <------- Delete this.

\section{RQ2 Findings: Challenges in Exploration}
\label{sec:RQ2-findings}

In this section, we present our findings for RQ2: What challenges do VIPs face while exploring unfamiliar environments, both independently and collaboratively? 
% Our analysis revealed challenges around two major means of exploration and our results are organized around them: independent exploration (Section~\ref{sec:ind_exploration}) and collaborative exploration (Section~\ref{sec:colab_exploration}).
% Our analysis revealed challenges that VIPs face, around two major means of exploration: independent exploration (Section~\ref{sec:ind_exploration}) and collaborative exploration (Section~\ref{sec:colab_exploration}).
% We note that whilst organized as two different sections, participants described exploring environments themselves (independently) and by seeking assistance from others (collaboratively) in an intertwined manner, often shifting between the two means of exploration.
Our analysis revealed several challenges that VIPs face during exploration, which we present around two major means of exploration, (1) \textit{independent exploration}: exploring by themselves (Section~\ref{sec:ind_exploration}), and (2) \textit{collaborative exploration}: exploring by seeking assistance from others (Section~\ref{sec:colab_exploration}). 
We note that whilst organized as two different sections, participants described exploring environments using both means of exploration in an intertwined manner, often shifting between one another. 
% Throughout our results, we highlight key insights that inform design implications for future NAS research.


% This paragraph can be removed, in case we run into space issues. Doesn't add new knowledge as such. But does lay a solid base of what is to come next and get a general sense of VIPs' preference for both these forms of exploration.
% Most participants (n=8) reported relying on their own abilities first, as they prefer to\todo{May omit this para.}  \textit{`figure things out'} (Nora) using their non-visual senses
% % (e.g., hearing, touch, smell)
% and their O\&M skills. However, participants described challenges in doing so reliably, indicating that independent exploration may not always be possible. In such situations, participants seek assistance from other people. In fact, some participants (n=4) prefer collaborating with other people --- over exploring independently --- as it is more \textit{``convenient''} (William) and also \textit{``saves time''} (Lucas). Despite this comfort, our participants shared some challenges in supervising the assistance they received when collaborating with others.  

% Below, we discuss the challenges that our participants reportedly face: first in independent exploration, and then in collaborative exploration. 
% Below, we discuss the challenges that our participants reportedly face in independent exploration first.


% Not surprisingly, we found - - - (something that is found in other papers). Interestingly, - - - (our new findings, or nuance).









\subsection{Challenges in Independent Exploration}
\label{sec:ind_exploration}
We discovered two major challenges in our participants' independent exploration endeavors.
First, participants reported difficulties in gathering spatial information precisely and reliably via their non-visual senses (e.g., hearing, touch, smell). Second, participants described challenges in acquiring appropriate O\&M training and maintaining their O\&M skills. We elaborate upon these challenges in the following sections.

% % Why independent exploration is important. <-- doesn't seem like a "very" important thing to say. 
% Most participants (n=8) emphasized that being able to explore on their\todo{May omit this para.}  own is crucial to their sense of independence and self-confidence, reinforcing findings by Lee et al.~\cite{lee2021designingIndependence}. 
% James, for instance, considers external assistance only as a last resort, indicating he would not ask for help from others, \textit{``unless I'm in an absolute hurry and have no choice''}. Despite such a strong preference, VIPs reported facing challenges in using their non-visual senses to gather spatial information and using their O\&M skills to explore environments. We elaborate upon these challenges in the following sections.

% In the following sections, we elaborate on these challenges.











\subsubsection{Gathering spatial information precisely and reliably}
\label{sec:precise-spatial-info}

% Participants described many instances in which they could not gather spatial information precisely and reliably as a major challenge to them being able to explore unfamiliar environments independently.

% Participants described their inability to gather spatial information precisely and reliably as a major challenge to them being able to explore unfamiliar environments independently. As we found in Section~\ref{sec:informationNeeds}, VIPs need two types of spatial information for exploration --- information about rooms' shape and information about the layout of objects within rooms --- so we define spatial information to be these two types of information. Participants described many instances in which they could not gather spatial information precisely and reliably using their non-visual senses (hearing and touch), impeding their ability to explore independently.


Interviewees shared many instances in which they gathered spatial information --- shape and layout information (see Section~\ref{sec:informationNeeds}) --- using their non-visual senses such as hearing, touch, and smell. Not surprisingly, VIPs' use of their non-visual senses for navigation has been reported by prior research as well~\cite{thinus-blanc_representation_1997, banovic_uncovering_2013, williams_pray_2013, williams_just_2014, thieme_i_2018}. Interestingly, though, we found that spatial information gathered through these senses was neither precise nor reliable for VIPs to make in-situ navigation decisions, severely impeding their ability to explore unfamiliar environments independently.


% James and Charles describe using their sense of hearing --- particularly, echolocation --- to gather shape information. INSERT JAMES SCENARIO INFO. INSERT CHARLES SCENARIO INFO.
% But that hearing was not precise or reliable.
% INSERT PARAGRAPHS ABOUT PRECISION

% SOUND
Some participants (n=3) described using their sense of hearing --- particularly, echolocation --- to gather shape information, but lamented that it only gives them a very rough idea of the environment's shape and lacks the precision to work well in large or crowded places. 
James recalled visiting a shopping mall in his neighbourhood, describing how echolocation was not precise enough for him to gather shape information, and how he had to use his white cane to learn more. \vspace{-0.25cm}\\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & %
 \textit{``... echolocation can tell me some things about the shape, but I want specifics. 
   So, I will go to each side of the entrance and check how big the entrance is, and then I can learn that there are two large openings from this foyer.''} --James
 & \\
\end{tabu}
\\\\
Similarly, Charles had concerns about relying on the shape information acquired via echolocation and noted that he resorts to seeking confirmation from others. 



We found that our participants trusted their sense of touch more than their sense of hearing due to its higher precision. However, participants also noted that their sense of touch is not a reliable option since it can not be used everywhere. 
Most participants (n=7) agreed that using touch is a brute force approach that does not scale well to large spaces such as grocery stores, airports, and shopping complexes.

Furthermore, participants expressed hesitation in using touch, including tactile feedback via their cane, to gather spatial information when other people are present in the environment. 
Charles mentioned concerns about hitting people with his cane in crowded places, while Olivia expressed fear of knocking objects over in front of others. Harper echoed the sentiment, stating that some behaviors are inappropriate in a public setting, making it extremely challenging to independently explore environments via touch.
 \vspace{-0.25cm} \\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & %
 \textit{``I mean, if you're somewhere by yourself, you could explore anything. But when you're in a public setting, people are really gonna look at you strangely if you get up at a restaurant and start walking around and feeling all the tables.''} --Harper
 & \\
\end{tabu}
\vspace{-0cm}\\\\
Approaching this finding from Easley et al.'s~\cite{easley_lets_2016} perspective --- majority of people who occupy the environment dictate the social norms --- we could in fact say that VIPs' independent exploration strategies using their non-visual senses is ``disruptive in predominantly sighted environments''. 

% Our findings align with prior work by Easley et al.~\cite{easley_lets_2016} and thus, VIPs' \todo{find a good word for association and extension}
% % and thus, by extension, we note that 
% independent exploration using non-visual senses could also be viewed as being ``disruptive in predominantly sighted environments''. 


Among the three non-visual senses, our participants mentioned relying the least on their sense of smell for exploration. Many participants recalled specific examples of detecting the smell of fries (Grace), laundry (Nora), and garbage (Leo) to identify certain landmarks, helping them make an educated guess about the possible layout of the space but the information was not concrete enough to be able to act upon. Leo expressed the shared sentiments among our participants, describing how the sense of smell merely supplements their other senses. \vspace{-0.25cm}\\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & %
 \textit{``That's usually not my first priority. [The sense of smell] is more maybe just providing some supplemental information. I would not say that that's something that I rely on in any capacity.''} --Leo
 & \\
\end{tabu}\\


We noticed an exception to the need for precision and reliability in spatial information. Participants with residual vision mentioned that they did not rely on their non-visual senses as much. Consequently, they were able to gather spatial information with some extra effort using their vision. However, participants with low-vision still expressed some frustrations while doing so and thus shared the need for assistance for improving the precision of information collected via their \textit{visual senses}, instead of non-visual senses. Our findings, in context of exploration, align with Szpiro et al.'s~\cite{szpiro_finding_2016} work on understanding challenges that people with low-vision face when shopping.

% learn the layout of the space. 
% As James explains, \textit{``stores often have a smell... clothing stores smell different from jewelry stores.''} 

\vspace{2mm}
\vspace{-0.0cm}\begin{center}
\setlength{\fboxsep}{0.8em}
\fbox{\begin{minipage}{0.5\textwidth}
\textbf{Insight 3}: VIPs face difficulties in making \mbox{navigation} decisions based on spatial information collected via their non-visual senses.
% Participants
% % VIPs 
% face difficulties in gathering precise and reliable spatial information %
%  via their non-visual senses%
% , impeding their ability to explore independently.
% them being able to explore unfamiliar environments independently
% Spatial information gathered via VIPs' non-visual senses is neither precise nor reliable, being a significant challenge in their ability to explore independently.
\end{minipage}}
\end{center}
\vspace{1mm}

% \yy{Again, for Gaurav's consideration - There might be more nuances here regarding individual differences in the need. Do all VIPs require precise info? I remember some low vision VIPs mentioned that they did not need super precise info, because once they are at the vicinity, they can use their residual vision to find it. I can look for the quote if you need. I might also find RW that talks about using residual vision.}

% Latest version of Brian's stab at it
% Participants described their inability to gather spatial information precisely and reliably as a major challenge to them being able to explore unfamiliar environments independently. As we found in Section~\ref{sec:informationNeeds}, VIPs need two types of spatial information for exploration --- information about rooms' shape and information about the layout of objects within rooms --- so we define spatial information to be these two types of information. Participants described many instances in which they could not gather spatial information precisely and reliably using their non-visual senses (hearing and touch), impeding their ability to explore independently.


% Participants described their inability to gather spatial information precisely and reliably as a major challenge to them being able to explore unfamiliar environments independently. As we found in Section~\ref{sec:informationNeeds}, VIPs need two types of spatial information for exploration: information about rooms' shape and information about the layout of objects within rooms. Our participants described how it is not possible for them to gather this type of information precisely and reliably using their non-visual senses (hearing and touch), and that they would be able to explore unfamiliar environments much more independently if they could gather spatial information more precisely and reliably.










% \subsubsection{Learning and maintaining O\&M skills for exploration}

\subsubsection{Acquiring appropriate O\&M training and maintaining O\&M skills} 
\label{sec:Acquire-O&M-Training}
We discovered that most participants (n=7) expressed difficulties in exploring environments independently because of lack of confidence in their O\&M proficiency. Participants indicated that this was not because O\&M techniques are not sufficient to support independent exploration, but rather attributed this hesitation to their lack of access to appropriate O\&M training and their inability to maintain O\&M skills. 


Upon further inquiry, we found three hindrances that prevent VIPs from acquiring adequate O\&M training resources: lack of funding, shortage of O\&M instructors, and difficulties in setting up O\&M sessions as an adult --- specifically those who developed vision impairments later in life. 
Most participants were aware of the power of O\&M skills and lamented on the lost opportunities to explore unfamiliar environments by themselves. 
As Charles exclaimed: \vspace{-0.25cm}\\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & \textit{``I feel like I would have benefited [with more O\&M training]. I don't want to feel like I'm over exaggerating, but at least 10 times more.''} --Charles & \\
\end{tabu}\\%
% This lack of O\&M training causes VIPs to lose confidence in their ability to ``figure things out'' on their own, surfacing as a major challenge to VIPs' desire for independent exploration.


% As a consequence, VIPs hesitate to ``figure things out'' on their own.




% Although prior work investigating VIPs' variability in O\&M training experiences~\cite{williams_pray_2013} 
% Our findings reinforce prior work by Williams and colleagues~\cite{williams_pray_2013} who studied variations in VIPs' O\&M training experiences to asse 

%  Williams and colleagues~\cite{williams_pray_2013} reported variations in VIPs' O\&M training and reported several factors including  . However,  



% Williams and colleagues~\cite{williams_pray_2013} found variability in when it was obtained, quality of instruction, and how the training is currently used.

% insufficiencies in their participant demographic as well, citing reasons such as funding and onset of vision impairments as factors. 

% participants believed that they would be able to use their O\&M skills to explore unfamiliar environments independently, had they received appropriate O\&M training.
% Upon further inquiry, participants revealed that their insufficiency in O\&M skills was attributed to difficulties in acquiring appropriate O\&M training. 

% This insufficiency further affected their sense of felt independence and autonomy in exploring environments independently.%
% % its immense importance as it empowers them with autonomy. 
% \vspace{-0.25cm}\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{``[O\&M skills are] vital because the world will walk over you if you don’t take control of your own abilities. [...] People will tell you where you can go and what you can do. If you don't know how to do those things, then you're just kind of meekly following along. It's self esteem shattering, and reduces your individuality.''} -James & \\
% \end{tabu} \\



% The first factor is \textit{onset of vision impairments}\todo{\cite{williams_pray_2013} says this as well}. Most of our participants (n=7) who developed vision impairments earlier in life or are blind by birth, reported easy access to O\&M instructors via their schools as a child. On the contrary, participants (n=3) who developed vision impairments later in life described challenges in arranging for one. Several participants (n=6) agreed that it much more difficult to set up an O\&M session as an adult, compared to when they were in school. For instance, Nora (who is blind by birth) explains:\vspace{-0.25cm}\\\\
%         \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%          & \textit{``For earlier years, I didn't need to reach out to O\&M instructors because that's something, that like, we automatically get in schools. Now, [as an adult,] I definitely would have to advocate for myself''.} -Nora & \\
%         \end{tabu}\\
% % As a result, most of Nora's O\&M training was done during her K-12 education.\vspace{0.2cm}
    
% The second factor is \textit{lack of access to O\&M instructors}\todo{\cite{williams_pray_2013} says this as well}. Some of our participants (n=2), despite being blind by birth and being assigned an O\&M instructor, did not receive appropriate training. Our follow up interviews with the leaders of blind-serving organization and the O\&M instructors revealed that this is primarily due to shortage of O\&M trainers and decentralization. Both the leaders and the instructor confirmed that O\&M instructors are assigned multiple students scattered over a geographical area, which makes it difficult for them to be physically present and provide enough time to all their students. As a result, many VIPs miss out on the appropriate amount of O\&M training they are promised. For instance, Charles, who was assigned an O\&M instructor during middle school explains that he never received formal O\&M training, despite his belief that it would have benefited him. \vspace{-0.25cm}\\\\
%     \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%     & \textit{``I was told that I would get an O\&M trainer back in middle school. [...] I never received that trainer. She came in once within the six years she was supposed to be training me.''} -Charles & \\
%     \end{tabu} \\
    
% Lastly, the third factor is \textit{lack of funding}\todo{\cite{williams_pray_2013} says this as well}. Most of our participants (n=9) reported being dependent upon their respective states to receive O\&M training or other accessibility services or devices. Few participants (n=2) noted that their access to O\&M training in the past has been affected due to shortage of state funding. Lucas explains that adult VIPs in his state are only provided vocational rehabilitation training, which is a form of training meant only to provide necessary skills to a VIP so that they can perform a specific job. However, as Lucas further notes, even this type of training was scarce, and VIPs have to prove their employment status in order to receive it. \vspace{-0.25cm}\\\\
%     \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%      & \textit{``It's just very hard to get O\&M training here because [anonymized state] is out of money. [...] It's very hard [because] you've got to prove that you’re working.''} -Lucas & \\
%     \end{tabu}\\\\
% We acknowledge that these factors are predominant in the United States where all our participants live. 
% Further research is needed to 
 
% [option 1]
% Although increasing awareness regarding the three factors we identified is important, NASs too can play an important in mitigating some of these issues.
% [option 2]Although the three factors we identified call for action from the concerned authorities due their systemic nature, NASs too can play an important in mitigating some of these issues.
% For instance, with respect to shortage of trainers, many participants described wanting to meet more frequently with their O\&M instructors: \textit{``... so I don't think once a week is enough training, that's why I already applied for [...] taking a mobility class every day''} (Grace). NASs can help support both O\&M instructors and VIPs by acting as virtual O\&M assistants to allow VIPs practice and learn regularly. 
% More on this in Section~\ref{sec:visions}.



% \begin{center}
% \fbox{\begin{minipage}{0.5\textwidth}
% \textbf{Insight 4:} Participants  face difficulties in acquiring appropriate O\&M training due to three factors: (1) onset of vision impairment, (2) lack of access to O\&M instructors, and (3) lack of funding.
% \end{minipage}}
% \end{center}
% \vspace{1mm}


% The three factors described above primarily concern with how the system is set up to provide VIPs support for O\&M training. While it is important to increase awareness about these issues and to warrant action from the concerned authorities, NASs too have the potential to help by serving as a . For instance, some participants mentioned that 
 


% \textit{``Yeah, so I don't think once a week is enough training, that's why I'm I already applied for a training centre that focuses on mobility and you'll be taking a mobility class every day and they blindfold you and they make you cross streets and I'm like, I need that because that will really push me out of my comfort zone and that will give me the confidence I need to cross any street.''} -Grace



% Providing an efficient systems-based solution to O\&M training could help democratize the skills necessary for VIPs to navigate independently. 
% Hence, we suggest that in order for NASs to facilitate exploration, they should not only provide a means of practicing O\&M skills but should also provide an effective way of developing these skills in the first place.

% Add a sentence about how there is opportunity for NASs (or in general) to help VIPs with O\&M training. - Done.








% \subsubsection{Maintaining O\&M skills}\todo{section 5.1.3 needs edit.}
% Interviewees described their inability to maintain their O\&M skills as a major challenge to them being able to explore independently. 

Few participants (n=3) reported receiving appropriate O\&M training, yet still did not feel confident in exploring environments independently. Participants noted that this was because of their inability to regularly use their O\&M skills safely, and thus were concerned about atrophy of their skills.
James elaborated how he denies assistance out of fear of his skills deteriorating if he relies too much on others.\vspace{-0.25cm}\\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & \textit{"It is very easy to let your [O\&M] skills atrophy as a blind person if you rely overly on sighted people[.] It's easy to [use a] sighted guide and become complacent and [not pay attention to] what turns you have taken and where you are in relation to other things." } --James & \\
\end{tabu}
\\\\However, he mentioned eventually relying on sighted guide assistance --- especially when exploring unfamiliar environments.

% We note that not all participants agreed to this sentiment. Some participants (n=4) prefer seeking assistance — over exploring independently — as it is more “convenient” (William) and also “saves time” (Lucas) and end up being guided by them.



% Participants felt strongly about maintaining their O\&M skills as it contributes significantly to their sense of autonomy. \vspace{-0.25cm}\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{``[O\&M skills are] vital because the world will walk over you if you don’t take control of your own abilities. [...] People will tell you where you can go and what you can do. And if you don't know how to do those things, then you're just kind of meekly following along. It's self esteem shattering, [and] reduces your individuality.''} -James & \\
% \end{tabu}% \vspace{-0.25cm}
% \vspace{-0.1cm}\\\\%
% We discovered two major facets to participants' challenge in maintaining their O\&M skills.


% Participants worried about their safety when exploring unfamiliar environments, thereby relying on others such as an O\&M instructor or a family member to accompany them. However, as we found previously (in Section~\ref{sec:Acquire-O&M-Training}), shortage of O\&M instructors and limited availability of family members makes it a virtually infeasible option.
% Grace shared how she needs regular practice to feel more confident about crossing streets independently. \vspace{-0.25cm}\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{``Yeah, so I don't think once a week is enough training, that's why I have already applied for [...] taking a mobility class every day. [...] I need that because that will really push me out of my comfort zone and that will give me the confidence I need to cross any street.''} -Grace & \\
% \end{tabu} \\


% Participants expressed frustrations as they found themselves caught in a vicious circle where they had to rely on others to maintain their O\&M skills.

% could not avoid other people's help due to lack of confidence, which in turn was caused by their inability to maintain their O\&M skills.   


% [decision to go somewhere depends on availability of family/friends] "Yes, it depends. Or it depends on whether they're free or whether or not they're going in general." -Daniel



% \textit{``Yeah, so I don't think once a week is enough training, that's why I'm I already applied for a training centre that focuses on mobility and you'll be taking a mobility class every day and they blindfold you and they make you cross streets and I'm like, I need that because that will really push me out of my comfort zone and that will give me the confidence I need to cross any street.''} -Grace
% Limited opportunities to practice and gain confidence. We found two reasons: One, they do not have the safety net of an instructor or a family member where they could go and practice. INSERT GRACE'S QUOTE ABOUT MORE TRAINING IS NEEDED.

% Two, they cannot always avoid help from other people even when they want to. INSERT QUOTE BY JAMES ABOUT HOW HE AVOIDS HELP, but then there are other VIPs (mixed opinions) who prefer to seek help rather than do it themselves because it is more convenient and safe for them to do so. INSERT MINI-QUOTES BY LUCAS AND WILLIAM (or whoever it was).

% SEEMS OVER GENERALIZED...
% Interestingly, we also learned that VIPs' inability to maintain their O\&M skills could even force their choice of mobility aid. Harper, who developed vision impairment later in life, described that her decision to use a guide dog was purely because of her discomfort in using a white cane, caused by not being able to maintain her skill. She explains:\vspace{-0.25cm}\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{``I think it was because at the time I got the training, I had too much vision left. So I was able to rely on not just the white cane, but also my vision. 
% %  So I was able to see the other, you know, I was able to see the white lines of the crosswalk, so I could stay in between. 
%  But as I lost more vision, I didn't go back for more orientation and mobility training, because by then I had to see my dog''} -Harper & \\
% \end{tabu} \\


\vspace{2mm}
\begin{center}
\setlength{\fboxsep}{0.8em}
\fbox{\begin{minipage}{0.5\textwidth}
\textbf{Insight 4:} VIPs face difficulties in acquiring \mbox{appropriate} O\&M training and maintaining their O\&M skills, negatively impacting their confidence to  explore independently.
\end{minipage}}
\end{center}
\vspace{1mm}








% \subsubsection{Different mobility aids pose different challenges.}


% Our findings revealed another interesting insight about the challenges faced when using different mobility aids, despite both being a part of VIP's independent exploration. Not surprisingly, we observe that all participants who use a white cane regularly (n=10) experienced independence when exploring environments with their cane
% ~\cite{lee2021designingIndependence}. Interestingly, we found that both Emily and Harper --- who are guide dog users --- expressed similar feelings of independence when navigating with their guide dogs.\vspace{-0.2cm} \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{``I will ask for people assistance in my life where I need it, you know, but not a whole lot that way. I pretty much am on my own. When I when we go on our walks around, [my dog] and I are by ourselves.''} -Emily
%  & \\
% \end{tabu} \\\\
% As discussed, while it is challenging to gather information in a self-directed manner for our participants with a white cane, we found that it is almost impossible to explore environments with a guide dog. Harper explains how her guide dog is instrumental in ensuring her safety, but exploring environments with its help is even more challenging than with a white cane.\vspace{-0.2cm} \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{``That's the only thing. That's the real downside for my seeing eye dog. To explore a new space, I am supposed to tell him, give him commands left right forward. If I don't know where I'm going, I can't tell him. So he is not good. The only thing he can do is get me out [...] and he will keep me from falling down steps.''} -Harper
%  & \\
% \end{tabu}
% \vspace{-0.4cm}\\\\ 


% Finally, Grace expressed frustration about not being able to explore environments independently in a self-directed manner. She further reinforces the fact that landmarks and GPS-based systems primarily support guidance-based navigation~\cite{clemenson_rethinking_2021}, and do not facilitate exploration. \vspace{-0.25cm}\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{``You can't really go anywhere unless you have like a plan and you know where you're going. And you have like a set address and like, route to go [and] you have [to have] like a plan B if you get lost [...] Coz like, we can't look at signs and be like, Oh, I'm in this street. You either use landmarks or your GPS or something.''} -Grace
%  & \\
% \end{tabu}
% \vspace{-0.4cm}\\\\ 





% \begin{center}
% \fbox{\begin{minipage}{0.5\textwidth}
% \textbf{Insight 4}: O\&M Skills and the issues related to it...
% \end{minipage}}
% \end{center}
% \vspace{1mm}




\subsection{Challenges in Collaborative Exploration}
\label{sec:colab_exploration}
We discovered two major challenges that VIPs face when exploring unfamiliar environments by seeking assistance from other people. 
First, our VIP-participants (n=4) expressed concerns about putting social pressure on others while seeking assistance from them. Follow-up interviews with others collaborating with the VIPs (e.g., grocery store employee) corroborated feeling some social anxiety when helping VIPs explore; particularly, when in public settings.
Second, many VIPs (n=5) described difficulties in supervising assistance from others. 
% communicating their preferred form of assistance (i.e., verbal assistance) and comprehending verbal assistance. 
More specifically, participants described wanting to stay in control of the type of assistance they receive and the format in which they receive spatial information. Doing so is important to both their ability to successfully explore unfamiliar environments and to their sense of independence. 
We elaborate on these challenges next.






% Not surprisingly, participated mentioned seeking assistance from others during exploration, as found in prior research by Williams et al.~\cite{williams_just_2014}. Participants mentioned relying 
% Interestingly, 

% copied from previous draft:
% \textit{The second means of exploration that we discovered as being challenging for VIPs is the ability to get information from others }--- specifically, from non-VIPs. Our VIP participants (n=4) expressed a desire to ask non-VIPs for directions as a means of exploring unfamiliar environments, and to do so while maintaining their independence and continuing to navigate the environment themselves.

% Specifically, the VIPs reported three challenges they often face in getting information from non-VIPs: that asking for information often leads to receiving full guidance, that the information they receive relies on having vision to understand, and that merely asking non-VIPs for information exerts social pressure on them. We describe these three challenges in the following subsections.


% We note that all quotes reported in this section are from our interviews with the 12 VIPs (Table \ref{tab:participants}) and follow up interviews with 6 other people (two leaders of blind-serving organization, a manager of disability services department at a university, an O\&M trainer, and two store employees). We interviewed these other people, who the VIPs constantly mentioned as shaping their behavior around navigation, to investigate specific challenges that VIPs reported in interviews.


\subsubsection{Social pressures in collaborative exploration}
% \subsubsection{Getting information without putting social pressure on the helper}
Participants cited instances where they felt uncomfortable receiving help from others, due to social pressure that the person helping them may face. 
James expressed frustrations about having to put her younger sister in a position where others feel that she is responsible for James's actions. He recalled going for shopping with his sister: \vspace{-0.25cm}\\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & \textit{“I know that my sister gets looks from people all the time, because of foolish assumptions they make out of ignorance. [People think] that she is my caretaker [and that] anything that they perceive as her not doing her job, is wrong.”} --James & \\
\end{tabu}%
\\\\
Many participants (n=4) indicated that they are most comfortable seeking assistance from O\&M instructors since they are trained professionals and somewhat immune to these social pressures. However, relying on O\&M instructors is not feasible, as we discussed earlier (Section~\ref{sec:Acquire-O&M-Training}).


% agreed that they are most comfortable seeking assistance from O\&M instructors since they are trained professionals and somewhat immune to these social pressures. However, relying on O\&M instructors is not feasible, as we discussed earlier (Section~\ref{sec:Acquire-O&M-Training}).


During our interviews, most VIPs (n=10) mentioned grocery stores as an example setting for collaborative exploration. Our participants described several different techniques for buying groceries. Daniel, for instance, stated that he calls the store ahead of time to arrange for a personal shopper. Despite the advance notice for assistance, Daniel describes sensing some discomfort when exploring the store with the store employee. To better understand this discomfort and to confirm Daniel's inkling, we followed up with a grocery store employee.



We found that the employees indeed feel the social anxiety, confirming Daniel's claim. 
The grocery store employee noted that despite his intention to help visually impaired customers, he is \textit{``... always concerned with invading somebody's personal space or [disregarding] their bodily autonomy.''} He also mentioned worrying about the company policies and feared getting in trouble if he makes a mistake. \vspace{-0.25cm}\\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & \textit{``[My manager] said that if you need to help a customer [...] who's disabled, definitely try to if they give you consent [...] Just be careful in that case. But if they don't say anything, then you shouldn't do anything. Because you don't want to actually [cause] issues where they say, `oh, why are you touching me'?''} --Grocery store employee & \\
\end{tabu} \\\\
We discovered that social pressures affect both VIPs and others, negatively impacting the frequency and quality of assistance that VIPs receive when exploring environment collaboratively. 
% While Easley et al.~\cite{easley_lets_2016}




\vspace{2mm}
\begin{center}
\setlength{\fboxsep}{0.8em}
\fbox{\begin{minipage}{0.5\textwidth}
\textbf{Insight 5}: Social pressures pose a major challenge to VIPs receiving help and to non-VIPs providing help when exploring environments collaboratively.
\end{minipage}}
\end{center}
\vspace{1mm}

% \yy{Contrast with "Let’s Get Lost: Exploring Social Norms.." paper, that paper describes a predominantly blind environment. Our findings focus on predominantly sighted people environment, where social pressure becomes heightened. Some behaviors / techniques, (Staff announces "Registration desk this way!", VIPs ask loudly "where is empty seats?") in "Let's Get Lost" paper is quite effective, but those behaviors are not practical in predominantly sighted environment due to social pressure. How can NASs support those VIP behaviors without the social pressure?}



\subsubsection{Supervising assistance for collaborative exploration}
\label{sec:supervising-collab-exploration}

Many participants (n=4) described wanting a loose form of collaboration, specifically verbal assistance, when exploring unfamiliar environments with the help of others. Verbal assistance comprises primarily of descriptions for shape and layout information, which enables them to \textit{``figure things out''} (Nora). 
By contrast, Williams et al.~\cite{williams_just_2014} found that VIPs prefer ``sighted guide'' assistance when walking with another person. This difference highlights that for VIPs, exploration is a self-driven activity and other people play a secondary role as per VIPs' requirement.
Our participants described challenges in communicating preference for verbal assistance. 
% \todo{"connection between space and language has long been a vexing issue to researchers and developers" 2
% \cite{giudice_use_2020}}



% Participants expressed difficulties in communicating their preference for verbal assistance, primarily because of other people's assumption about VIPs' need for guided assistance. 
% Similar to Guerreiro et al.'s findings~\cite{guerreiro_airport_2019}, several participants (n=5) shared their experiences navigating at an airport and most of them %
% % agreed with Emily that they \textit{``... have always gotten very good ground assistance at the airport''}. However, some of them also 
% expressed annoyance when the staff assumes they need a wheelchair: \textit{``... the very first thing they always do, and I will never understand this, is they give you a wheelchair''} (James).


% While some participants said that they refuse this offer as it negatively impacts their sense of independence, Lucas says that he would use it. He further explains that he prefers receiving verbal instructions only in scenarios where he does not have a specific destination to reach within a time constraint.  




% \vspace{-0.25cm} \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{``... the very first thing they always do, and I will never understand this, is they give you a wheelchair''} -James & \\
% \end{tabu}
% \vspace{0.2cm} \\\\

In addition, participants mentioned  challenges in comprehending verbal assistance. In situations where VIPs do get verbal assistance, they noted that the information they received was often not useful. We found that participants struggle to comprehend spatial information received from non-VIPs because of non-VIPs' predominantly visual descriptions.
% \vspace{-0.25cm} \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{``... they'll say, just go down `there' a little. That's not [enough]. I need to really know, take about 10 paces, and turn left or turn sharp left. And people just aren't used to being that descriptive.''} -Harper & \\
% \end{tabu} \\
\vspace{-0.25cm} \\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & \textit{``[I need to ask for clarification] because a lot of people describe [shapes with letters] like `U' shaped or `H' shaped. ... I just prefer geometric shapes [for descriptions.]''} --James & \\
\end{tabu} \\\\
While several studies have noted that VIPs' perceptions of space is different from those of sighted people~\cite{williams_just_2014, thieme_i_2018}, we identified VIPs' preferred format for spatial information --- geometric shape descriptions --- to inform NAS design.



Interestingly, we found that for this reason many participants (n=3) collaborate with other VIPs who have already been to a location. Nora recounted calling her friend, who is also visually impaired, to ask for verbal assistance. Through her friend she obtained spatial information in a more useful format, along with additional cues for her non-visual senses. \vspace{-0.25cm}\\\\
\begin{tabu} to \linewidth { X[l] X[28l] X[l]}
 & \textit{“So for example, my friend will tell me this train [...] doesn't talk. And I'm really gonna have to pay attention and count the stops.”} --Nora & \\
\end{tabu} \\\\
Another successful instance of such a collaboration is using remote sighted assistance such as AIRA~\cite{aira}. Although participants are content with verbal descriptions provided by AIRA professionals, many participants (n=5) noted that it is too expensive for them.


% We note that a VIP-VIP form of collaboration is usually not observed in turn-by-turn navigation, and has untapped design opportunities for NASs.

% \textbf{May add later:} Some VIPs also mentioned using remote sighted assistance like AIRA, but said that it was too expensive for them to use. -- later in visions, talk about how vip-vip and aira dataset can be used to for descriptions and stuff -- since it is VIPs' language. In fact, we could keep sighted people in the loop, which could guide these translation systems to make predictions better -- which may not be super accurate since data is very small and these models are data intensive.




\vspace{2mm}
\begin{center}
\setlength{\fboxsep}{0.8em}
\fbox{\begin{minipage}{0.5\textwidth}
\textbf{Insight 6}: VIPs want verbal assistance in a \mbox{comprehensible format} when exploring \mbox{collaboratively} but find it challenging to \mbox{communicate this} preference to others.
\end{minipage}}
\end{center}
\vspace{2mm}



% Table~\ref{tab:findings} summarizes our findings for our two research questions. Based on these findings, we synthesize design guidelines for future NASs that facilitate exploration; described in the next section.













% COPY OF THE TABLE
% % Pasted from Friendscope paper
% \begin{table}[th]
% \renewcommand{\arraystretch}{1.3}
% \caption{Summary of our study findings for our two research questions.}
% \label{tab:results-summary}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{{p{0.14\textwidth}p{0.36\textwidth}p{0.49\textwidth}}}
% \toprule
% \textbf{Research Question} & \textbf{Theme} & \textbf{Findings}\\
% \midrule
% Fellowship & Users emphasized the sense of being directly connected --- live --- to each other when using Friendscope and described it as a more intimate form of livestreaming. 
% & While \textit{continuous streaming} is a popular approach for sharing live experiences, consider supporting \textit{continuous access} instead or in addition. The mere feeling of having access can promote the feeling of closeness. \\

% & Lightweight signals such as “trigger requests” signaled to both Wearers and Friends that their partners were connected ``live.''
% & Even very minimal interaction techniques can provide feelings of immediacy and intimacy in experience sharing systems. Consider incorporating “trigger requests” and other forms of lightweight signals in addition to standard message types such as text and voice notes. \\

% \hline
% Privacy & 1:1 sharing enhanced participants' comfort with the shared camera.
% & To mitigate privacy concerns, consider allowing users to choose small, private groups to share content with. \\

%  & Manually approving trigger requests assuaged Wearers' concerns about sending content accidentally.
%  & Designing interactivity into a system can help communicate users’ intent. Consider enabling explicit actions to signal explicit consent. \\ 
% \hline
% Control & Both Friends and Wearers preferred Wearers to have complete control over what was shared. & Consider using multiple, complementary techniques to give Wearers control --– from allowing them to invite selected friends only, to switch sharing modes anytime, and to reject or approve each trigger request. \\
% \hline
% Screenlessness & Many participants preferred the spontaneity of having no screen. 
% & Consider embracing screenlessness. Not having a preview can support spontaneous, low-stakes communication by preventing users from polishing their output. \\

%  & Friends who wished the system had a screen wanted to use it for mostly low-fidelity responses.
% & Bidirectional interaction between friends is important, but consider keeping things simple even if the form factor allows higher fidelity.  For instance, emojis or icons may be sufficient or preferred over text or photo responses for many. \\

% \bottomrule
% \end{tabular}
% }
% \end{table}




% \newpage

% \subsubsection{Gathering information in a self-directed manner}
% % Our participants described wanting to gather information about the environment themselves, i.e., in a self-directed manner. 
% All our participants (n=12) shared their experiences of exploring environments using their non-visual senses, enabling them to actively engage with the environment and thereby build more robust mental maps~\cite{chrastil2013active, chrastil2012active}. Furthermore, our participants expressed a sense of independence in their ability to explore the environment on their own~\cite{lee2021designingIndependence}. 

% % James recalls visiting a shopping mall in his neighbourhood, describing how he uses a combination of echolocation and tactile feedback from the white cane to gather shape information of the mall entrance. \vspace{-0.25cm}\\\\
% % \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
% %  & %
% %  \textit{``[At the mall,] echolocation can tell me some things about the shape, but I want specifics. So, I will go to each side of the entrance and check how big the entrance is, and then I can learn that there are two large openings from this foyer.''} -James 
% %  & \\
% % \end{tabu}
% % \\\\
% % However, participants agreed that it is challenging to gather information in a self-directed manner using their non-visual senses. Our participants cited three main reasons. 

% First, information collected in this manner is not robust enough for participants to reliably make navigation decisions. Charles had concerns about relying on the shape information gathered through echolocation and resorts to seeking confirmation from others. Similarly, Leo noted a specific example of using olfactory cues as merely supplemental information. \vspace{-0.25cm}\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{``That's usually not my first priority. That's more maybe just providing some supplemental information. I would not say that that's something that I rely on in any capacity.''} -Leo
%  & \\
% \end{tabu}\\\\
% Second, some participants (n=4) indicated that while tactile feedback is more reliable, it is challenging to apply this brute force technique to larger spaces such as airports, department stores, and shopping complexes. Such an approach doesn't scale well. 
% Third, few participants (n=3) also noted that presence of other people in the environment made it challenging for them to explore environments. Charles indicated concerns about hitting people with his cane in crowded places, while Olivia expressed fear of knocking objects off in front of others. Harper echoed the sentiment, stating that some behaviors are simply inappropriate in a public setting, making it extremely challenging to independently explore environments. \vspace{-0.2cm} \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & %
%  \textit{``I mean, if you're somewhere by yourself, you could explore anything. But when you're in a public setting, people are really gonna look at you strangely if you get up at a restaurant and start walking around and feeling all the tables.''} -Harper
%  & \\
% \end{tabu}
% \vspace{-0.4cm}\\\\






% \begin{center}
% \fbox{\begin{minipage}{0.5\textwidth}
% \textbf{Insight 3}: Self-directed exploration... 
% \end{minipage}}
% \end{center}
% \vspace{1mm}


% VIPs' confidence in their O\&M skills is one of the most crucial elements to their sense of independence~\cite{hersh_mental_2020}. Many of our participants (n=4) acknowledged the importance of O\&M skills in their lives and described how these techniques empower them with autonomy. James explains that O\&M skills are \textit{``vital because the world will walk over you if you don’t take control of your own abilities''} and further emphasizes its role in gaining control of one's life: \textit{``people will tell you where you can go and what you can do. And if you don't know how to do those things, then you're just kind of meekly following along. It's self esteem shattering.''}

% As P4 explained:  \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{“[O\&M skills are] vital because the world will walk over you if you [don’t] take control of your own abilities. [...] People will tell you where you can go and what you can do[.] And if you don't know how to do those things, then you're just kind of meekly following along. It's self esteem shattering, [and] reduces your individuality.”} - \textbf{P4} & \\
% \end{tabu} \\\\


% Given the immense importance O\&M skills in VIPs' lives, we asked our participants about the extent to which they are comfortable in exploring unfamiliar environments using their O\&M skills. We discovered that almost all our participants are not confident in their current proficiency of O\&M skills to explore unfamiliar environments independently. We found that many participants (n=7) acknowledged their insufficiency and attributed it to the lack of access to good O\&M training. While the remaining participants (n=5), who self-reported as receiving appropriate amount of O\&M training, expressed some doubts in their abilities and attributed it to the lack of opportunities to practice O\&M skills on a daily basis.   


% Below, we describe challenges faced by VIPs in learning and maintaining O\&M skills, which is crucial to VIPs' ability to explore unfamiliar environments.

% Many participants (n=5) described wanting a more comprehensive O\&M training. We  

% A sizeable number of participants (n=5) reported that they have received only limited O\&M training in their lives. Upon further inquiry, we identified three main factors that hinder VIPs' access to adequate O\&M training:



% \textbf{Learning O\&M skills.} 
% A sizeable number of participants (n=5) reported that they have received only limited O\&M training in their lives. Upon further inquiry, we identified three main factors that hinder VIPs' access to adequate O\&M training: 
% \begin{itemize}
%     \item[(i)]\text{Onset of vision impairments}: Most of our participants (n=7) who developed vision impairments earlier in life or are blind by birth, reported easy access to O\&M instructors via their schools, as a child. On the other hand, participants (n=3) who developed vision impairments later in life described challenges in arranging for one. Furthermore, many participants (n=6) stated that it much more difficult to set up an O\&M session as an adult, compared to when they were in school. For instance, Nora (who is blind by birth) explains:\vspace{-0.25cm}\\\\
%         \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%          & \textit{``For earlier years, I didn't need to reach out to O\&M instructors because that's something, that like, we automatically get in schools. Now, [as an adult,] I definitely would have to advocate for myself''.} -Nora & \\
%         \end{tabu}
%         \\\\
%     As a result, most of Nora's O\&M training was done during her K-12 education.\vspace{0.2cm}
    
%     \item[(ii)] \text{Lack of access to O\&M instructors}: Some of our participants (n=2), despite being blind by birth and being assigned an O\&M instructor, did not receive appropriate training. Our follow up interviews with the leaders of blind-serving organization and the O\&M instructors revealed that this is primarily due to shortage of O\&M trainers and decentralization. Both the leaders and the instructor confirmed that O\&M instructors are assigned multiple students scattered over a geographical area, which makes it difficult for them to be physically present and provide enough time to all their students. As a result, many VIPs miss out on the appropriate amount of O\&M training they are promised. For instance, Charles, who was assigned an O\&M instructor during middle school explains that he never received formal O\&M training, despite his belief that it would have benefited him. \vspace{-0.25cm}\\\\
%         \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%         & \textit{``I was told that I would get an O\&M trainer back in middle school. [...] I never received that trainer. She came in once within the six years she was supposed to be training me.''} -Charles & \\
%         \end{tabu}
%         \vspace{-0.4cm}\\
        
%     \item[(iii)] \text{Lack of funding}: Most of our participants (n=9) reported being dependent upon their respective states to receive O\&M training or other accessibility services or devices. Few participants (n=2) noted that their access to O\&M training in the past has been affected due to shortage of state funding. Lucas explains that adult VIPs in his state are only provided vocational rehabilitation training, which is a form of training meant only to provide necessary skills to a VIP so that they can perform a specific job. However, as Lucas further notes, even this type of training was scarce, and VIPs have to prove their employment status in order to receive it. \vspace{-0.25cm}\\\\
%         \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%          & \textit{``It's just very hard to get O\&M training here because [anonymized state] is out of money. [...] It's very hard [because] you've got to prove that you’re working.''} -Lucas & \\
%         \end{tabu}
%         \vspace{-0.4cm}\\
% \end{itemize}
 
 
 % Descriptions from the VIP friend not only matched Nora's perception of space, but also included other relevant details that Nora found important or useful. In fact, all VIP participants (n=8) almost always prefer to ask for descriptions from their friends who are visually impaired over non-VIP peers. All VIP participants (n=8) also reported that non-VIPs often struggle to match their descriptive preferences, leaving them frustrated. 






% We further found that despite these preferences, VIPs are often offered inappropriately excessive assistance.
% For example, James described an instance when non-VIPs have forced wheelchair service onto him out of ignorance:\\\\
% \vspace{0.2cm}
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{“[Airport staff are] relatively good at adapting [to our needs] usually, but the very first thing they always do [when they assist you] is they give you a wheelchair, and [some staff] insist that you use it." } - \textbf{James} & \\
% \end{tabu}
% \vspace{0.2cm} \\
% While wheelchair service might be more convenient, it does not match James's preference for autonomy, specifically in that it assumes and reinforces a passive role instead of promoting exploration. VIPs often prefer to receive information from others, instead of sighted guidance.
% In fact, excessive assistance in this case was not only unnecessary but also demeaning to James. James explained that while he understood their actions were due to inadequate training, he still felt uncomfortable being forced to accept a type of assistance that overemphasized his level of disability and ignored his preferences.
% In short, we learned that VIPs often just want information from non-VIPs instead of being guided. \\


% Participants described challenges in supervising the form of assistance, where they preferred a more loose form of collaboration when exploring environments. More specifically, we found that VIPs prefer receiving verbal information during collaborative exploration which is in contrast with how VIPs would not mind a more guided form of assistance when navigating to a specific destination.

% Many participants (n=3) noted that while it was relatively straight forward to moderate assistance for reaching a specific destination, supervising assistance for exploration was challenging. More specifically, we found that when receiving help from others VIPs preferred to get verbal information and then preferred to figure things out on their own, when exploring unfamiliar environments. This is in contrast with how participants wanted to reach their destination



% that VIPs prefer that others give them verbal directions only rather than escort them to their destination.



% Supervising help from other people meant several things: safety, getting the useful information, and above all, a sense of control and independence which is important to VIPs.


% \textbf{Avoid Getting Guided After Asking for Information.}
% We found that some VIP participants (n=4) strongly prefer that others give them verbal directions only rather than escort them to their destination.
% Nearly half (n=3) of our VIP participants reported that they avoid sighted guide assistance in most situations because the guides will be too helpful, and instead opt to use their O\&M skills to actively navigate to their destination despite the inconvenience. 

% We further found that despite these preferences, VIPs are often offered inappropriately excessive assistance.
% For example, James described an instance when non-VIPs have forced wheelchair service onto him out of ignorance:\\\\
% \vspace{0.2cm}
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{“[Airport staff are] relatively good at adapting [to our needs] usually, but the very first thing they always do [when they assist you] is they give you a wheelchair, and [some staff] insist that you use it." } - \textbf{James} & \\
% \end{tabu}
% \vspace{0.2cm} \\
% While wheelchair service might be more convenient, it does not match James's preference for autonomy, specifically in that it assumes and reinforces a passive role instead of promoting exploration. VIPs often prefer to receive information from others, instead of sighted guidance.
% In fact, excessive assistance in this case was not only unnecessary but also demeaning to James. James explained that while he understood their actions were due to inadequate training, he still felt uncomfortable being forced to accept a type of assistance that overemphasized his level of disability and ignored his preferences.
% In short, we learned that VIPs often just want information from non-VIPs instead of being guided. \\

% \begin{center}
% \fbox{\begin{minipage}{0.5\linewidth}
% \textbf{Insight 3}: There is a mismatch between type and amount of information provided by non-VIPs and VIPs' preferences for them. 
% \end{minipage}}
% \end{center}
% \vspace{2mm}


% \textbf{Get Information in a Comprehensible Format.}


% We found that VIPs often struggle to receive information for navigating independently such as directions or room descriptions from non-VIPs, and that they struggle because the information they get requires vision to understand or interpret.

% MAY BE ADDED IF NEEDED, BUT I DON'T THINK THIS EXAMPLE CORRESPONDS TO SPATIAL INFORMATION.
% For example, Nora reported a time when a description from a non-VIP caused confusion: \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{"Sometimes there will be [situations] where [a non-VIP tells me], ‘Oh, [the place I’m looking for is] the third door.’ [...] But there's a storage room [next to the classroom]. [I didn’t know] they d[id]n't count that as a door or a room."} - \textbf{Nora} & \\
% \end{tabu}
% \vspace{0.2cm} \\\\
% While the presence of a fourth door may have been trivial to the non-VIP, providing this detail proved to be necessary for Nora to adequately understand the space.




% As another example, James states that he finds it difficult to understand the shape and layout of an environment based on non-VIP's descriptions. 
% He explained:\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{"[I need to ask for clarification] because a lot of people describe [shapes with letters] like `U' shaped or `H' shaped. I know what U shaped is, but sometimes I forget what H shaped means[.] I just prefer geometric shapes [for descriptions.]"} - \textbf{James} & \\
% \end{tabu}
% \vspace{0.2cm} \\\\
% Non-VIPs often utilize visual details when describing a space. 
% As James explained, however, this is not always applicable to VIPs. 
% In fact, we found that VIPs often prefer non-visual descriptions for navigation, such as describing how the floor texture changes from one location to another.


% Last, our VIP participants expressed that they often need details beyond the presence of POIs and landmarks to successfully navigate a space, especially if they are visiting a place independently. These additional details include the presence of other accessibility features or notes of caution. 
% In short, we learned that a major challenge hampering VIPs' ability to explore is ensuring that VIPs can get information from non-VIPs communicated to them in a way that they can interpret without vision. \\
% % 
% \begin{center}
% \fbox{\begin{minipage}{0.5\linewidth}
% \textbf{Insight 4}: Non-VIPs' perception of spaces differ from that of VIPs, 
% which causes a barrier to VIPs receiving verbal instructions or directions from non-VIPs. 
% \end{minipage}}
% \end{center}
% \vspace{1mm}








% Non-VIP staff have difficulty determining whether or not to give assistive information to a VIP, and they often opt to not interfere out of fear that they may act in a socially unacceptable manner or get in trouble due to some company policies. 
% In short, we find that social pressures can negatively impact both the frequency and quality of exploration information that VIPs receive. As a result, minimizing the social tensions that non-VIP helpers face is integral for VIPs to receive effective navigational information from them.\\



% We discovered that this discomfort stems from their fear of not being able to help them in the right manner or for getting in trouble due to company policies regarding this. \vspace{-0.25cm}\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{``I'm always concerned with invading somebody's personal space or [disregarding] their bodily autonomy.''} -Grocery store employee & \\
% \end{tabu}
% \\\\
% Both Daniel and Emily shared their experiences doing grocery shopping. Daniel told us that he usually orders online


% doesn't fit here as much.
% Emily, who lives in a small city, shares her experience with the change in management at her grocery store near her house. Earlier, she knew everyone in the store so it was easy for her to get help, but with the new management in place, she finds herself not going their often because of how the management feels about catering to her special needs. MAY INSERT QUOTE IF NEEDED.



% VIPs expressed that another aspect of why getting information from others is challenging is the fact that non-VIPs often face social pressure from others whenever they are helping VIPs, even if it is just to provide information or directions.


% \textcolor{magenta}{Add: Guidance (A->B) is easier in the sense that you can ask simple questions, and get to the destination. However, when exploring environments, it is very different: (1) requires more time because you don't have anything specific in your mind; (2) more socially anxious because it takes more time, you feel like people are watching you and that is very inconvenient; (3) you cannot touch everything (that's the only way to explore) which is even more socially uncomfortable because you cannot touch something you do not know. }


% We observed that this feeling applies even when VIPs receive assistance from their friends and/or family. 
% For example, James said:\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{“I know that my sister gets looks from people all the time [when she acts as my sighted guide], because of foolish assumptions they make out of ignorance. [People think] that she is my caretaker, [and that] anything that they perceive as her not doing her job is wrong.”} - \textbf{James} & \\
% \end{tabu}
% \vspace{0.2cm} \\\\
% He added that it is for this reason that he prefers receiving help information from professionals, such as O\&M instructors, as he feels less guilt towards having to subject them to such "embarrassment." It is clear from participants' remarks that social pressures are preventing VIPs from utilizing the full potential of non-VIP information available to them.

% Hi YY! How's it going? 
% hello :)

% In addition, our interviews with business staff confirmed that non-VIPs feel social pressure when offering help to VIPs.
% For example, the grocery store employee reported their difficulty determining whether or not they should offer help information to VIPs they see: \\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{“I'm always concerned with invading somebody's personal space or [disregarding] their bodily autonomy. So I think it's a matter of just trying to be cognizant [...] if somebody seems like they need help [or] if somebody seems like they are totally fine. [It] is not a perfect system, obviously, [and] mistakes will be made.”} - \textbf{Grocery store employee} & \\
% \end{tabu}
% \vspace{0.2cm} \\\\

% Furthermore, the grocery store employee expressed some social anxiety while helping VIP customers. As the employee explains, for him it was due to the company policies and lack of training.\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{“[My manager] said, if you need to help a customer [...] who's disabled, definitely try to. If they give you consent that you can drive my wheelchair, or you can grab my arm [...] Just be careful in that case, if they do say you can. But if they don't say anything, then you shouldn't do anything. Because you don't want to, you know, actually causing issues where they say, `oh, why are you touching me'?”} - \textbf{Grocery store employee} & \\
% \end{tabu}
% \vspace{0.2cm} \\\\





% \begin{center}
% \fbox{\begin{minipage}{0.5\linewidth}
% \textbf{Insight 5}: Social pressure prevents VIPs from receiving and non-VIPs from providing useful information.
% \end{minipage}}
% \end{center}
% \vspace{2mm}


% \textcolor{magenta}{Nice quote from Paige about: how some people get frustrated when they ask too many questions. Eventually, they've learned to say sorry for now reason, and that is something they don't like. This could be used to motivate why NASs can play a better role (than people), and hence motivate the translation vision.}




% Participants reported a significant drop in their O\&M proficiency without regular use, and that too in challenging environments. 

%  Thus, it is important that VIPs make use of their O\&M skills on a regular basis and incorporate them for everyday navigation activities.
% Many of our participants (n=4) acknowledged the importance of O\&M skills in their lives and described how these techniques empower them with independence and autonomy during navigation. 
% As P4 explained:  \\\\

% P4 further elaborated that he even denies assistance out of fear of his skills deteriorating if he relied too much on sighted assistance:\\\\
% \begin{tabu} to \linewidth { X[l] X[28l] X[l]}
%  & \textit{"It is very easy to let your [O\&M] skills atrophy as a blind person if you rely overly on sighted people and it's an easy trap to fall into. It's easy to [use a] sighted guide and become complacent and [not pay attention to] what turns you have taken and where you are in relation to other things." } -James & \\
% \end{tabu}
% \vspace{0.2cm} \\\\
% While P4 knows that taking advantage of any assistance offered may be immediately convenient, he also understands that it may harm his ability to be independent in the long run.
% % by deteriorating the skills that he needs to explore the space on his own.
% Several of our participants (n=3) share this sentiment and prefer to use their O\&M skills as much as possible, denying sighted assistance whenever they can.  
% As O\&M skills are crucial for VIPs to remain independent, there is an opportunity for NASs to promote exploration by providing a means of maintaining these skills and preventing them from deteriorating. \\



% \textit{``Yeah, so I don't think once a week is enough training, that's why I'm I already applied for a training centre that focuses on mobility and you'll be taking a mobility class every day and they blindfold you and they make you cross streets and I'm like, I need that because that will really push me out of my comfort zone and that will give me the confidence I need to cross any street.''} -Grace



% Not using the O\&M skills may lead to loss of skills. One of our participants (Harper) is a living example of this -





% NASs can help support both O\&M instructors and VIPs by acting as virtual O\&M assistants to allow VIPs practice and learn regularly. 



% \begin{center}
% \fbox{\begin{minipage}{0.5\textwidth}
% \textbf{Insight 5}: Participants face difficulties in maintaining their O\&M skills due to lack of opportunities to practice safely, and hence lack the confidence to explore independently.
% \end{minipage}}
% \end{center}
% \vspace{1mm}


==> 5-Design Guidelines/v1.tex <==
The new prospect for future NASs is to empower VIPs' active engagement abilities, detailed in our findings. We applied qualitative coding to our findings in order to understand how VIPs engage with different layers of information in their active engagement behaviors, and how NAS design can support and augment those behavioral needs in those layers. The qualitative coding revealed three layers of technological design: Information, Representation of Information and Human-Computer Interaction. In each layer, active engagement abilities inspire a new light of thinking, and calls for a new set of system design guidelines.  

\subsection{Information Collection}

\subsubsection{\textbf{DG-1: Types of Information}}
Active engagement navigation technology must collect types of information aligned with VIPs’ sensory and perceptual abilities. These types of information would be instrumental to help VIPs activate their spatial awareness and stay actively engaged with indoor environments. Existing guidance navigation systems focus on route-planning via waypoints, underrepresenting VIPs' needs in collecting geometric and non-visual information of the space.

\textit{Geometric Information of Space}. 
Indoor environments are outlined by boundaries. The geometric shape of the boundaries help set a foundational layer for mental maps. VIPs learn the shape of a space by either asking for verbal descriptions of the shape, which are usually inaccurate, or by slowly tracing their hands along the walls, which is time-consuming. Additionally, VIPs benefit from learning the objective and accurate counts of physical geometries in space, such as the number of doors or steps. There is an opportunity for technology to collect and display the geometric information of spaces accurately and efficiently.

\textit{Non-Visual Information.}
Due to the lack of visual information, non-visual information becomes the building blocks for VIPs’ spatial awareness. Non-visual information includes ambient sounds, touch of texture, temperature, air current, echolocation, smell and more. VIPs engage a tremendous amount of mental effort in capturing useful non-visual information. There is an opportunity for technology to collect non-visual information and augment VIPs’ sensory abilities. 

\subsubsection{\textbf{DG-2: Characteristics of Landmarks}} 
Active engagement navigation technology ought to collect spatial landmarks that are essential components of VIPs mental maps. VIPs’ landmarks are different from objective waypoints and destination points of interest on navigation maps. Rather, VIPs’ landmarks should be designed for storing and recognizing local features helpful for spatial memory and orientation. Therefore, the useful spatial landmarks for active engagement are composed of non-visual information, fluid in time contexts, and must be verifiable by VIPs sensory abilities. 

\textit{Landmarks are multi-sensory information.}
A landmark is only recognizable [to VIPs?] when multiple pieces of sensory information are present at the same time. For example, an air-conditioning unit is perceived by the collection of cold air flow, the fan blade noise and the engine vibration. It is important for technology to collect all pieces of information in support of a recognizable landmark.

\textit{Landmarks are fluid.}
A landmark could perform differently during different times of the day. For example, the bakery landmark might only emit a fresh smell of bread and warmth from the oven in the morning but not in the evening. It is important for technology to collect the fluid contextual characteristics matching the particular landmark.

\textit{Landmarks are verifiable by VIPs.}
In order to promote active engagement with the environment, the information provided by technology must be verifiable by VIPs with their sensory abilities. Technology should take a supporting role rather than a leading / guiding role. Verifiable information is key to building VIPs' confidence and independence in active engagement, rather than to replacing their abilities with reliance on technology. 

\subsection{Information Representation}

\subsubsection{\textbf{DG-3: Organization of Information}}
Active engagement navigation technology ought to represent the geometric and non-visual information aligned with VIPs’ perceptual abilities. VIPs organize spatial information to compose their mental map, and correlate non-visual landmarks to orient themselves to the locations in the mental map. Technological design should align the organization of information with VIPs' cognitive processes, in order to augment their abilities in orienting and exploring through active engagement with environments.


\textit{Organize Geometric Shapes to Form Maps.}
Geometric information of spaces are useful for mental map building, however, indoor environments often are complex in shapes, containing multiple interconnected spaces and rooms linked by connection landmarks: doorways, stairs, elevators, etc. It is important for technology to organize the shapes of spaces along with the connection landmarks in a readable format by VIPs. The organization of geometric maps should support active reading or surveying by VIPs.


\textit{Organize Non-visual Information to Reinforce Maps.}
Due to the multi-sensory and fluidity characteristics of non-visual landmarks, it is crucial for technology to pertain these characteristics and to organize them in correspondence with the geometric map. Each location on a geometric map is characterized by multiple landmarks in multiple modalities. With landmarks being fluid in time, technology should weigh their presence likelihood and determinative order in supporting the recognition of the location. [just say that having redundant multi-modal landmarks can help make recognition better. Based on context, for example time of the day in the bakery example, NASs should weigh confidence on each landmark in order to localize themselves on the map.]



\subsubsection{\textbf{DG-4: Interpretation of Information}}
When VIPs try to make use of spatial information offered by non-VIPs, there is often a mismatch between sensory modalities, making the information inaccurate or unperceivable for VIPs. There is an opportunity for technology to mediate the differences and interpret the information to achieve usefulness to VIPs.

\textit{Translate visual information to non-visual information.}
Non-VIPs intuitively describe the environment with visual information, however, it needs to be translated to non-visual information for VIPs. For example, non-VIPs may describe a pot of flowers by its colors, while VIPs perceive them by its smell. There is an opportunity for technology to make cross-modality information translation with artificial intelligence, such that information communicated by non-VIPs can also support VIPs in their active engagement with environments. 


\textit{Verify and complete non-VIP provided information.}
Information provided by non-VIPs often contains unintentional bias, which need to be verified and completed for VIPs. For example, non-VIPs may omit a storage door when giving directions by the count of doors. Non-VIPs may give a generic shape using a letter form metaphor while VIPs would need a more detailed geometric description. There is an opportunity for technology to verify and complete the information provided by non-VIPs, such that the information is accurate and with the appropriate level of details for VIPs usefulness.


\subsection{Agency in Interaction and Skill-building}

\subsubsection{\textbf{DG-5: Active Agency with Help}}
Active engagement navigation technology should facilitate active agency in VIPs toward others in requesting and receiving help information. (From findings) Caused by current social unawareness toward visual impairments, there is a mismatch between VIPs’ abilities and non-VIPs’ expectations [of what], and a mismatch between VIPs’ needs and non-VIPs’ offers of assistance. There is an opportunity for technology to combat this imbalance by giving VIPs the active agency in requesting ability-based assistive information, and exact level of needed information.  

\textit{Signal Abilities, not Disabilities.} 
Help offered to VIPs often magnify their disabilities and ignore their abilities. There is an opportunity for technology to combat this prejudice by masking VIPs disabilities, and signal their abilities associated with help requests. Giving VIPs active agency in requesting information matching their abilities, technology has the potential to promote social identity equality between VIPs and non-VIPs.

\textit{Request Transactional Help, Reject Unwanted Help.}
Help available to VIPs is often more than they need causing reliance [on sighted people], or less than what they need causing burden. There is an opportunity for technology to facilitate exact transactional help requests, by giving VIPs the active agency in the request and by informing non-VIPs the precise needs.

\subsubsection{\textbf{DG-6: Active Agency with Education}}
Ultimate aim: No reliance on the system FOR EXPLORATION (self-exploration is key, or independent exploration w/o the system) -- Enable creating / deciding their own routes based on mental map that they create during exploration
To achieve this: Nudge towards cognitive improvements / skill building. NASs should serve as educational tools, that help build O\&M skills, and attention capabilities toward non-visual information



% So many points. how to consolidate to 2-3 points more logically ?

% % Discover and add their own sensory landmarks to the layout map 
% Self-orient and self-explore with proper-agency help from the system 
% Learning with optimized cognitive demand 
% Less clutch feedback as skills go up
% Nudge towards cognitive improvements / skill building
% doable for an active VIP, and they still get the feeling that they did it.
% Passive VIPs have this doable threshold set extremely low. Over time, this should go up. 
% Move from passive to active behavior
% Enable creating / deciding their own routes based on mental map
% % Maintain non-visual skills not to atrophy
% Build confidence in safety and autonomy
% No reliance on the system


==> 5-Design Guidelines/v2.tex <==
The new prospect for future NASs is to empower VIPs' exploration in navigation, detailed in our findings. We applied qualitative coding to our findings in order to understand how VIPs engage with different layers of information in their exploration behaviors, and how NAS design can support and augment those behavioral needs in those layers. Our analysis revealed three layers of technological design: Information Collection, Representation of Information and Agency in Interaction and Skill-building. In each layer, exploration abilities inspire a new light of thinking, and calls for a new set of system design guidelines.  

\subsection{Information Collection}

\subsubsection{\textbf{DG-1: Types of Information}}
Exploration NASs must collect types of information aligned with VIPs’ sensory and perceptual abilities. These types of information would be instrumental to help VIPs activate their spatial awareness and stay actively engaged with indoor environments. Existing turn-by-turn NASs focus on route-planning via waypoints, underrepresenting VIPs' needs in collecting geometric and non-visual information of the space.

\textit{Geometric Information of Space}. 
Indoor environments are outlined by boundaries. The geometric shape of the boundaries help set a foundational layer for mental maps. VIPs learn the shape of a space by either asking for verbal descriptions of the shape, which are usually inaccurate, or by slowly tracing their hands along the walls, which is time-consuming. Additionally, VIPs benefit from learning the objective and accurate counts of physical geometries in space, such as the number of doors. There is an opportunity for technology to collect and display the geometric information of spaces accurately and efficiently.

\textit{Non-Visual Information.}
Due to the lack of visual information, non-visual information becomes the building blocks for VIPs’ spatial awareness. Non-visual information includes ambient sounds, touch of texture, temperature, air current, echolocation, smell and more. VIPs engage a tremendous amount of mental effort in capturing useful non-visual information. There is an opportunity for technology to collect non-visual information and augment VIPs’ sensory abilities. 

\subsubsection{\textbf{DG-2: Characteristics of Landmarks}} 
Active engagement navigation technology ought to collect spatial landmarks that are essential components of VIPs mental maps. VIPs’ landmarks are different from objective waypoints and destination points of interest on navigation maps. Rather, VIPs’ landmarks should be designed for storing and recognizing local features helpful for spatial memory and orientation. Therefore, the useful spatial landmarks for active engagement are composed of non-visual information, fluid in time contexts, and must be verifiable by VIPs sensory abilities. 

\textit{Landmarks are multi-sensory information.}
A landmark is recognizable to VIPs when multiple pieces of sensory information are present at the same time. For example, an air-conditioning unit is perceived by the collection of cold air flow, the fan blade noise and the engine vibration. It is important for technology to collect all pieces of information in support of a recognizable landmark.

\textit{Landmarks are fluid.}
A landmark could perform differently during different times of the day. For example, a bakery may act as a landmark,  might only emit a fresh smell of bread and warmth from the oven in the morning but not in the evening. It is important for technology to collect the fluid contextual characteristics matching the particular landmark.

\textit{Landmarks are verifiable by VIPs.}
In order to promote active engagement with the environment, the information provided by technology must be verifiable by VIPs with their sensory abilities. Technology should take a supporting role rather than a leading / guiding role. Verifiable information is key to building VIPs' confidence and independence in active engagement, rather than to replacing their abilities with reliance on technology. 

\subsection{Information Representation}

\subsubsection{\textbf{DG-3: Organization of Information}}
Active engagement navigation technology ought to represent the geometric and non-visual information aligned with VIPs’ perceptual abilities. VIPs organize spatial information to compose their mental map, and correlate non-visual landmarks to orient themselves to the locations in the mental map. Technological design should align the organization of information with VIPs' cognitive processes, in order to augment their abilities in orienting and exploring through active engagement with environments.


\textit{Organize Geometric Shapes to Form Maps.}
Geometric information of spaces are useful for mental map building, however, indoor environments often are complex in shapes, containing multiple interconnected spaces and rooms linked by connection landmarks: doorways, stairs, elevators, etc. It is important for technology to organize the shapes of spaces along with the connection landmarks in a readable format by VIPs. The organization of geometric maps should support active reading or surveying by VIPs.


\textit{Organize Non-visual Information to Reinforce Maps.}
Due to the multi-sensory and fluidity characteristics of non-visual landmarks, it is crucial for technology to pertain these characteristics and to organize them in correspondence with the geometric map. Each location on a geometric map is characterized by multiple landmarks in multiple modalities. With landmarks being fluid in time, technology should weigh their presence likelihood and determinative order in supporting the recognition of the location. [just say that having redundant multi-modal landmarks can help make recognition better. Based on context, for example time of the day in the bakery example, NASs should weigh confidence on each landmark in order to localize themselves on the map.]



\subsubsection{\textbf{DG-4: Interpretation of Information}}
When VIPs try to make use of spatial information offered by non-VIPs, there is often a mismatch between sensory modalities, making the information inaccurate or unperceivable for VIPs. There is an opportunity for technology to mediate the differences and interpret the information to achieve usefulness to VIPs.

\textit{Translate visual information to non-visual information.}
Non-VIPs intuitively describe the environment with visual information, however, it needs to be translated to non-visual information for VIPs. For example, non-VIPs may describe a pot of flowers by its colors, while VIPs perceive them by its smell. There is an opportunity for technology to make cross-modality information translation with artificial intelligence, such that information communicated by non-VIPs can also support VIPs in their active engagement with environments. 


\textit{Verify and complete non-VIP provided information.}
Information provided by non-VIPs often contains unintentional bias, which need to be verified and completed for VIPs. For example, non-VIPs may omit a storage door when giving directions by the count of doors. Non-VIPs may give a generic shape using a letter form metaphor while VIPs would need a more detailed geometric description. There is an opportunity for technology to verify and complete the information provided by non-VIPs, such that the information is accurate and with the appropriate level of details for VIPs usefulness.


\subsection{Agency in Interaction and Skill-building}

\subsubsection{\textbf{DG-5: Active Agency with Help}}
Active engagement navigation technology should facilitate active agency in VIPs toward others in requesting and receiving help information. (From findings) Caused by current social unawareness toward visual impairments, there is a mismatch between VIPs’ abilities and non-VIPs’ expectations [of what], and a mismatch between VIPs’ needs and non-VIPs’ offers of assistance. There is an opportunity for technology to combat this imbalance by giving VIPs the active agency in requesting ability-based assistive information, and exact level of needed information.  

\textit{Signal Abilities, not Disabilities.} 
Help offered to VIPs often magnify their disabilities and ignore their abilities. There is an opportunity for technology to combat this prejudice by masking VIPs disabilities, and signal their abilities associated with help requests. Giving VIPs active agency in requesting information matching their abilities, technology has the potential to promote social identity equality between VIPs and non-VIPs.

\textit{Request Transactional Help, Reject Unwanted Help.}
Help available to VIPs is often more than they need causing reliance [on sighted people], or less than what they need causing burden. There is an opportunity for technology to facilitate exact transactional help requests, by giving VIPs the active agency in the request and by informing non-VIPs the precise needs.

\subsubsection{\textbf{DG-6: Active Agency with Education}}
Ultimate aim: No reliance on the system FOR EXPLORATION (self-exploration is key, or independent exploration w/o the system) -- Enable creating / deciding their own routes based on mental map that they create during exploration
To achieve this: Nudge towards cognitive improvements / skill building. NASs should serve as educational tools, that help build O\&M skills, and attention capabilities toward non-visual information



% So many points. how to consolidate to 2-3 points more logically ?

% % Discover and add their own sensory landmarks to the layout map 
% Self-orient and self-explore with proper-agency help from the system 
% Learning with optimized cognitive demand 
% Less clutch feedback as skills go up
% Nudge towards cognitive improvements / skill building
% doable for an active VIP, and they still get the feeling that they did it.
% Passive VIPs have this doable threshold set extremely low. Over time, this should go up. 
% Move from passive to active behavior
% Enable creating / deciding their own routes based on mental map
% % Maintain non-visual skills not to atrophy
% Build confidence in safety and autonomy
% No reliance on the system


==> 5-Design Guidelines/v3.tex <==
\label{sec:DGs}
The new prospect for future NASs is to support VIPs’ exploration in navigation, detailed in our findings. We applied qualitative coding to the findings in order to understand how VIPs engage with different layers of information in their exploration behaviors, and how NAS design can support and augment those behavioral needs. 

Our analysis reveals new perspectives in all three layers of NAS design: \textit{Information Collection, Information Representation and Agency in Requesting and Skill-Building}. The first layer, Information Collection, provides guidelines on how NASs should collect raw information from the environment for exploration. The second layer, Information Representation, builds upon the first layer and provides guidelines on how the NASs should represent the collected raw information to VIPs. The third layer, Agency in Requesting and Skill-Building, addresses interaction with aforementioned information and provides guidelines on how agency should be allocated when people and NASs interact with the exploration information. In each layer, VIPs' exploration behaviors inspire a new light of thinking, and calls for a new set of design guidelines.

\subsection{Information Collection}

Spatial information that supports VIPs' exploration of environments differs from that of guidance. We provide guidelines on the specific types of information and characteristics of landmark information that are useful in supporting exploration and should be collected by NASs. 

\noindent\textbf{DG-1: NASs must collect the types of information used during VIPs’ exploration, including geometric information of space and non-visual information.}


NASs must collect the types of information used by VIPs during their exploration of the environment. The types of information must align with VIPs’ sensory and perceptual abilities. They are instrumental to help VIPs pay attention and collect spatial information as they explore the indoor environment. Existing turn-by-turn NASs provide directional cues to the next waypoints; however, they do not support the exploration of the environment, which requires geometric and non-visual information about the space.


\textit{Geometric Information Of Space.} Indoor environments are outlined by boundaries. The geometric shape of the boundaries help set a base layer for mental maps. VIPs may learn the shape of a space by asking for verbal descriptions, which are usually inaccurate. They may also learn the shape of a space by slowly tracing along the walls using their tactile senses, which is time consuming, especially for large spaces. Additionally, VIPs benefit from learning the objective and accurate counts of physical geometries in space, such as the number of doors. There is an opportunity for NASs to collect and display the geometric information of spaces accurately and efficiently. 

\textit{Non-Visual Information.}
Due to the lack of visual information, non-visual information becomes the building blocks for VIPs’ spatial exploration and mental maps. Non-visual information includes ambient sounds, textures, temperature, air current, echolocation, smell, and more. VIPs must use a huge amount of mental effort to capture useful non-visual information. There is an opportunity for NASs to collect non-visual information and augment VIPs’ sensory abilities.  

\noindent\textbf{DG-2: NASs must collect VIPs’ spatial landmark information including multisensory, dynamic and VIP-verifiable characteristics.}

NASs must collect spatial landmarks that are essential components of VIPs' mental maps. VIPs’ landmarks are different from turn-by-turn waypoints and destinations in guidance-based navigation. Rather, VIPs’ landmarks should be designed for storing and recognizing local features helpful for spatial exploration, orientation and memory. Therefore, the useful spatial landmarks for exploration are composed of non-visual multisensory information, fluid in time contexts, and must be verifiable by VIPs sensory abilities.

\textit{Landmarks Must Be Multisensory.}
A landmark is recognizable to VIPs when multiple pieces of sensory information are present at the same time. For example, an air-conditioning unit is perceived by the collection of cold air flow, the fan blade noise and the engine vibration. It is important for NASs to collect all pieces of information in support of a recognizable landmark. 


\textit{Landmarks Must Be Fluid.} 
A landmark could present itself differently during different times of the day. For example, a bakery may act as a fluid location landmark, and it emits a fresh smell of bread and warmth from the oven in the morning but not in the evening. It is important for NASs to collect the fluid contextual characteristics matching the particular landmark.  


\textit{Landmarks Must Be Verifiable by VIPs.}
In order to enable VIP’s independent exploration of the environment, the information provided by NASs must be verifiable by VIPs with their sensory abilities. NASs should take a supporting role rather than a directing role. Verifiable information is key to building VIPs’ confidence and independence in exploration, rather than replacing their abilities with a reliance on NASs.



\subsection{Information Representation}

Due to VIPs' unique sensing and perceiving abilities of spatial information, the collected raw information from the first layer must be represented in a way that aligns with their abilities and supports their exploration behaviors. We provide guidelines on how NASs should organize and interpret information in order to render a useful representation for VIPs. 

\noindent\textbf{DG-3: NASs must align the organization of information with VIPs’ exploration cognitive process, including organizing geometric information, to form maps and non-visual information to reinforce the maps.}

NASs must represent the geometric and non-visual information aligned with VIPs’ exploration process. Through exploration, VIPs organize spatial information to compose their mental map, and correlate non-visual landmarks to orient themselves. NASs’ design should align the organization of information with VIPs’ cognitive process, in order to augment their abilities in exploring various environments. 

3.a: NASs should help room shape info, connection landmarks, and where those 

\textit{Organize Geometric Information To Form Maps.}
Geometric information of spaces is useful for mental map building; however, indoor environments often have complex shapes, containing multiple interconnected spaces and rooms, linked by connection landmarks: doorways, stairs, elevators, etc. It is important for NASs to organize the shapes of spaces along with the connection landmarks in a readable format for VIPs. The organization of geometric maps should support active surveying by VIPs. 

\textit{Organize Non-visual Information To Reinforce Maps. }
Due to the multi-sensory and fluid characteristics of non-visual landmarks, it is crucial for NASs to accommodate these characteristics and to organize them in correspondence with the geometric map. Each location on a geometric map is characterized by multiple landmarks in multisensory modalities. Moreover, each landmark presents time fluid characteristics. NASs should weigh statistical confidence in their presence and their prominence, in order to support an augmented recognition of the location.  


\noindent\textbf{DG-4: When information sources differ from VIPs’ sensory abilities, NASs must provide an interpretation of information, which includes translating visual information to non-visual information, and verifying and completing the provided information.}


Not all spatial information is directly collected from the environment by NASs. Some information is provided by other sources and collected indirectly via NASs. An example of this other source is another person (non-VIP) offering help, who might have vision or different sensory abilities. In this case, the information offered by a non-VIP would often mismatch with the VIPs' sensory modalities, making the information inaccurate or unperceivable for VIPs. NASs must mediate the differences and interpret the information to make it useful for VIPs.


\textit{Translate Visual Information To Non-visual Information. }
Non-VIPs intuitively describe the environment with visual information; however, this must be translated to non-visual information for VIPs. For example, non-VIPs may describe a pot of flowers by its colors, while VIPs perceive them by its smell. NASs should make cross-modality information translation with artificial intelligence, such that information communicated by non-VIPs can also support VIPs in exploration of environments.


\textit{Verify And Complete Non-VIP Provided Information. } 
Information provided by non-VIPs often contains unintentional bias, which needs to be verified and completed for VIPs. For example, non-VIPs may omit a storage door when giving directions by the count of doors. Non-VIPs may give a generic shape using a letter shape metaphor while VIPs may not remember letters by shape and would need a more detailed geometric description. NASs should verify and complete the information provided by non-VIPs, such that the information is accurate and with the appropriate level of details to be useful for VIPs.

\subsection{Agency in Requesting and Skill-Building}

% Need a small intro paragraph here 

\noindent\textbf{DG-5: NASs must facilitate active agency in VIPs toward others in requesting help information, in a way that signals abilities rather than disabilities, and that accepts needed information and rejects the unwanted.}


NASs must facilitate active agency in VIPs toward others in requesting and accepting help information. Due to current social unawareness toward visual impairments, there is a mismatch between VIPs’ abilities and non-VIPs’ expectations of their disabilities, and a mismatch between VIPs’ needs and non-VIPs’ offers of assistance. NASs must combat this imbalance by giving VIPs active agency in requesting ability-based information, and the precise level of needed information.

\textit{Signal Abilities Rather Than Disabilities. }
In some cases, help offered to VIPs is prejudicial, often magnifying their disabilities and ignoring their abilities. NASs must combat this prejudice by signaling their abilities associated with help requests, and placing zero emphasis on their disabilities. Giving VIPs an active agency in requesting information matching their abilities, NASs have the potential to promote social identity equality between VIPs and non-VIPs.



\textit{Accept Needed Information And Reject The Unwanted. }
In some cases, help available to VIPs is often more than what they need. Abundance of help forces VIPs to rely on non-VIPs for guidance, and deprives VIPs of the choice for exploration. In other cases, no help is available to VIPs when they need it. Insufficiency in help forces VIPs to struggle with difficulty, causes a burden on their cognitive load and their self-confidence could suffer. NASs must facilitate the exchange of precise help information, by giving VIPs the active agency to request and accept exactly the needed information and reject the unwanted help. 


\noindent\textbf{DG-6: NASs must facilitate mixed agency in skill-building, including taking agency to nudge VIPs for more challenging skills, and giving agency to VIPs for independent exploration. }

NASs must facilitate VIPs' skill-building for exploration. VIPs desire to build, practice and maintain their non-visual and O\&M skills for independent spatial problem-solving. Building skills is the essential process for increasing self-confidence, cognitive advantages and independence in exploration. The process requires NASs to take agency nudging VIPs to challenge and improve their skills. The ultimate goal is for NASs to give agency back to VIPs, enabling them to engage in independent exploration, without reliance on NASs for guidance.


\textit{NASs Take Agency to Nudge VIPs In Skill-building.}



\textit{NASs Give Agency to VIPs In Independent Exploration.}


==> 5-Design Guidelines/v4.tex <==
\label{sec:DGs}
The new prospect for future NASs is to support VIPs’ exploration in navigation, detailed in our findings. We applied qualitative coding to the findings in order to understand how VIPs engage with different layers of information in their exploration behaviors, and how NAS design can support and augment those behavioral needs. 

Our analysis reveals new perspectives in all three layers of NAS design: \textit{Information Collection, Information Representation and Agency in Requesting and Skill-Building}. The first layer, Information Collection, provides guidelines on how NASs should collect raw information from the environment for exploration. The second layer, Information Representation, builds upon the first layer and provides guidelines on how the NASs should represent the collected raw information to VIPs. The third layer, Agency in Requesting and Skill-Building, addresses interaction with aforementioned information and provides guidelines on how agency should be allocated when people and NASs interact with the exploration information. In each layer, VIPs' exploration behaviors inspire a new light of thinking, and calls for a new set of design guidelines.

\subsection{Information Collection}


VIPs' exploration requires different 
basic types of information 
and define exploratory landmarks, which we call exploratory landmarks, that are different what they use for guidance.
We elaborate on them in DG1 and DG2 respectively.
and define what characterizes landmarks 

may also be different from what they use for guidance.

define landmarks through their characteristics



Specifically, DG1 
We define guideline for what these basic information types are in DG-1, and elaborate on new characteristics for the landmark information in DG2. - like the emphasis on charactersitics
that builds on top of these basic units in DG2.
- not sure about building on top of - because geometry info is not mentioned in DG2 - perhaps no need to mention one is on top of another relationship. rather, types and characteristics are parallel


% Spatial 
Information that supports VIPs' exploration of environments differs from that of guidance. 



We provide guidelines on the 

specific types of information and characteristics of landmark information that are useful in supporting exploration and should be collected by NASs. 



\noindent\textbf{DG-1: NASs must collect the types of information used during VIPs’ exploration, including geometric information of space and non-visual information.}


%Come back with insight 
VIPs' exploration is based on two basic types of information: geometric shape of the space, and information gathered via non-visual senses. 
NASs must collect these in order to facilitate exploration. 
[connect with insight]
how to introduce the two sub-points 
- what is the guideline in high level 
- where it comes from - insight
- NAS should do [this] 


% NASs must collect the types of information used by VIPs during their exploration of the environment. 
% The types of information must align with VIPs’ sensory and perceptual abilities. 
% They are instrumental to help VIPs pay attention and collect spatial information as they explore the indoor environment. 
% Existing turn-by-turn NASs provide directional cues to the next waypoints; however, they do not support the exploration of the environment, which requires geometric and non-visual information about the space.


\textit{Geometric Information Of Space.} Indoor environments are outlined by boundaries. The geometric shape of the boundaries help set a base layer for mental maps. VIPs may learn the shape of a space by asking for verbal descriptions, which are usually inaccurate. They may also learn the shape of a space by slowly tracing along the walls using their tactile senses, which is time consuming, especially for large spaces. Additionally, VIPs benefit from learning the objective and accurate counts of physical geometries in space, such as the number of doors. There is an opportunity for NASs to collect and display the geometric information of spaces accurately and efficiently. 

\textit{Non-Visual Information.}
Due to the lack of visual information, non-visual information becomes the building blocks for VIPs’ spatial exploration and mental maps. Non-visual information includes ambient sounds, textures, temperature, air current, echolocation, smell, and more. VIPs must use a huge amount of mental effort to capture useful non-visual information. There is an opportunity for NASs to collect non-visual information and augment VIPs’ sensory abilities.  

\noindent\textbf{DG-2: NASs must collect VIPs’ spatial landmark information including multisensory, fluid and VIP-verifiable characteristics.}

alt title DG-2: NASs must collect exploratory landmarks defined through characteristics: multi-sensory, fluid and VIP-Verifiable
%characteristics is key word



NASs must collect spatial landmarks that are essential components of VIPs' mental maps. VIPs’ landmarks are different from turn-by-turn waypoints and destinations in guidance-based navigation. Rather, VIPs’ landmarks should be designed for storing and recognizing local features helpful for spatial exploration, orientation and memory. Therefore, the useful spatial landmarks for exploration are composed of non-visual multisensory information, fluid in time contexts, and must be verifiable by VIPs sensory abilities.

\textit{Landmarks Must Be non-visual Multisensory.}
A landmark is recognizable to VIPs when multiple pieces of sensory information are present at the same time. The multiple sense should

For example, an air-conditioning unit is perceived by the collection of cold air flow, the fan blade noise and the engine vibration. It is important for NASs to collect all pieces of information in support of a recognizable landmark. 


\textit{Landmarks Must Be Fluid.} 
A landmark could present itself differently during different times of the day. For example, a bakery may act as a fluid location landmark, and it emits a fresh smell of bread and warmth from the oven in the morning but not in the evening. It is important for NASs to collect the fluid contextual characteristics matching the particular landmark.  


\textit{Landmarks Must Be Verifiable by VIPs.}
NASs should define landmarks in a way that VIPs can verify the presence of a landmarks either using their own senses alone, or by using additional supportive information from the NASs. 
NASs should adapt to VIPs' information formats -- which is primarily non-visual, and augment, and not replace, it so that they can detect presence of landmarks on their own. 
The ability to verify landmarks boosts VIPs confidence to enable independent exploration.

% NASs play by the rules of VIPs, and not the other way round. 

% - Landmarks must be defined by both NASs and VIPs in using the same sensory information.


% - detect the presence of a landmarks using their own senses as well, NASs should provide support for this detection but not do it for VIPs directly.


% - landmarks should be both collectable by NASs and VIPs

% - When landmarks is collected by VIPs - independent exploration
% - the same landmark collected by NASs - to provide support
% - if NASs provided landmark is not verifiable, NASs is guidance, VIPs must trust what NASs give them 
% - if NASs provided landmark is verifiable, VIPs can learn from it. 
% Since landmarks are a key component for .... for reinforcing VIPs' location, VIPs must be able to detect/verify landmarks using their existing senses. 


% In order to enable VIP’s independent exploration of the environment, the information provided by NASs must be verifiable by VIPs with their sensory abilities. NASs should take a supporting role rather than a directing role. 

% Verifiable information is key to building VIPs’

% confidence and independence in exploration, 

% rather than replacing their abilities with a reliance on NASs.



\subsection{Information Representation}


% - [raw] information needs processing and organization to be represented to the VIPs in the correct/comprehensible/useful format. 

% organizing the units of information important for exploration and sometimes process. information from alternative sources such as non-VIPs.



In order to support VIPs' exploration, NASs must support VIPs in organizing the basic units of information (from DG1) into maps. In addition, NASs MUST ~sometimes~ process information from alternative sources --- such as non-VIPs --- in order to render a useful representation for VIPs.


% Due to VIPs' unique sensory abilities of spatial information, the collected raw information from the first layer must be represented in a way that aligns with their abilities and supports their exploration behaviors. We provide guidelines on how NASs should organize and interpret information in order to render a useful representation for VIPs. 

\noindent\textbf{DG-3: NASs must align the organization of information with VIPs’ exploration cognitive process, including organizing geometric information, to form maps and non-visual information to reinforce the maps.}

NASs must represent the geometric and non-visual information aligned with VIPs’ exploration process. Through exploration, VIPs organize spatial information to compose their mental map, and correlate non-visual landmarks to orient themselves. NASs’ design should align the organization of information with VIPs’ cognitive process, in order to augment their abilities in exploring various environments. 

3.a: NASs should help room shape info, connection landmarks, and where those 

\textit{Organize Geometric Information To Form Maps.}
Geometric information of spaces is useful for mental map building; however, indoor environments often have complex shapes, containing multiple interconnected spaces and rooms, linked by connection landmarks: doorways, stairs, elevators, etc. 
connection nodes? to not clash with our defined "landmark"
It is important for NASs to organize the shapes of spaces along with the connection landmarks in a readable format for VIPs. The organization of geometric maps should support active surveying by VIPs. 


\textit{Organize landmarks To Strengthen Maps}
Since exploratory landmarks are contextual in nature: i.e., dependent upon time and is also multi-sensory (DG2), there may scenarios where one more landmark may be more relevant than the other and vice versa.
In such cases, NASs should support VIPs in organizing multiple complementary landmarks for each location to form robust mental maps. 
In such cases, NASs must automatically cue/hint/inform VIPs to look for other landmarks instead. 
For instance, 
morning, evening --> bagels (morning) and trash can (evening)
% a landmark defined by AC may become irrelevant when it's turned off in the evening. 
% reason: characteristics - fluid
% action: organize
% goal: reinforce for robustness


% \textit{Adapt to Contextual Nature of Landmarks To Reinforce Maps.}
% Since exploratory landmarks are contextual in nature: i.e., dependent upon time and is also multi-sensory (DG2), NASs must help VIPs define context in order to direct user's attention to the most reliable information in that context in time and space. For instance, a landmark defined by AC may become irrelevant when it's turned off in the evening. In such cases, NASs must automatically cue/hint/inform VIPs to look for other landmarks instead.
% - how NASs 

% if air conditioners is stops running, all informatio
% , NASs should support VIPs in dealing with this dynamic nature. For this, NASs should support VIPs in 
% Due to the multi-sensory and fluid characteristics of non-visual landmarks, NASs should add support for reinforcing the mental map with landmarks.


% it is crucial for NASs to accommodate these characteristics and to organize them in correspondence with the geometric map. 
% Each location on a geometric map is characterized by multiple landmarks in multisensory modalities. 
% Moreover, each landmark presents time fluid characteristics. NASs should weigh statistical confidence in their presence and their prominence, in order to support an augmented recognition of the location.


\noindent\textbf{DG-4: When information sources differ from VIPs’ sensory abilities, NASs must provide an interpretation of information, which includes translating visual information to non-visual information, and verifying and completing the provided information.}




Not all spatial information is directly collected from the environment by NASs. Some information is provided by other sources and collected indirectly via NASs. An example of this other source is another person (non-VIP) offering help, who might have vision or different sensory abilities. In this case, the information offered by a non-VIP would often mismatch with the VIPs' sensory modalities, making the information inaccurate or unperceivable for VIPs. NASs must mediate the differences and interpret the information to make it useful for VIPs.


\textit{Translate Visual Information To Non-visual Information. }
Non-VIPs intuitively describe the environment with visual information; however, this must be translated to non-visual information for VIPs. For example, non-VIPs may describe a pot of flowers by its colors, while VIPs perceive them by its smell. NASs should make cross-modality information translation with artificial intelligence, such that information communicated by non-VIPs can also support VIPs in exploration of environments.


\textit{Complete Non-VIP Provided Information. } 
Information provided by non-VIPs often contains unintentional bias, which needs to be completed for VIPs. 
% For example, non-VIPs may omit a storage door when giving directions by the count of doors. 
While giving directions non-VIPs may provide incomplete directions for VIPs to act on. For example, non-VIPs may ask VIPs to take a left turn from "there" (pointing their finger in a specific direction). NASs must act as interface between VIPs and non-VIPs to establish a communication link in order to complete the information.



Non-VIPs may give a generic shape using a letter shape metaphor while VIPs may not remember letters by shape and would need a more detailed geometric description. 

NASs should complete the information provided by non-VIPs, such that the information is accurate and with the appropriate level of details to be useful for VIPs.







\subsection{Agency in Requesting and Skill-Building}

% Need a small intro paragraph here 

\noindent\textbf{DG-5: NASs must facilitate active agency in VIPs toward others in requesting help information, in a way that signals abilities rather than disabilities, and that accepts needed information and rejects the unwanted.}


NASs must facilitate active agency in VIPs toward others in requesting and accepting help information. Due to current social unawareness toward visual impairments, there is a mismatch between VIPs’ abilities and non-VIPs’ expectations of their disabilities, and a mismatch between VIPs’ needs and non-VIPs’ offers of assistance. NASs must combat this imbalance by giving VIPs active agency in requesting ability-based information, and the precise level of needed information.

\textit{Signal Abilities Rather Than Disabilities. }
In some cases, help offered to VIPs is prejudicial, often magnifying their disabilities and ignoring their abilities. NASs must combat this prejudice by signaling their abilities associated with help requests, and placing zero emphasis on their disabilities. Giving VIPs an active agency in requesting information matching their abilities, NASs have the potential to promote social identity equality between VIPs and non-VIPs.



\textit{Moderate Help from Others.}
Insight \#[TODO] highlights the mismatch between the help VIPs want and what non-VIPs have to offer. To this end, 
NASs must act as a ~bridge~ between the two parties and help VIPs moderate the amount and type of help they want to receive from others. For example, while grocery shopping, VIPs can decide the type of help they want on a spectrum of "here's my shopping list, can you please find these for me?" vs. "can you give me an overview of the store and I'll find my stuff?"


% which may be just about getting them to the right aisle or
% "shopping list example".


% In some cases, help available to VIPs is often more than what they need. Abundance of help forces VIPs to rely on non-VIPs for guidance, and deprives VIPs of the choice for exploration. In other cases, no help is available to VIPs when they need it. Insufficiency in help forces VIPs to struggle with difficulty, causes a burden on their cognitive load and their self-confidence could suffer.
% NASs must facilitate the exchange of precise help information, by giving VIPs the active agency to request and accept exactly the needed information and reject the unwanted help. 


\noindent\textbf{DG-6: NASs must facilitate mixed agency in skill-building, including taking agency to nudge VIPs for more challenging skills, and giving agency to VIPs for independent exploration. }

NASs must facilitate VIPs' skill-building for exploration. VIPs desire to build, practice and maintain their non-visual and O\&M skills for independent spatial problem-solving. Building skills is the essential process for increasing self-confidence, cognitive advantages and independence in exploration. The process requires NASs to take agency nudging VIPs to challenge and improve their skills. The ultimate goal is for NASs to give agency back to VIPs, enabling them to engage in independent exploration, without reliance on NASs for guidance.


\textit{NASs Take Agency to Nudge VIPs In Skill-building.}

NASs take initiative 


\textit{NASs Give Agency to VIPs In Independent Exploration.}

VIPs take initiative 

==> 5-Design Guidelines/v5.tex <==
\label{sec:DGs}
Our findings uncover a new set of design guidelines for helping NASs become exploration assistance systems rather than guidance systems. We group the design guidelines under three themes: 
(1) \textit{information collection}: which types of raw information NASs should gather from the environment (DG1, DG2), 
(2) \textit{information representation}: how this information should be processed and organized (DG3, DG4), 
(3) \textit{agency in requesting information}: how NASs should support, and not replace, VIPs' natural exploration behaviors such as interaction with non-VIPs (DG5), and
(4) \textit{skill-building}: how NASs  should support the growth of VIPs' spatial cognitive abilities (DG6).
% how should NASs support and develop VIPs' exploration to achieve independent navigation.


% ------------------------------------------------------------------------------------
\subsection{Information Collection}
Through our findings, we learn that the information collected by an NAS in order to support exploration is different from what is required for guiding a user.
In our recommended design guidelines, we define the basic types of information (DG1) and a new class of landmarks, namely \textit{exploratory landmarks} (DG2), that NASs should collect in order to support exploration in navigation for VIPs.

% ------------------------------------------------------------------------------------

\begin{itemize}
    \item [\textbf{DG1.}] 
    % \textbf{NASs should collect raw information from the environment useful to VIPs: geometric shape and non-visual information.}
    \textbf{NASs should collect raw information from the environment in a way that aligns with VIPs' sensory and perceptual capabilities}
    (\texttt{from Insight 1}).
\end{itemize}
From our findings, we learned that VIPs use non-visual senses to explore and understand the general layout of a space (Insight 1). To facilitate exploration, NASs should also collect the same raw information to align with VIPs' sensory and perceptual capabilities. Doing so would allow NASs to help VIPs form mental maps of an environment in a more natural way.
Below, we elaborate on these two basic types of information required to support exploration.



\textit{Geometric Shape Information.} 
Environments, especially indoors, are characterized by their boundaries which  may be represented in the form of geometric shapes such as squares (for rooms) or rectangles (for hallways). These shapes form the first layer of VIPs' mental map, which develops over time as they explore the space more. In practice, however, VIPs find it challenging to gather this formation. They may acquire this information by asking for verbal descriptions from others, which is seldom accurate. Alternatively, they may also trace along the boundaries using their tactile senses which is time consuming and tedious. Hence, NASs should collect the geometric shape information of the environment to initiate the formation of VIPs' mental map of a space.


\textit{Non-Visual Sensory Information.}
VIPs reported that they constantly augment their mental map (containing the geometric shape information) with additional information gathered via non-visual senses during exploration. 
Non-visual information may include ambient sounds, change in floor textures, temperature, air-current, smell, or some combination thereof. 
Non-visual information has a significantly lower bandwidth, when compared to visual information. As a result, VIPs have to put in a lot of effort to gather detailed non-visual information~\cite{tversky1993cognitive}.
Hence, NASs should collect and communicate non-visual information in a way that augments VIPs' existing perceptual capabilities and fosters a sense of exploration.
  




% ------------------------------------------------------------------------------------



\begin{itemize}
    \item [\textbf{DG2.}] 
    \textbf{NASs should define \textit{exploratory landmarks} using multi-sensory, fluid, and VIP-verifiable characteristics}
    (\texttt{from Insight 2}).
\end{itemize}



% NASs should define exploratory landmarks using multi-sensory, fluid and VIP-Verifiable characteristics. 


From our findings, we learned that VIPs use a more complex form of landmarks during exploration than during guidance --- we name them as \textit{exploratory landmarks}. Unlike physical landmarks such as destinations (e.g., restroom, doors, office) or waypoints along the routes, exploratory landmarks are characterized by different properties: multi-sensory, fluid in time, and verifiable by VIPs. 
% Due to the complex nature of these landmarks, NASs should support VIPs in collecting information about these landmarks. 
We now explain each of the three characteristics in detail.

\textit{Multi-sensory:}
Each exploratory landmarks is composed of multiple pieces of non-visual sensory information.
For example, an air-conditioning unit may be composed of cold air flow (temperature, air-currents), rotating fan blades (sound), and an engine vibration (haptics). 
NASs should help VIPs collect all these pieces of information. 
                
\textit{Fluid in Time:} 
Exploratory landmarks' relevance changes with time. 
For example, consider a bakery in a shopping mall as an exploratory landmark. It is characterized by the aroma of breads and warmth from the oven. Note that this landmark is more prominent during the day when the shop is open, as opposed to during the evenings when it may be closed. 
NASs should collect contextual information for each landmarks to determine its relevance at a given time.

\textit{Verifiable by VIPs:}
Landmarks must be defined such that VIPs can verify the presence of said landmarks either using their own senses alone, or by using additional supportive information from the NASs. 
NASs should adapt to VIPs' information formats -- which is primarily non-visual -- to augment, and not replace, the detection of these landmarks.


% ------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------



\subsection{Information Representation}
Basic information collected by the NASs should be organized and used to form larger and more complex representations of mental maps (DG3). 
In addition, NASs should also process information from alternative sources, such as non-VIPs, in order to render a more comprehensible representation for VIPs to use and act upon (DG4).


\begin{itemize}
    \item [\textbf{DG3.}] 
    \textbf{NASs should organize raw information and exploratory landmarks in a way that leads to mental maps}
    (\texttt{from Insight 1, 2}).
\end{itemize}


As a follow-up to DG1 and DG2, once the NASs have collected the basic information, they must help VIPs make sense of individual pieces of information by suggesting logical connections between them. Doing so would help VIPs understand the space better. In addition, NASs should help VIPs establish context for exploratory landmarks in order to confirm their relevance and thus reinforce their mental maps.



\textit{Organize Geometric Shape Information To Complete Mental Maps.}
VIPs mentioned that it is challenging for them to organize different shape information on a global level to understand the space as a whole. For instance, 
environments often have complex shapes, with multiple interconnected spaces such as rooms linked by doorways, stairs, or elevators.
NASs should inform VIPs of these connections in a way that is comprehensible to VIPs. 
One suggestion is to organize shape information via connections such as doors, elevators, or any landmark which leads to another piece of shape information.


\textit{Organize Exploratory Landmarks To Reinforce Mental Maps.}
Since exploratory landmarks are fluid in time, there may be scenarios where one landmark may be more relevant than another at a given time.
In such cases, NASs should utilize multiple complementary landmarks for each location to reinforce VIPs' mental maps. 
For instance, consider a location defined by two landmarks: a bakery and a trash can. Here, the bakery may be more relevant in the morning due to the odor and sound (from the oven), whereas the trash can may grow in relevance by evening as it fills up throughout the day (due to the smell).


% ------------------------------------------------------------------------------------


% \noindent\textbf{DG-4: When information sources differ from VIPs’ sensory abilities, NASs should provide an interpretation of information, which includes translating visual information to non-visual information, and verifying and completing the provided information.}
\begin{itemize}
    \item [\textbf{DG4.}] 
    \textbf{ NASs should process information from alternate sources for useful representation to VIPs 
    }
    % interpretation of information, which includes translating visual information to non-visual information, and verifying and completing the provided information, when information sources differ from VIPs’ sensory abilities,.}
    (\texttt{from Insight 3, 4}).
\end{itemize}

From our findings, we learned that one of the major alternate sources of information for VIPs is non-VIPs. However, there is often a mismatch between how VIPs perceive spaces both in terms of type of information (predominantly visual for non-VIPs), and the level of detail required to describe a space (higher for VIPs). NASs should act as an interface to mediate these differences via translation and completion.


% Not all spatial information is directly collected from the environment by NASs. Some information is provided by other sources and collected indirectly via NASs. An example of this other source is another person (non-VIP) offering help, who might have vision or different sensory abilities. In this case, the information offered by a non-VIP would often mismatch with the VIPs' sensory modalities, making the information inaccurate or unperceivable for VIPs. NASs should mediate the differences and interpret the information to make it useful for VIPs.


\textit{Translate Visual Information To Non-visual Information. }
Non-VIPs intuitively perceive and describe the environment through visual information, which may not be useful for VIPs.
% this must be translated to non-visual information for VIPs. 
For example, non-VIPs may describe a flower pot by its size and color (sense of vision), while VIPs may depict it through its scent (sense of smell). NASs should provide information translation such that information communicated by non-VIPs can  support VIPs' exploration.


\textit{Complete Information Provided by Non-VIPs. } 
Non-VIPs often provide incomplete information to VIPs, which may not be useful for VIPs.
% Information provided by non-VIPs often contains unintentional bias, which needs to be completed for VIPs. 
% For example, non-VIPs may omit a storage door when giving directions by the count of doors. 
% While giving directions non-VIPs may provide incomplete directions for VIPs to act on. 
For example, a non-VIP may attempt to give directions like, ``Take a left from \textit{there}'' while pointing with their finger. Such directions are difficult, if not impossible, for a VIP to interpret without further clarification.
% non-VIPs may ask VIPs to take a left turn from "there" (pointing their finger in a specific direction). 
NASs should act as an interface between VIPs and non-VIPs to ensure completeness of information.



% Non-VIPs may give a generic shape using a letter shape metaphor while VIPs may not remember letters by shape and would need a more detailed geometric description. 

% NASs should complete the information provided by non-VIPs, such that the information is accurate and with the appropriate level of details to be useful for VIPs.


% ------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------

\subsection{Agency in Requesting Information from Others}

From our findings, we learned that VIPs want to explore environments in a self-directed manner. Hence, it is important that NASs aim to support, and not crutch, VIPs' exploration efforts while navigating. To this end, NASs should support VIPs' natural exploration strategies such as requesting information from others (DG5).


\begin{itemize}
    \item [\textbf{DG5.}]
    \textbf{NASs should help VIPs request information from others while emphasizing and maintaining their own abilities}
    (\texttt{from Insight 3, 5}).
\end{itemize}
Our findings reveal that VIPs struggle with requesting and getting information from others. Because non-VIPs are often unaware of VIPs' abilities, they often end up making incorrect assumptions and causing unwanted social anxiety for all involved parties.
NASs should mitigate this by giving VIPs active agency in requesting spatial or environmental information and by allowing VIPs to moderate the type and amount of information that others can give back.

\textit{Signal Abilities, Not Disabilities. }
Social anxiety is often caused by false assumptions about VIPs' disabilities. For example, in airports, VIPs often complain about being helped with a wheelchair when they do not have any motor impairments~\cite{guerreiro_airport_2019, abdolrahmani2021towards}.
% In some cases, help offered to VIPs is prejudicial, often magnifying their disabilities and ignoring their abilities. 
NASs should combat this prejudice by signaling VIPs' abilities associated with help requests and de-emphasizing their disabilities. 
% A universal help platform for both VIPs and non-VIPs would promote social identity equality.



\textit{Moderate Information from Others.}
The type and amount of information VIPs want is often misjudged by non-VIPs. VIPs must be allowed to take initiative and gain agency over the kind of information they want. For example, VIPs may have differing preferences for assistance while grocery shopping. Their requests could range anywhere on the spectrum from, "Can you give me an overview of the store aisles? I can help myself from there." (i.e., descriptions) to "Here's my shopping list, can you please help me find all of them?" (i.e., guided assistance). NASs should provide VIPs a platform to communicate and moderate information from others to match their preferences. 

% Insight \#[TODO] highlights the mismatch between the help VIPs want and what non-VIPs have to offer. To this end, 
% NASs should act as a ~bridge~ between the two parties and help VIPs moderate the amount and type of help they want to receive from others. For example, while grocery shopping, VIPs can decide the type of help they want on a spectrum of "here's my shopping list, can you please find these for me?" vs. "can you give me an overview of the store and I'll find my stuff?"


% which may be just about getting them to the right aisle or
% "shopping list example".


% In some cases, help available to VIPs is often more than what they need. Abundance of help forces VIPs to rely on non-VIPs for guidance, and deprives VIPs of the choice for exploration. In other cases, no help is available to VIPs when they need it. Insufficiency in help forces VIPs to struggle with difficulty, causes a burden on their cognitive load and their self-confidence could suffer.
% NASs should facilitate the exchange of precise help information, by giving VIPs the active agency to request and accept exactly the needed information and reject the unwanted help. 

% ------------------------------------------------------------------------------------

\subsection{Skill-Building}

In our findings, VIPs expressed the desire to maintain and learn O\&M skills. They also reported that they found it difficult to do so without regular access to either O\&M trainers or sighted guides.
Hence, NASs should help VIPs develop their O\&M skills until they reach a stage where they no longer need an NAS (DG6). 
% There is an opportunity for NASs to play a different role, than what most NASs are thought to be playing, 


% Building and actively practicing O\&M skills is a means of environmental exploration. 
% In order for VIPs To explore independently, it is critical to build and maintain O\&M skills. NASs should fill the gap between lack of access to O\&M training and insufficient approach to O\&M training. 



\begin{itemize}
    \item [\textbf{DG6.}] 
    \textbf{NASs should nudge VIPs toward building O\&M skills and not needing an NAS.
    % must not act as a crutch, and instead should nudge VIPs toward building their O\&M skills in order to achieve independent navigation, so that they can ultimately explore environments alone, without the help of an NAS 
    }
    (\texttt{from Insight 6, 7}).
\end{itemize}
From our findings, we learned that VIPs want the ability to navigate independently, but lack the O\&M skills needed for independent exploration. As a result,   
% \noindent\textbf{DG-6: NASs should not act as a crutch, but nudge VIPs toward building their skills in order to achieve independent navigation and explore environment alone}
% facilitate mixed agency in skill-building, including taking agency to nudge VIPs for more challenging skills, and giving agency to VIPs for independent exploration. 
% NASs should facilitate VIPs' skill-building for exploration. 
VIPs need support to build, practice, and maintain their O\&M skills and their ability to process non-visual information.
% for independent spatial problem-solving. 
Building these skills is essential for increasing VIPs' self-confidence, which is a big step towards independent navigation. Hence, NASs should facilitate skill-building in a mixed-initiative manner, nudging VIPs to improve their O\&M skills on a daily basis.
% , cognitive advantages and independence in exploration. 
% The process requires NASs to take agency nudging VIPs to challenge and improve their skills. 
The ultimate goal is for NASs to give agency back to VIPs, enabling them to engage in independent exploration without needing to rely on NASs.


\textit{Facilitate Skill-building via Mixed-Initiative Interaction.}
NASs have an immense potential to serve as skill-building or educational tools to help VIPs achieve independent navigation. To this end, NASs should first help a VIP build the O\&M skills needed to explore their environments, then reduce their support over time, until the VIP is no longer dependent on the NAS for exploration.
In this mixed-initiative interaction, NASs nudge VIPs toward playing a more active role in their navigation, but VIPs too provide constant feedback to NASs in order to help determine the right amount of support NASs need to provide.


==> 6-Visions/v1.tex <==
We now articulate visions for future NAS research that are informed by our design guidelines. Each vision finds its motivation from an \texttt{Insight} --- VIPs' exploration need --- highlighted in our findings. We then map the insight to relevant design guidelines to inform our vision of how future NASs can support VIPs's exploration needs. Each vision may be informed by one or several of the design guidelines. 

While we acknowledge that there will be alternate solutions to VIPs' exploration needs and several practical considerations also shape the design of an NAS, our aim of presenting these visions is two-fold. One, we believe that these visions will spur discussion, experiment, and further insight into how we might rethink NAS design to support exploration, in addition to guidance. Two, we hope to provide system developers a more elaborate account of how they might use the design guidelines to inform their work in service of facilitating exploration for VIPs.

% how we might rethink NAS design to support exploration.
% % Each vision outlines an NAS design framework that solves a challenge in exploration discovered from our interviews, informed by one or several of the design guidelines. Our hope is that these visions will spur discussion, experiment, and further insight into how we might rethink NAS design to support exploration in navigation for VIPs.



\subsection{Active Environment Shape Surveying}
VIPs explore their immediate surroundings through tactile feedback via a white cane. However, it is difficult to gather information about the environment beyond the reach of the white cane. From our interviews, we found that VIPs want to learn about the general layout of the space in a self-directed manner, specifically in indoor environments (see \texttt{Insight 1}). This form of exploration derives from two of the design guidelines. First, \texttt{DG-1}, which highlights the importance of geometric shape information of the space. Second, \texttt{DG-3}, which mentions the importance of helping VIPs organize the geometric shape information in a way that supports their spatial understanding of the environment to form mental maps.  

Figure.~\ref{fig:vision1} presents our vision of an NAS design that enables VIPs to survey the shape of an environment in a natural way. The system constitutes a wearable sensor --- e.g., head or chest-mounted camera, smartglasses --- which scans the environment to compute the required shape information. As the user moves around the environment, the NAS offers them the ability to receive shape information on-demand via audio cues. Using spatialized audio, the system gives user a sense of how far the walls are in front of them. Similar to how VIPs use echolocation, the system provides VIPs non-visual cues for them to process instead of directly telling them the shape of the room. Doing so would help them form a better mental map, as it allows them to integrate this new information with their other sensory information.
% [IS THIS NEEDED?]% they can integrate this additional information with the raw information they gathered from their other senses.



% In fact, the camera feed can also be used to compute other types of information such as objects, obstacles, people, and scene descriptions, to provide users the freedom to choose between different types and levels of information. Since the camera is mounted onto the user, linking the their orientation with the information would help their spatial understanding of the space.

% The system offers VIPs two levels of control. First, control over the type and granularity of information being provided by the NAS. Second, ability to survey the environment in a direction of their choice.

% our vision of an NAS that enables VIPs to survey the environment in a self-directed manner. The user wears a head-mounted RGB-D camera, which scans the environment to gather (1) distance to the wall, (2) semantic information, (3) ... . As the user moves around the environment, they have the ability to get gather different types of information such as shape layout, object information, obstacle information, scene descriptions, ... . Note that the user exercises two levels of control over exploration. First, the head-mounted camera offers a more natural way of providing NAS the direction in which they wish to get information. Second, they have control over the type and granularity of information being provided by the NAS. The ability to gather information in a more natural would help them link the information with their spatial understanding of the space better.




% --



\subsection{Support for `Fluid' Landmarks}
During exploration, VIPs use a more nuanced/complex form of landmarks which are multi-modal (i.e., use information from multiple senses) and dynamic (i.e., may change over time and space). This helps them account for the dynamic nature of the environment (\textit{Insight 2}). The concept of fluid landmarks emerge from DG-2, which highlights that NASs should support VIPs in creating, modifying, and automatically updating fluid landmarks.

Figure~\ref{fig:vision2} presents our vision of an NAS that supports fluid landmarks. The system maintains a list of landmarks, each defined by new attributes such as (1) \textit{modality}: which senses are used to detect the landmark, (2) \textit{persistence in time}: when is the landmark active/inactive, (3) \textit{persistence in space}: what was the previous location of this landmark (if any), and (4) \textit{confidence}: a derived attribute that is computed in real-time to assess how relevant is this landmark in the current context of time and space. The NAS supports two major functions through this concept. First, it helps with detection of new landmarks via a host of sensors, augmenting VIPs' non-visual senses and filtering out any noise in the environment. Second, it assists VIPs in reinforcing their location by presenting them with a ranked list of landmarks. Ranking is based on the \textit{confidence} attribute to reflect dynamic changes in the environment. Fluid landmarks may be integrated with existing guidance-based systems while also assisting VIPs' exploration.





% - list of landmarks
% - where each location is defined by multiple landmarks ranked by their importance. The importance is based on several factors like their persistence, recognizability -- both by system and by VIPs, 


% Existing NASs use predefined NASs that are usually physical landmarks such as doors, elevators, stairs, and bathrooms; which act as destinations in a guidance-based system. However, as highlighted by DG-2, there is a need to integrate a broader sense of what landmarks mean to VIPs when exploring an environment. Specifically, VIPs should have the ability to add dynamic landmarks beyond physical landmarks and modify them as well.


% \textit{Design Consideration.}
% The motivation touches upon two streams of design guidelines: information. Specifically, DG-2.


% \textit{System Description.}
% Figure.~\ref{fig:teaser} presents our vision of an NAS that enables the concept of an enhanced landmarks. NASs must allow VIPs to add, modify, and delete landmarks while automatically creating a hierarchy for them. Since VIPs employ a host of different senses, NASs should enable VIPs to save non-visual information from multiple different senses to help them identify landmarks in a more natural way, i.e., using their other senses. Further, the ability to combine landmarks would also mimic their natural behavior of using multiple different landmarks to reorient/confirm their location. As DG-2 suggests, landmarks may vary over time and space, and hence the ability to modify landmarks is crucial to how VIPs can keep NASs up to date about their new mental maps, instead of using static, pre-determined set of physical landmarks.


% --


\subsection{Cross-Modality Translation}
% \textit{Motivation.}
Exploration of unfamiliar environments often require VIPs to ask for directions from sighted people nearby. However, the difference in perception of environments --- which is primarily visual for sighted people --- make it challenging for VIPs to use their navigational instructions effectively (\texttt{Insight 4}). This form of exploration touches upon \texttt{DG-4}, which highlights the opportunity for NASs to serve as an interface for navigational help between VIPs and sighted people. 


% Several research efforts, including ours, have corroborated that VIPs' perception of space is different from how sighted people perceive spaces. This arises primarily from the dependence on different senses or modalities of gathering and processing information. While sighted people rely on vision, VIPs tend to combine information all other senses. Due to this, when sighted people describe a place or provide instructions, VIPs find it challenging to understand that information without visual context.
% Hence, there is an opportunity for NASs to perform this cross-modality description translation to facilitate ease of exploration.


% \textit{Design Consideration.}
% [representation] DG-4


% \textit{System Description.}





Figure~\ref{fig:vision3} presents our vision of an NAS that facilitates translation of sighted person's navigational instruction to a format appropriate for VIPs. First, there is a need to identify the standard format which fits the VIPs' needs. A similar effort has been made by Lee et al.~\cite{lee2021designing} to identify product descriptions for grocery shopping. The NAS takes as input directions from a sighted person in natural language and converts them to the standard format. Natural language processing, with its sophisticated models, has the potential to automate this translation. There may be scenarios where sighted person's instruction may not satisfactorily complete the standard format. In such cases, the system plays a transactional role in raising specific queries to fix the missing pieces. Such systems have the potential to help standardize the help provided by remote-assistance based systems such as AIRA~\cite{} and BeMyEyes~\cite{}.


% help remote assistance-based systems such as AIRA~\cite{} and BeMyEyes~\cite{} by standardizing the assistance provided by different helpers/volunteers/experts/people.
% [In case the format is not satisfactorily filled up, the system should ask non-VIPs for specific pieces of information that they missed out.]


% --


\subsection{Integrated Assistance Platform}
\textit{Motivation.}
VIPs often find themselves being treated as a separate class, which causes social anxiety both for them and the helper (Insight \#X). To address this, DG-3 suggests that help should be ability-based, and not identity-based. Hence there is a need to design assistance platforms that allow both VIPs and sighted people to ask for assistance without necessarily revealing their identity. In fact, such an assistance platform should be integrated in the NAS design. 



\textit{Design Consideration.}
DG-3


\textit{System Description.}
Figure.~\ref{fig:teaser} presents our vision of an NAS design with an integrated assistance platform. NASs must integrate assistance from others within them (on the VIP side). On the non-VIPs side, they should receive assistance requests on the same platform from both VIPs and non-VIPs. 



% --

\subsection{Real-time/Virtual O\&M Assistance}
\textit{Motivation.}
% Recently, remote assistance-based solutions such as AIRA~\cite{cite aira} and BeMyEyes~\cite{cite bemyeyes} have gained popularity amongst the VIP community. These approaches help VIPs solve the issue of not being able find sighted assistance by helping them connect to either paid experts (AIRA) or volunteers (BeMyEyes). We belive that this concept can be extended to O\&M trainers as well, in order to solve the problem of lack of access to O\&M trainers. 
There is an immense potential for NASs to not just support exploration, but also to help VIPs gain necessary O\&M skills that would help them explore an environment on their own. Due to the lack of access to O\&M trainers, NASs may be used as educational tools that provide real-time O\&M assistance. O\&M techniques are powerful in that they are designed to help VIPs ``solve'' any environment. However, it may be difficult for some individuals to identify which technique suits best in a particular situation.
[Based on the immediate surroundings, what is the best O\&M skill that can be used at that point of time.]


\textit{Design Consideration.}
DG-6.


\textit{System Description.}
Figure.~\ref{fig:teaser} presents our vision of an NAS that enables VIPs to receive real-time O\&M assistance. Whenever VIPs get stuck, or cannot determine the best possible technique to use, NASs can help them. Based upon the current camera view, NASs may automatically compute the best possible O\&M technique or next steps to take in order to solve the environment. From an NASs' perspective, each of these environments can be imagined as a problem set where O\&M techniques are solutions to each of these problems. 
In addition, NASs can save logs of VIPs' quest to solve an environment. These logs can later be reviewed by O\&M experts to identify areas of improvement for the VIP. Such a system would allow one O\&M trainer to cater to several VIPs.
Through this real-time assistance, VIPs would not only gain confidence to explore an environment by themselves, but would also help them build their O\&M skills. We believe that NASs that replace sighted assistance with AI should also think about NASs that build skills in order to ultimately replace NASs and make VIPs independent navigators/travellers.









==> 6-Visions/v2.tex <==
\label{sec:visions}


We now articulate visions for future NAS research that are informed by our design guidelines. Each vision finds its motivation from an \texttt{Insight} --- one of VIPs' exploration needs --- that our findings in Section~\ref{sec:findings} highlight.
While we acknowledge that there will be alternate solutions to VIPs' exploration needs and that practical considerations also shape the design of NASs, our reason for presenting these visions is two-fold. First, we believe that these visions will spur discussion among the research community about how we might rethink NAS design to support exploration in addition to guidance. Second, we hope to provide system developers a more explicit account of how they might use our design guidelines from Section~\ref{sec:DGs} to inform their design of future NAS features. 
% Note that we followed a co-design process by brainstorming ideas for these visions with the two VIPs in our research team. [Add co-design here?]




\subsection{Active Environment Shape Surveying}




VIPs explore their immediate surroundings through tactile feedback via a white cane. However, it is difficult to gather information about the environment beyond the reach of the white cane. From our interviews, we found that VIPs want to learn about the general layout of the space in a self-directed manner, specifically in unfamiliar indoor environments (\texttt{Insight 1}). This means of exploration derives from two of the design guidelines: \texttt{DG1} and \texttt{DG3}. \texttt{DG1} highlights the importance of geometric shape information of the space, while \texttt{DG3} mentions the importance of helping VIPs organize that information in a way that supports the formation of complete mental maps via connection information.  

Figure~\ref{fig:surveying} presents our vision of an NAS design that enables VIPs to survey the shape of an environment in a natural way. The system constitutes a wearable sensor --- e.g., head or chest-mounted camera, smartglasses --- which scans the environment to compute the required shape and connection information. As the user moves around the environment, the NAS offers them the ability to receive shape information --- straight edges and corners ---  on-demand via audio cues, where loudness indicates the distance to the boundaries. 
% Using spatialized audio, the system gives user a sense of how far the walls are in front of them.
In addition, VIPs also receive audio cues for connections such as elevators and stairs, in order to help them form a complete image of the environment when transition to other rooms, floors, or even buildings.
Similar to how VIPs use echolocation, the system provides VIPs non-visual cues for them to process instead of directly telling them the shape of the room. Doing so can help them form a better mental map~\cite{clemenson_rethinking_2021}, as it would allow them to integrate this new information with their other sensory information.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{images/surveying.pdf}
    \caption{Our vision of a navigation assistance system (NAS) facilitating active environment shape surveying. The system constitutes a wearable sensor (head-mounted camera) which scans the environment to compute environment shape and connection information. As the user moves around the space, they hear shape information such as straight edges and corners via audio cues; and announcements for connections such as stairs and elevators. Loudness of the audio cues indicate the distance of the information.}
    \label{fig:surveying}
\end{figure}

\subsection{Support for Exploratory Landmarks}
During exploration, VIPs use exploratory landmarks which are multi-sensory (i.e., comprised of information from multiple senses), fluid (i.e., may change over time), and verifiable by VIPs themselves (\texttt{DG2}). This helps them account for the dynamic nature of the environment (\texttt{Insight 2}). Exploratory Landmarks emerge from (\texttt{DG2}), which highlights that NASs should support VIPs in collecting and managing information about these landmarks.

% Figure~\ref{fig:vision2} presents our vision of an NAS that supports fluid landmarks. 
% NASs may incorporate the concept of exploratory landmarks by extending the definition of physical landmarks which are used in guidance.
% % concept by extending the capabilities of what a physical landmarks does for guidance. 
% Doing so would help facilitate both exploration and guidance.
Our vision of such a system maintains a list of landmarks, each defined by three additional attributes, (1) \textit{modality}: which senses are used to detect the landmark, (2) \textit{persistence in time}: when is the landmark active/inactive, and (3) \textit{confidence}: a derived attribute that is computed in real-time to assess the relevance of a landmark along with keeping track of which sensory information are active at any given time.


NASs, through their system components, may support two major functionalities. First, it can help detect new landmarks via a host of different sensors that augment VIPs' non-visual senses. It also filters out any noise in the environment to reduce VIPs' cognitive load during exploration. Second, it assists VIPs in reinforcing their location by directing their attention toward more relevant landmarks in order to account for the dynamic changes in the environment. It does this by maintaining a ranked list of landmarks which is based on the \textit{confidence} attribute. Exploratory landmarks may very well be integrated with existing guidance-based systems to add support for VIPs' exploration of the environment.



\subsection{Cross-modality Translation Interface}
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/translation.pdf}
    \caption{Our vision of a navigation assistance system (NAS) serving as an interface for navigational help between VIPs and non-VIPs to perform cross-modality translation. A VIP asks for directions from a non-VIP, to which the non-VIP responds with incomplete information that primarily constitutes visual cues. The NAS queries the non-VIP to provide additional details in order to complete the information, and then translates visual cues such as colors (red flowers) to non-visual cues such as smell (scent of the flowers) to help VIPs get effective navigational help.}
    \label{fig:translation}
\end{figure}
Exploration of unfamiliar environments often require VIPs to ask for directions from non-VIPs nearby. However, the difference in perception of environments --- which is primarily visual for non-VIPs --- make it challenging for VIPs to use their navigational instructions effectively (\texttt{Insight 4}). This means of exploration touches upon \texttt{DG4}, which highlights the opportunity for NASs to serve as an interface for navigational help between VIPs and non-VIPs. 

Figure~\ref{fig:translation} presents our vision of an NAS that facilitates translation of a non-VIP's navigational instruction to a format appropriate for VIPs.  The system takes as input directions from a sighted person in natural language and converts them into a format that aligns with VIPs' preferred sensory information. The recent advancements in Natural language processing (NLP) have the potential to automate this translation and realize our vision of a cross-modality translation interface. 

The interface is also transactional is nature. Consider a scenario where
non-VIP's instruction may not satisfactorily conform to VIPs' need. In such cases, the system plays a transactional role by raising specific queries to the non-VIP in order to comply with VIPs' need. Figure~\ref{fig:translation} illustrates the transactional nature of the system. This feature also has the potential to help remote-assistance based systems such as AIRA~\cite{aira} and BeMyEyes~\cite{holton2015review}, to develop a framework that ensures that all VIPs receive a uniform assistance. 


\color{magenta}{Talk about how creating awareness is also an important area of further research. Cite Refs. 1 and 3 from "Just let the cane hit it" paper. Social acceptance + social interactions -- Let's get lost paper.}

\color{black}{}
% In addition, there is also an opportunity for research to identify the standard format which fits the VIPs' needs. Similar efforts has been made by Lee et al.~\cite{lee2021designing} to identify product descriptions for grocery shopping, and \cite{scheuerman2017learning} to ----[Complete]\todo{complete}.


% [add verification]



\subsection{Real-time O\&M Tutoring}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\linewidth]{images/tutor.pdf}
    \caption{Our vision of a navigation assistance system (NAS) as an educational tool, providing real-time orientation and mobility (O\&M) tutoring to VIPs. (a) User comes across an environment that they might need help with in order to navigate; (b) system scans the environment to create a challenge and compute the hint based on user's skill-level; (c) the user accepts the challenge and asks for the hint which is computed in a way that it nudges the user to use their O\&M skills; (d) the user makes it through to the environment by minimal support from the NAS, mostly relying on their own abilities.}
    \label{fig:tutor}
\end{figure}
NASs have an immense potential for empowering VIPs to explore environments independently, by serving as educational tools. Many of the VIPs expressed the need to build and maintain O\&M skills (\texttt{Insight 6}). Empowering VIPs through educational NASs derives from \texttt{DG6}, which highlights the importance of nudging VIPs to constantly improve their O\&M skills, attention toward non-visual information, and ability to navigate through complex environments. 


Figure~\ref{fig:tutor} presents our vision of an NAS to serve as an educational tool. The NAS constitutes a wearable camera which scans the environment to create \textit{challenges} for VIPs. A challenge is essentially an environment that VIPs must navigate through on their own using NASs limited support.
These challenges can be thought of as a teacher creating problem sets for the their students. Based on the immediate surroundings, the system provides the user with a general strategy they can follow in the form of \textit{hints}.
Instead of guiding the user through the environment, system announces a strategy which is broken down in terms of VIPs' O\&M techniques. 


% From an NASs' perspective, each of these environments can be imagined as a problem set where O\&M techniques are solutions to each of these problems.

The NAS personalizes the difficulty level of a challenge, and the amount of support (hints) it should provide the user based on system logs. The system saves logs which are used to analyse the user's past performances. As the user develops skills over time, the system logs reflect the change in performance and the NAS can reduce its support until it is no longer required. The ultimate goal of this educational tool is empowering VIPs to explore an environment all by themselves.

% In addition, the NAS saves system logs which can can be used in two ways. First, logs can help determine the level of support needed for a specific user, with an aim to reduce support over time.  Second, the logs can later be shared with O\&M trainers to help VIPs get recommendations for areas of improvement.   
% We believe that NASs should constantly reduce the support over time, ultimately aiming to empower VIPs 

==> 6-Visions/v3.tex <==
  \label{sec:visions}

%Through answering our research questions, we discovered new needs of VIPs for exploration, in addition to turn-by-turn guidance. These new discoveries point to future research opportunities of exploration assistance systems. 


% \subsection{Spatial Information Augmentation}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\linewidth]{images/Figure4.pdf}
%     \caption{A vision of a navigation assistance system (NAS) facilitating Spatial Information Augmentation. The system constitutes computer vision which scans the environment for shape and layout information, and customizable information display format meeting early-blind users' preference of sonification and late-blind users' preference of speech. }
%     \label{fig:spatialinfo}
% \end{figure}

% % . As the user moves around the space, they hear shape information such as straight edges and corners via audio cues; and announcements for connections such as stairs and elevators. Loudness of the audio cues indicate the distance of the information. 

% Our research findings reveal that VIPs want to gather spatial shape and layout information of the space (\texttt{Insight 1}). Acquiring spatial information provides a foundation for VIPs to explore the environment independently. NASs have the potential to enhance VIPs current practices and extend their abilities to survey the shape and layout of the environment. Additionally, information format preferences differ depending on VIPs onset of vision impairment (\texttt{Insight 2}). The NASs can display the spatial information to VIPs in a format that matches their needs. 

% The NAS is equipped with a wearable sensor, such as a head or chest-mounted camera or smart glasses. The sensor is combined with machine learning detection models to recognize the shape and layout information meeting VIPs’ needs. For shape information, the sensor scans for edge conditions in the environment, for example, corners, straight edge or curved edge. For layout information, the sensor scans the environment with scene object detection focusing on the categories of objects that inform layouts, for example, doors, stairs, and hallways.

% The information feedback format is customizable based on the VIPs preference, as they differ due to onset of visual impairment. For early-blind  VIPs who prefer sensory augmentation, the information can be displayed using sensory substitution techniques \cite{meijer_seeingwithsound_1992}. Different audio sonification cues can be used to describe different shapes of the space and shapes of objects, mimicking sounds produced by echolocation. For late-blind VIPs who prefer verbal description, the information can be displayed using speech announcements, directly calling out shapes and object names in natural language. Spatialized audio can also be integrated with information feedback to display spatial direction and distance. The loudness of the sound indicates the distance to the detected information. 


% \subsection{Commodity O\&M Education Tool}

% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[width=0.65\linewidth]{images/tutor.pdf}
% %     \caption{Our vision of a navigation assistance system (NAS) as an educational tool, providing real-time orientation and mobility (O\&M) tutoring to VIPs. (a) User comes across an environment that they need additional skills in order to navigate; (b) system scans the environment to create a challenge and compute the hint based on user's skill-level; (c) the user accepts the challenge and asks for the hint which is computed in a way that it nudges the user to use their O\&M skills; (d) the user makes it through to the environment by minimal support from the NAS, mostly relying on their own abilities.}
% %     \label{fig:tutor}
% % \end{figure}

% Many VIPs face the lack of O\&M instructors and funding to receive training, as well as difficulties to maintain O\&M skills in their daily practice (\texttt{Insight 4 \& 5}). NASs have the potential to serve as inexpensive commodity tools for educational assistance, providing supports for both O\&M training and day-to-day maintenance of the skills. Such commodity education tools can fill the gap of instructor and funding shortage, provide VIPs with access to O\&M support anywhere and anytime, and help VIPs become more confidence in exploring unfamiliar environments. 

% %and empower VIPs to explore environments independently. Building and maintaining O\&M skills highlights the importance of nudging VIPs to constantly improve their O\&M skills, attention toward non-visual information, and ability to navigate through complex environments. 

% % Figure~\ref{fig:tutor} presents our vision of an NAS to serve as an educational tool. 
% % The NAS constitutes a wearable camera which scans the environment to create \textit{challenges} for VIPs. A challenge is essentially an environment that VIPs must navigate through on their own using NASs limited support.

% The NASs constitute a wearable camera and a smartphone app, that can detect challenges and training opportunities in the real world environment. These challenges can be thought of as a teacher creating problem sets for their students. Based on the immediate surroundings, the system provides the user with a general strategy they can follow in the form of \textit{hints}. Instead of guiding the user through the environment, the system announces a strategy which is broken down in terms of VIPs' O\&M techniques. The NAS personalizes the difficulty level of a challenge, and the amount of support (hints) it should provide the user based on system logs. The system saves logs which are used to analyse the user's past performances. As the user develops skills over time, the system logs reflect the change in performance and the NAS can reduce its support as the VIP user's O\&M skills and confidence increase. 


% %until it is no longer required. 

% %The ultimate goal of this educational tool is empowering VIPs to explore an environment all by themselves.

% % \yy{I pitched this vision towards commodity education tool to reflect the findings on lack of instructors and funding. However, I feel the older version was more exciting - nudging out of comfort zone and build independence over time.}


\subsection{Collaboration and Translation Interface}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{images/translation.pdf}
%     \caption{Our vision of a NAS serving as an interface for navigational help between VIPs and non-VIPs to perform cross-modality translation. A VIP asks for directions from a non-VIP, to which the non-VIP responds with incomplete information that primarily constitutes visual cues. The NAS queries the non-VIP to provide additional details in order to complete the information, and then translates visual cues such as colors (red flowers) to non-visual cues such as smell (scent of the flowers) to help VIPs get effective navigational help.}
%     \label{fig:translation}
% \end{figure}

NASs can mitigate social pressure by serving as a discrete collaboration platform, removing potential social pressure projected by bystanders on both VIPs and sighted people who help VIPs (\texttt{Insight 5}). 
%Existing apps, such as AIRA and Be My Eyes (CITE), provide verbal remote assistance through video-conferencing. 
Our vision of NASs could provide a private channel to support collaboration between VIPs and sighted helpers in public, allowing them to communicate without social pressure. The NASs could also mediate communication differences between VIPs and sighted helpers, giving VIPs the active agency in requesting and moderating assistance. Additionally, the NASs could translate the language difference between VIPs and sighted people with Natural Language Processing (NLP) algorithms, forming more effective collaboration (\texttt{Insight 6}). 

%As our design implication reveals, sighted people should speak VIPs' language in order to provide effective assistance. The differences in communication is 
%The difference in perception of environments --- which is primarily visual for non-VIPs --- make it challenging for VIPs to use their navigational instructions effectively.
%highlights the opportunity for NASs to serve as an interface for navigational help between VIPs and non-VIPs. 

% Figure~\ref{fig:translation} 

The NAS provides a private collaboration channel in a transactional nature centered on VIPs needs. In the case when sighted people's instruction may not satisfactorily conform to VIPs' need, the system plays a transactional role by raising specific queries to the sighted people in order to comply with VIPs' need. The NAS also facilitates NLP algorithms that translates a sighted people's navigational instruction to a format appropriate for VIPs. The system takes as input directions from a sighted person in natural language and converts them into a format that aligns with VIPs' preferred sensory information. For example, if the sighted people gives direction to turn at the red flower planter, however red is a visual attribute that VIPs cannot perceive, the NLP algorithms can translate the visual attribute to olfactory attribute instructing the VIP to follow the scent of flowers instead. Recent advancements in NLP have the potential to automate this type of cross-modal translation and realize our vision. 

% The recent advancements in Natural language processing (NLP) have the potential to automate this translation and realize our vision of a cross-modality translation interface. 
% Figure~\ref{fig:translation} illustrates the transactional nature of the system. This feature also has the potential to help remote-assistance based systems such as AIRA~\cite{aira} and BeMyEyes~\cite{holton2015review}, to develop a framework that ensures that all VIPs receive a uniform assistance. 

==> 7-Limitations/v1.tex <==
While this work provides interesting key insights into "beyond guidance" navigation goals of VIPs, we acknowledge that our study has some limitations. First, [what is the issue?] [what can we do next?] [what is the justification, if any]
Second, [what is the issue?] [what can we do next?]  [what is the justification, if any]
Third, [what is the issue?] [what can we do next?]  [what is the justification, if any]
Finally, [what is the issue?] [what can we do next?]  [what is the justification, if any]
We would like to better understand these attitudes in quantitative terms through online surveys and questionnaires that can be directed at a larger set of participants (in future).

the experiences of VIPs, there were several limiting factors that should be considered. First, we had a limited number of participants, which may not give a complete representation of the VIP community. Our participants were predominantly male, young, and from the US. Future studies could further explore the preferences of VIPs from a broader perspective, via an online questionnaire. Another limitation was that the majority of our interviews were conducted remotely. Because most of our interviews were conducted online, we may have missed some of the nuances that may otherwise have been visible in person. While interviews provide an overview of the experiences and preferences of the participants, observation sessions could provide further insight into the needs and preferences of VIPs for navigation. Another limitation of this study was that we focused primarily on VIPs’ navigation practices in indoor environments, and lacked a comprehensive evaluation of VIP’s preferences for outdoor navigation. Nevertheless our findings provide strong evidence that NAS design should adopt a more agency-oriented approach that enhances and enriches both passive and active VIPs’ navigation experience.


% ---- Possible points -----
% 1. (Age and Location) Not representative of the world -- interview diverse people
% 2. Small sample size
% 3. Clusters we created were found in the ptcpts that we interviewed (which was small), a follow-up study [or an online survey] could now be designed to find the ratio of active to passive within a larger set of VIPs to get a better sense of how many people are active.
% 4. We asked VIPs to remember where they went and what they did, which may not always be comprehensive. For this, a longitudinal study such as a diary study or observation session could be conducted.
% 5. Only one female -- but this is not common because there are more male VIPs than females (there should be a paper that we can cite here)
% 6. Not generalizable: our results are based on a small sample of interviews, meaning that they are not necessarily generalizable to all populations of people with visual impairments. Further investigation with a large set of VIPs is needed to concretely establish ..

% ---- Final points -----
% small size, not representative of the world (only one female, young folks, from US), hence the results may not be generalizable -- for this, first justify why it is okay to do this. And then talk about possible solutions
% We asked VIPs to remember where they went and what they did, which may not always be comprehensive. For this, a longitudinal study such as a diary study or observation session could be conducted. -- be explicit about what else can we learn (example 5)
% Our small sample showed a 50-50 split but that may not be true. We would like to better understand these attitudes in quantitative terms through online surveys and questionnaires that can be directed at a larger set of participants in future. (example 3)


% Example 1: Our sample of participants were from the United States of America, used mobility aids (white cane and guide dogs) and some form of technology to assist with navigation. This is likely not represen- tative of the larger population of people with visual impairments within the US or abroad. Additionally, our results are based on a small sample of interviews and a single diary study, meaning that they are not necessarily generalizable to all populations of people with visual impairments.

% Example 2: A challenge faced by accessibility researchers relates to recruitment of disabled users, due to the smaller number of individuals in their population. Consequently, it is not uncommon to recruit smaller samples and from venues local to the researchers, where the researchers have links with community-based organizations [70] -- Towards More Transactional Voice Assistants: Investigating the Potential for a Multimodal Voice-Activated Indoor Navigation Assistant for Blind and Sighted Travelers
\cite{abdolrahmani2021towards}




% Example 3: Additionally, this study focused on participants’ individual travel experiences rather than understanding the experiences of those who may have been trav- eling in a group (e.g., blind parents with sighted children, groups of blind or sighted travelers). The findings of this study could be extended by eliciting experiences of travelers who travel in a group, have a wider range of travel frequency (e.g., those who travel rarely or on a frequent basis), frequently make multiple connections on the same journey, or identify as having other disabilities (e.g., mobility impairments). 

% Example 4: One limitation of our research is inherent sampling bias, as all of our interviewees were Aira employees who volunteered to participate. This group has unique expertise in RSA, which was crucial to this study. Even though the participants’ identities were protected, their employment relationship with Aira may have affected how candid they were. However, our data shows a balance of positive and negative findings, and all agents seemed happy to discuss challenges and shortcomings in Aira’s service. --- safeguard against a limitation.

% Example 5: Look at the limitations of this paper: Ahmetovic, Dragan, João Guerreiro, Eshed Ohn-Bar, Kris M. Kitani, and Chieko Asakawa. ‘Impact of Expertise on Interaction Preferences for Navigation Assistance of Visually Impaired Individuals’. In Proceedings of the 16th International Web for All Conference, 1–9. San Francisco CA USA: ACM, 2019. https://doi.org/10.1145/3315002.3317561.
% They get into the details of what might be missing in our current study, and how a longitudinal study can help with that. example: While our approach is the frst to explore how prior knowledge infuences navigation assistance requirements and preferences for PVI, we can see how a longitudinal study could complement and verify the fndings. For instance, it is still not clear how fast a PVI builds a mental model of the environment while being assisted by a NAT, as well as how the navigation needs of PVI change during that time. 

==> 7-Limitations/v2.tex <==
While our work provides key insights into VIPs' `\textit{beyond guidance}' navigation goals, we acknowledge that our study has some limitations. 
% 
First, we had a small sample of participants. Our participants were predominantly male, were relatively young, and were all white cane users from the United States. This is likely not representative of the visually impaired population around the world, and thus our results may not necessarily be generalizable to all populations. Since recruiting disabled participants is a challenge faced by the accessibility research community at large, due to the small size of this population and skewed gender ratio,
% Private correspondences with CEO of blind-serving organizations.
there is an increased understanding among the HCI community to recruit smaller samples from local venues through community-based organizations~\cite{sears2011representing}. Still, we must acknowledge this limitation in our sample of VIPs.
% 
Our small sample size leads to a second limitation, which is the fact that we are not able to estimate the proportion of the VIP population at large that is wants ``beyond guidance'' navigation vs.\ being satisfied with receiving guidance only. We found an equal split in the VIPs that we interviewed, with four VIPs on each side, but this may not generalize to the VIP population at large. The findings of this study could be extended by eliciting responses of a large sample through other study methods such as an online survey. Such a survey could also help us understand, in quantitative terms, the factors that influence these attitudes.
% 
Finally, during the interviews we relied on participants' memory of their past experiences and behaviours, which may not always be comprehensive or accurate. While our approach is the first to explore VIPs' ``\textit{beyond guidance}'' navigation goals, we realize how a contextual inquiry or a longitudinal study such as a diary study could complement and support our findings more concretely. 
% For instance, it is still not clear how VIPs' behaviour would be affected by the presence of an NAS, as well as how fast does a VIP build their mental map of an environment. 
% 
% Finally, our samples were found to be distributed equally between active (n=4) and passive (n=4) attitudes, but this ratio is likely not an accurate representation of the population at large. 



